Learning to Play: Reinforcement Learning and Games

Amazing breakthroughs in reinforcement learning have taken place. Computers teach themselves to play Chess and Go and beat world champions. There is talk about expanding application areas towards general artificial intelligence (AI). The breakthroughs in Backgammon, Checkers, Chess, Atari, Go, Poker, and StarCraft have shown that we can build machines that exhibit intelligent game playing of the highest level. These successes have been widely publicized in the media, and inspire AI entrepreneurs and scientists alike. Reinforcement learning in games has become a mainstream AI research topic. It is a broad topic, and the successes build on a range of diverse techniques, from exact planning algorithms, to adaptive sampling, deep function approximation, and ingenious self-play methods. Perhaps because of the breadth of these technologies, or because of the recency of the breakthroughs, there are few books that explain these methods in depth. This book covers all methods in one comprehensive volume, explaining the latest research, bringing you as close as possible to working implementations, with many references to the original research papers. The programming examples in this book are in Python, the language in which most current reinforcement learning research is conducted. We help you to get started with machine learning frameworks such as Gym, TensorFlow, and Keras, and provide exercises to help understand how AI is learning to play.

==> chapters/04search__MBPAske-2.local_s_conflicted_copy_2019-01-09_.tex <==
%% 3:
%% section: eval: linear combiation
%% section: search: fixed depth fixed width
%% section: b and d, crit tree, alpha beta,
%% *section: bounds, solution tree, null window search, mtdf
%% section: id/tt/hh
%% *section: null move
%% section: small program with heur eval and ab
%% section: system 1 and system 2 (this is system 2: planning)

% Search-eval as arachitecture is in previous chapter

%\section{Plan/Learn}

The {\bf problem} of this chapter is that the
value of a state must be computed.
The {\bf topic} of this chapter is to introduce the first methods of how to
enumerate state spaces.  
We will find that the mathematical definition
of the states gives us a convenient algorithm, the minimax algorithm,
that can then further be refined. In doing so, this chapter introduces
the search-eval architecture, that is the basis for the rest of this book.

\section*{Learning Goals}
\begin{itemize}
\item Search-Eval Architecture
\item Heuristics
\item State Space, complexity
\item Minimax,  alpaha-beta, window, cut off
\end{itemize}
    

% of: section on  heuristic eval?
The previous chapter provided us with the theoretical framework
of reinforcement learning and Markov Decision Processes, which neatly
formalize many intuitive 
notions of learning by trial and error. We  discussed the
importance that algorithms do exploitation and exploration, part of
the trial part of trial and error, and do recursive backup of reward
values, part of the error part of trial and error. The formalizations
allow us to  precisely 
reason about our algorithms.

Towards the end, the chapter also mentioned a way to deal with state spaces
that are very large, by using function approximation and
generalization. In this chapter we will see a different
solution to deal with large spaces: the heuristic evaluation function.

The problem of dealing with  large state space has been around
since the beginning of research into games. It is a central element in
Artificial Intelligence, and finding ways to successfully search
 large state spaces is an important  element of AI.

In this chapter, we will focus on the use of basic heuristics to be
able to search large state spaces. In the next chapter we look at advanced
methods to use heuristics, such as used in state of the art Chess and
Checkers programs. Next, we will look at heuristics-free
methods to search large state space efficiently, that caused a
breakthrough in Go.  

 A
heuristic is a function that encodes domain specific knowledge. For
example, in Chess, having two pawns is better than having  one pawn,
and  the Queen is more valuable than the Rook. Heuristic evaluation
functions have been a center piece of combinatorial search. In fact,
the name heuristic planning has been the name of field that has
studied methods for solving difficult decision making problems with
state spaces that are of exponential  size~\cite{pearl1984heuristics}.

The downside of a heuristic is, of course, that it is  domain
specific---it does not work in another domain. Non-heuristic machine
learning methods such as random forests, support vector machines or neural networks
(see the next part) are more general. Another problem of heuristics is
that it may be hard to find good ones, and that hand coding them
correctly can be challenging, requiring many hours of manual
debugging. To achieve world campionship level,
the teams behind Chinook and Deep Blue spend years of refining their
heuristics.

Furthermore, heuristic evaluations are, in almost all games, crude
approximations of the  value of the states. They  often only capture static
elements of a position, and lack insight into the dynamics. Achieving high
performance requires either extra work on heuristics or capturing
dynamics with planning algorithms. In reinforcement learning the two
approaches  (dynamic programming and function approximation) are often 
studied separately and seen as mutually exclusive approaches.

In most
board games, however, they are studies together, due to
the lack of performance of heuristic evaluation 
functions without search, and conversely the lack of performance of
search without heuristic evaluation functions. In Chess and Checkers
they are studies in an integrated setting, where
search is  responsible for dynamics (tactics), and evaluation
for static aspects of the game (strategy).

In the field of heuristic
search the value function is a heuristic evaluation function, and
dynamic programming is done by a search procedure. This two-way architecture
has been the dominant paradigm ever since Turing's and Shannon's  papers
on how to have a machine play chess~\cite{turing1953digital,shannon1988programming}.

For that reason we use the terminology from heuristic search in this
book, and call this architecture the {\em search-eval\/} architecture
(which is also shorter than dynamic programming-function
approximation architecture, which would have been correct
reinforcement learning terminology).

\section{The Search-Eval Architecture}
The search-eval architecture consists of a search function and an eval
function. It has the search function because the evaluation
function misses game dynamics and an evaluation
function because the search space is too large to search completely. 
Together, search and eval
are  strong enough to achieve a level of play that beats the best humans
in Chess and Checkers.
\index{search-eval architecture}

\subsection{State Space}
Finding the best move of a board position is hard. Let us try to see
why it is so 
difficult. An often used measure is to
calculate an upper bound on the size of the state space, i.e., how
many legal  states would be traversed if all successors are
eavaluated. 
In general, finding 
the exact state space size of games is 
a surprisingly challenging problem, that has attracted many
interesting research papers~\cite{shannon1988programming,schaeffer2007checkers,bonnet2013complexity,allis1994searching,fraenkel1981computing,iwata1994othello,hsieh2007fairness,iida2002computer,tromp2006combinatorics}.


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/Tic-tac-toe-game-tree.png}
\caption{Tic Tac Toe Game Tree (part)}\label{fig:ttt-tree2}
\end{center}
\end{figure}
\index{Tic Tac Toe}


Listing~\ref{lst:smalltree} gives an example in Python code of a very
small tree, with one max node (the root), three min nodes, and 9
leaves. In a short while we will compute the value of the tree by
looking at the leaf values, and later on by looking at the material.

\lstset{label={lst:smalltree}}
\lstset{caption={Small Tree code}}
\lstinputlisting[language=Python]{python/smalltree.py}


For small games, such as Tic Tac Toe, the state space is small enough
to enumerate with a computer.
See Fig.~\ref{fig:ttt-tree2} for a 
two ply tree of how the possible states are enumerated. 
To compute the size of the Tic Tac Toe state space, we note that there are 9 squares
of the board that can be either empty, cross, or circle. This number, $3\times
3\times\ldots\times 3= 3^9=19,683$ is an over-estimate, since it
contains unreachable and illegal positions.
When we remove illegal positions we come to $5,478$ states. When
rotations and reflections of positions are removed there are only $765$ positions left~\cite{schaefer2002}.

Beyond Tic Tac Toe, for more challenging games such as Chess or Go, calculating the
precise number of legal and reachable game positions is harder.
For Chess the size of state space is often given as $10^{47}$ and for
Go on the standard $19\times 19$ board this number is
$10^{170}$~\cite{allis1994searching}.\index{state space complexity}

Note that the state space size is different from the game tree
size. The former is the number of unique game states reachable
from the start position, the latter is the number of possible games
that can be played. For Tic Tac Toe an upper bound for the former is
$3^9=19,683$ (pieces on squares), for the latter it is $9!=362,880$
(different full game sequences
of moves). The former is the game graph, the latter is the
game tree. The same position from the graph can occur in many
different lines of play, that consitute the tree. These shared
position are often called transpositions. The difference between the
game graph and the game tree is large~\cite{shannon1988programming,allis1994searching,plaat1996exploiting,plaat1996exploiting}. An
essential element of Chess and Checkers programs is the transposition
table, a cache of positions, preventing the generation of states that
have already been searched before. In Section~\ref{sec:tt} we will go
deeper into transposition tables and their advantages.



\subsection{Search: Depth First}
How can we determine if a position is won, lost, or drawn, and how can
we find the best move that leads to this outcome? In a two player zero
sum game players want to win, and should choose moves
that lead to successor positions that  have the highest probability of
winning. More formally, if node $n$ represents the  position of which
we wish to determine the value, then the value of node $n$ is the
maximum of the value of its children $C_n$. The value of these child
nodes is determined analogously, although here the moves are made by our
opponent, who chooses positions that will minimize the outcome for
us. Next it is our move again, and we choose the position that
maximizes our winning probability. This alternating of maximizing and
minimizing is the reason the procedure is called {\em minimax}.

%% The intiution behind minimax is familiar: If Anna and Beth are
%% playing, then Anna will try to find the best move, assuming Beth will
%% look for Beth's best reply,  assuming that Anna will play Anna's
%% best reply, assuming that Beth \ldots
%% From Anna's point of view, Anna will choose the move maximizing
%% Anna's value, Beth the move minimizing Anna's value; Anna goes for max,
%% Beth for min. The max/min/max/min/max/min/\ldots sequence is
%% abbreviated as minimax (although maximin would be more logical).

In Figure~\ref{fig:TTTminimax} a Tic Tac Toe tree is drawn with
values. In Figure~\ref{fig:minimax} another, larger, minimax tree is
shown. Maximizing nodes are drawn as squares, minimizing nodes as
circles. By following the values we can see how the values of the
nodes are determined. The shaded nodes are explained later in the
discussion on alpha-beta.

Listing~\ref{lst:minimax} gives example Python code for the minimax
algorithm. % Listing~\ref{lst:smalltree} defines a small tree with 9
% leaves.
The minimax function will determine the value of a node by taking the minimum
of the value of the children of the MIN nodes, and the maximum of the
values of the children of the MAX nodes. In the case of the tree in Listing~\ref{lst:smalltree}, the value of
nodes \verb|min_node1| and \verb|min_node3| is both 1, and the value
of \verb|min_node2| is 2. The maximum of 1 and 2 is 2, so the minimax
value of the root is 2.\index{minimax}



\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/minimax-TTT.png}
\caption{Tic Tac Toe Game Tree}\label{fig:TTTminimax}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/AB_pruning.png}
\caption{Minimax Tree}\label{fig:minimax}
\end{center}
\end{figure}


\lstset{label={lst:minimax}}
\lstset{caption={Minimax code}}
\lstinputlisting[language=Python]{python/minimax.py}


\subsubsection{Search Tree}
The minimax procedure recursively traverses the entire game tree. It starts at the
root, and does a depth first traversal of the tree by calling itself
recursively for each child node. The nodes that are
actually expanded during a search procedure are  called the {\em
search tree}. For the minimax procedure the search tree is identical
to the game tree. In the rest of this book we will see 
many examples of procedures whose search tree is significantly smaller
than the game tree. Minimax does a full-depth  full-width expansion of
the game tree.  For regular trees, where all nodes have the same
number of children, the number of leaves of the game tree is $w^d$, where $w$ is
the width of the nodes (the number of children of a node) and $d$ is
the depth of the tree. For the tree in Listing~\ref{lst:smalltree} the
width is $3$ and the depth is $2$, so the number of leaves is
$3^2=9$. The size of the game tree is exponential in the depth
parameter, and is dominated by the number of leaves. The size
therefore is $O(w^d)$, and so is the running time of the minimax
procedure, since it visits every node.
\index{search tree}

Calling the minimax function on a Chess position, whose game tree is
of size $O(10^{47})$ would take too long.\footnote{Even if node evaluation
would take a ridiculously fast one nanosecond, it would still take $O(10^{38})$ seconds,
or $O(3\times 10^{30})$ years.} In order to reduce the size of the
search tree, the search depth can be reduced.\footnote{Also the width
of the tree can be reduced. With forward pruning fewer  children are
expanded at inner nodes. See Section~\ref{forward}.} To do so, the
earliest Chess and   
Checkers program (Turing, Samuel) used a heuristic evaluation
function as an approximation of the true value. The heuristic is based
on domain knowledge, provided by domain experts. In Chess and Checkers,
the most important heuristic is material balance. Instead of traversing the tree to the full depth where the
game ends due to an end game position, we create artificial leaves, at
much shallower search depth. The deeper search is artificially limited,
and a heuristic is called to evaluate whatever position happens to
occur at that depth.

Listing~\ref{lst:depthmm} adds depth-limiting to our Python code of
minimax. New is
parameter \verb|d| which is decremented in the recursive call of the
function, and that the \verb|eval| function no longer uses the score
at the leaves, but takes a heuristic value of the node whenever the
depth parameter happens to be 0. The heuristic eval in the example
code is quite straightforward, it uses the \verb|material| value of the
node (see Listing~\ref{lst:smalltree}). 

\lstset{label={lst:depthmm}}
\lstset{caption={Depth Limited Minimax code}}
\lstinputlisting[language=Python]{python/depthmm.py}


\subsection{Eval: Heuristic Features}\label{sec:eval}

In real Chess and Checkers programs the heuristic evaluation function
is a highly advanced piece of code, using many features. The features
are typically heuristic,  manually chosen, and manually optimized
and tuned. This feature engineering is quite labor intensive.
Debugging a manual evaluation function is especially hard, because the
search space is large and pathological behavipr may be difficult to pinpoint.

In Chess and Checkers  material balance is the dominant factor in
the strength of a position. For this reason, the heuristic
evaluation function of Listing~\ref{lst:depthmm} 
uses the \verb|material| field of the nodes defined in
Listing~\ref{lst:smalltree}.
\index{heuristic evaluation}

Heuristic evaluation functions are linear combinations of features.
A typical chess evaluation function consists of the following
features: material, mobility, king safety, center control. The
evalution function is static. Dynamic aspects are taken care of by the
search. To achieve good search performance, speed of evaluation is
important. For that reason heuristics are
often optimized for speed, not for accuracy.

Today, many  Chess programs are open source, including one of the top programs,
Stockfish~\cite{stockfish},\footnote{The name reflects the countries of programmers
Romstad and Costalba: ``produced in Norway
and cooked in Italy.''}. To get an idea of just how extensive current
state of the art heuristic 
evaluation function have become, you may want to have a look at the Stockfish
source at Github: \href{https://github.com/official-stockfish/Stockfish}{Stockfish}.\footnote{\url{https://github.com/official-stockfish/Stockfish}}

Stockfish has a conventional  evaluation function with manual features and manually
tuned weights. In other games evaluation functions based on machine
learning have been succesful, such as
Othello (Logistello~\cite{buro1995statistical}) and Backgammon
(Neurogammon~\cite{tesauro1989neurogammon}) and of course Go
(AlphaGo~\cite{silver2016mastering}). Despite some effort to
automate tuning of weights by Samuel~\cite{samuel1959some} and in Deep
Blue~\cite{hsu2004behind}, in Chess manual evaluation   
functions have reigned supreme, although one paper describes success in
evolving coefficients of manual features~\cite{david2014genetic}, and
in AlphaGo both the features themselves and the coefficients are
learned~\cite{silver2016mastering,silver2017mastering,silver2018general}.

The machine learning evaluation functions have the advantage of being
more general and easier to debug.



\subsection{Search and Eval}
Game playing programs consist of both a search function and an
evaluation function. Together these two form the search-eval architecture:
finding the best move  is done by lookahead {\em search},
and by {\em evaluation}, after the position 
has been searched sufficiently deep. See Figure~\ref{fig:se-arch} for an illustration.

In the early days of Turing and Shannon's papers, when search-eval was
conceived~\cite{turing1953digital,shannon1988programming}, the searhc
and eval functions were quite straightforward. The heuristic function
was the most basic eval function that worked,  and the search function
was a minimax(-like) function to
traverse the nodes in standard depth first order. This simple model proved quite
versatile and amenable to successive refinements. Over the years many
enhancements were  introduced and  performance has reached world
champion level  in games such as Chess and
Checkers. The enhancements are very important---they elevate the level
of performance from being barely able to follow the rules to state of the
art. Chapter~\ref{chap:idtt} will discuss many of the major
enhancements, such as iterative deepening and transposition tables.

\begin{figure}
\begin{center}
\input searchevaltree
\caption{Search-Eval Architecture in a Tree}\label{fig:se-arch}
\end{center}
\end{figure}

Let us see how all this fits into the general picture of the field of
game playing programs. Table~\ref{tab:arch2} gives an overview of the
different paradigms in this book. The entry for
Chapter~\ref{chap:search}   shows the heuristic search approach in the 
search-eval architecture. 
\index{search-eval architecture}
The focus of  this chapter is on  full width search and manual
heuristic evaluation functions, and value backup via the minimax
rule. Future chapters will discuss variable 
width and variable depth search and learning evaluation functions.
The search-eval architecture  allows us to compare the main features
of different search functions and different eval functions.


\begin{table}
  \begin{center}
    \begin{small}
\input paradigm
  \caption{Search-Eval Architecture}\label{tab:arch2}
  \end{small}
  \end{center}
\end{table}

As the table indicates, in the following chapters different, more
advanced, techniques will be introduced. In Chapter~\ref{chap:plan}
this will culminate in functions 
that are able to self learn to play a game as complicated as Go with
as only knowledge the rules of the game.
% Zero heuristics, learning
% adaptively, by trial and error, presumably in a way reminiscent of how
% young humans learn to play the game well.


But first, we should explore in more depth the  advances that
have been made to the minimax function. The algorithms that have been
devised allow to double the search depth compared to minimax, with equal computational
cost and yielding the same quality of the answer.
% These insights have
% pointed the way to research finding better and better algorithms to
% find the value of a position and the corresponding best moves. They are
% the basis on which the techniques of future chapters are built.

%\section{Theory}
\subsection{*State Space Complexity}
We will start by having a careful look at the minimax tree. We will try to
find what part of tree is the  essential part that proves the value of
the minimax tree. We will see that  there is
quite some redundancy in the tree, which allows us to create a much more
efficient search algorithm.

\subsubsection{Width and Depth}
Let us start with a fixed width fixed
depth tree. The size of this tree is dominated by the number of leaf
nodes, which is $w^d$ for width $w$ (number of moves per board
position) and depth  $d$ (number of  moves that will be looked ahead). 

\subsubsection{Critical Path}\index{critical path}
Figure~\ref{fig:prooftree} shows a minimax tree,
with leaf alues, and values at the inner nodes. As usual, the root is a max
node, its value is the maximum of its child values, and the children of
the root are min nodes, whose value  is the minimum of their child values.
illustrated in the example tree. The child nodes that have the same
value as their parent are shown blue. The tree of blue links is called
the {\em critical path}, the path of nodes whose value is equal to the value of the
root.
\begin{figure}[t]
\begin{center}
\input crittree
%\includegraphics[width=6cm]{figures/prooftree.png}
\caption{{\bf\em $\pm$ Critical Path}, {\bf + Max
Solution Tree}, {\em - Min Solution Tree}}\label{fig:prooftree}
\end{center}
\end{figure}


\subsubsection{Critical Tree}
It turns out that not all nodes in the minimax tree are necessary do
determine the value at the root. Let us try to construct the smallest possible tree that defines the
minimax value. At max nodes, the highest child
determines the value of the parent node. All other children are
unnecessary, they are non-critical nodes that are ``dominated'' by their critical
sibling. Likewise, at min nodes, only the lowest child determines the value of
the node. There is a complication, however. If we only expand
one child, then we do not know for certain what the value of a node
is, even if it is the critical child. At a max parent, the single expanded child creates a
{\em lower bound\/} on the minimax value (since expansions of subsequent
children can only increase the value upwards, in a max node). Likewise,
a min node whose children have been partly expanded has an upperbound
on its final value, since subsequent expansion can only lower the value
further.

A partly expanded max node defines a lowerbound on the minimax value. Lower bounds
of {\em min\/} nodes, however, require all children of that min node
to be expanded (since, if it were partly expanded, then expansion of
another child could lower the value further, and the lower bound
evidently was not a lower bound).

Likewise, a partly expanded min node is an upperbound on the min node
value. Upper bounds of {\em max\/} nodes, however, require all
children of that max node to be expanded.

Now we have enough information to construct the smallest tree that
defines the minimax value. If we wish to have an upper bound at the
root node,  then we need a tree where at least {\em one\/} child of
the min nodes is present, and {\em all\/}
children of all the nodes are present. Figure~\ref{fig:maxsoltree}
shows such a tree. This tree is called a max solution tree in the
literature, the tree determining an upper
bound. There is an extensive literature on solution trees, see for
example
~\cite{kumar1988general,pijls1990another,stockman1979minimax,pearl1984heuristics,plaat1996best}.\index{solution
  tree}\index{max solution tree}

Conversely, if we wish to have a lower bound at the root node, then we have to
construct a tree where at least one child of all max nodes is present,
and all children of all min nodes. Figure~\ref{fig:minsoltree} shows 
such a tree, which is called a min solution tree, a tree determining a
lower bound in a minimax tree.\index{min solution tree}

\begin{table}
\begin{center}
\begin{tabular}{c|c|c|c}
solution tree & bound \# children at MAX node & \# children at MIN node\\ \hline\hline
Max & upper & all & $geq 1$\\ \hline
Min & lower & $\geq 1$ & all
\end{tabular}
\caption{Solution Trees and Bounds}

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/maxsoltree.png}
\caption{Max Solution Tree}\label{fig:maxsoltree}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/minsoltree.png}
\caption{Min Solution Tree}\label{fig:minsoltree}
\end{center}
\end{figure}



The minimax value of a position is, of course, defined by  two  solution
trees of equal value, one min solution tree defining a lower bound of
the same value as the upper bound defined by its max solution tree.
The intersection of the 
min solution tree and the max solution tree is the critical path. 
Figure~\ref{fig:crittree}  shows such an intersection of a
min solution tree and a max solution tree. The union of the two
solution trees is called the
critical tree, or the proof tree. It is the smallest tree that proves
the value of the position. It proves that the minimax value is not less than the
value of the min solution tree, and not larger than the value of the
max solution tree. Every algorithm that wishes to find the minimax
value, has to at least traverse this critical tree, otherwise it has
not seen enough of the tree to know its value~\cite{knuth1975analysis}.\index{critical tree}

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/crittree.png}
\caption{Critical Tree}\label{fig:crittree}
\end{center}
\end{figure}

The size (the number of leaf nodes) of a max rooted max solution tree
is $w^{\lceil d/2\rceil}$, or the quare root of the size of the minimax tree. The number of leaves of a max rooted min solution
tree is $w^{\lfloor d/2\rfloor}$. 

Likewise, the size of the critical tree (the union of the two solution
trees) is $w^{\lceil d/2\rceil}+w^{\lfloor d/2\rfloor}-1$, the square root of the size of the
minimax tree, $O(\sqrt{w^d})$. In order to determine the value of a
minimax tree with $1000000$ leaves, only $1000$ leaves have to be
examined. In the same time as minimax would search to depth $5$, an
optimal algorithm would search to depth $10$, double the depth.

In Listing~\ref{lst:minimax} we have seen an $O(w^d)$ algorithm for
traversing the tree and finding the minimax value.

Next, we will describe alpha-beta, an $O(\sqrt{w^d})$ algorithm for
traversing the tree and finding the minimax value, much more efficiently.

\section{Alpha-Beta}\index{alpha-beta}
The listing~\ref{lst:alphabeta} shows the alpha-beta algorithm, an
$O(\sqrt{w^d})$ algorithm that has been the basis of almost all Chess and
Checkers programs since the 1960s. A seminal analysis of the alpha-beta
algorithm is~\cite{knuth1975analysis}, although without the concept of
solution trees, which has been studied in later publications on the
Stockman's SSS*
algorithm~\cite{pijls1990another,stockman1979minimax,pearl1984heuristics},
which turned out to be related to alpha-beta~\cite{plaat1996best}.\index{SSS*}

So, how does alpha-beta work, how can it search the minimax tree and
find the value without searching all of the tree?

\subsection{Alpha-Beta Window}\index{alpha-beta window}
alpha-beta maintains a window on the value of the position. This window
starts out as the widest possible window, which we write as
$\langle-\infty,+\infty\rangle$. The window is updated in each node
with results of its child nodes, and each recursive call of alpha-beta
uses the latest version of the window. When, at a certain node, the
window collapses, the search can be stopped, since the value of that
node is known. alpha-beta is said to {\em cut off\/} the search of the
other children.\index{alpha-beta cut off}

As we perform  lookahead in minimax games such as Chess and
Checkers, we encounter child positions, some of which are good. These
good positions provide a
lower bound on our value (since we are the maximizer). Now, the positions
that 
that our opponent searches, lower the values it finds (since our
opponent is the minimizer). As soon as the opponent finds positions equal
to or below
that good move that we found, the overall search can be stopped at
{\em its\/} node, since it can not influence {\em our\/} value anymore. For us, this
child position has become irrelevant as soon as it has been proven
that its value will be lower than the good move that we had
encountered earlier. The subsequent positions are said to be cut
off by the good position that we found and the position that the
opponent found.

This principle of cut offs that are possible due to the intermeshing of
maximization and minimization is said to have been reinvented
independently by several authors, among them 
John McCarthy, Arthur Samuel, Alexander Brudno, Richard, Hart and Levine~\cite{newellcomputer}.


\lstset{label={lst:alphabeta}}
\lstset{caption={alpha-beta code}}
\lstinputlisting[language=Python]{python/alphabeta.py}

\subsection{Alpha-Beta Example}
Let's look at an example which will make this more clear.

In Figure~\ref{fig:abtree} a small tree is show. The root $r$ is a max
node, indicate by the rectagnle shape, the level below the root are
two min nodes, repsenting the two child positions of the player. Each
of these has two child positions (again max nodes) for which the
opponent moves. These are leaf positions (it is a very small
tree). The leaves have
values $3, 6, 2, \cdot$.

Let us start now. alpha-beta starts at the root, with a window
of $\langle-\infty,+\infty\rangle$.  alpha-beta is called with
$n=r, a=-\infty,b=+\infty$. alpha-beta starts at the root node. It finds
this is a max node, and it expands the max node $r$'s first child
$a$. It finds node $a$ is of type min, and alpha-beta expands min node $a$'s first
child, leaf node $c$. Next, alpha-beta finds node $c$ is a leaf node,
adn returns its value $3$. Coming out of the recursion back in node
$a$ alpha-beta updates the variables $g=\min(+\infty,3)$ and
$b=\min(+\infty,3)$ to $3$. It then expands the second child of min
node $a$, leaf node $d$. This node $d$ is expanded with window
$\langle-\infty,3\rangle$, a tighter beta bound. Its value is $6$, coming out of the recursion
back in $a$ alpha-beta updates the variables  $g=\min(3,6)$ and
$b=\min(3,6)$ to $3$, finds no other children at $a$, and returns
$g=3$ to $r$. Back out of the recursion at the root $r$ alpha-beta
updates  $g=\max(-\infty,3)$ and
$a=\max(-\infty,3)$ to $3$. It sees that there is another child $b$,
which it expands with window $\langle 3,+\infty\rangle$, and it
expands the first child of node $b$ with the same window, finding 
leaf node $e$. The value of $2$ is returned to parent $b$, who updates
the variables $g=\min(+\infty,2)$ and $b=\min(+\infty,2)$ to $2$. At this point the
if statement is tested and $3\geq2$ is true, so the break statement
breaks out of the loop, returning the value of $g=2$ to parent $r$,
cutting off the expansion of child $f$. At parent $r$, the root, the variables are
updated to  $g=\max(3,2)$ and
$a=\max(3,2)$ to $3$. alpha-beta is ready and returns $g=3$ to the
caller as the minimax value of position $n$ {\em without having
expanded all nodes of the tree}.

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}
\tikzstyle{max node}=[rectangle,draw,inner sep=9]
\tikzstyle{min node}=[circle,draw,inner sep=2]
\tikzstyle{cut node}=[rectangle,draw,fill,inner sep=5]
\node[max node,label=left:{$r$}](0){$3$}
          child[sibling distance=30mm]{node[min node,label=left:{$a$}]{$=3$}
                         child[sibling distance=15mm]{node[max node,label=left:{$c$}]{$3$}}
                         child[sibling distance=15mm]{node[max node,label=left:{$d$}]{$6$}}}
          child[sibling distance=30mm]{node[min node,label=left:{$b$}]{$\leq2$}
                         child[sibling distance=15mm]{node[max node,label=left:{$e$}]{$2$}}
                         child[sibling distance=15mm]{node[cut node,label=left:{$f$}]{}}};
\end{tikzpicture}
\caption{alpha-beta Example Tree}\label{fig:abtree}
\end{center}
\end{figure}

The impact of alpha-beta on the development of early Chess and Checkers
programs was large. Through this simple algorithmic trick programs could
search twice as deep as before, achieving a much better quality of
play.
\index{alpha-beta}

It should be noted, however, that there is a catch. alpha-beta can
perform cutoffs only if the trees are well ordered. The example tree
in Figure~\ref{fig:abtree} is well ordered: the root has two sub
trees, one with value $3$ and one with value $\leq2$. It just so
happens that hte higest (best) occurred first. If the sub trees had
been ordered the other way around, then node $b$ woudl have been
expanded first, and leaf $f$ woudl have been expanded, along with all
other leaves, arriving ot the same minimax value of $3$. The ordering
of successor positions does not influence the value of the position,
but it does influence the efficiency with which alpha-beta can compute
it.

Thus, much research in move ordering heuristics has been performed. In
Chapter~\ref{chap:idtt} we will devote a whole chapter to these methods,
that were essential for the success of Chess and Checkers programs.

\subsection{*Null Window Search \& MTD($f$)}\index{null window}
Before we go to more heuristics, however, we will look further into
the alpha-beta window. The window is a powerful concept, with which more
efficiency can be gained.
\subsubsection{Postcondition/Bounds}
In addition to searching well ordered trees, there is another way to
improve search efficiecny, and that is  searching smaller
windows. A narrow window causes more cut offs than a window with
wider bounds.

So far we have only used alpha-beta as a routine that searches with a
wide wondow. Can we exploit narrow window to generate more cut offs?

Let us look in more detail at the post condition of the alpha-beta
function. We know that it is supposed to return the minimax value if
it is called with the window $\langle-\infty,+\infty\rangle$. But what
about other windows? What is the meaning of the result of the function
if the result falls outside the window? This is less hypothetical than
it may seem at first sight, since most inner nodes of the tree are
called with an alpha-beta window smaller than
$\langle-\infty,+\infty\rangle$. And in case of a cutoff, their return
value falls outside the window. What is the meaning of this return
value?
\index{alpha-beta postcondition}

The postcondition of $g = \mbox{alpha-beta}(n, \alpha,\beta)$ is as
follows~\cite{knuth1975analysis,plaat1996best}:\label{postcondition}
\begin{enumerate}
\item $\alpha<g<\beta$: $g$ is the minimax value of the tree
rooted in $n$. alpha-beta has traversed at least the critical tree, the
union of a max and a min solution tree.
\item $g\leq\alpha$: $g$ is an upper bound on the minimax value of the tree
rooted in $n$. AlhaBeta has traversed at least the max solution tree
whose value is upper bound $g$.
\item $\beta\leq g$: $g$ is a lower bound on the minimax value of the tree
rooted in $n$. AlhaBeta has traversed at least the min solution tree
whose value is lower bound $g$.
\end{enumerate}

This postcondition allows the construction of the ultimate in efficient
decision procedures: the Null Window Search, or NWS. A null window, of $\alpha =\beta-1$ (we assume
that all values are integer values) guarantees that alpha-beta performs
the most efficient search possible, at the cost of returning only a
boolean answer: the minimax value is either above or below the input
window. Finding the minimax value with the NWS decision procedure
requires a sequence of NWS calls. The literature contains two main
algorithms, Scout, which uses NWS recursively, and MTD($f$), which
uses NWS iteratively.

\subsubsection{Scout}
Scout~\cite{pearl1980scout,reinefeld1989spielbaum}
works on the assumption that the tree is well ordered, and that 
the first child is the principal variation (Scout is also knowns as
Principal Variation Search~\cite{fishburn1982analysis}). Assuming such a well
ordered tree, Scout searches the first child with a 
wide window, and then uses NWS 
to see efficiently if the other children are indeed inferior. If not,
they are searched with a wide window.
Listing~\ref{lst:scout} shows the code.\index{Scout}


\lstset{label={lst:scout}}
\lstset{caption={Scout code}}
\lstinputlisting[language=Python]{python/scout.py}

The re-searches may seem inefficient, and they would be, if alpha-beta
would recompute search results for each search anew. As we shall see
in Chapter~\ref{chap:idtt}, actual game playing versions of alpha-beta
use transposition tables, large lookup tables in which all nodes and their
search resuls are efficiently stored. Re-searching is therefore not
more expensive, since no new  nodes are expanded.

\subsubsection{MTD($f$)}
MTD($f$)~\cite{plaat1996best} takes as input a first
guess to the minimax value, and then 
iteratively calls a sequence of NWS decision procedures to home in on
the minimax value. If the first guess is too high, then NWS will
return a lower bound, which is fed into the next NWS call, until the
minimax value is found and NWS returns an upper bound.  In contrast to
Scout, which uses some wide window searches, MTD($f$) uses only NWS. Experimental
comparisons showed indeed that MTD($f$) expands less nodes than
Scout on average, although trees can be constructed in which either
algorithm performs best~\cite{plaat1996best,plaat1996research}. Even more so than Scout,
MTD($f$) relies  on a well 
functioning lookup table to store intermediate search results in
(Chapter~\ref{chap:idtt}), which requires care with inconsistencies in
the tree, which may be caused by cycles.

Listing~\ref{lst:mtdf} shows the code for MTD($f$).

\lstset{label={lst:mtdf}}
\lstset{caption={MTD($f$) code}}
\lstinputlisting[language=Python]{python/mtdf.py}

\index{MTD($f$)}
MTD($f$) starts the search for the minimax value at a heuristic first
guess, and then iterating in the direction of the minimax value based
on the outcome of the null window search. When the granularity of the
evlaution function is fine, the number of iterations can become large,
and the overhead of traversing through the tree too.

An alternative approach is to use a binary search~\cite{knuth1997art}
to interpolate between the upper and the lower bound, to use that
value as the pivot for the null window search, which will produce a
new bound, and to repeat the binary search. This may result in fewer
iterations of null window search to find the minimax value. This
algorithm is called MTD-bi~\cite{plaat1996best}, the idea of bisecting
the search goes back to \index{MTD-bi}
C*~\cite{coplan1982special,weill1992negac} where it is used in end
game search. MTD-bi is used in Sunfish,
 a tiny fully functional Chess program in 111 lines of Python code.




\section{Practice} 
\subsection{Sunfish---Chess in 111 lines of Python}\label{sec:sunfish}
Chess programs based on heuristic evaluation functions and highly
tuned search function are often large pieces of code. Although there
are many open source programs available that allow study of the code,
the size of the codes requires a large investment of study time. There
are also short programs Chess programs. For example, the program
Micro-Max, by Harm Geert Muller, is a minimalist Chess progam in 133
lines of C code, in less than 2000 characters (not counting
comments). Inspired by this, Thomas Ahle wrote Sunfish, a Chess
program in 111 lines of Python. You can download it from
Github \href{https://github.com/thomasahle/sunfish}{Sunfish}.\footnote{\url{https://github.com/thomasahle/sunfish}} The
entire program is in a single file, \verb|sunfish.py|.
\index{Sunfish}

The program consists of a heuristic evaluation function based on piece
square tables. It uses null window search in MTD-bi, enhanced with iterative
deepening, transposition tables, null moves, and killer moves. These
enhancements are discussed in the next Chapter. Sunfish is small
enough to play around with and study, to learn how a real working
Chess program functions.

The small size and organization of the code also allow easy
modification. Things to try are, for example, changes to the piece
square table, to see the effect on playing style of a different
evaluation function (see the assignments in section~\ref{sec:assignments}). Or taking out search enhancements, such as the
null move or the killer move. Another thing to try out is to replace
null window search by an ordinary wide window alpha-beta
searcher, or by the null window version of SSS* and see how large the
difference is~\cite{plaat1996best,plaat1994sss}. Seeing differences between the full program and the changed
program might actually be subtle. Some changes may only turn up in a large
suite of test positions or after careful analysis of tournament
play. In the next section we shall look at one way to measure playing strength.
\index{SSS*}

Do practice as assignment?


%Small chess program: alpha beta + heuristic eval
%go program? mvgen + ab + eval.
%code on github.
%and gnugo, or hex?
%aim: writing a working program with the knowledge of this chapter,
%which is full width fixed depth plus manual eval. so hex. simple
%or go? will not play well, but will provide code base for mvgen, data structures


\subsection{Playing Strength: Elo}
Playing strength is a proxy for intelligence. Playing strength can be
determined by playing tournaments, and computing a rating based on the
outcome and the strength of the opponent. In board games the Elo
rating is often used. It computes the rating by comparing the rating
of player 1 and player 2. If player 1 has a rating $R_1$ and player 2
has a rating $R_2$ then the expected score of player 1 is
$E_1=\over{1}{1+10^{(R_2-R_1)/400}}$. If the actual score of player 1
was $S_1$ then the new rating of player 1 is
$R_1\prime=R_1+K(S_1-E_1)$ where $K$ is a constant that signifies the
maximum adjustment per game. It is typically set from 16
for master players to 32 for weak players.
\index{Elo rating}

Code for computing the Elo rating is at \href{https://github.com/ddugovic/BayesianElo}{BayesElo}\footnote{\url{https://github.com/ddugovic/BayesianElo}}

Python libraries for computing the Elo rating exist. Just
\verb|pip install bayeselo| and you should be able to use it. 

You can use the Elo rating to compute the strength of the different
programs that you have created in the previous section.



\subsubsection{Exercises}\label{sec:assignments}
\begin{enumerate}
\item Download and install Sunfish and BayesElo for Python. Play your first
game against Sunfish. Write a script that performs a tournament of two
identical instances with the same time controls of
Sunfish. Suggestion: 10 seconds per move.

\item Make a graph with on the $x$ axis the
number of games played (the size of the tournament) and on the $y$
axis the Elo rating of the first program. What do you see? Provide an
explanation.

\item Running tournaments costs compute time. How long should a
tournament be? Add confidence intervals or error bars  to the graph
showing the standard deviation of the Elo rating. 

\item Make a change: halve the playing time of the second player. How
does the Elo rating change?

\item Study the influence of search enhancements and evaluation
heuristics. Perform tournaments between variations of the program. The
baseline is standard Sunfish with all enhancements and all
heuristics. Try the following: Replace MTD-bi by SSS*
(see~\cite{plaat1996best}, SSS* is a loop of null window searches that starts at the
upperbound). Replace MTD-bi by MTD($f$). Replace the null window search by wide window
alpha-beta. Replace the move ordering heuristics: put killer moves last
in the move list that is generated by the move generator.

\item Read Part 1 of Kahneman~\cite{kahneman2011thinking}, on
the Two Systems (less than a hundred pages of easy, enjoyable and
illuminating reading. Part 2 is about
heuristics, but not the kind we have used to in our evaluation
functions). How is the thinking of a computer chess program related to
human thinking? Is alpha-beta like System 1 or Sytem 2? Is heuristics
evaluation like System 1 or System 2?
\end{enumerate}

\section{Summary}
\subsubsection{Fast and Slow}
In this chapter we have covered a lot of ground. We have discussed the
general architecture of the search-eval architecture. We have also
discussed in quite some depth different search functions and different
evaluation functions.

The search functions covered in this chapter
have been conceptually simple, in the sense that they are directly
based on the mathematical definition of a zero sum game: the maximization
and minimization of the reward values.

The evaluation functions are equally simple, and close to a first
order approximation of the heuristics that humans use when playing the
games.

When the early AI researchers such as Turing, Shannon and Samuel discussed
Chess playing computers, they believed to learn about human thought
and to learn about human intelligence. When 40 to 50 years later Deep
Blue finally beat Kasparov, it was said that brute force had won from
human intellect. We had not learned about how humans think, but we had
learned hwo to mke a fast computer search many positions.

The work of psychologist Kahneman can be interpreted to mean that this
is view not true at all. Chess computers think in exactly the same way as
humans. Humans have a fast, heuristic, System 1, and a slow,
deliberative, System 2. Just as Chess computers have a fast heuristics
evaluation function, and a slow planning function, that painstakingly
reasons through some of the possible positions. Humans and computers
think or play Chess in the same way. The search-eval architecture is
not only a good architecture to organize the functions of a chess
program in a clean way, it is also how humans play think. Turing and
Shannon's dream of creating a mechanical model of thought has succeeded
in a great way, and teaches us many interesting aspects of the way in
which we think.

Of course the ``brute force'' argument is not without merit. It is
very true that computers always blindly follow their program, and do
not deviate. Human System 2 thinking is not so perfect, and is easily
distracted by System 1 associations. Indeed, computers can search many more
positions than humans can.

Computer Chess has also thaught
us that computer programming is hard. It has taken four to five
decades of research by a dedicated community of researchers before
machine intelligence has risen to the challenge. Much of this time has
been spent in removing errors from heuristic evaluation functions that
were hard to understand and hard to debug. When looking at the piece
square table of Sunfish, we look at the accumulated wisdom of many
years of study, and the reasons behind the values in the table is not
immeidately obvious if we want to go beyond the concept of more
material is better than less, and center control is advantageous.

Conceptually the way in which computers and humans play chess is
hihgly related. In the details, there are important differences. 

%Thinking Fast and slow:
%give general intro of fast and slow
%this is slow (planning)
%using heuristics

%Do we really want this section in every chapter?


\section*{Historical and Bibliographical Notes}
alpha-beta McCarthy, Russia, Knuth. alpha-beta is a simple depth first
search. Heuristic search distinguishes between depth first, breadth
first, and best first search. 
In 1979 the field of computer chess SSS* was shocked when Stockman
introduced a procedure that was said to be best first~\cite{stockman1979minimax}. It was
subsequently studied by many
researchers~\cite{pearl1980scout,pearl1984heuristics,ibaraki1986generalization}. 15 years later
 a straightforward relation between alpha-beta and SSS*,
between depth first and best first minimax was published~\cite{plaat1995best}. The concept of solution
trees, introduced by Stockman, and null window alpha-beta searches play
an important role~\cite{de1994solution,plaat1996best}, this work also
introduced MTD($f$)~\cite{plaat1995best} and showed how SSS* can be
implmented in game playing programs.


First open source program Crafty~\cite{hyatt1997crafty}.
Parallel Cilkchess~\cite{leiserson1998programming}.
Fruit is an influential open source program by Fabien Letouzey, GNU
Chess is now based on Fruit~\cite{fruit}.

In many board games the Elo-rating is calculated,
a system devised by the Hungarian-American physicist  Arpad Elo based
on pairwise comparison \cite{elo1978rating}.


The \href{https://www.chessprogramming.org/Main\_Page}{Chess programming wiki} contains a wealth of information on how to
write your own Chess program.~\footnote{\url{https://www.chessprogramming.org/Main_Page}}

%
% \section{Challenge}
%
% Understand Alphabeta and solution trees
%
% Critical Tree is proof tree
%
 


==> chapters/07supervised__Aske___s_MacBook_s_conflicted_copy_2019-02-16_.tex <==
{\bf this chapter is light on juicy content. more should be added,
  about the theory why deep learning is so hard, and on overfitting.}


This chapter shows how deep networks can learn layered
representations. we briefly introduce supervised learning, a basic machine
learning technique for generalizing state representations.
%% The {\bf problem} of this chapter is function approximation: 
%% can features be found automatically to provide a reliable
%% representation or categorization, even for unseen states?

This chapter provides an answer to the problem of  how to find the determining features of a
high dimensional and large state space, so that their value can be
generalized. Finding a good value function for a state space so large
that not all states can be seen is a challenging generalization
problem.

The learning goals of this chapter are to understand how we can
compute approximations of states of which most have not have been encountered
while training, simply because the state space is so large. This will
be accoplished through feature generalization. We will
look at deep learning and representation at multiple levels, at
feature recognition, and at error functions and backpropagation. We
will discuss building blocks such as convolutions and residual
networks, we will look at examples of specific network architectures such as
AlexNet, and we will discuss tools such as TensorFlow and Keras.

%% \section*{Learning Goals}
%% \begin{itemize}
%% %\item {\bf It is exciting to learn about the deep learning history. full of emotion, AI breakthrough. now we know how to keep the learning from overfitting, to keep it in place}
%% \item general function approximation, neural net, feature recognition
%% \item deep neural net: multi level representation abstraction
%% \item supervised learning; error function, back propagation, SGD
%% \item 2012 AlexNet, convolution net, ResNet
%% \item Tensorflow, Keras
%% \end{itemize}
The previous chapters covered exact planning methods. The emphasis was
on search algorithms, and evaluation was  treated as a heuristic black box,
in the sense that it was up to the programmer to handcraft top down heuristic
functions based on knowledge of the domain. If there was learning,
then at most the weights of handcrafted heuristic features were
learned.

Around the change of the millennium advances in computing power in CPUs
and GPUs
made it feasible for researchers to consider learnign of end-to-end training of raw,
unpreprocessed inputs data.


In this chapter we will turn to learning those heuristic features
bottom up from data. We will be 
concerned with value functions, generalization, 
features, neural networks, state evaluation, and training and learning.

%% In this chapter we will first start with supervised learning, in the following chapter
%% we will turn to function approximation in reinforcement learning.

Learning is the adaptation of behavior from experience. Supervised
learning is concerned with learning an input/output mapping, to
categorize input data into a number of output categories. Supervised
learning is closely related to generalization, which is the
identification of common properties in instances of data. When we
perform a generalization, we  extract the essence of a concept based
on similarities with other objects. By finding commonalities we
simplify  many instances into fewer,  higher-level, concepts. These
concepts are more abstract, or general, than the many lower level
instances. 
In the context of AI and generalization, the commonalities are usually
called features, and finding the higher level abstractions is called 
representation learning~\cite{lecun2015deep}. It is one of the 
core technologies used in function approximation.

\section*{Core Concepts}
\begin{itemize}
\item Value Function by Generalizing Features
\item Layered Representations in Deep Networks
\item Generalization, CNN, Vanishing Gradients, ReLU, Batch Normalization
\item Overfitting, Dropouts
\end{itemize}

%\section{Deep Learning}
\section{Supervised Learning}\index{supervised learning}\index{neural
  network}\index{function approximation}
Towards the end of Chapter~\ref{chap:rl}, in section~\ref{sec:approx}
we discussed ways to approximate functions when the state space
becomes so large that it becomes unlikey that states will have been seen
before in training. Statistical learning theory provides a framework for machine
learning methods such as supervised learning and reinforcement
learning~\cite{russell2016artificial,friedman2001elements}. Supervised
learning learns a function from
an explicit set of labeled training
data. For example, the training set may be a set of pictures, labeled
with a description, such as {\em CAT\/} or {\em DOG}.\footnote{In reinforcement
learning there is no explicit training set, but the training is achieved through
interaction with an environment, that returns positive or negative rewards when an action
is taken in a state (see Chapter~\ref{chap:rl} and~\cite{sutton2018introduction}).} 

Supervised learning is a basic and widely studied problem in
artificial intelligence. A wide range of algorithms exist for
supervised learning: Support Vector Machines, linear regression,
Bayesian classification, decision trees, random forests, nearest
neighbor, and artificial neural networks, to name just a
few~\cite{russell2016artificial}. 

Since around 2010 artificial neural networks have achieved
impressive results in image recognition, speech recognition, and game
playing. 

The next chapter covers function approximation in reinforcement
learning. Many of the techniques are from supervised learning, and can
be easily understood with the supervised learning paradigm. Therefore, in
this chapter we start with supervised learning techniques.

\subsubsection{Training Set and Test Set}\index{overfitting}\index{underfitting}\index{training
  set}\index{test set}\label{sec:trainset}
A standard method in machine learning to test how good an 
algorithm can categorize a data set is to divide the data set in a
training part and a test part~\cite{bishop2006pattern}. A typical
split is 90\% of the data for the training set, and the remaining 10\%
for the test set. The algorithm
is allowed to train on the training part. The
quality of the algorithm is then tested on the remaining (unseen) 10\%
to see how well it generalizes. If the percentage of correct
predictions on the test set is about the same as on the training set,
then the  algorithm generalizes well to the test set. If not, the training
may have underfitted or overfitted.


\subsubsection{Feature Recognition}
Function approximation was introduced in Chapter~\ref{chap:rl} for
large state spaces. Its purpose is to learn generalizable state
representations that work well even when is is unlikely that states have been
seen during training. Deep neural networks are a popular approximation
method.
We have  seen that deep nets perform feature recognition through a
layered hierarchy of increasingly abstract 
representations~\cite{hinton2006fast,lecun2015deep}.



In Chapter~\ref{chap:search}, heuristic value functions were
introduced as a way to search the large state spaces of Chess and
Checkers (section~\ref{sec:eval}). 
The difference is that the
features in the Chess evaluation function are manually designed
heuristics, combined in a linear function whose coefficients are
manually tuned, whereas the features in a deep net are trained
(generalized) on a large set of examples in an automatic training process.

From a
scientific point of view, the hand
crafting and hand tuning is much less reproducible than the training
of deep function approximators by stochastic gradient descent. Furthermore, and
most importantly, the hand crafted heuristics do not generalize well
to other domains, whereas deep  feature recognizers have been
shown to work well in many domains. (Although each time the network
archictecture has to be adapted to the domain, which is a non-trivial
manual operation.)


\subsection{Shallow Network}
Figure~\ref{fig:nn} show a simple neural network, with an input layer,
an output layer, and a shallow hidden layer.
Artificial neural networks have achieved recent fame through the
success of deep learning. However, neural networks have a long history,
and much work has been done, before success happened. Already in 1943 McCulloch and
Pitts~\cite{mcculloch1943logical} provided a computational model for
neural networks.
The history of development of neural networks is quite interesting and
rich, with high ups and deep downs. Training neural networks is
not trivial, and many years of research were necessary to achieve the
current day impressive results. Section~\ref{sec:bib:neural} provides
some pointers to background papers.

\begin{figure}[t]
\begin{center}
\includegraphics[width=5cm]{figures/shallownet}
\caption{Neural Network}\label{fig:nn}
\end{center}
\end{figure}
%% The basic approach to train a neural net is as follows. Examples are
%% shown to the net and coded in the input layer, values are propagated through
%% the hidden layers to the output layer, where the results are compared to
%% the output labels. An error is computed, and it is propagated back through
%% the network to the input layer, allowing the calculation of
%% derivatives for the adjustment of the weights of the
%% layers. The propagation of the errors is called
%% backpropagation, and is part of the gradient descent algorithm to
%% update the weights in the training of the network~\cite{goodfellow2016deep}.

Much work has been done to formulate this backpropagation
algorithm~\cite{werbos1974beyond}. It allowed the training of
multi-layer networks, paving the way for deep learning's success.
%% (again, getting deep networks to work well took a lot of hard work, see the
%% references to the literature). 



%\section{Algorithms}

\subsubsection{Algorithms}\label{sec:algo}\index{backpropagation}\index{SGD}
We will now discuss the networks and training algorithms in more detail.

%\subsubsection{Weights, Backpropagation, SGD}
The neural network consists of neurons and connections, typically
organized in layers (see Figure~\ref{fig:nn}). The neurons
consist of a function that processes their input signal, producing an output
signal.  This function is called  an activation function. Popular
activiation functions are the rectified linear unit (ReLU: partly
linear, partly zero), the hyperbolic tangent, and the
sigmoid or logistic function $\frac{1}{1+e^{-x}}$ (these will be
discussed in more detail shortly). The connections
between the neurons are called the weights. Weights are summed at the
input of the neurons $\sum_i o_iw_{ij}$ for input $j$ of output $o_i$ of
predecessor neuron $i$.

When training starts, the weights of the
network are initialized to small random numbers. The network is
then  exposed to the training examples. The examples are pairs, such
as pictures and labels. The input layer is exposed to the input
(the picture), which is propagated through the network to the output
layers, using the weights and activation functions. At the output
layer the propagated value is compared to the other part of the 
example pair, the label. The difference with the label is calculated, yielding
the {\em error}. Then, in the backward phase, this error is propagated back
to the input layer, adjusting the weights in the direction so that the
error becomes smaller. This method uses the gradient over the weights,
and is called backpropagation.

Most neural nets are trained using a stochastic
version of backpropagation, stochastic gradient descent, or
SGD~\cite{song2018mean}, that does not compute the gradients in the
order of the samples in the training set, but shuffles them. Popular
variants of SGD are AdaGrad~\cite{duchi2011adaptive} and
Adam~\cite{kinga2015method}, methods that adaptively change the
learning rate and momentum of the backpropagation.


\begin{figure}[t]
    \centering{\includegraphics[width=6cm]{figures/leelayers}
     \caption{Deep Layers\cite{lee2009convolutional}}\label{fig:leelayers}}
\end{figure}

\subsection{Deep Network}\index{deep learning}\label{sec:deepnetwork}
{\bf hier dus toevoegen hoe moeilijk het wel niet was. CNN nodig, deep
  learning, backprop, vanishing gradients, overfitting. Eigenlijk
  staat het er allemaal wel, maar het is te kort en te makkelijk}
Some functions can
only be represented compactly with an architecture of at least a
certain
depth~\cite{bengio2009curriculum,bengio2007greedy,haastad1991power}.
For complex tasks such as image recognition  shallow
networks do not perform well, or need pre-processing with handcoded
feature recognizers.  A breakthrough in end-to-end (direct image) recognition was
achieved only when deep networks  were being used, and ways 
were found to train them. This breakthrough created a surge of
interest into neural nets and deep learning.

In deep learning, each layer  transforms its input data into a
 more abstract  representation.
The  hierarchy of network layers can more easily 
recognize a hierarchy of low to high level
concepts~\cite{lecun2015deep,lee2009convolutional} (see
Figure~\ref{fig:leelayers}). In 2006 Hinton et al.~\cite{hinton2006fast} 
published work on efficiently learning 
a high-level representation using successive layers of variables in a
restricted Boltzmann machine. Later, researchers
were able to  create multi level networks that
learned to recognize high level concepts such as cats from watching
unlabeled images from Youtube videos~\cite{le2012building}.


%% Although a single hidden layer in theory is enough to approximate  any
%% function, in practice, 

After  impressive results in 2012~\cite{krizhevsky2012imagenet},
LeCunn, Bengio and Hinton 
recently published an overview  paper on deep learning~\cite{lecun2015deep},
explaining in detail how multiple hidden layers in networks learn increasingly
abstract representations. For example, in face recognition (see
Figure~\ref{fig:leelayers}) the first hidden layer may 
encode edges; the second layer then composes and 
encodes simple structures of edges; the third layer may encode higher
level concepts such as nose or
eyes; and the fourth layer works at the abstraction level of a
face. Note that deep feature learning finds what to abstract at
which level on its own~\cite{bengio2013representation}. 
Especially in image and speech recognition impressive results have
been reported by deep
networks~\cite{bengio2009learning}. Section~\ref{sec:zflayers} goes
deeper into the features of deep layers.

For deep learning to work, a
number of problems had to be solved, that we will now discuss.

\subsection{Generalization}
The universal appoximation theorem states that a feed forward network
with a single hidden layer can approximate a wide variety of
interesting continuous functions. However, the theorem does not give
an indication on how easy it is to learn this
representation~\cite{cybenko1989approximations}, and some complex functions can
only be represented compactly with an architecture of at least a
certain depth. Therefore multi level networks,  or deep networks, are
used.

\begin{figure}[t]
  \centering{\includegraphics[width=8cm]{figures/mnist}\caption{MNIST images}}\label{fig:mnist}
\end{figure}

Standard  MNIST images are low-resolution $32\times 32$ pixel images
of single handwritten digits (Figure~\ref{fig:mnist}). 
To achieve higher accuracy, and to process more complex scenes,
researchers looked to grow the networks in size and complexity. This can be done in
three ways. First, the width of the network can be increased, by
having more neurons in each layer. Second, the depth of the network
can be increased, by having more layers. And third, the complexity of
the network can be increased, by using a more complex type of
processing at the neurons, a different interconnection structure, or
different training schemes.

As might be expected, all three were necessary, and in unexpected and
non-trivial ways.

\subsubsection{Width Increasing: Slow learnign and Overfitting}



\begin{figure}[t]
  \centering{\includegraphics[width=8cm]{figures/overfitting}\caption{Overfitting:
    Which line captures the Essence of the Data best?}}\label{fig:overfitting}
\end{figure}

Simply increasing the width of a fully connected network is
not a scalable solution. More width creates three problems. First, it
causes a quadratic increase of the number of weights, and 
the same holds for the training time. The training time becomes
unacceptably long. Second,  overfitting becomes
a problem, since after increasing the capacity of the network, the
number of parameters may become 
greater than the number of observations, and the network will
overfit. Figure~\ref{fig:overfitting} illustrates overfitting, which will
be described more fully in Section~\ref{sec:overfitting}.
Third, only increasing the width does not address the problem that some
complex functions can only be approximated with a network of 
a certain depth~\cite{bengio2009curriculum,bengio2007greedy,haastad1991power}.


cnn feature extraction. locally connected, recognizes local features
fcn classification. globally connected, finds global classes


\begin{figure}[t]
  \centering{\includegraphics[width=8cm]{figures/layers}\caption{Increasing
      number of Layers}}\label{fig:layers}
\end{figure}

\subsubsection{Depth: Preventing Exploding Number of Weights}
Increasing the width of a fully connected network runs into problems
since the number of weights explodes (or rather, increases quadratically).
Let us look what happens when we increase the depth of the network.

As 
the depth increases, the number of weights increases linearly (see
Figure~\ref{fig:layers})  and so does the
training time. The overfitting problem also increases
linearly. However, complicated functions  can be approximated better by
the deeper network. 


Therefore, it seems that increasing the  depth of the network is the
way forward. This is indeed the case, but it does not solve all our
problems. 
If we want to approximate a function, especially one with a high
dimensional input such as a higher definition image, then at least our input layer has
to have a corresponding number of inputs. For high dimensional  input
we simply have to build a network with at least wider lower  
network layers, in combination with deep
layers to be able to reacognize complex composite
representations and to reduce the weight explosion as much as
possible. So, it we still have not solved the problem of exploding
numbers of weights of fully connected networks learning slowly and
generalizing badly. 

\subsection{Convolution Neural Nets}\index{convolutional network}\index{CNN}

The solution lies in the third element: using a more complex type of
processing at the neurons, a different interconnection structure, and
different training schemes. 

Convolutional neural nets take their inspiration from biology. The
visual cortex in animals and humans is not fully connected, but
locally connected.

\subsubsection{Local Connectivity, receptive field}
Local connectivity: following the concept of receptive fields, CNNs
exploit spatial locality by enforcing a local connectivity pattern
between neurons of adjacent layers. The architecture thus ensures that
the learned "filters" produce the strongest response to a spatially
local input pattern. Stacking many such layers leads to non-linear
filters that become increasingly global (i.e. responsive to a larger
region of pixel space) so that the network first creates
representations of small parts of the input, then from them assembles
representations of larger areas.

By connecting only locally, the number of weihgts is dramatically
reduced in comparison to a fully connected net. The recognition
ability of CNNs is less, and this is where deep stacks come into
play. By stacking convolutional layers on top of each other, they can
recognize and represent increasingly complex concepts.


\subsubsection{Weight-Sharing in CNN. Reduce Capacity, Reduce
  Overfitting, go deep, complex composed functions, hierarchical
  represenations}

If local connectvivty was not enough there is a second weight
reduction element in CNN: weight sharing.

cnn translates width to depth. deep not possible with FCN.
CNN does weight sharing and does small translations, per
layer. anchoring optim to small changes, weight sharing very
important to prevent overfitting
 
problem is too many connections, too many weights.

w/ cnn can get deeper. + less overfitting due to weight sharing. +
locality of reference. width, height

can we substantiate this?

3D volumes of neurons. The layers of a CNN have neurons arranged in 3
dimensions: width, height and depth. The neurons inside a layer are
connected to only a small region of the layer before it, called a
receptive field. Distinct types of layers, both locally and completely
connected, are stacked to form a CNN architecture.



\subsubsection{Shared Weights} 
Shared weights: In CNNs, each filter is replicated across the entire
visual field. These replicated units share the same parameterization
(weight vector and bias) and form a feature map. This means that all
the neurons in a given convolutional layer respond to the same feature
within their specific response field. Replicating units in this way
allows for features to be detected regardless of their position in the
visual field, thus constituting a property of translation invariance. 
 



\subsubsection{CNN}
Convolutional neural nets (CNN) are an integral part of the deep learning
revolution~\cite{lecun1989backpropagation}. CNNs are inspired by the biological process of visual 
processing. The connectivity pattern of CNNs resembles the animal
visual cortex~\cite{hubel1963shape,matsugu2003subject}. A CNN consists
of a convolutional operator or filter. A tyical convolution operator
has a small {\em receptive field\/} (it only connects to a limited number of
neurons, say $5\times 5$) whereas a fully connected neuron connects to
all neurons in the layer below. CNNs thus work as small local
transformations, such as translations or rotations. A CNN layer can be
seen as a set of learnable 
filters (or kernels)~\cite{goodfellow2016deep}. Also, the weights of the links are
shared, resulting in a large reduction in the number of weights that
have to be trained. This is a significant advantage of CNNs, since the
computational requirements of training the weights of many fully
connected layers would be prohibitive. 

CNNs work well in image recognition tasks, for visual filtering
operations in spatial dependencies, and for feature recognition
(edges, shapes)~\cite{lecun1989backpropagation}.
For recognition tasks with temporal dependencies, such as in speech or
text recognition, other networks have been developed. Long Short Term
Memory (LSTM) has been introduced by~\cite{hochreiter1997long}, and
recurrent neural nets (RNN) by~\cite{goller1996learning}.\index{LSTM}\index{RNN}

\subsubsection{Max Pooling}\index{max pooling}
An operation related to convolving is pooling. Pooling is a kind of
non linear down sampling.  Typically, a $2\times 2$ block is down sampled to a scalar
value. Pooling reduces the dimension of the
network. The most frequently used is max pooling. It
is an important component for object
detection~\cite{cirecsan2012multi}.

\subsubsection{CNN solves all: deep representations, efficient computation}

why deep? because big pictures too many weights. increases quadratically. impossible to learn fcn
so need alternative from fcn with fewer weights (and if it would, it
would learn too much noise). idea: look at biology. cnn has local
connections, very few connections, acts like filter. Filters can be
stacked in layers, weights increases linearly. filters learn small
translations. They share weights, very weight efficient, shared
weights very low overfitting, and generalizes translations over the image. computationally
feasible, less overfitting. And it turns out to learn intermediate
representations. (small learning steps, edges, circles)
Also theory argument that need certain depth for learning complex
functions.
The architectural structure forces learning into limited type of
learning, which turns out to work when stacked. (it is efficient, and
when stacked, and combined with small FCN, it generalizes translations
and learns categorization)


Traditional multilayer perceptron (MLP) models were successfully used
for image recognition.[example needed] However, due to the full
connectivity between nodes they suffer from the curse of
dimensionality, and thus do not scale well to higher resolution
images.

A 1000×1000 pixel image with RGB color channels has 3 million
dimensions, which is too high to feasibly process efficiently at scale
with full connectivity. 

FCN not generalizing, structure forces optim in certain
direction. Too many choices for optim not good.
CNN, is generalizing self tuning filter for small changes.

CNN shared weights

The convolution operation brings a solution to this problem as it
reduces the number of free parameters, allowing the network to be
deeper with fewer parameters

receptive field
by reducing number of weights can be deeper. CNN have allowed deep
networks. and: lower capacity: overfitting resolved
and: shared weights same translations.

neocognitron 1980 fukushima
receptive field + down sampling

breakthrough after gpu impl: 2004


\subsection{Vanishing Gradients}
\subsubsection{Vanishing gradients}\index{vanishing
gradients}\index{batch renormalization}
The vanishing gradient problem was one of the problems that have held
back progress in multi level neural 
networks for some time. Multiple solutions to this problem have been
found. One solution  is to model the network as a
multi level hierarchy of networks pre trained on level at a
time~\cite{schmidhuber1992learning}.  Also, Hinton's work on deep
belief networks addresses this
problem~\cite{hinton2006fast}. Batch renormalization periodically normalizes the
weights~\cite{ioffe2017batch}. Finally, the ReLU activiation function
is less susceptible to the vanishing gradient problem.

\subsubsection{What is it? sigmoid and backpropagation}
Hochreiter

http://neuralnetworksanddeeplearning.com/chap5.html
 Gradient flow in recurrent nets: the difficulty of learning long-term
 dependencies
 
 the gradient tends to get smaller as we move backward through the
 hidden layers. This means that neurons in the earlier layers learn
 much more slowly than neurons in later layers.

 More generally, it turns out that the gradient in deep neural
 networks is unstable, tending to either explode or vanish in earlier
 layers. This instability is a fundamental problem for gradient-based
 learning in deep neural networks.

 might the small gradient in early layers of a deep network mean that
 we don't need to do much adjustment of the weights and biases?

 What's causing the vanishing gradient problem? Unstable gradients in
 deep neural nets.

 The derivative of sigmoid reaches a maximum at σ′(0)=1/4. So all get
 smaller and smaller deeper down, since derivative of sigmoid is max
 .25

 As we've seen, such terms are typically less than 1/4
 in magnitude. And so the gradient ∂C/∂b1
 will usually be a factor of 16
 (or more) smaller than ∂C/∂b3
 This is the essential origin of the vanishing gradient problem.

long  product of many layers yields low value at deep layer.



The problem is that in some cases, the gradient will be vanishingly
small, effectively preventing the weight from changing its value.
As one example of the problem cause, traditional activation functions
such as the hyperbolic tangent function have gradients in the range
(0, 1), and backpropagation computes gradients by the chain rule. This
has the effect of multiplying n of these small numbers to compute
gradients of the "front" layers in an n-layer network, meaning that
the gradient (error signal) decreases exponentially with n while the
front layers train very slowly.

gradient descent cannot learn long range



\subsubsection{ReLU, residual, LSTM, multi-level hierarchy of
  networks}

\subsubsection{batch normalization}
speedup training, reduce overfitting, reduce vanishing gradient

\subsubsection{ReLU}\index{ReLU}
Traditionally the activation function of neurons is a well
differentiable function such as $\tanh$ or the sigmoid function
$\sigma(x) = \frac{1}{1+e^{-x}}$. For CNNs the ReLU (short for
rectified linear unit) is often used: $f(x)=\max(0,x)$. Over the positive part of
its input ReLU is linear, otherwise it is zero. ReLU is a simple
function that is quick to calculate, is
non linear, and removes negative values from the activations~\cite{krizhevsky2012imagenet}.




\subsection{Overfitting}\index{dropouts}\index{regularization}\index{overfitting}\label{sec:dropouts}\label{sec:overfitting}



\subsubsection{Overfitting is putting the noise before the signal}
wider and deeper gives exploding number of weights.
problem with too many parameters is twofold: computation overhead;
overfitting freedom. the seen training set may not be a perfect
generalizer of essence for test set

overfitting is you fit the noise in the training set, not the signal
The essence of overfitting is to have unknowingly extracted some of the residual variation (i.e. the noise) as if that variation represented underlying model structure



the network can memorize
the training data, perfectly modeling the noise with the signal  in
the training set, an extreme case of the noise drowning out the
signal.
\subsubsection{Overfitting is putting the noise before the signal,
  fitting too complex a fucntion to the data, possibly creating more noise}
Since the number of weights in
deep networks is often in the millions, it is typically greater than the
number of observations. In such a situation overfitting is a problem
that reduces the generality of the network.
Overfitting is said to have happened when a trained model corresponds
too closely to a particular 
data set, and therefore fails to reliably predict a future
observation. The network has been fitted to the particular training set, not the underlying
structure of the data. Therefore, the model fits the
training data set, but fails on the test set. Overfitting occurs frequently when a model has
more parameters than the data set has observations. 

https://towardsdatascience.com/preventing-deep-neural-network-from-overfitting-953458db800a
\subsubsection{Dropout}

\subsubsection{Early stop}

\subsubsection{Batch Renormalization}

\subsubsection{Capacity reduction}

\subsubsection{L1 or L2 regularization}



Much of the neural network research is aimed at reducing overfitting,
through regularization. One (crude) method is to stop the training of the
network early. Another way is to reduce the number of
parameters in the network, so that it can hold less information. This
is also called reducing the capacity of the network. A related method
that is often used is
dropout~\cite{hinton2012improving,srivastava2014dropout}. With this
method a certain percentage of neurons is stochastically dropped
during backpropagation. Dropout is an effective method to reduce
overfitting~\cite{goodfellow2016deep}.




\section{ImageNet, TensorFlow: Datasets and Networks}
%\subsection{Data Sets}
Datasets have been of great importance to the progress of supervised
learning. The algorithmic advances that were discussed in
Section~\ref{sec:algo} were facilitated by the availability of large
training sets  of labeled training examples.
A well known  repository of  data sets is
the University of California at Irvine Machine Learning
repository~\href{https://archive.ics.uci.edu/ml/index.php}{UCI}.\footnote{\url{https://archive.ics.uci.edu/ml/index.php}}\index{UCI}

MNIST may well be the best known of these data sets. MNIST
is a database of 60,000 handwritten digits provided by the National
Institute of Standards and Technology. The original MNIST database is
available at \href{http://yann.lecun.com/exdb/mnist/}{MNIST}.\footnote{\url{http://yann.lecun.com/exdb/mnist/}}\index{MNIST} 
Another major data set  is ImageNet.\index{ImageNet}
ImageNet is available at \href{http://www.image-net.org}{ImageNet}.\footnote{\url{http://www.image-net.org}}
It is a collection of more than 14 million URLs of images that have
been hand annotated with what objects are in the picture. It contains
more than 20,000 categories. A typical category contains several
hundred training images. Since 2010 ImageNet runs an annual software
contest, the ImageNet Large Scale Visual Recognition Challenge
(ILSVRC)~\cite{deng2009imagenet}. Since 2012 ILSVRC has been won by deep
networks, starting the deep learning boom in science and industry.

We will now mention some influential networks architectures.

%\section{Networks}

\subsubsection{LeNet-5}
Towards the end of the 1990s the work on neural networks moved into
deep learning, a term coined in~\cite{dechter1986learning}. Early work
on monkey and cat visual cortexes indicated neurons that respond to
small regions in the visual field~\cite{hubel1963shape,hubel1968receptive}. After the
introduction of deep convolutional neural nets by LeCun et
al.~\cite{lecun1998gradient} CNNs became highly popular. This paper
introduced the architecture LeNet-5.\index{LeNet-5} LeNet-5 is a 7
layer convolutional neural net trained to classify handwritten digits
from $32\times 32$ pixel images from MNIST. It is a successful network that was
used commerically to recognize digits in banking checks. The paper
also has a thorough comparison of LeNet-5 to other methods such as
PCA.\index{CNN}\index{convolutional network}\index{MNIST}\index{Keras}


A Keras implementation of LeNet (and of AlexNet  and VGG) is available
at
\href{https://github.com/eweill/keras-deepcv/tree/master/models/classification}{Models Keras}.\footnote{\url{https://github.com/eweill/keras-deepcv/tree/master/models/classification}} The code straightforwardly lists the layer definitions, shown in
listing~\ref{lst:lenet}.


\lstset{label={lst:lenet}}
\lstset{caption={LeNet code~\cite{lecun1998gradient,weill}}}
\lstinputlisting[language=Python,float]{python/lenet.py}

\subsection{AlexNet}\index{AlexNet}\index{GPU}
In 2012 Krizhevsky et al.\ published
the AlexNet architecture~\cite{krizhevsky2012imagenet} with
breakthrough performance on the ImageNet dataset. They  used a deep
network of 8 layers. The first 5 layers were convolutional layers,
some with max pooling, and 3 layers were fully connected
layers. Krizhevsky et al.\ overcame problems of vanishing 
gradients and overfitting, and effectively used the power of
GPUs to train a large network. Their work created many follow up works 
showing even better performance, and attracted much attention, setting
off the general interest in deep learning.

Deep networks have since grown in size, with many more layers, and
different learning algorithms and connection structures. The number of weights in
such networks is often in the millions, greater than the number of observations on
which the network is trained. This makes it  easy for the network
to overfit. Overfitting is for the network to match precisely the
training data set, but fail on the test data set, since it fails to
generalize to fit additional data or to predict future observations
well.

%% Much of  neural network research is aimed at regularization,
%% to reduce overfitting~\cite{goodfellow2016deep}.\index{overfitting}





\subsection{TensorFlow}\index{TensorFlow}\index{GPU}\index{Torch}\index{Theano}\index{Caffe}\index{Keras}


%\subsection{GPU, Tensorflow, Keras}
Another crucial factor in the deep learning breakthrough is the
availability of computational power. GPUs have been originally
developed for fast processing of image and video data. GPU development
has been largely driven by the video gaming industry. Modern GPUs consist of
thousands of processing units optimized to process linear algebra matrix operations
 in parallel~\cite{sanders2010cuda,liu2012sparse,oh2004gpu,cirecsan2010deep,sze2017efficient,song2014scaling}.

Matrix operations are at the basis of image processing and neural
network training. Many neural network training packages support
GPUs. Well known dedicated deep learning packages are
Caffe~\cite{jia2014caffe}, Torch~\cite{paszke2017automatic}, Theano~\cite{bergstra2011theano}, Tensorflow~\cite{tensorflow2015whitepaper,abadi2016tensorflow}, and
its user friendly add-on Keras~\cite{chollet2017deep}. Most packages have Python interfaces. Some machine learning and mathematical
packages also offer deep learning tools, such as Matlab and R. 

The free availability of these packages has stimulated progress in deep supervised learning  in
deep reinforcement learning (Chapter~\ref{chap:dqn}) and in self play
(Chapter~\ref{chap:plan}). TensorFlow provides high quality
implementations of many machine learning and neural network algorithms
and operations.  (A
tensor is a  multi dimensional array, often used for transformations.)
The programming concept of
TensorFlow takes some getting used to.  Programs are constructed as a dataflow
graph in which the sequence of tensors defines the operations. A
higher level, easier, interface is provided by Keras. Keras comes with
TensorFlow. It is recommended to start with Keras.





\section{Practice}\index{keras}\label{sec:keras}
Let us start with some exercises. 
First make sure that Python is installed on your computer (see
Appendix~\ref{chap:python} or \href{https://www.python.org}{Python}).\footnote{\url{https://www.python.org}}
When you have Python installed, go to the TensorFlow page at
\href{https://www.tensorflow.org}{TensorFlow}.\footnote{\url{https://www.tensorflow.org}} Tensorflow allows easy
experimentation with deep function approximators. Of many of the
algorithms of the field high quality implementations exist, including
GPU versions. Tensorflow is a large and extensive software
package. Learning it would take quite some time. Keras is a more
userfriendly interface that runs on top of Tensorflow. The assignments
below are meant to be done in Keras.

\subsubsection{Exercises}
\begin{itemize}
\item Download and install Tensorflow and Keras. Check if everything is
  working by executing the MNIST training example. Run it on a
  training set, and then test the trained network on a testset. How
  well does it predict?
\item Which optimizer does the example use? Use ImageNet. Try a different optimizer,
  such as Adam or simple Backprop.
\item What is the effect of a different learning rate? Does
  performance increase?
\item How fast is your training going? Are you working on a laptop or
  do you have a high power CPU/CPU combo? Would you like more? The Cloud provides ample
  compute power at cheap prices, often with free sign up bonuses. Go
  to AWS, the Google Cloud, or Microsoft Azure, and explore ways to
  speed up your learning.
  \item One of the biggest problems of supervised learning is
    overfitting. Create an experiment in which you force overfitting
    to occur. What will you do: change the algorithm (change cnn,
    relu, dropout) or change a parameter (learning rate, dropout
    percentage)? How can you see if overfitting has occurred? When has
    it reduced?
\end{itemize}


\section{Summary}
%{\bf central concept: approximate method: deep learning generalizes better features than hand crafted}
In this chapter we introduced our first methods for function
approximation. The field of function
approximation (or neural networks) is large, rich, and deep. This
chapter can only give a glimpse of the work that has been
done. However, such a glimpse is necessary because of the important
role that function approzimation plays in reinforcement learning.

The goal of function approximation is to find a reliable value
function for large state spaces, so large, that test examples will not
be seen during training. In this way, the function approximators of
this chapter are an alternative tio the heuristic feature function of
chapter~\ref{chap:search} and the average random values of
chapter~\ref{chap:trial}.

We have discussed how supervised learning provides a simple paradigm
of learning by example. We have discussed how the representation power
of networks can be improved by deep hierarchies of layers of
neurons. The trained deep layers of features replace the hand crafted heuristic features Training these deep networks is not trivial, and many
techniques have been discussed, from vanishing gradients (ReLU, batch normalization), to dropouts (to prevent
overfitting), to convolutional layers (to both reduce the number of
weights and allow efficient translations and rotations), and we have
of course covered training methods such as SGD and its variants.

Function approximation has blossomed when large labeled data sets
became available {\em and\/} when the necessary computational power in
the form of GPUs arrived. In addition to the data sets, easy to use
free software packages such as Tensorflow and Keras have lowered the
barrier of entry for researfch significantly, and have played a large
role in the success of the field.


\subsubsection{Fast and Slow}
This has been the first chapter of the part on learning. In it, we discussed
how generalization in neural nets can create function
approximators. These function approximators encode learned knowledge,
learned features, just as the heuristics did in the part on
planning. If we look at Kahneman's System 1 (thinking fast) and System
2 (thinking slow), then the using function approximators is like
Thinking Fast. Function approximators act fast, like reflexes,
providing  quick answers delivered by
association or lookup. This is in sharp contrast to planning, which
provides exact answers through tree traversal. System 2's thinking
slow performs  reasoning.



\section*{Historical and Bibliographical Notes}\label{sec:bib:neural}
In 1958 Rosenblatt~\cite{rosenblatt1958perceptron}
introduced the perceptron, a simple neural network for pattern
recognition. An key element of neural networks is how to train
them. Training consists of a forward and a backward phase. In the
forward phase an input is shown to the network, which then calculates
an output based on the weights and activation functions. At the output layer,
the difference with the label is calculated, the {\em error}. In the
backward phase, this error is propagated back to the input layer,
adjusting the weights in the direction so that the error becomes
smaller~\cite{bengio2012practical}.


Much work has been done to formulate this backpropagation
algorithm~\cite{werbos1974beyond}. It allowed the training of multi
layer networks, paving the way for deep learning's success. In the
1980s McClelland and Rumelhart published an influential work coining
the terms parallel distributed processing and
connectionism~\cite{rumelhart1987parallel}. However, Support Vector
Machines and other simpler classifiers became popular~\cite{boser1992training,smola1998learning}. They were easier to reason
about and performed better~\cite{rost1993prediction}. Later,
max-pooling was introduced, and GPU methods were created to speed up
backpropagation. The performance of neural nets was further plagued
by the vanishing gradient problem, especially in deeper (multi level)
networks. Schmidhuber devised a hierarchy of networks that were pre
trained one network at a time, to overcome this
problem~\cite{schmidhuber1992learning}. Other methods were later
designed, such as ReLU threshold functions and batch renormalization~\cite{ioffe2017batch}. 


\subsubsection{Early Games}\index{NeuroGammon}
In game playing, the advantage of neural networks for function approximation
has been recognized early. Let us give a brief overview of the
approaches that have been tried.


Twenty years before AlexNet, in 1990, Tesauro published a paper on
NeuroGammon~\cite{tesauro1990neurogammon}, his program for playing
Backgammon. (Figure~\ref{fig:bg} shows a Backgammon board.)
Neurogammon used supervised learning to train the coefficients of human designed heuristic
input features, by using 400 example games played by Tesauro
himself. A later version of Neurogammon, TD-Gammon, used
reainforcement learning to train the samen heuristic input
features. TD-Gammon achieved  world class human tournament level
play~\cite{tesauro1995td,tesauro1995temporal}.
\index{backgammon}\index{TD-Gammon}\index{NeuroGammon}

In 1996 Enzenberger created NeuroGo~\cite{enzenberger1996integration},
His Go playing program. NeuroGo uses temporal difference learning and backpropagation to
train the coefficients of manually crafted heuristics features. Its
performance did not surpass that of heuristic programs of its time.\index{NeuroGo}

In 1990 there was insufficient computer power for training of large
networks, nor were there large 
databases of example games to achieve strong play.

In 1999 Chellapilla and Fogel~\cite{chellapilla1999evolving,fogel2001blondie24} used a
fully connected network to evolve board features in Checkers, achieving a good results.

Maddison et al.~\cite{maddison2014move} show how convolutional neural
nets can be used in the context of Go to generate moves. 
Sutskever and Nair~\cite{sutskever2008mimicking} used CNNs to learn from
Go expert games.

Convolutional neural nets were also used in Go by Clark and
Storkey~\cite{clark2014teaching,clark2015training} who had used a CNN for supervised learning
from a database of human professional games, showing that it
outperformed GNU Go and scored wins against Fuego.

David et al.~\cite{david2016deepchess} report on end to end deep
learning in Chess, achieving results on par with Falcon and Crafty,
two  AlphaBeta based programs.





\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/Backgammon.png}
\caption{Backgammon}\label{fig:bg}
\end{center}
\end{figure}





==> chapters/Ago.tex <==

The research in this book may have piqued your interest in learning to
play Go. This tutorial contains a brief introduction to the game of Go.
It is based on 
\url{https://www.kiseido.com/ff.htm}, Kiseido Publishing Company,
Japan (permission pending). Go is a fascinating game of strategy
providing endless challenge and enormous joy to millions of players
worldwide. This appendix contains a basic tutorial to get you started.  Other tutorials can be found in your bookstore and on the
Internet. As you are surfing, you may want to see if there is a Go
club nearby. There is no better way  to learn to play Go than  from real people.

\subsubsection*{The Board}
Go is usually played on a 19x19 grid, or board. Dia.~1 shows an empty board.
Notice the nine marked points. These points are usually referred to as
the star points. They serve as reference points as well as markers on
which the handicap stones are placed in handicap games.


%\begin{figure}[h]
%  \centering{
\includegraphics[width=4cm]{figures/go1.jpg}
%     \caption{The Board}\label{fig:go1}}
%   \end{figure}
%\begin{figure}[h]
%  \centering{
\includegraphics[width=4cm]{figures/go2.jpg}
%     \caption{Move Types}\label{fig:go2}}
%\end{figure}


\subsubsection*{The Stones}
The pieces used are black and white lens-shaped disks, called stones.
Black starts out with 181 stones and White with 180. The total of 361 stones corresponds to the number of intersections on the standard 19x19 Go board. 
The stones are usually kept in wooden bowls next to the board.

\subsubsection*{How Go Is Played}
At the beginning of the game, the board is empty.
One player takes the black stones, the other player the white ones.

The player with the black stones, referred to as ``Black,'' makes the
first move. The player with the white stones, referred to as ``White,''
makes the second move. Thereafter, they alternate making their moves.

A move is made by placing a stone on an intersection.
A player can play on any unoccupied intersection.

A stone does not move after being played, unless it is captured and
taken off the board.

Dia. 2 shows the beginning of a game.
Black plays the first move in the upper right corner.

White plays 2 in the lower right corner.

Black plays 3 and White plays 4.

This is a typical opening where each player has staked out a position in  two of the four corners.

Next Black approaches White 2 with 5, and White pincers 5 with 6.

Black escapes into the center with 7, and White stakes out a position in the bottom right with 8.

Next Black pincers the white stone at 6 with 9.

\subsubsection*{The Object of Go Is to Control Territory}

The object of Go is to control more territory than your opponent. At
the end of the game, the player who controls  more territory wins
the game.

We are going to show you how territory is formed in a game on a 9x9
board. Although Go is usually played on a 19x19 board, it can also be
played on a 9x9 board, or any size board from 5x5 up. Explaining the
rules on a 9x9 board is convenient because the game is over quickly
and the beginner can immediately grasp the flow of the game and how
the score is counted. We also recommend that you play your first games
on a 9x9 board and, when you have mastered the rules, start playing on
the 19x19 board.

\subsubsection*{An Example Game}

%\begin{figure}[h]
%  \centering{
\includegraphics[width=2.80cm]{figures/go3.jpg}
%     \caption{Moves}\label{fig:go3}}
%   \end{figure}
%\begin{figure}[h]
%  \centering{
\includegraphics[width=2.95cm]{figures/go4.jpg}
%     \caption{Moves}\label{fig:go4}}
%\end{figure}
%\begin{figure}[h]
%  \centering{
\includegraphics[width=2.75cm]{figures/go5.jpg}
%     \caption{Moves}\label{fig:go5}}
%\end{figure}

As shown in Figure 1, Black makes the first move on the 4-4 point, after which
White makes its move.

Thereafter, both sides continue to alternate in making their moves. With White 6, the territories of both sides are beginning to take shape.
Black has staked out the right side, and White has laid claim to the left side.

Once you have mapped out your territory, there are two basic strategies to choose from.

One is to expand your own territory while reducing your opponent's
territory. The other is to invade the territory your opponent has
mapped out.



Black 7 in Figure 2 follows the first strategy:
Black expands the territory on the lower right while
preventing White from expanding its own with a move at White ``a.''

White must defend at 8 to block an incursion by Black into the
territory on the left. 
Next, Black reinforces the territory on the right with 9.


It is now White's turn to expand the territory.
White does this by first expanding the center
with 10 and 12 in Figure 3, then expanding the upper
left territory with 14.
Black must defend the top right territory with 15.
The points around ``a'' at the top and bottom must now be decided.


%\begin{figure}[h]
%  \centering{
\includegraphics[width=3cm]{figures/go6.jpg}
%     \caption{Moves}\label{fig:go6}}
%\end{figure}
%\begin{figure}[h]
%  \centering{
\includegraphics[width=3cm]{figures/go7.jpg}
%     \caption{Moves}\label{fig:go7}}
%\end{figure}
%\begin{figure}[h]
%  \centering{
\includegraphics[width=3cm]{figures/go8.jpg}
%     \caption{Moves}\label{fig:go8}}
% \end{figure}



The moves from White 16 to Black 19 in Figure 4 are a common sequence.
The same kind of sequence is next played at the bottom
from White 20 to Black 23.
By playing these moves, White is able to expand the territory
while reducing Black's.


White 24 to White 26 in Figure 5 are the last moves of the game.
It is now possible to determine the winner.
In this case, counting the score is easy.



 Black's territory here consists of all the vacant points Black controls 
on the right side, while White's territory consists of all the vacant point White controls on the left.
More precisely, Black's territory is all the points marked ``b''
in Figure 6 and White's territory is all the points marked ``w.''
If you count these points, you will find that Black has 28 points,
while White has 27. Therefore, Black wins by one point.


This was a very simple game, and some of the rules did not
arise. However, playing over this game will show you what Go is about.

\subsubsection*{The Rule of Capture}

An important rule of Go concerns the capturing of stones. We will
first show you how stones are captured, then show how this occurs in a
game.

\subsubsection*{Liberties}

%\begin{figure}[h]
%  \centering{
\includegraphics[width=8cm]{figures/go9.jpg}
%     \caption{Liberties}\label{fig:go9}}
% \end{figure}

 The lone white stone in Dia. 3 has four liberties.
Namely, the four points ``a'' in Dia.~4. If Black can occupy all four of these points, black captures the white stone.
Suppose, for example, that Black occupies three of these liberties in Dia.~5. The white stone would be in Atari and Black would be able to capture it on the next move, that is with 1 in Dia.~6.
Black would then remove the white stone from the board and put it in
the prisoner pile. The result of this capture is shown in Dia.~7.

%\begin{figure}[h]
%  \centering{
\includegraphics[width=8cm]{figures/go10.jpg}
%     \caption{Liberties}\label{fig:go10}}
% \end{figure}

 At the edge of the board a stone has only three liberties. The white stone in Dia.~8 is on the edge of the board; that is on the first line.
Its three liberties are at ``a'' in Dia.~9.
If Black occupies two of these liberties, as in Dia.~10, the white stone would be in Atari.
Black captures this stone with 1 in Dia.~11.
The result of this capture is shown in Dia.~12.

%\begin{figure}[h]
%  \centering{
\includegraphics[width=8cm]{figures/go11.jpg}
%     \caption{Liberties}\label{fig:go11}}
% \end{figure}

 A stone in the corner has only two liberties. The white stone in Dia.~13 is on the 1-1 point.
Its two liberties are at ``a'' in Dia.14.
If Black occupies one of these points, as in Dia.~15, the white stone would be in Atari.
Black captures this stone with 1 in Dia.~16.
The result is shown in Dia.~17.


%\begin{figure}[h]
%  \centering{
\includegraphics[width=7cm]{figures/go12.jpg}
%     \caption{Liberties}\label{fig:go12}}
%   \end{figure}

It is also possible to capture two or more stones if you occupy all their liberties. In Dia.~18, there are three positions in which two white stones are in Atari.
Black captures these stones with 1 in Dia.~19.
The results are shown in Dia.~20.

%\begin{figure}[h]
%  \centering{
\includegraphics[width=5cm]{figures/go13.jpg}
%     \caption{Liberties}\label{fig:go13}}
%   \end{figure}

 Any number of stones making up any kind of shape can be captured if all their liberties are occupied.

In Dia.~21, there are four different positions.


Black 1 captures twelve stones in the upper left, four stones in the lower left, three stones in the upper right, and three stones in the lower right.

When you capture stones in a game, you put them in your prisoner pile.

Then, at the end of the game, these captured stones are placed inside your opponent's territory.

\subsubsection*{A Game}
Let's look at a game to see how this actually works.


%\begin{figure}[h]
%  \centering{
%    \begin{tabular}{cc}

\includegraphics[width=3cm]{figures/go14.jpg}
%
\includegraphics[width=3cm]{figures/go15.jpg}
%      \end{tabular}
%     \caption{Liberties}\label{fig:go14}}
% \end{figure}
 
 After Black plays 3 in Figure~7, White makes an invasion inside Black's sphere of influence with 4. White 10 Atari's the black stone at 7.
This stones has only one liberty remaining at the point ``a.''

If Black doesn't play the next move at ``a,'' White will play on this point
and capture the black stone at 7.


Therefore, black connects at 11 in Figure~8,
but White Atari's again at 12.
The marked stone cannot be rescued, so Black has to sacrifice it.

%\begin{figure}[h]
%  \centering{
%    \begin{tabular}{cc}

\includegraphics[width=3cm]{figures/go16.jpg}
%
\includegraphics[width=3cm]{figures/go17.jpg}
%      \end{tabular}                                                     
%     \caption{Liberties}\label{fig:go16}}
%   \end{figure}

Black plays its own Atari with 13 in Figure~9. White then captures with 14 and Black Atari's two white stones with 15.
That is, it threatens to capture them by playing at ``a.''


 With 16 in Figure~10,
White maps out the territory on the left side,
and Black expands the territory on the right side with 17 to 21.

The moves from White 22 to Black 24 are the same kind of endgame
sequence we saw in Figure~4 of the first game.


%\begin{figure}[h]
%  \centering{
%   \begin{tabular}[t]{cc}
\begin{minipage}[t]{0.3\textwidth}
  \vspace{0pt}
  \includegraphics[width=3cm]{figures/go18.jpg}
\end{minipage}%
\begin{minipage}[t]{0.3\textwidth}
  \vspace{0pt}
  \includegraphics[width=3cm]{figures/go19.jpg}
\end{minipage}


%      \end{tabular}                                           
%     \caption{Liberties}\label{fig:go18}}
% \end{figure}

 White 26 forces Black to capture two white stones with 27
in Figure~11.
Next, the moves at White 28 and 30 each reduce Black's territory by one point.
Black 31 Atari's the two white stones at 26 and 30, so White must connect at 32 to save them.

Finally, Black 33 reduces White's territory on the left by one
point. The game ends when White blocks at 34.



 Figure~12 shows what the board looks like at the end of this game.

White has one black stone in the prisoner pile, while Black has two
white stones.


%\begin{figure}[h]
%  \centering{
%    \begin{tabular}{cc}    

\includegraphics[width=3cm]{figures/go20.jpg}
%
\includegraphics[width=3cm]{figures/go21.jpg}
%      \end{tabular}                                                 
%     \caption{Liberties}\label{fig:go20}}
% \end{figure}

 In Figure~13, each side places the prisoners in the opponent's territory.
White places  one black prisoner (the marked black stone) inside Black's territory,
and Black places  two white prisoners (the two marked white stones)
inside White's territory.




 It is customary to rearrange the stones a bit to make the counting of territory simple and rapid.
In Figure~14, the three marked black stones and the two marked white stones were moved.


Calculation of the size of the territories can now be made at a glance.
Black has 23 points; White has 24 points. White wins by one point.


\subsubsection*{Questions and Answers}
 After White 12 in Figure 8, why didn't Black try to escape with the
 marked stone?

 
%\begin{figure}[h]
%  \centering{
\includegraphics[width=3cm]{figures/go22.jpg}
%     \caption{Liberties}\label{fig:go22}}
% \end{figure}
% 
%\begin{figure}[h]
%  \centering{
%    \begin{tabular}{cc}
%
 \includegraphics[width=3cm]{figures/go23.jpg}
%
 \includegraphics[width=3cm]{figures/go24.jpg}

%\end{tabular}
%    \caption{Liberties}\label{fig:go23}}
% \end{figure}

Black could try to escape by playing 1 in Dia.~22,
but White would pursue him and the black stones would still
be in Atari.
If Black persists with 3, Black can Atari the marked white stone,
but White captures three stones by taking Black's last liberty with 4.





 After Black 15 in Figure~9, it might seem as if the two White stones
 in Atari could escape by extending to `a'. Why doesn't White try
 this?
 The reason White doesn't try to escape is because White can't, unless
Black blunders.

If White extends to 1 in Dia.~23, White increases the liberties to
three but Black pursues white with 2 and, after 4,
White is at the end of its rope:
white has no way to increase  liberties. If White plays 5,
Black Atari's with 6 and captures with 8.


%\begin{figure}[h]
%  \centering{
\includegraphics[width=3cm]{figures/go25.jpg}
%     \caption{Liberties}\label{fig:go25}}
% \end{figure}

 However, Black must not play 2 from the outside as in Dia.~24.
White would then turn at 3 and now the two marked black stones
have only two liberties,
while the white group on the right has three liberties.
White captures the two marked stones with 5 and 7.



% \begin{figure}[ht]
%     \centering{\includegraphics[width=4cm]{figures/go26.jpg}
%      \caption{Liberties}\label{fig:go26}}
%  \end{figure}

 Is Black 25 in Figure~10 necessary?

 It certainly is. If Black omitted this move,
White would Atari the marked black stone with 1 in Dia.~25.
If Black tries to run away with 2 and 4, White pursues him with 3
and 5, forcing the black stones into the corner,
where they run out of liberties.
White would then capture four black stones with 7.

% \begin{figure}[ht]
%     \centering{\includegraphics[width=4cm]{figures/go27.jpg}
%      \caption{Liberties}\label{fig:go27}}
%  \end{figure}

 These are most of the rules of Go. There is one other rule: the ko
 rule, which prevents repetitive capture. The rule simply states:
 The previous board position cannot be recreated.
 
 If you are a beginner who wishes to learn the game of Go, we
 recommend that you start with the book  \emph{Go: A Complete Introduction to
 the Game} by Cho Chikun~\cite{ch1997go}, from which this brief introduction was
 taken. 

==> chapters/conclusion.tex <==

%% 7:
%% section: did we achieve intelligence/special intelligence
%% section did achieve learning
%% *section: how generally applicable is search-eval architecture
%% section: other apporaches towards general artificial intelligence


\section{Intelligence}
Special Intelligence, general intelligence

\section{Learning}
We did achieve learning

\section{*How General is the Search-Eval architecture?}

\section{Challenges and The Future}
Towards artificial general intelligence



\subsection{Games}
\subsubsection{Gym/ALE}
\subsubsection{Starcraft}
\subsubsection{Poker}
\subsubsection{Bridge}
\subsubsection{GVGGP}

\subsection{Reinforcement Learning}
\subsubsection{hierarchical RL}
\subsubsection{Meta learning}
\subsubsection{imperfect info}
\subsubsection{sparse spaces}
\subsubsection{delayed reward}
\subsubsection{transfer learning}
\subsubsection{agi}


==> chapters/curr-summary.tex <==
\section{curriculum learning}
summarize bengio, weinshal, silver.

bengio 2009
deep training is hard
Elman 1993: curriculum: start small increase difficulty, also: small capacity
learn possible unlearnable
multi-stage curriculum strategies improved generalization and faster convergence

Bengio writes: deep architecture training. Some have good solutions in local minima that are almost impossible to find by random initialization. (Erhan 2009)
Deep learning attempts to learn feature hierarchies. Features at
higher levels are formed by composition of lower level
features. Automatically learning multiple levels of abstraction,
creating a complex function mapping from input to output, without
depending on human crafted features.

Training deep architectures involves a potentially intractable
optimiztation problem. Before Hinton 2006 there were no good
algorothms for training fully-connected deep architectures, when they
introduced greedily training one layer at a time. It exploits
an unsupervised generative learning algorithm for each layer: a
restricted Boltzmann Machine.  Now, it is conceivable that by training
each layer one after the other, we first learn the cimpler concepts,
represented in the first layer, then silightly more abstract concepts
in the second layer, etc. Further works introduced other algorithms
for training deep architectures, all showing advantage of deep
architectures over shallow ones, and using unsupervised pre-training. 

Out of the study for better deep learning algorithms, and the success
of unsupervised pre-training, curriculum
learning arose. Unsupervised pre-training starts the supervised
poptimzation in a region of parameter space that were not much better
in terms of final trainign error, but substantially better in terms
of test error (they generalized better). This suggests a dual effect
of unsupervised pre-training. It helps opitmization by starting in
better basins of attraction of the descent procedure in parameter
space, and as a kind of regularizer.

A curriculum can be seen as a sequence of training criteria. Each
training criterion in the sequence is associated with a different set
of weights on the training examples. Initially, the weights favir
easier examples, or examples illustrating the simplest concepts, that
can be learned most easily. The next training criterion involves a
slight change in the weightingof examples that increases the
probability of sampling more difficult examples. At the end of the
sequence, the reweighting of the examples is uniform and we train on
the target training set of the target training distribution.

Advantage of a curriculum strategy is: faster training in the online
setting because the learner wastes less time with the noisy or harder
to predict examples (when it is not ready to incorporate them).

And guiding training towards better regions in parameter space, into
basins of attraction (local minima) of the descent procedure
associated with better generalization: a curriculum can be seen as a
particular continuation method. (...)

Curriculum strategies are also connected to transfer (or mukti-task)
learning
Curriculum strategies are also connected to transfer (or multi-task)
learning and lifelong learning (Thrun, 1996). Curriculum learn- ing
strategies can be seen as a special form of trans- fer learning where
the initial tasks are used to guide the learner so that it will
perform better on the final task. Whereas the traditional motivation
for multi- task learning is to improve generalization by sharing
across tasks, curriculum learning adds the notion of guiding the
optimization process, either to converge faster, or more importantly,
to guide the learner to- wards better local minima.


Weinshall:
in human learning supervision is often accompanied by a
curriculum. Thus the order of presented examples is rarely random when
a human teacher teaches another human. Like- wise, the task may be
divided by the teacher into smaller sub-tasks, a process sometimes
called shaping (Krueger \& Dayan, 2009) and typically studied in the
context of reinforcement learning (e.g. Graves et al., 2017). Although
it remained for the most part in the fringes of machine learning
research, curriculum learning has been identified as a key challenge
for machine learning throughout (e.g., Mitchell, 1980; 2006; Wang \&
Cottrell, 2015). 

We focus here on curriculum learning based on ranking (or weighting as
in (Bengio et al., 2009)) of the training exam- ples, which is used to
guide the order of presentation of examples to the learner. Risking
over simplification, the idea is to first present the learner
primarily with examples of higher weight or rank, later to be followed
by examples with lower weight or rank. Ranking may be based on the
dif- ficulty of each training example as evaluated by the teacher,
from easiest to the most difficult. 

curriculum learning, when given the ranking of training points by
their difficulty thus defined, is expected (probabilistically) to
significantly speed up learn- ing especially at the beginning of
training. This theoretical result is supported by empirical evidence
obtained in the deep learning scenario of curriculum learning
described in Section 3, where similar behavior is observed. We also
show that when the difficulty of the sampled training points is fixed,
convergence is faster when sampling points that incur higher loss with
respect to the current hypothesis as suggested in (Shrivastava et al.,
2016). This result is not al- ways true when the difficulty of the
sampled training points is not fixed.
But such ideal ranking is rarely available. In fact, the need for such
supervision has rendered curriculum learning less useful in machine
learning, since ranking by difficulty is hard to obtain.

However, self play

Learning rate is always faster with curriculum learning, especially at
the beginning of training. (ii) Final generalization is sometimes
improved with curriculum learn- ing, especially when the conditions
for learning are hard: the task is difficult, the network is small, or
when strong regularization is enforced. These results are consistent
with priorart(see e.g. Bengioetal.,2009). 

\section{pre-training as transfer learning for curriculum learning}
Join both.

Pre-training with a curriculum strategy might act similarly to
unsupervised pre-training, acting to find better local minima and as a
regularizer, and help to reach faster convergence to a minimum of the
error function.

Curriculum is like transfer from stage to stage.
Pre training.

notion of transfer discussed in (Bengio et al., 2009) in the context
of multi-task and life- long learning (Thrun \& Pratt, 2012), where
knowledge is transferred from earlier tasks (e.g. the discrimination
of easy examples) to later tasks (e.g. the discrimination of difficult
examples).


Continuation methods (smoothing)?

\section{transfer learning}
Summarize transfer learning.
normal training adjust net for each new example.
for an example the net is not blank, but initialized by the previous
training examples.
pre-training is that another batch of examples are used as
initializer, possibly per layer.

transfer learning is that another batch of examples is use for entire
net as inistializer

curriculum learning, is that examples are increasingly difficult

curriculum learning takes other examples (input to training)
transfer learning takes other weights (result of training)

while doing curriculum leanring, the intermediate results are used as
in transfer learning. It learns from different examples.
doing transfer learning thus needs different examples as input


pre-training.




\section{self play as curriculum learning}
Self play is curriculum. Self play is pre training. Self
play is transfer.

\section{transfer learning as general game playing}
But also: alphazero 3 games is transfer. And: it is
not. No transfer of learnd weights. Need more research there.  Net viz
to learn knowledge.




 


==> chapters/epilogue.tex <==




%\section{Open Mind}
This has been a story of many surprises.
      Breakthroughs do not come by accident, but are the result
        of hard work towards more insight, and an open mind towards
        unexpected outcomes.

        If there is one lesson, it is that breakthroughs
        come by combining methods from different fields.

        Everybody knew that minimax was the only backup rule that made sense, until it
        wasn't.

        Everybody knew that Monte Carlo evaluations is crazy, until
        it worked.

        Everybody knew neural nets were too slow, until
        they were not.

        Everybody knew that end-to-end neural nets do not work for
        Chess, until they did.

        Everybody knew that deep reinforcement learning
        was unstable, until it was stable.

        Everybody knew that self-play maxes out  early, until it kept on learning.

        Everybody knew that a Go
        architecture would never work for Chess, until it
        did.

        Everybody knows that Poker is too hard, until it
        was not.

        And now, everybody knows that AGI is  
        impossible.\\

        The future will surprise

==> chapters/old-11transfer.tex <==

%% The problems of this chapter are performance and applicability: we
%% wish to increase the 
%% quality of self-play, and we wish to enlarge the range of applications
%% that it can be applied to. We will 

Self-play is still a young technique, 
despite
being around since the dawn of AI. There are still many opportunities
for enhancing performance. 
In this chapter we  deepen our understanding of self-play to
improve performance and increase the number and kinds of problems that
it can be applied to.

We start with the open questions from the previous chapter. SInce
self-play is still young, the enhancements in this  chapter are more
suggestions for future enhancements than a report on experiences with the
enhancements. Self-play is young, and most of the suggestions have not
yet been applied to self-play.




%% \section*{Learning Goals}
%% \begin{itemize}
%% \item stability: learning process improvements. deadly triad?
%% \item generalization to other problems. arch, hier rl, other self play work
%% %% \item
%% %% For which other domains can self play work? Does self play only work
%% %% games, or also for other Markov problems, or for non-Markovian problems?
%% %% \item
%% %% Why is performance of self play levelling off? How can learning be
%% %% improved further? 
%% %% \item
%% %% Did self play kill the deadly triangle? Is learning stability no
%% %% longer a problem? Is overfitting solved?
%% %% \item
%% %% Can learning be sped up, can learning efficiency be improved?
%% %% \item
%% %% Can the network architecture be learned automatically?
%% %% \item
%% %% Why do resnets perform so well in self play? Are there other
%% %% architectures that work better?
%% %% \item
%% %% How general are the concepts learned by self play? How can learned
%% %% concepts be transferred to other games? (Note that in AlphaZero each
%% %% game needed to start training from scratch.)
%% %% \item
%% %% Does self play work well in imperfect information games such as
%% %% Bridge, Poker, and Starcraft? 
%% \end{itemize}

%% These questions can be grouped into two categories: questions about
%% the training process, and questions about generalization towards more
%% applications.

\section{Training Efficiency}
The questions are concerned with the  efficiency of the
training process, and with generalization of training results
(transfer learning). We will first discuss the efficiency of the
training process.

\subsection{Learning Stability}
Issue: Stability: correlations
solution: replay buffers
self-play: with replay buffers seems solved
saturation does not seem to be caused by stability issues.

Previously, training reinforcement learning function approximators
required careful attention to stability, due to correlations between
subsequent states and target values. Replay buffers were introduced,
and actor critic networks, to achieve sufficiently stable
training. Training sets were large, to provide sufficient variation in
training examples, causing training times to be large.

Self play combines planning and learning. Examples are generated by a
planner (such as MCTS). This lookahead creates examples of higher quality and
greater independence, creating a more  diverse  and stable training
process.

The ``deadly triad'' of function approximation, bootstrapping and  off policy
learning did not occur in AlphaZero, or, if it did, it did not
preclude reaching a high level of play.

{\bf
  Did others encounter this in self play? other studies into learning stability of self play?}

well, bengio curriculum learning, epstein perfect teacher, tesauro add heuristics


It should be noted that no in depth study 
Stable learning? more efficient self play due to suitable opponent?
 Did self play kill the deadly triangle? Is learning stability no
 longer a problem? Is overfitting solved?

Is curriculum learning, learning by small steps, applicable to more
problems?

This remains very much an open question
 
\subsection{Learning efficiency}\label{sec:curr}\index{curriculum
learning}\index{transfer learning}
We also saw in the previous chapter that supervised and
reinforcement learning can be slow when there is a large gap between
training targets and  the initial state of the approximator. When errors are
large, it takes many steps for the net to converge.

Tabula rasa self play has the advantage that the quality of the
training examples are never too far off. The training targets are
generated in lock step with the trainee, both trainer and trainee grow
in quality together. 

Thus each training iteration converges much quicker than when large
steps must be taken. Indeed, this has been observed in other works as
well and sometimes named curriculum
learning~\cite{bengio2009curriculum,matiisen2017teacher}, or
pre-training~\cite{erhan2010does}. Specifically, the pre-training has
been reported to guide the learning towards basins of attraction of
minima that support better generalization from the training data
set~\cite{erhan2010does,bengio2012practical}. Recently, curriculum
learning has been studied in relation to transfer
learning~\cite{weinshall2018curriculum}. Curriculum learning is 
also important for life long learning, or never ending
learning~\cite{mitchell2018never}, and has been reported to be
necessary on other domains as well~\cite{zaremba2014learning}.

A question that remains is why performance of self play is levelling
off, and, importantly, how this point can be pushed further off?
Perhaps there is nothing left to learn in $19\times 19$ Go? This
question can be tested by running the program on smaller and larger
boards, and seeing if the learning curves scale up and down
accordingly.

Perhaps the network is saturating? This can be tested, and has been to
some extent, by decreasing or increasing the network complexity. The
AlphaGo Zero paper describes a comparison between 20 block and 40
block residual nets, finding the improvement of the larger network to
be small~\cite{silver2017mastering}.

Perhaps there is a more fundamental limit to what self play can teach
a neural net? This situation is described by Tesauro in his TD-gammon
papers. His single layer network did not learn more complicated
patterns, and he added a small amount of planning (a 2 level search) and
certain hand crafted heuristic knowledge, improving performance of the
program significantly~\cite{tesauro2002programming}.

Perhaps the self play training scheme should be improved. Already
Epstein~\cite{epstein1994toward,epstein1993toward} noted the importance of a good
trainer in self play, and has suggestions on how to avoid self play training
pathologies. Or perhaps the planner needs to imporve as the level of
play increases. Perhaps the number of MCTS simulations should increase
as Elo increases.

The question how to improve learning  further is perhaps the most
important question to ask in machine learning. 
This remains very much an open question that will be actively
researched in the field.

Need saturation study into the reasons of sturation

\subsection{Learning Architecture}
\subsubsection{Hyperparameter Optimization}

Deep learning and self play systems have many hyper
parameters. AlphaGo Zero lists the following: number of self play games per iteration
(25000), MCTS
simulations (1600), exploration temperature (1 for first 30 moves, 0
afterwards), Dirichlet noise ($\eta=0.03, \epsilon=0.25$), resignation
threshold (5\%), regularization parameter ($c=10^{0.4}$), mini batch size (2048, 32 per worker), self play positions
(500,000), learning rate (annealed with momentum parameter 0.9), cross
entropy loss and mean squared error are weighted equally in the loss
function, optimization checkpoint for new batch of self play games
(1000), self play evaluator (400), win margin for acceptance (55\%),
network architecture (19 residual blocks)~\cite{silver2017mastering}.

The effects of some of these hyperparameters interfere. A recurring theme of AI is
that some decision making tasks are best left to computers. This holds
for hyperparameter. Finding the
optimal setting for all parameters is a daunting task, best left to
machine optimization.\footnote{just as finding the best coefficients for an
evaluation funciton of hand crafted heuristics is best left to machine
learning, and, for that matter, crafting the evaluation features
themselves  is also best left to machine learning, and crafting a database of
training positions is best left to self play. Some would even say that
crafting machine learning algorithms is best left to machine learning,
but that is a topic for another book.} Many optimization algorithms
have a large set of hyperparameters, and hyperparameter optimization
is an active field of research. Well known methods are exhaustive
search~\cite{hoos2004stochastic}, random search~\cite{bergstra2012random,wang2016bayesian},
Bayesian optimization~\cite{bergstra2011algorithms,hutter2011sequential,thornton2013auto,snoek2012practical}, gradient based methods (including neural
networks and SVM)~\cite{bergstra2011algorithms,chapelle2002choosing},
and evolutionary
optimization~\cite{back1993overview,burke2013hyper,pappa2014contrasting,van2015optimally}.
Some
software packages for hyperparameter optimization are
\href{https://github.com/automl/SMAC3}{SMAC}\footnote{\url{https://github.com/automl/SMAC3}}~\cite{hutter2011sequential},
\href{https://automl.github.io/auto-sklearn/stable/}{auto-sklearn}\footnote{\url{https://automl.github.io/auto-sklearn/stable/}}~\cite{feurer2015efficient},
\href{http://www.cs.ubc.ca/labs/beta/Projects/autoweka/}{Auto-WEKA}\footnote{\url{http://www.cs.ubc.ca/labs/beta/Projects/autoweka/}}~\cite{kotthoff2017auto},
\href{https://scikit-learn.org/stable/}{scikit-learn}\footnote{\url{https://scikit-learn.org/stable/}}~\cite{pedregosa2011scikit},
  \href{http://iridia.ulb.ac.be/irace/}{irace}\footnote{\url{http://iridia.ulb.ac.be/irace/}}~\cite{lopez2016irace}
  and
  \href{https://code.fb.com/ai-research/nevergrad/}{nevergrad}\footnote{\url{https://code.fb.com/ai-research/nevergrad/}}~\cite{nevergrad}.\index{nevergrad}\index{irace}\index{scikit-learn}\index{AutoML}\index{AutoWeka}\index{auto-sklearn}\index{SMAC}

AlphaGo Zero optimized its hyperparameters with Bayesian optimization,
AlphaZero used the same set. 


\subsubsection{Network Architecture}
The  architecture of the network is
also a  hyperparameter to optimize. Among the decision to make are
how many layers, of what type, and how many
neurons, also of what type, whethr to have cells, and how they are
connected. Getting the architecture 
right for your problem can be a timeconsuming problem, perhaps also
best left to machine learning. 
Network architecture optimization can be based the same methods as for
hyperparameter optimization, random search, bayesian
optimization~\cite{yoshinari2018probabilistic}, 
evolutionary algorithms~\cite{kitano1990designing,van2018automatic,jaderberg2017population,miikkulainen2019evolving}, although reinforcement learning has also been
used~\cite{zoph2016neural,baker2016designing}. Two surveys
  are~\cite{yao1999evolving} and \cite{elsken2018neural}. A standard
  work on evolutionary strategies is B\"ack~\cite{back1996evolutionary}.

\subsubsection{Network Type}
In Chapter~\ref{chap:super} we saw an evolution of different network
types for image recognition, and in Chapter~\ref{chap:dqn} the same
occurred in  reinforcement learning. For AlphaGo Zero
Figure~\ref{fig:slrl} compared convolutional and residual nets. So
far, there is little other work reported that compares different
network types. A
complicating factor is that running self play experiments is
computationally expensive. Running experiments to find out what type
of network and which
hyperparameters work best for a problem may be computationally
infeasible. 

\subsubsection{Network Optimization}
An important element of all neural network function approximators is
the optimization algorithm. Stochastic gradient descent has been the
optimization algorithm of
choice, although alternatives exist. Recently works
report on evolution
strategies~\cite{chrabaszcz2018back,salimans2017evolution,wierstra2008natural}. An
advantage of evolution strategies is that they are well suited for
parallelization, providing possible speedups for the training phases
of self play.

\subsection{Generalization in Reinforcement Learning}
To improve performance several ideas to further develop reinforcement
learning are being pursued.

\subsubsection{hierarchical RL}\index{hierarchical reinforcement learning}
\cite{barto2003recent}
\cite{bakker2004hierarchical}
\subsubsection{Meta learning}
\subsubsection{imperfect info}
\subsubsection{sparse spaces}
\subsubsection{delayed reward}
\subsubsection{DQN vs planning}
\subsubsection{DQN}
Question: much of current research is dqn without planning. can all
planning be folded into multilayer backprop? Is planning essential for
self learning? Atari learns good play (reflexes) without planning. Is
planning needed for strategy (= long distance between credit
assignment)?




\section{Transfer Learning: Generalization to other Problems}\index{transfer learning}
There are two kinds of generalization that we are interested in:
system generalization and knowledge generalization. In system
generalization the question is to build a system that can learn to
solve multiple problems. This is the kind of generalization that GGP
seeks to achieve. AlphaZero succeeded in this aspect for three
board games. Algorithms, network architecture and hyperparameters generalized to three
games, although it needed hand crafted input and output
layers, and, significantly, the network had to be retrained from
scratch for each game: trained nets do not generalize accross games. Extending system generalization tries to extend this to more
and different kinds of problems.

The goal of knowledge generalization is to build a system where the
whole system generalizes to solving different kinds of problems
(including the trained net). This type of generalization tries to
transfer knowledge that is learned in one domain to solve problems in
another domain, without retraining. This kind of knowledge
generalization is known as {\em transfer 
  learning\/}~\cite{pratt1993discriminability,thrun2012learning}. Chapter~\ref{chap:agi}
is about artificial general intelligence and will cover this topic in
more depth.

\subsection{Visualizing Neural Net Weights}\label{sec:zflayers}
Deep supervised learning was designed to facilitate feature learning, or
representation learning. The layers learn concepts of increasing
generality~\cite{bengio2013representation,lecun2015deep}, creating a
hierarchy of concepts,together representing high level concepts, such
as a whole face. How general are the concepts learned by self play?
What do they ``look'' like (can they be represented as a two
dimensional picture for humans to interpret).?

Montavon et al.~\cite{montavon2018methods} provides an tutorial of
methods for interpreting deep nets.
Zeiler and Fergus ZF paper~\cite{zeiler2014visualizing} gives
insightful pictures of the different layers (one of which is
reproduced in Figure~\ref{fig:zfnetlayers11}). They developed a
visualization technique to interpret the layers of a CNN.
Noh et al.~\cite{noh2015learning} use deconvolution for semantic segmentation.


\begin{figure}[t]
    \centering{\includegraphics[width=10cm]{figures/zfnetlayers}
     \caption{ZFnet layers\cite{zeiler2014visualizing}}\label{fig:zfnetlayers11}}
\end{figure}

During supervised learning the accumulating knowledge is refined with
each training epoch and is generalized in the deep layer. In self
play, there is an extra dimension, in addition to epoch and layer. In
each self play iteration the level of difficulty of the concepts learned
increases. In this sense, AlphaGo Zero's joseki picture illustrates
how ovr time the self players learned each other more advanced concepts  (see Figure~\ref{fig:joseki11}).
Table~\ref{tab:concepts11} illustrates the three kinds of self play learning.
  
\begin{figure}[ht]
    \centering{\includegraphics[width=13cm]{figures/joseki}
     \caption{AlphaGo Zero is Learning Joseki~\cite{silver2017mastering}}\label{fig:joseki11}}
\end{figure}

\begin{table}
  \centering{
    \begin{tabular}{c|c|c}
      {\bf supervised} & {\bf self play} & {\bf learn}\\ \hline
      epoch & epoch & optimize  error\\ \hline
      layer & layer & generalize concept \\ \hline
      -     & iteration & increasing difficulty
    \end{tabular}
    \caption{Three Kinds of Learning in Supervised and Self
      Play}\label{tab:concepts11}
  }
\end{table}

Ever since Samuel's Checkers player self play has a long history in research . The recent breakthrough by
AlphaGo Zero, and the subsequent reimplentations (A0G, Elf OpenGo,
PhoenixGo and Leela) will stimulate research in this area.
Future work may find other insightful ways to visualize knowledge accumulation.

\subsection{Other  Problems Domains}
Self play is a natural training paradigm for two agent games.
Self play is also being tried in other games, such as Starcraft and
Poker~\cite{heinrich2016deep}. Many optimization problems in science
are single agent NP hard optimization problems such as the Traveling
Salesperson Problem, the 15 puzzle, and
Satisfiablity~\cite{russell2016artificial}. The question arises if
self play can be 
used for single agent optimization as well.





Approximating single solutions for instances of single agent combinatorial optimization with neural nets has been studied for quite
some time~\cite{smith1999neural}.
Work  for self play learning of solvers for a {\em problem domain\/} (which
contains many instances) is more recent.
Recently, after work reformulating MCTS based self play to single player
problems~\cite{moerland2018a0c} and work on reformulating
combinatorial problems to neural networks~\cite{vinyals2015pointer}, a deep learning algorithm applying self play to
single agent combinatorial optimization was
published~\cite{laterre2018ranked}, showing that it outperforms
MCTS. Also, other work aplies approximate reinforcement learning to
TSP~\cite{kool2018attention,bello2016neural,gambardella1995ant}. It
can be expected that more research into single agent self play approximators will
appear, benefiting from the
curriculum learning~\cite{bengio2009curriculum,matiisen2017teacher} that appears to be
inherent in self-play approximators.


\subsubsection{Recent Self-Play Work}
Recent work on self-play explores the idea further. Sodhani and Pahuja~\cite{sodhani2018memory} augment self-play with
memory resulting in faster exploration of the environment.
Charlesworth~\cite{charlesworth2018application} applies self-play in a
multi-player game of imperfect information.
Sukhbaatar et al.~\cite{sukhbaatar2018learning} experimemt with
self-play in hierarchical reinforcement learning to automatically
learn sub-goals. Previously, they studied intrinsic
motivation and curriculm learning through
self-play~\cite{sukhbaatar2017intrinsic}.
Zhao et al.~\cite{zhaotraining} study self-play in modern games.

\section{Practice}
\subsubsection{Exercises}
A0G:
\begin{enumerate}
\item play with tensorboard to understand training process
\item do a bit of hyper para tuning
\item play with diff nets automation
\item implement 15 puzz in A0G
\item see if transfer learning of 4x4 Oth, to 6x6 to 8x8 works, and works faster
\end{enumerate}

\section{Summary}
{\bf central concept: learning generalization: hyper par optim,
network arch; transfer/generalization to other problems: hier rl, imperfect info}
\begin{itemize}
\item learning process improvements. deadly triad?
\item generalization to other problems
\end{itemize}
This is still an active field of research. Improving performance of
the learning process through automation with optimization
methods. Visualizing knowledge, generalizing it to other domains. 

\section*{Historical and Bibliographical Notes}
Hyperparameter
optimization~\cite{bergstra2011algorithms,hutter2011sequential}.

Evolutionary Strategies the reference is~\cite{back1993overview}.

Curriculum learning~\cite{bengio2009curriculum,matiisen2017teacher}.

For GGP go to~\cite{genesereth2005general}.

Readable and insightful introduction into the field of Abstraction in
deep representation learning are~\cite{bengio2013representation,lecun2015deep}.

For Network visualization start with the ZFnet paper
insight~\cite{zeiler2014visualizing}.

Poker~\cite{bowling2015heads}
\cite{moravvcik2017deepstack}
\cite{brown2018superhuman}




==> chapters/old01intro.tex <==
Amazing breakthroughs in reinforcement learning in games have taken
place. Computers teach themselves how to play Chess and Go at world
champion level, and they learn faster than humans.
The road towards artificial general intelligence is being taken. The
breakthroughs are by 
a combination of key technologies.
%Written by the head of the
%reinforcement learning group of Leiden University,
This book covers
them all in depth The
book is intended for a  graduate course on reinforcement learning in
games, and can be a starting point for research.  

The breakthroughs in Backgammon, Checkers, Chess, Atari, Go, Poker,
and StarCraft have shown that we can build machines that exhibit
intelligent behavior of 
the highest level. These successes have been widely published in the
media, and inspired AI entrepreneurs and scientists alike. The topic
of reinforcement learning in games is a broad topic.  The 
successes build on a broad range of techniques, from exact planning
methods, to learning of deep approximate  representations, to
ingenious self-play methods.

Perhaps because of the breadth of these
technologies, or 
because of the recency of the breakthroughs, there are few books that
explain what it takes to achieve this level of
achievement. This book covers all these methods in
one compact and comprehensive volume, with a clear focus on games,
eplaining the research papers, bringing you as close as possible to working implementations. The
programming examples  in this book are in Python, the language in which most
current reinforcement learning research is
conducted. Appendix~\ref{chap:python} provides entry points for
learning Python. 

The rest  of this chapter will give an overview of the contents of
this book.

\section{Main Story}


\begin{itemize}
  \item architecture: search-eval/exact-approx/slow-fast/plan-learn
\item two trends: performance and generalization. 
  First start with problem description, do a shortcut towards high
  performance, exploiting heuristic specifics, then understand what is
  going on, and generalize the specific features through
  learning.
  \item And this is the real lesson that you should take away from
  this book: an experimental approach to creating intelligent problem
  solvers of amazingly good performance. Try, understand, generalize/automate, try
  again. (not really which methods to
  use to achieve AGI, although we teach some pretty strong methods in
  this book, but even more, an approach to research, a mentality, that allows you to
  keep inventing better methods yourself, to work towards AGI)
\item Try, Fail. Try again, Fail better.
  \item Try harder, and always in the direction of more automation/learning/generalization
  \item (4) minimax+heuristic, (5) ab, id/tt, search extensions, quiescence, coeff
    learning, (6) avg backup, monte carlo eval, exploration selection,
    (7) function approx, (8) stable learning, (9) performance
    learning, (10) self tuning through self play, (11) hyper par
    optim
    \item from rigid to flexible to learned flexibility (which is even
      more flexible than hard coded ``flexibility'')
    \item This is a story of many suprises.
      Breakthroughs do not come by accident, but are the result
        of hard work towards more insight, and an open mind towards
        new methods. If there is one lesson, it is that breakthroughs
        came by combining methods from suprising fields. Everybody in
        Chess knew that minimax was the only backup rule that made sense, until it
        wasn't. Everybody knew that monte carlo eval is crazy, until
        it worked.  Everybody knew neural nets were too slow, until
        they weren't. Everybody knew that end-to-end neural nets don't work for
        Chess, until they did. Everybody knew that deep reinforcement learning
        was unstable, until it was stable. Everybody knew that self
        play maxed out, until it kept on learning. Everybody knew that a Go
        architecture would never work for Chess. Until it
        did. Everybody knows that Poker is too hard, until it
        wasn't. And now, everybody knows that AGI is still 
        impossible. So, may I beg you to please keep an open mind?
\end{itemize}


\section*{Learning Goals}
\begin{itemize}
\item {\bf It  is exciting to learns about the quest for machine intelligence, and the 4 paradigms. Bring the emotion in understanding our own thinking}
  \item The DeepMind AlphaGo Zero work is truly senstional. Beating
    the human Go champions has shaken the world of AI, indeed it has
    shaken the world. The goal of this book is to teach you how they
    did it, by the best possible scientific means, by allowing you to
    replicate their work, or at least as close as possible. To truly
    appreciate where we are coming from, you will build an old school heuristic Chess
    program (planning), and understand what is behind it, you will
    build a MCTS program, and understand what is behind it, and see
    how very different it is from the heuristic approach, you will
    understand the basics of this field {\em reinforcement learning\/} that
    everybody is talking about, you will understand another very
    important field, deep learning, and
    replicate the Atari experiments that set off the reinforcement
    learning interest (learning), and you will put it all together and
    build a version of AlphaGo Zero that achieves something one of the
    major feats of recent AI: self learning. It learns to play games from
    scratch (tabula rasa) so that you can create programs to play the
    old school heuristic games programs.

    This book is built on two
    pillars: the excitement of knowing you are learning  the
    most exciting AI development of the decade, and the excitement of
    thinking of what this might hold for the future. Because, after
    this book, you are ready.
  \item Thinking=Fast+Slow
  \item AI=Plan+Learn
  \item Learning=Generalized planning examples (Fast is internalized Slow)
\end{itemize}

\subsubsection{Excitement}
This book is built on excitement. 
Excitement because the advances in game playing certainly appear to be
approaching true intelligence; excitement because some of the
intelligence is applicable to more than one domain, giving a glimpse
of general intelligence; excitement because in doing so two old
schools in AI, symbolic and connectionst, have joined forces;
excitement because likewise planning and learning are working
together; excitement because we are leaving behind the world of
heuristic (special) knwoledge, to enter the world of general methods;
excitement because, simply, it is exciting to understand what is
inside a Chess machine and to know what makes a Go machine tick;
excitement because the path of discovery of the scientists reads like
a detective story with many unexpected turns of events; and finally
excitement because this knowledge might enable you to take us further
on the road to machine intelligence$\ldots$  


%% section: topic (background) legitimization (why this book): to explain the tech behind the big breakthrough
%% section: problem statement
%% section: methods: theory and running practic eexample
%% section: outline

\section{Homo Ludens}
This is a book about intelligence and a book about games. In 1938 the great
Dutch historian and cultural theorist Johan Huizinga published Homo
Ludens. In this book he discussed the importance of the element of play in
human culture~\cite{huizinga1938homo}. In education and psychology the
concept of learning through play is well known. This book is not about human
culture or human learning, but about  artificial
intelligence. This book is about the
importance of the element of self play for learning, and
intelligence. AI is about creating mechanical devices that exhibit
intelligent behavior.  AI is a study of how
intelligence can be realized outside the human body. This book is
about how, through self play, computers can learn to play games of
intelligence (Go, Chess, and Shogi). The links of self play, and
reinforcement learning, between learning in AI and learning in
children is inescapable. To provide a glimpse of this link we will
highlight parallels between chapters of this book and the book
``Thinking, Fast and Slow,'' a book by psychologist and behavioral
economist Daniel Kahneman~\cite{kahneman2011thinking}.

\subsubsection{15 March 2016}
15 March 2016 is an important day in the history of intelligence. That
Tuesday was the final day of a five game match in which a computer
program challenged one of the strongest Go players known to
humanity. Go is an ancient game of strategy, played by millions around
the world, originating in South-east Asia. Playing the game well
requires a considerable amount of training and intelligence. Dedicated
Go-schools exist in China, Korea, and Japan, and professional Go
players achieve star-status in their countries and receive lucrative
prize money. 

On 15 March, at the Four Seasons hotel in Seoul, the computer program
AlphaGo beat top Go-professional Lee Sedol. The prize money, 1 million dollars, was donated by DeepMind
to charities. Lee Sedol received 170,000 dollars for his
efforts. Although the match consisted only of 5 games, the human
champion was beaten 4-1, and a subsequent match against Ke Jie was
also won by the computer. Commentators described AlphaGo's level of
play as strong, and the style of play as refreshing, with a few highly
surprising moves. AlphaGo was awarded a 9 dan professional rank, the
highest rank possible, by the Chinese Weiqi association, and the journal
Science chose the event as one of the breakthrough of the year runners
up. Today, human Go players are taking inspiration from the games
played by AlphaGo, trying to learn from its deep insights and unusual moves.

To add insult to injury, in 2017 
DeepMind team went even further. They created a version of AlphaGo, AlphaZero, that learned
to play the game from scratch, with zero human knowledge added, no
grandmaster games studied, and no Go knowledge
preprogrammed \cite{silver2016mastering,silver2017mastering,silver2017shogi,silver2018general}. Some
consider this AlphaZero work even more impressive, since it is said to
closely
resemble learning processes in human children.

The breakthrough performance of AlphaGo came as a surprise. The level
of play of computer Go programs had been languishing around the strong
amateur level for years. Experts in computer games had expected grand
master level play to be at least 10 years off, let alone beating the
world's strongest players.



\section{What is this book about?}
Therefore the main question that we are concerned with in this book is
the following.
{\em What caused the unexpected improvement in playing strength, what
technologies are combined in Go and got to work so well,
surprising Go experts and artifical intelligence researchers alike?}

Among the technologies are heuristic search methods, neural nets, and
compute power in the form of GPUs and cloud-computing. This book
provides an in depth introduction to them all, how they work, example
code, and references to the literature for more info. 

This book is about the  search-eval
architecture, and how it allowed advanced planning and learning
methods to work synergistically together. The book describes the
architecture, and the technologies that have been fitted into to it
that have been so successful, form heuristisc search,
exploration/exploitation, Monte Carlo, to neural nets and Deep Q
Learning. 

Planning (more
specifically Bandits and MCTS) and
Learning (more specifically DQN) are separate and active fields of study in their own
right. When they came together, in Turing's classic search-eval
architecture, they
caused a quantum leap, in Go. Getting techniques from two fields
to work together requires large efforts to understand (1) two fields and
(2) how they can work together. It is our hope that the explanations in
this book stimulate more efforts of scientists like
the DeepMind team to
cross boundaries and join efforts in both fields, allowing AI to solve
harder and harder problems.

An alternative problem statement, and a driving question, is: {\em What is
intelligence? Or more precise:  for Chess and Go, games for which humans
require intelligence, what  mechanical methods work? And what kind of
problems can these methods solve, and how can these methods be
extended?}

As you will see, although the methods for Chess and Go are quite
different (from brute force minimax to deep reinforcement learning)
there is a  commonality in both approaches, which is called the
search-eval architecture in this book. This architecture, devised by Turing around
the Second World War, is at the center of many intelligent machines.



\section{Search-Eval Exact-Approximate}
Finding the optimal policy in a game of intelligence entails searching
through extremely large state spaces. For small state spaces exact
methods that traverse the states one by one are suitable. They have
the advantage of giving precise answers, but are unsuitable for large
state spaces since it woudl just take too long. An alternative are approximation methods, that use
combinations of features of a state to approximate the value of a
state. They are fast, but not as precise as the exact methods. The
search-eval architecture provides a framework in which to 
combine the two approaches: exact search methods traverse a part of
the state spaces, and approximation methods evaluate states at some
point to prevent the traversal to take too long.

Exact methods are appropriate for low-dimensional spaces. Approximate
methods are appropriate for high-dimensional spaces. 

In the search-eval architecture
we can categorize different solutions for the search challenge and the
eval challenges. Originally,
when compute power was low, heuristics were used for both search and
eval, for both move selecting
and position feature evaluation. Section~\ref{forward} covers heuristic
forward pruning, and section~\ref{sec:eval} covers heuristic feature
evaluation. Plain heuristic forward pruning does not work well in most
games, although null move pruning~\cite{donninger1993null} and
Prob-cut~\cite{buro1997experiments} can be considered a kind of
forward pruning. Heuristic evaluation does work well in Chess and
Checkers, and when more compute power became available, the backward
pruning power of AlphaBeta turned out to achieve good results with full width
(no selectivity) search.

In Chapter~\ref{chap:trial} we will discuss alternatives
for heuristic selective search and evaluation by heuristic features. MCTS uses UCT
to trade off exploitation/exploration and averaged Monte Carlo
playouts for evaluation. In the next Chapters we will cover
position and policy approximation by feature recognition with neural
networks, and finally how planning can be used to train these networks.

\section{Symbolic and Connectionist}
Throughout the history of AI there have been two dominant schools of
thought: symbolic AI and connectionist AI. The school of symbolic AI
is rooted in logic and reasoning, and gave rise to expert systems. The
idea is that many aspects of intelligence can be studied
thorugh the manipulation of symbols. Symbolic AI is sometimes seen as
top down, theory driven. Dichotomies are always oversimplifications,
but if forced, planning and search would be symbolic AI.

Connectionist AI is bottom up, it believes that intelligence emerges
out of interactions of complex networks with their environment. Neural
networks and deep learning are prime examples of connectionist
AI. Learning would be connectionist.

As noted, forcing the real world into dichotomies does not always do
justice to the complexity of the real world. Learning may be
connectionist, but if an important part of the success of deep
learning is due to efficient backpropagation optimizers. And
optimizers are search algorithms, or symbolic AI.

It will be clear by now that this book is about the success of both: planning and
learning, symbolic and connectionist AI. 


\section{Planning and Learning}

The essence of the search-eval architecture is an intricate interplay
between two reinforcement learning methods: planning, and
learning. In the planning phase an exact lookahead algorithm generates
possible future states of the game, that are scored by an approximate value
function. This value function, for its part, can be a deep network
that is trained with the future states generated by the planner. The
planner generates states that the learner uses to improve the value
function (that is itself used by the planner to generate the states
(that are used by the learner (whose value function is used by the
planner (whose generated states are used by the learner
$\ldots$)))). See Fig.~\ref{fig:arch}.

The search-eval architecture consists of a virtuous circle of
planning and learning that help each other to improve their outcomes,
leading to an ever improving quality of play.
See Fig.~\ref{fig:dragon}.

The goal of this book is to familiarize the reader with this
architecture, and to discuss in depth the techniques that constitute
machine intelligence, so that the reader is well equipped to take the
next steps and perhaps help bring the field forward.



\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/arch.jpg}
\caption{Search--Eval Architecture}\label{fig:arch}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=5cm]{figures/dragon.jpg} &
\includegraphics[width=5cm]{figures/DrawingHands.jpg}
\end{tabular}
\caption{A Dragon biting in his own Tail and Escher's Self-drawing Hands}\label{fig:dragon}
\end{center}
\end{figure}

\section{From Heuristics to Learning}
The history of this book is from special to general. The chapters in
this book start with methods that need domain specific heuristics, and
end with methods that learn how to generalize features for many
domains. It is a story showiing how the first steps from  ASI towards
AGI were taken, tiny steps from Artificial Special
Intelligence towards Artificial General Intelligence.



\section{Learning to Learn}
This book also documents the path of AI researchers towards self
learning systems. It has been a long road, that started with trying to
mimic human knowledge. It started with coding heuristics,
approximations of what was thought to be relevant domain specific
knowledge. Quickly, a planner or searcher was put on top, to resolve
tactical and strategic issues. Then, adaptive search was invented, and
latern on generalizaiton. The role of heuristics steadily diminished,
as the success of general learning systems increased. Two parallel
developments helped:  the availability of large training databases
with labeled examples, and the avialability of large amounts of
compute power, especially in the form of GPUs.

This book covers all technologies behind the major AI breakthroughs in
playing games of intelligence: Chess, Atari, and Go. We
cover surprisingly diverse techniques, from heuristic planning to
deep learning to self-play.
\begin{itemize}
\item Heuristic Planning: Heuristic evaluation functions and
  alpha-beta search, and many important enhancements such as iterative
  deepening and transposition tables, all necessary ingredients for
  world championship level Chess
\item Monte Carlo Tree Search, the algorithm at the basis of the
  breakthrough in Go, including reinforcement learning, the paradigm
  necessary to understand how it works
\item Deep learning and deep reinforcement learning (DQN), which
  caused a sensation iby playing Atari from the raw pixels of the
  Arcade games
\item Self-play, the technology behing AlphaZero, allowing it to learn
  world championship level play in Go, from firsst principles, without
  any heuristic input
\item Current research in reinforcement learning are discussed, such
  as imperfect information, transfer
  learning, curriculum learning, and hierachical reinforcement
  learning, and how these techniques may develop and influence the
  future of AI, and the quest to artificial general intelligence
\end{itemize}


Thus, this book is also the story of AI researchers that were learning
to learn, and learning to forget about heuristics and 
knowledge engineering.



\section{Plan to Learn}
Table~\ref{tab:concepts} connects the main concepts covered in this
book from AI
and Psychology (or better, Kahneman). Note that Kahneman does not
feature reinforcement learning prominently, and does not label
explicitly the activity of using rational planning to generate
examples to train the patterns from. Since this training is quite
important in our architecture, we took the liberty of adding as 
a system 3, a system in which rational reasoning creates examples from 
which fast reflexes are trained.

Table~\ref{tab:paradigms} translates the main concepts to paradigms
for planing and learning on which the game players are based.

Table~\ref{tab:techniques} relates these paradigms  the techniques that
are used in the players.


Table~\ref{tab:architecture} concerns the search-eval and provides
details of the different algorithms that are used in the search, eval,
and two other important elements of the game players.




\begin{table}[ht]
\begin{center}
  \begin{tabular}{c|c}
    \hline\hline
     {\bf AI} &  {\bf  Kahneman}\\ \hline
    Feature Recognition  & System 1, Thinking Fast
    \\ \hline
    Planning, Reasoning & System 2, Thinking Slow \\ \hline
    Reinforcement Learning & {\em System 3, Training Very Slowly?}\\ \hline\hline
  \end{tabular}
  \caption{Concepts in Artificial Intelligence and Psychology}\label{tab:concepts}
  \end{center}
\end{table}

\begin{table}[ht]
\begin{center}
\input paradigm
\caption{Four Reinforcement Learning Paradigms}\label{tab:paradigms}
  \end{center}
\end{table}

\begin{table}[ht]
\begin{center}
\input technique
\caption{Techniques}\label{tab:techniques}
  \end{center}
\end{table}

\begin{table}[ht]
\begin{center}
\input searcheval
\caption{Search-Eval Architecture}\label{tab:architecture}
  \end{center}
\end{table}


\section{Hands on}
The following chapters will document these methods. We will take a
hands on artifical intelligence perspective. After each new method is
described, we will show how the concepts can be implemented in a
running example, which is a small Go program, naturally. Although you
probably do not have access to Google-scale computer power, at the end of
this book, a fully functional Go program that learns itself to play Go
will be in your hands.

\section{Graduate Course}
This book was designed also to be suited for an advanced/specialized
graduate course in Artificial Intelligence Game Playing. The material
is organized in chapters that should correspond to a one semester
course. The availability of source code should provide for practical
assignments where students can get their hands dirty and immerse
themselves in this fascinating topic, and having working pieces of
code that they can extend to their liking for further study. The book
will be used for such a Master-level course at Leiden University.

This book is designed ot be self-contained, necessary pieces of
information from other fields has been included to that purpose.

\section{Preliminary Knowledge}
This book is meant to be self contained. A basic introduction into
Markov Decision Process and reinforcement learning is provided. To
make the exercisses in this book, some proficiency on Python is
necessary. A general background uderstand into artificial intelligence
and neural networks is advantageous.

\section{Thinking Fast and Slow}
The philosophical implications of the AlphaGo achievement are
large. Although some humans knew that we are not the only intelligent race on
the planet (ask any dog, monkey or dolphin trainer) the realization
that we are now able to create a machine to learn to play such a
tremendously challenging and rich game of strategy, beating the
smartest professionals who have devoted their lives to learn the
intricacies of the game, is baffling. Indeed, if the goal of artificial
intelligence research is to understand intelligence, through the
creation of artificial versions of it, than we have made a tremendous
step. It now certainly appears that, 
at least for the narrow domain of a the most complicated board games,
we have succeeded at replicating learning processes and level of
intelligent reasoning for which humans need large amounts of
intelligence. 

Daniel Kahneman is a psychlogist and winner of the Nobel prize in
Economics. He is one of the founders of the field of behavioral
economics, through his work on prospect theory and many other works,
in which he combines psychology and economics. Based on his many
publications he has written a highly accessible book, which has been
on best sellers lists for many years now. It is called  
{\em Thinking Fast and Slow}, published in 2011~\cite{kahneman2011thinking}. In this book he presents the topics of his
most famous scientific works in a highly accessible way
\cite{kahneman2011thinking}. Kahneman describes System 1
thinking, or fast, approximate, intuitive thinking, and System 2
thinking, or exact, slow,
reasoned thinking. These two concepts fit well with the AI methods
described in these chapters.

For this reason we will highlight links between the  methods described here and the
concepts in Kahneman's book. In a way, since the philosophical
implications of the AI progress are undoubtedly large, we respectfully
point you to the work of Kahneman for these implications,
allowing us to focus in this book on the more technical AI methods. If
you think of this book as the companion of Kahneman's book for robots,
then that is somewhat appropriate, although current AI technology is
just starting to be intelligent in a very limited way. But the model
of thinking fast and slow is present. We call it planning and
learning. 


\section{Outline}
A major element in AI is to formalize problems in state spaces. For
interesting problems these
state spaces are very large, and much of AI is concerned with how to
efficienlty find solutions in these very large state spaces. In the following chapters, we will describe in depth the Artificial
Intelligence technologies that are behind these breakthroughs.

This book is organized in parts, from planning to learning to self
play, with chapters on the main discoveries, and three chapters for
advanced material. Depending on your interests, or the aim of the
course, some material can be skipped. Figure~\ref{fig:overview} shows
the structure of the chapters. The further to the right, the more
technical the chapters are.


\begin{figure}
\begin{center}
\input overview
\caption{Overview of the Chapters of this Book. Roman: General
  Content {\bf Bold: Technical Content} {\em Italics: Advanced Content}}\label{fig:overview}
  \end{center}
\end{figure}



We will
start in chapter~\ref{chap:games} with early thoughts on intelligent
machines, Alan Turing's chess program, the role of games in AI, and
the outline of the basic 
search-eval architecture. The techniques are rooted in different paradigms
(see Table~\ref{tab:paradigms}.)

Next, in
chapter~\ref{chap:search}, we 
introduce planning (thinking slow). The mathematical structure of the
large state space is used to traverse it in a smart way. When it is
still too large, heuristics are used for evaluation.  In this chapter we treat
in depth heuristic search methods at the basis of earlier AI breakthroughs, in
checkers and chess \cite{schaeffer1997kasparov}. These are based on
fixed depth fixed width 
methods minimax and AlphaBeta, and a first small program in
Python. Heuristics, encoding domain knowledge, were the first methods
used to deal with very large state spaces. Heuristics have been very
successful in some games and other domains.

It turns out that more is needed to achieve good performance. The
following chapter, chapter~\ref{chap:idtt} introduces many
enhancements to overcome some of the rigidity of the mathematical
approach. In this chapter variable depth and variabl width
enhancements are introduced.

In the next chapter, chapter~\ref{chap:trial}, we delve deeper in  the
principles of learning by trial and error. Major principles in this chapter are the
exploration/exploitaiton trade off, the concept of evaluation by
random play out, MCTS, and convergence concepts such as Q
learning. The algorithm in this chapter is variable depth and variable
width by design, and great performance improvements, especially in Go,
are achieved.

Then, we switch from planning to learning (thinking fast). We focus on the evaluation
function, and try to generalize features from the states. We start in
chapter~\ref{chap:super} with a short review of deep learning
methods for supervised learning. In 2012 these methods caused a
breakthrough in image recognition performance, and much of the
current intrest in AI is caused by these methods.

Chapter~\ref{chap:dqn} looks at how these methods can be used in a
reinforcement learning setting:
generalization of features in deep neural networks for learning by
trial and error, or Deep Q Networks,
DQN. We find that generalization is an effective method to deal with large
state spaces, and that DQN can be an effective way to replace
heuristic evaluation functions. 

In the next chapter, chapter~\ref{chap:conv}, we turn to self play. A
powerful paradigm where the machine teaches itself what to learn, by playing. We go deeper into
the methods that are needed to achieve good performance. Specifically,
we cover impediments, such as overfitting and myopia, in deep
reinforcement learning.

The next chapter,
chapter~\ref{chap:plan}, combines planning and learning, or MCTS and
DQN, the two major building 
blocks of AlphaGo. Here we will see how the two planning and
generalization can be combined to create self-learning systems. The
kind of learning of these systems resembles human learning. Finally,
we conclude in chapter~\ref{chap:conclusions} by reflecting on the
artificial intelligence progres and the relations to natural
intelligence.


%% \begin{table}\label{tab:arch}
%%   \begin{center}
%%     \begin{small}
%% \input tab-arch
%%   \caption{Search-Eval Architecture in different chapters}
%%   \end{small}
%%   \end{center}
%% \end{table}

\section{From Special to General}
The story in this book is also a history, and one on multiple
levels. It is a history of a specific kind of AI, the history of
computer playing intelligent board games. That history shows how
technology evolved, form the specific to the general---from
exploitative enumerative search and domain specific heuristics, to
exploration, generalization and domain specific features that are
learned by general methods.

At a deeper level, this is the story of
AI---from specific to general.  It is the story of a how a young field
with limited computional power tried to model a game of intelligence
through manual heuristics,
and through roadblocks and setbacks develops more general methods that
are applicable to other domains, that can learn and generalize. It is the story of how two areas of AI
that were quite distinct---symbolic AI and connectionist AI---came
together to create a success. It is the story of planning and learning. It is
also the story of one constant: 
the search-eval architecture.

These are the first baby steps on the road to
Artificial General Intelligence---a history worth to be documented and
learned from. Hold on tight, for the story of 70 years of artificial intelligence.

\section{Stories}
There are many stories in this book, and they are all related. 
See Figure~\ref{fig:stories}.

\begin{figure}
\begin{center}
\input stories2
\caption{Overview of the Story Lines in this Book}\label{fig:stories}
  \end{center}
\end{figure}

\begin{itemize}
\item In Eval, From Heuristics to Learning is Special to General is
  Weak to Powerful
\item In Search (planning), From alpha-beta to MCTS is Rigid to Adaptive
  
  \item From Plan to Learn to Self Play is Plan+Learn
    
\item From Slow to Fast to ??? (become a pro in $x$ in 10,000 hour of training?)
  \item From Symbolic to Connectionist is indeed from Heuristics to
    Learning
    \item Heuristics is not search, Learning is not eval

  \item A constant is the search-eval architecture---in all programs
    there is a search component interacting with an eval component
    (except Atari)
  \item The coming of age of Self Play---Learning to Play

\end{itemize}
And: note that computers are now learning faster than humans. AlphaZero
learns to play Go in a few days, where humans take years to master the
game.

If you forgive the blatant anthropomorphization, not only are computers better
at playing Chess and Go, they are now also better at {\em learning\/} to
play Chess and Go, and what is more, they teach themselves.

\section{Outlook}
\begin{itemize}
\item Self play works
\item  Computers can now learn faster than humans and they teach themselves.
  \item Future research will yield many new developments in self learning:
  \begin{itemize}
  \item in applications, such as medicine, and new uses of intelligent
    decision making
    \item in fundamental learning. Through self play, learning will
      be  more powerful
  \end{itemize}
\item The reason is that self play generates an efficient curriculum
  learning method for self learning
 
% \item Message: Self Play is Plan + Learn. We need Plan. Machine
% learning needs reasoning 
\end{itemize}
Students studying AI should learn about this, hence this book.

%% \section{Old Stuff}
%% % This stuff is more like a preface
%% \section{why this book}
%% To explain what makes alphago tick, this book explains the recent leaps in reinforcement learning.

%% The AlphaGo Nature papers explained. The AlphaGo technology is truly
%% breathtaking. As any good science, the technology has been published
%% in scientific papers. The Nature publications of 2015, 2016, and 2017
%% by the DeepMind team are the prime source of information
%% \cite{mnih2015human,silver2016mastering,silver2017mastering}. They are
%% well written, explaining all details. However, the articles are full
%% with details, and expect much background knowledge. Even for insiders
%% it is a daunting task to understand all details. The purpose of this
%% book is to collect all necessary information and to explain it in a
%% comprehensive way to make it easier to understand. For AI researchers,
%% and for those aspiring to become one. 

%% \section{intended audience}
%% Researchers and Graduate Students interested in planning and learning,
%% the technology behind AlphaGo. I have tried to make the text self
%% contained, and as accessible as possible to a wider audience, since
%% the field of computer games has traditionally thrived by the attention
%% and contributions of scientists and non-scientists alike. 

%% This book is the reult of three lectures on the technology behind the
%% successes of modern reinforcement learning. The first was an early
%% lecture in October 2016 for the KNAW, for a general audience, given
%% together with my colleagues Max Welling and Tom Heskes. The second was
%% a guest lecture in the Master course Reinforcement Learning at Leiden
%% University. The lecture was crammed with details, I talked as fast as
%% I could, and there was not nearly enough time to explain many of the
%% deep concepts in full. Thus, the idea for a longer treatment was
%% born. The third lecture was for an audience of physicists, at
%% Innsbruck University. In all lectures, the audience wanted to know all
%% details to understand, essentially, how AlphaGo thinks. In all three
%% lectures there was barely enough time to scratch the surface. This
%% book is my way of making amends to these three audiences.  

%% \section{what we will discuss}
%% planning and learning

%% \section{contributions}
%% The search-eval architecture has been with us since the start of AI,
%% it was the basis of the first chess program design. Now, with AlphaGo,
%% a new incarnation has shown the great power of this classic
%% architecture. The architecure may be old, but the technology inside is
%% brand new. This book explains both the architecture and the
%% technology inside needed to make a truly self-learning computer
%% program for one of the hardest games known to mankind.
%% The question is, where can it lead us further, what kind of
%% problems can be solved next?

%% \begin{itemize}
%% \item First coherent treatment of planning and learning, the two
%%   technology working in synergy in AlphaGo (see nature paper)
%% \item document important new incarnation of search-eval architecture
%%   as it allowed step towards general artifical intelligence  (see
%%   nature paper)
%% \item comprehensive overview of all necessary technology, from
%%   minimax, hash tables, to nets and DQN 
%% \item the book has two main threads: A practical one, in each chapter
%%   you will build elements of a working Hex program (or 9x9 go?); A
%%   philosophical one, in each chapter the learned mechaisms are
%%   compared with what we know of human thought, thinking fast and
%%   slow. 
  
%% \end{itemize}  


==> chapters/old02games.tex <==
%% 2: games
%% section: behaviorist view of intelligence: memory, reasoning, and learning. turing test
%% section: games in ai: drosophila: simpler reality, strict rules
%% section: history checkers, chess (turing, russians, deep blue-kasparav)
%% section: lookahead: search-eval architecture
%% section: example: 9x9 go in python, or hex or ttt

%FIRST WRITE TOP DOWN STRUCTURE

%add words to the sections $\rightarrow$ make subsections

%Landmarks

%Methods

The topic of this chapter is to introduce the reason why to study the
topic of this book. We discuss the behavioristic approach to
intelligence, and further narrow the scope of the study of artificial
intelligence to domains  with clear and well defined rules, yet
providing exciting challenges to human intelligence: board games such
as Chess, Checkers, and Go. We will provide a short historic overview
of early work in these fields. 
\section*{Learning Goals}
\begin{itemize}
\item {\bf It is exciting to learn the history of the old AI-ers, and
  their dreams of creating machine intelligence. Emotion in the old
  guys and their dreams}
  \item intelligent behavior and games
  \item history of games
\end{itemize}


\section{Intelligent Behavior}
What is intelligence? Human intelligence is embodied, humans are conscious,
self-aware. Intelligence implies reasoning, memory, learning,
problem solving skills, emotion, adaptivity, and creativity. The former is about {\em
being\/} intelligent. The latter list is about {\em acting\/}
intelligent.

We will now discuss these aspects in more depth.

\subsection{Cognition}
           Intelligence has been defined in many ways, including
           cognitive aspects: the
           capacity for logic, understanding, self-awareness,
           learning, emotional knowledge, reasoning, planning,
           creativity, and problem solving. 

           Intelligence gives humans the cognitive abilities to learn, form
           concepts, understand, and reason, including the capacities
           to recognize patterns, comprehend ideas, plan, solve
           problems, and use language to communicate. Intelligence
           enables humans to experience and think.

\subsection{Embodiment}
           {\bf embodied intelligence discussion}
           {\bf skills list: memory, reasoning, learning, creativity,
             emotion, consciousness, interaction, adaptation, language, speech}
           {\bf behaviorist view}
More generally, it can be
           described as the ability to perceive or infer information,
           and to retain it as knowledge to be applied towards
           adaptive behaviors within an environment or context, in a more
           embodied sense.
           
Embodied cognition is the theory that many features of cognition,
whether human or otherwise, are shaped by aspects of the entire body
of the organism. The features of cognition include high level mental
constructs (such as concepts and categories) and performance on
various cognitive tasks (such as reasoning or judgment). The aspects
of the body include the motor system, the perceptual system, bodily
interactions with the environment (situatedness) and the assumptions
about the world that are built into the structure of the organism. 

The embodied mind thesis challenges other theories, such as
cognitivism, computationalism, and Cartesian dualism.[1][2] It is
closely related to the extended mind thesis, situated cognition and
enactivism. The modern version depends on insights drawn from recent
research in psychology, linguistics, cognitive science, dynamical
systems, artificial intelligence, robotics, animal cognition, plant
cognition and neurobiology.

At the heart of the Computational Theory of Mind is the idea that
thoughts are a form of computation, and a computation is by definition
a systematic set of laws for the relations among representations.  
           
\subsection{Artificial Intelligence}
           Among the traits that researchers hope machines will
           exhibit are reasoning, knowledge, planning, learning,
           communication, perception, and the ability to move and to
           manipulate objects.[27][28] In the field of artificial
           intelligence there is no consensus on how closely the brain
           should be simulated. 

\subsubsection{Behavior: Turing Test}
behaviorist view of intelligence: memory, reasoning, and
learning. turing test

The Turing test, developed by Alan Turing in 1950, is a test of a
machine's ability to exhibit intelligent behavior equivalent to, or
indistinguishable from, that of a human. Turing proposed that a human
evaluator would judge natural language conversations between a human
and a machine designed to generate human-like responses. The evaluator
would be aware that one of the two partners in conversation is a
machine, and all participants would be separated from one another. The
conversation would be limited to a text-only channel such as a
computer keyboard and screen so the result would not depend on the
machine's ability to render words as speech.[2] If the evaluator
cannot reliably tell the machine from the human, the machine is said
to have passed the test. The test results do not depend on the
machine's ability to give correct answers to questions, only how
closely its answers resemble those a human would give. 

The test was introduced by Turing in his 1950 paper, "Computing
Machinery and Intelligence", while working at the University of
Manchester (Turing, 1950; p. 460).[3] It opens with the words: "I
propose to consider the question, 'Can machines think?'"  

\subsection{Generalization}
           {\bf general discussion}
           general is common, is essential features. generalization is
           learning is intelligence

           A generalization (or generalisation) is the formulation of
           general concepts from specific instances by abstracting
           common properties.

           Generalization is the process of identifying the parts of a
           whole, as belonging to the whole

           When the mind makes a generalization, it extracts the
           essence of a concept based on its analysis of similarities
           from many discrete objects. The resulting simplification
           enables higher-level thinking.

In the context of AI, generalization is feature learning, one of the
core technologies used in function approximation.

           
\subsection{Special and General Intelligence}
           Artificial general intelligence (AGI) is the intelligence of a machine that could successfully perform any intellectual task that a human being can. It is a primary goal of some artificial intelligence research and a common topic in science fiction and future studies. Some researchers refer to Artificial general intelligence as "strong AI",[1] "full AI"[2] or as the ability of a machine to perform "general intelligent action"[3]; others reserve "strong AI" for machines capable of experiencing consciousness.

Some references emphasize a distinction between strong AI and "applied AI"[4] (also called "narrow AI"[1] or "weak AI"[5]): the use of software to study or accomplish specific problem solving or reasoning tasks. Weak AI, in contrast to strong AI, does not attempt to perform the full range of human cognitive abilities.

As of 2017, over forty organizations worldwide are doing active
research on AGI.[6]



\section{Games, the Drosophila of AI}
In 1965, the Soviet mathematician Aleksandr Kronrod called chess the
Drosophila Melanogaster of Artificial Intelligence~\cite{landis2001aleksandr},
see Fig.~\ref{fig:drosophila}. The Drosophila Melanogaster, a type of
fruit fly, has been used by developmental biologists in genetics
experiments, because of it fast procreation cycle. Researchers could see quickly results of their
experiments.
\index{Drosophila Melanogaster}

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/drosophila.jpg}
\caption{Drosophila Melanogaster (fruit fly)}\label{fig:drosophila}
\end{center}
\end{figure}

AI research was also in need of a suitable domain for experimentation
that would yield rapid turnaround times. Chess was a convenient domain
that was well suited for experimentation. It was considered the game
of intelligence par excellence, requiring highly intelligent human
beings to study for many years to acquire proficiency. The rules are
clear and unambiguous. Results are easily measured, all one needs to
do is let different programs play against eachother, and it is known
which is the strongest. 

Indeed, dedicated research  all over the world created quick
progress. In only three decades the dream of beating the human world
champion was realized. On May 11, 1997 Garry Kasparov, the highest
rated human chess player ever, was defeated by the computer
program \textsc{Deep Blue}, in a highly publicized six game match in
New York.  

\subsubsection{Limited Scope}
Ever since the start of AI games have played an important role to
experiment with new ideas and to measure progress. The goal of AI is
to create mechanisms for inelligent behavior, to be measured,
ultimately, by how well a device performs in the real world. Smart
researchers start small, with challenges that are large, require
intelligence, but are nevertheless manageable. The scope of a game is
defined by its rules, and games are used frequently within AI as a
domain of study. 

\subsubsection{Clear Rules}
In addition to limited scope, a second advantage of games are the
clarity of the rules. Games have a clear goal, and the possible
actions are well defined by the rules. In this, games differ from the
real world, where rules are often implicit and vague. Thus, games are
easier to solve than many real world tasks, an advantage for
researchers that want to achieve the larger goal in small steps.

\subsubsection{Clear Performance}
Games allow for a clear and undisputed way to measure progress. Games
define winners, and the intellignece of programs can be measured by
letting them play against eachother or against humans. Many games have
rating systems, such as in tennis, where the best of the world are
ranked based on how many wins have been scored against players of
different rankings. In many board games the Elo-rating is calculated,
a system devised by the Hungarian-American physicist  Arpad Elo based
on pairwise comparison \cite{elo1978rating}.

\subsubsection{Special Intelligence}
If our goal is to pass the Turing test, in which {\em any\/} question
can be asked of our machine, then this would test for General
Intelligence, the same kind of intelligence that humans have. Limiting
the scope of our domain to a single game clearly cannot be used to
achieve general intelligence, all we can hope is to achieve special
intelligence, the kind of intelligence needed to win a certain
game. Still, achievements in special intelligence, such as by Deep
Blue, Watson and AlphaGo, attract large publicity. This may be in part
because the human mind generalizes easily, and
anthropomorphizes\footnote{I.e., treat as if human.}
easily. When we see a device do something in a particular domain for
which a human must be incredibly smart, we often assume that the device
must {\em be\/} smart, and will do just as well in another domain {\em
because that is what a human would do}. We forget that a machine is
not a human. And when the machine does not know how to do the simplest thing in
another domain, such as how to make a sandwich, or play another game
for that matter, we are disappointed.

Because of this, we are interested not just in special intelligence,
but also in general intelligence, or at least in AI's that are
intelligent in more than one domain.
The field of transfer learning studies how knowledge that is learned
in one domain can be transfered to another
domain. Chapter~\ref{chap:transfer} discusses transfer learning.

\subsubsection{Drosophila Melanogaster}
Thus, games are a suitable testbed for AI experimentation~\cite{mandziuk2007computational}. The first
game to be heavily studied was Chess, thought to be the game of
intelligence par excellence. For this reason Kronrod named Chess the
Drosophila Melanogaster, or experimental testbed of choice, of AI. And
indeed, for many decades many researchers used it to great advantage,
achieving great progress, and developing many ingenious computational methods to
achieve a level of play, ultimately beating the strongest human minds
in the world.

Then, a new Drosophila had to be found, which would become Go.

\subsection{History of AI}
{\bf show that AI has fascinated humans for ages. It is one of the big
qurstions. short. 2 paragraphs}

``The history of Artificial Intelligence (AI) began in antiquity, with
myths, stories and rumors of artificial beings endowed with
intelligence or consciousness by master craftsmen; as Pamela McCorduck
writes, AI began with "an ancient wish to forge the gods."[1] 

Mary Shelley published the story of Frankenstein; or the Modern
Prometheus, a fictional consideration of the ethics of creating
sentient beings. 


The seeds of modern AI were planted by classical philosophers who
attempted to describe the process of human thinking as the mechanical
manipulation of symbols. This work culminated in the invention of the
programmable digital computer in the 1940s, a machine based on the
abstract essence of mathematical reasoning. This device and the ideas
behind it inspired a handful of scientists to begin seriously
discussing the possibility of building an electronic brain. 

The field of AI research was founded at a workshop held on the campus
of Dartmouth College during the summer of 1956.[2] Those who attended
would become the leaders of AI research for decades. Many of them
predicted that a machine as intelligent as a human being would exist
in no more than a generation and they were given millions of dollars
to make this vision come true. 

Eventually it became obvious that they had grossly underestimated the
difficulty of the project.

In 1973, in response to the criticism from
James Lighthill and ongoing pressure from congress, the U.S. and
British Governments stopped funding undirected research into
artificial intelligence, and the difficult years that followed would
later be known as an "AI winter". Seven years later, a visionary
initiative by the Japanese Government inspired governments and
industry to provide AI with billions of dollars, but by the late 80s
the investors became disillusioned by the absence of the needed
computer power (hardware) and withdrew funding again. 

Investment and interest in AI boomed in the first decades of the 21st
century, when machine learning was successfully applied to many
problems in academia and industry due to the presence of powerful
computer hardware.'' 

The dream of artificial intelligence was first thought of in Indian
philosophies like those of Charvaka, a famous philosophy tradition
dating back to 1500 BCE and surviving documents around 600
BCE. McCorduck (2004) writes "artificial intelligence in one form or
another is an idea that has pervaded intellectual history, a dream in
urgent need of being realized," expressed in humanity's myths,
legends, stories, speculation and clockwork automatons.[3] 

AI in myth, fiction and speculation[edit]
Main article: Artificial intelligence in fiction
Mechanical men and artificial beings appear in Greek myths, such as
the golden robots of Hephaestus and Pygmalion's Galatea.[4] In the
Middle Ages, there were rumors of secret mystical or alchemical means
of placing mind into matter, such as Jābir ibn Hayyān's Takwin,
Paracelsus' homunculus and Rabbi Judah Loew's Golem.[5] By the 19th
century, ideas about artificial men and thinking machines were
developed in fiction, as in Mary Shelley's Frankenstein or Karel
Čapek's R.U.R. (Rossum's Universal Robots),[6] and speculation, such
as Samuel Butler's "Darwin among the Machines."[7] AI has continued to
be an important element of science fiction into the present. 

Automatons[edit]
Main article: Automaton

Al-Jazari's programmable automata (1206 CE)
Realistic humanoid automatons were built by craftsman from every
civilization, including Yan Shi,[8] Hero of Alexandria,[9]
Al-Jazari[10] , Pierre Jaquet-Droz, and Wolfgang von Kempelen.[11] The
oldest known automatons were the sacred statues of ancient Egypt and
Greece. The faithful believed that craftsman had imbued these figures
with very real minds, capable of wisdom and emotion—Hermes
Trismegistus wrote that "by discovering the true nature of the gods,
man has been able to reproduce it.

Artificial intelligence is based on the assumption that the process of
human thought can be mechanized. The study of mechanical—or
"formal"—reasoning has a long history. Chinese, Indian and Greek
philosophers all developed structured methods of formal deduction in
the first millennium BCE. Their ideas were developed over the
centuries by philosophers such as Aristotle (who gave a formal
analysis of the syllogism), Euclid (whose Elements was a model of
formal reasoning), al-Khwārizmī (who developed algebra and gave his
name to "algorithm") and European scholastic philosophers such as
William of Ockham and Duns Scotus.[14] 

Majorcan philosopher Ramon Llull (1232–1315) developed several logical
machines devoted to the production of knowledge by logical means;[15]
Llull described his machines as mechanical entities that could combine
basic and undeniable truths by simple logical operations, produced by
the machine by mechanical meanings, in such ways as to produce all the
possible knowledge.[16] Llull's work had a great influence on
Gottfried Leibniz, who redeveloped his ideas.[17] 

In the 20th century, the study of mathematical logic provided the
essential breakthrough that made artificial intelligence seem
plausible. The foundations had been set by such works as Boole's The
Laws of Thought and Frege's Begriffsschrift. Building on Frege's
system, Russell and Whitehead presented a formal treatment of the
foundations of mathematics in their masterpiece, the Principia
Mathematica in 1913. Inspired by Russell's success, David Hilbert
challenged mathematicians of the 1920s and 30s to answer this
fundamental question: "can all of mathematical reasoning be
formalized?"[14] His question was answered by Gödel's incompleteness
proof, Turing's machine and Church's Lambda calculus.[14][21] 


The ENIAC, at the Moore School of Electrical Engineering. This photo has been artificially darkened, obscuring details such as the women who were present and the IBM equipment in use.[22]
Their answer was surprising in two ways. First, they proved that there
were, in fact, limits to what mathematical logic could accomplish. But
second (and more important for AI) their work suggested that, within
these limits, any form of mathematical reasoning could be
mechanized. The Church-Turing thesis implied that a mechanical device,
shuffling symbols as simple as 0 and 1, could imitate any conceivable
process of mathematical deduction. The key insight was the Turing
machine—a simple theoretical construct that captured the essence of
abstract symbol manipulation. This invention would inspire a handful
of scientists to begin discussing the possibility of thinking
machines.

``The Dartmouth Conference of 1956[39] was organized by Marvin Minsky,
John McCarthy and two senior scientists: Claude Shannon and Nathan
Rochester of IBM. The proposal for the conference included this
assertion: "every aspect of learning or any other feature of
intelligence can be so precisely described that a machine can be made
to simulate it".[40] The participants included Ray Solomonoff, Oliver
Selfridge, Trenchard More, Arthur Samuel, Allen Newell and Herbert
A. Simon, all of whom would create important programs during the first
decades of AI research.[41] At the conference Newell and Simon debuted
the "Logic Theorist" and McCarthy persuaded the attendees to accept
"Artificial Intelligence" as the name of the field.[42] The 1956
Dartmouth conference was the moment that AI gained its name, its
mission, its first success and its major players, and is widely
considered the birth of AI.[43]''

In June 1963, MIT received a \$2.2 million grant from the newly created
Advanced Research Projects Agency (later known as DARPA). The money
was used to fund project MAC which subsumed the "AI Group" founded by
Minsky and McCarthy five years earlier. DARPA continued to provide
three million dollars a year until the 70s.[63] DARPA made similar
grants to Newell and Simon's program at CMU and to the Stanford AI
Project (founded by John McCarthy in 1963).[64] Another important AI
laboratory was established at Edinburgh University by Donald Michie in
1965.[65] These four institutions would continue to be the main
centers of AI research (and funding) in academia for many years.[66] 



\subsection{History of Computing}
{\bf delete. replace by history of AI. Add females. Move Shannon and
  Turing to the Games Programs section as inventors of the search-eval
architecture}

AI is old. It has been around at least as long as computer science. A strong
case  can be made that the vision of creating a machine that thinks is
what caused computers to be  
conceived at all. The history of computation is also rich with names of
people behind important inventions.

``Around 1621, Wilhelm Schickard
built a machine based on gears for doing simplified multiplications
involved in Johannes Kepler's calculations of the orbit of the Moon.
Gottfried Leibniz became one of the most prolific inventors in the
field of mechanical calculators. While working on adding automatic
multiplication and division to Pascal's calculator, he was the first
to describe a pinwheel calculator in 1685 and invented the Leibniz
wheel, used in the arithmometer, the first mass-produced mechanical
calculator.

John Napier 1550-1617 John Napier is best known as the discoverer of
logarithms, John Napier was famous for his devices to assist with
computation. He invented a well-known mathematical artifact, the
ingenious numbering rods more quaintly known as “Napier's bones,” that
offered mechanical means for facilitating computation.

Charles Babbage  is credited with inventing the first mechanical
computer that eventually led to more complex electronic designs,
though all the essential ideas of modern computers are to be found in
Babbage's analytical engine.

Augusta Ada King, Countess of Lovelace
(née Byron; 10 December 1815 – 27 November 1852) was an English
mathematician and writer, chiefly known for her work on Charles
Babbage's proposed mechanical general-purpose computer, the Analytical
Engine. She was the first to recognise that the machine had
applications beyond pure calculation, and published the first
algorithm intended to be carried out by such a machine. As a result,
she is sometimes regarded as the first to recognise the full potential
of a "computing machine" and the first computer programmer.

Joseph
Marie Jacquard, Joseph Marie Charles Jacquard (1752-1834) was a French
weaver and merchant. He played an important role in the development of
the earliest programmable loom (the "Jacquard loom"), which in turn
played an important role in the development of other programmable
machines, such as an early version of digital compiler used by IBM to
develop the modern day computer.

Maria Mitchell (1818-1889) was an American
astronomer who computed the motion of the planet Venus.

Herman
Hollerith (1860 - 1929) was an American
inventor who developed an electromechanical punched card tabulator to
assist in summarizing information and, later, accounting. He was the
founder of the Tabulating Machine Company that was amalgamated (via
stock acquisition) in 1911 with three other companies to form a fifth
company, the Computing-Tabulating-Recording Company later renamed
IBM. Hollerith is regarded as one of the seminal figures in the
development of data processing. His invention of the punched card
tabulating machine marks the beginning of the era of semiautomatic
data processing systems, and his concept dominated that landscape for
nearly a century.

Grace Brewster Murray Hopper (1906–1992) was an American computer
scientist and United States Navy 
rear admiral. One of the first programmers of the Harvard Mark I
computer, she was a pioneer of computer programming who invented one
of the first compiler related tools. She popularized the idea of
machine-independent programming languages, which led to the
development of COBOL, an early high-level programming language still
in use today. Prior to joining the Navy, Hopper attained a Ph.D. in
mathematics from Yale University and was a professor of mathematics at
Vassar College.

Howard Hathaway Aiken (1900–1973) was an American
physicist and a pioneer in computing, being the original conceptual
designer behind IBM's Harvard Mark I computer

Claude Elwood Shannon (April 30, 1916 – February 24, 2001) was an
American mathematician, electrical engineer, and cryptographer known
as "the father of information theory". Shannon is noted for having
founded information theory with a landmark paper, A Mathematical
Theory of Communication, that he published in 1948. He is, perhaps,
equally well known for founding digital circuit design theory in 1937,
when—as a 21-year-old master's degree student at the Massachusetts
Institute of Technology (MIT)—he wrote his thesis demonstrating that
electrical applications of Boolean algebra could construct any logical
numerical relationship. On March 9, 1949, Shannon presented a paper
called "Programming a Computer for playing Chess." The paper was
presented at the National Institute for Radio Engineers Convention in
New York. He described how to program a computer to play chess based
on position scoring and move selection. He proposed basic strategies
for restricting the number of possibilities to be considered in a game
of chess. In March 1950 it was published in Philosophical Magazine,
and is considered one of the first articles published on the topic of
programming a computer for playing chess, and using a computer to
solve the game~\cite{shannon1988programming}. 


Joan Elisabeth Lowther Murray, MBE (née Clarke; 24 June 1917 – 4
September 1996) was an English cryptanalyst and numismatist best known
for her work as a code-breaker at Bletchley Park during the Second
World War. Though she did not personally seek the spotlight, her role
in the Enigma project that decrypted Nazi Germany's secret
communications earned her awards and citations, such as appointment as
a Member of the Order of the British Empire (MBE), in 1946.


Alan Mathison Turing OBE FRS (1912-1954)
was an English mathematician, computer scientist, logician,
cryptanalyst, philosopher and theoretical biologist.[6] Turing was
highly influential in the development of theoretical computer science,
providing a formalisation of the concepts of algorithm and computation
with the Turing machine, which can be considered a model of a
general-purpose computer. Turing is widely considered to be
the father of theoretical computer science and artificial
intelligence. Despite these accomplishments, he was never fully
recognized in his home country during his lifetime due to his
homosexuality, which was then a crime in the UK.

Turing addressed the problem of artificial intelligence, and proposed
an experiment that became known as the Turing test, an attempt to
define a standard for a machine to be called "intelligent". The idea
was that a computer could be said to "think" if a human interrogator
could not tell it apart, through conversation, from a human being



Adele Goldstine (1920 – 1964) was an
American mathematician and computer programmer. She wrote the manual
for the first electronic digital computer, ENIAC. Through her work
programming the computer, she was also an instrumental player in
converting the ENIAC from a computer that needed to be reprogrammed
each time it was used to one that was able to perform a set of fifty
stored instructions

Konrad Zuse (1910–1995) was a German civil engineer, inventor and
computer pioneer. His 
greatest achievement was the world's first programmable computer; the
functional program-controlled Turing-complete Z3 became operational in
May 1941. Thanks to this machine and its predecessors, Zuse has often
been regarded as the inventor of the modern computer.''

We will now look at a short history of significant achievements in
computer game programming.

\subsection{Strachey}
{\bf why? first working games program}
In 1951, using the Ferranti Mark 1 machine of the University of
Manchester, Christopher Strachey wrote a checkers program and Dietrich
Prinz wrote one for chess.[33] Arthur Samuel's checkers program,
developed in the middle 50s and early 60s, eventually achieved
sufficient skill to challenge a respectable amateur.[34] Game AI would
continue to be used as a measure of progress in AI throughout its
history. 

\subsection{Alan Turing 1950}
{\bf why? first paper chess program. search-eval arch}

``In 1948 Turing, working with his former undergraduate colleague,
D.G. Champernowne, began writing a chess program for a computer that
did not yet exist. By 1950, the program was completed and dubbed the
Turbochamp.[108] In 1952, he tried to implement it on a Ferranti Mark
1, but lacking enough power, the computer was unable to execute the
program. Instead, Turing "ran" the program by flipping through the
pages of the algorithm and carrying out its instructions on a
chessboard, taking about half an hour per move. The game was
recorded.[109] According to Garry Kasparov, Turing's program "played a
recognizable game of chess."[110] The program lost to Turing's
colleague Alick Glennie, although it is said that it won a game
against Champernowne's wife, Isabel''


\begin{figure}[t]
\begin{center}
\includegraphics[width=3cm]{figures/turing}
\caption{Alan Turing}\label{fig:turing}
\end{center}
\end{figure}
\index{Alan Turing}

\subsection{Samuel Checkers 1960}
{\bf why? first reasonable checkers program, first search eval self play
  machine learning}

\cite{samuel1959some}
Arthur Samuel (IBM) wrote the first game-playing program,[30] for checkers (draughts), to achieve sufficient skill to challenge a respectable amateur. His first checkers-playing program was written in 1952, and in 1955 he created a version that learned to play.[31]

Samuel is most known within the AI community for his groundbreaking
work in computer checkers in 1959, and seminal research on machine
learning, beginning in 1949.[6] He graduated from MIT and taught at
MIT and UIUC from 1946 to 1949.[10] He believed teaching computers to
play games was very fruitful for developing tactics appropriate to
general problems, and he chose checkers as it is relatively simple
though has a depth of strategy. The main driver of the machine was a
search tree of the board positions reachable from the current
state. Since he had only a very limited amount of available computer
memory, Samuel implemented what is now called alpha-beta pruning.[11]
Instead of searching each path until it came to the game's conclusion,
Samuel developed a scoring function based on the position of the board
at any given time. This function tried to measure the chance of
winning for each side at the given position. It took into account such
things as the number of pieces on each side, the number of kings, and
the proximity of pieces to being “kinged”. The program chose its move
based on a minimax strategy, meaning it made the move that optimized
the value of this function, assuming that the opponent was trying to
optimize the value of the same function from its point of view.[12] 

Samuel also designed various mechanisms by which his program could
become better. In what he called rote learning, the program remembered
every position it had already seen, along with the terminal value of
the reward function. This technique effectively extended the search
depth at each of these positions. Samuel's later programs reevaluated
the reward function based on input from professional games. He also
had it play thousands of games against itself as another way of
learning. With all of this work, Samuel's program reached a
respectable amateur status, and was the first to play any board game
at this high a level. He continued to work on checkers until the
mid-1970s, at which point his program achieved sufficient skill to
challenge a respectable amateur.[13 

\subsection{Backgammon 1992}
{\bf why? first world class level games program. self play
  reinforcement learning eval. neural net, mostly eval. Inspiration
  for the moderns: Atari and AlphaGo}
  
1992 TD Gammon \cite{tesauro2002programming} Tesauro. A
reimplementation in Tensorflow is at
\href{https://github.com/fomorians/td-gammon}{TD-gammon}.

TD-Gammon, a backgammon program written by Gerry Tesauro, demonstrates
that reinforcement (learning) is powerful enough to create a
championship-level game-playing program by competing favorably with
world-class players.

During play, TD-Gammon examines on each turn all possible legal moves and all their possible responses (two-ply look-ahead), feeds each resulting board position into its evaluation function, and chooses the move that leads to the board position that got the highest score. In this respect, TD-Gammon is no different than almost any other computer board-game program. TD-Gammon's innovation was in how it learned its evaluation function.

TD-Gammon's learning algorithm consists of updating the weights in its neural net after each turn to reduce the difference between its evaluation of previous turns' board positions and its evaluation of the present turn's board position—hence "temporal-difference learning". The score of any board position is a set of four numbers reflecting the program's estimate of the likelihood of each possible game result: White wins normally, Black wins normally, White wins a gammon, Black wins a gammon. For the final board position of the game, the algorithm compares with the actual result of the game rather than its own evaluation of the board position.[1]

Unlike previous neural-net backgammon programs such as Neurogammon (also written by Tesauro), where an expert trained the program by supplying the "correct" evaluation of each position, TD-Gammon was at first programmed "knowledge-free".[1] In early experimentation, using only a raw board encoding with no human-designed features, TD-Gammon reached a level of play comparable to Neurogammon: that of an intermediate-level human backgammon player.

Even though TD-Gammon discovered insightful features on its own,
Tesauro wondered if its play could be improved by using hand-designed
features like Neurogammon's. Indeed, the self-training TD-Gammon with
expert-designed features soon surpassed all previous computer
backgammon programs. It stopped improving after about 1,500,000 games
(self-play) using 80 hidden units.[2]

Backgammon expert Kit Woolsey found that TD-Gammon's positional judgement, especially its weighing of risk against safety, was superior to his own or any human's.[1]

TD-Gammon's excellent positional play was undercut by occasional poor
endgame play. The endgame requires a more analytical approach,
sometimes with extensive lookahead. TD-Gammon's limitation to two-ply
lookahead put a ceiling on what it could achieve in this part of the
game. TD-Gammon's strengths and weaknesses were the opposite of
symbolic artificial intelligence programs and most computer software
in general: it was good at matters that require an intuitive "feel"
but bad at systematic analysis.


\subsection{Schaeffer Checkers 1994}
{\bf why? first world champion program. Also: first solved game (after
TTT (picture), nine Men's Morris (picture), Connect4 (picture), etc)}
           
\cite{schaeffer1992world,schaeffer1996chinook}
\index{Chinook}
\index{Checkers}
\index{Tinsley}
English draughts (checkers) world champion Tinsley resigned a match against computer program Chinook. Chinook defeated 2nd highest rated player, Lafferty. Chinook won the USA National Tournament by the widest margin ever.

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/checkers}
\caption{Checkers}\label{fig:checkers}
\end{center}
\end{figure}
\cite{schaeffer2008one}
Chinook is the first computer program to win the world champion title in a competition against humans. In 1990 it won the right to play in the human World Championship by being second to Marion Tinsley in the US Nationals. At first the American Checkers Federation and English Draughts Association were against the participation of a computer in a human championship. When Tinsley resigned his title in protest, the ACF and EDA created the new title Man vs. Machine World Championship, and competition proceeded. Tinsley won with four wins to Chinook's two, with 33 draws.

In a rematch, Chinook was declared the Man-Machine World Champion in checkers in 1994 in a match against Marion Tinsley after six drawn games, and Tinsley's withdrawal due to pancreatic cancer. While Chinook became the world champion, it never defeated the best checkers player of all time, Tinsley, who was significantly superior to even his closest peer.[1]

In 1995, Chinook defended its man-machine title against Don Lafferty
in a 32-game match. The final score was 1–0 with 31 draws for Chinook
over Lafferty.[2] After the match, Jonathan Schaeffer decided not to
let Chinook compete any more, but instead try to solve checkers. At
the time it was rated at 2814 Elo. The solution was achieved, and the
result published in 2007.[3]

Chinook's program algorithm includes an opening book, a library of opening moves from games played by grandmasters; a deep search algorithm; a good move evaluation function; and an end-game database for all positions with eight pieces or fewer. The linear handcrafted evaluation function considers several features of the game board, including piece count, kings count, trapped kings, turn, runaway checkers (unimpeded path to be kinged) and other minor factors. All of Chinook's knowledge was programmed by its creators, rather than learned with artificial intelligence.

\subsection{Deep Blue Kasparov 1996/1997}\label{sec:deepblue}
{\bf why? first world champion chess program, the Drosophila. classic search
  eval, purely heuristic. excellent example of the field ``heuristic
  search''. Very high profile, impact in public perception of humans
  as the sole proprietors of intelligence on the planet. Now
  superseded by open source program Stockfish.}

\index{Deep Blue}
\index{Kasparov}
\index{Chess}
In 1996 IBM Sponsored the first match between the human world Chess
champion Garry Kasparov and IBM's Chess supercomputer Deep
Blue at the ACM Compuing Conference in Philidelphia. Kasparov won the match ...
A year later, in May 1997, the rematch was played in New
York. Kasparov was defeated in a highly publicized match. Several
accounts of the match, its historical significance, and the technology
have been
written~\cite{schaeffer1997kasparov,campbell2002deep,hsu1990grandmaster,hsu2004behind,levy1991computers}. 

Reference on how computers play chess is \cite{levy1991computers}.

The Deep Blue chess machine (IBM) defeats the (then) world chess
champion, Garry Kasparov.

Deep Blue was a chess-playing computer developed by IBM. It is known for being the first computer chess-playing system to win both a chess game and a chess match against a reigning world champion under regular time controls.

Deep Blue won its first game against a world champion on 10 February 1996, when it defeated Garry Kasparov in game one of a six-game match. However, Kasparov won three and drew two of the following five games, defeating Deep Blue by a score of 4–2. Deep Blue was then heavily upgraded, and played Kasparov again in May 1997.[1] Deep Blue won game six, therefore winning the six-game rematch 3½–2½ and becoming the first computer system to defeat a reigning world champion in a match under standard chess tournament time controls.[2] Kasparov accused IBM of cheating[3] and demanded a rematch. IBM refused and retired Deep Blue.

Development for Deep Blue began in 1985 with the ChipTest project at
Carnegie Mellon University. This project eventually evolved into Deep
Thought, at which point the development team was hired by IBM.[4] The
project evolved once more with the new name Deep Blue in
1989. Grandmaster Joel Benjamin was also part of the development team.

The project was started as ChipTest at Carnegie Mellon University by Feng-hsiung Hsu, followed by its successor, Deep Thought. After their graduation from Carnegie Mellon, Hsu, Thomas Anantharaman, and Murray Campbell from the Deep Thought team were hired by IBM Research to continue their quest to build a chess machine that could defeat the world champion.[5] Hsu and Campbell joined IBM in autumn 1989, with Anantharaman following later.[6] Anantharaman subsequently left IBM for Wall Street and Arthur Joseph Hoane joined the team to perform programming tasks.[7] Jerry Brody, a long-time employee of IBM Research, was recruited for the team in 1990.[8] The team was managed first by Randy Moulic, followed by Chung-Jen (C J) Tan.[9]

After Deep Thought's 1989 match against Kasparov, IBM held a contest to rename the chess machine and it became "Deep Blue", a play on IBM's nickname, "Big Blue".[10] After a scaled-down version of Deep Blue, Deep Blue Jr., played Grandmaster Joel Benjamin, Hsu and Campbell decided that Benjamin was the expert they were looking for to develop Deep Blue's opening book, and Benjamin was signed by IBM Research to assist with the preparations for Deep Blue's matches against Garry Kasparov.[11]

In 1995 "Deep Blue prototype" (actually Deep Thought II, renamed for PR reasons) played in the 8th World Computer Chess Championship. Deep Blue prototype played the computer program Wchess to a draw while Wchess was running on a personal computer. In round 5 Deep Blue prototype had the white pieces and lost to the computer program Fritz 3 in 39 moves while Fritz was running on an Intel Pentium 90 MHz personal computer. In the end of the championship Deep Blue prototype was tied for second place with the computer program Junior while Junior was running on a personal computer.[12]

Design[edit]
Deep Blue employed custom VLSI chips to execute the alpha-beta search
algorithm in parallel,[13] an example of GOFAI (Good Old-Fashioned
Artificial Intelligence) rather than of deep learning which would come
a decade later. It was a brute force approach, and one of its
developers even disclaimed that it was artificial intelligence at
all.[14]

Deep Blue, with its capability of evaluating 200 million positions per second, was the fastest computer to face a world chess champion. Today, in computer chess research and matches of world class players against computers, the focus of play has often shifted to software chess programs, rather than using dedicated chess hardware. Modern chess programs like Houdini, Rybka, Deep Fritz or Deep Junior are more efficient than the programs during Deep Blue's era. In a November 2006 match between Deep Fritz and world chess champion Vladimir Kramnik, the program ran on a computer system containing a dual-core Intel Xeon 5160 CPU, capable of evaluating only 8 million positions per second, but searching to an average depth of 17 to 18 plies in the middlegame thanks to heuristics; it won 4–2.[30][31]

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/chess}
\caption{Chess}\label{fig:chess}
\end{center}
\end{figure}
\cite{campbell2002deep,hsu2004behind}

\subsubsection{Impact of Deep Blue Win}
how chess is now learned
Watson, medical diagnoses.

Deep Blue and Kasparov played each other on two occasions. The first match began on 10 February 1996, in which Deep Blue became the first machine to win a chess game against a reigning world champion (Garry Kasparov) under regular time controls. However, Kasparov won three and drew two of the following five games, beating Deep Blue by a score of 4–2 (wins count 1 point, draws count ½ point). The match concluded on 17 February 1996.

Deep Blue was then heavily upgraded (unofficially nicknamed "Deeper Blue")[15] and played Kasparov again in May 1997, winning the six-game rematch 3½–2½, ending on 11 May. Deep Blue won the deciding game six after Kasparov made a mistake in the opening, becoming the first computer system to defeat a reigning world champion in a match under standard chess tournament time controls.

The system derived its playing strength mainly from brute force computing power. It was a massively parallel, RS/6000 SP Thin P2SC-based system with 30 nodes, with each node containing a 120 MHz P2SC microprocessor, enhanced with 480 special purpose VLSI chess chips. Its chess playing program was written in C and ran under the AIX operating system. It was capable of evaluating 200 million positions per second, twice as fast as the 1996 version. In June 1997, Deep Blue was the 259th most powerful supercomputer according to the TOP500 list, achieving 11.38 GFLOPS on the High-Performance LINPACK benchmark.[16]

The Deep Blue chess computer that defeated Kasparov in 1997 would typically search to a depth of between six and eight moves to a maximum of twenty or even more moves in some situations.[17] David Levy and Monty Newborn estimate that one additional ply (half-move) increases the playing strength 50 to 70 Elo points.[18]


Kasparov in 1985
Deep Blue's evaluation function was initially written in a generalized form, with many to-be-determined parameters (e.g. how important is a safe king position compared to a space advantage in the center, etc.). The optimal values for these parameters were then determined by the system itself, by analyzing thousands of master games. The evaluation function had been split into 8,000 parts, many of them designed for special positions. In the opening book there were over 4,000 positions and 700,000 grandmaster games. The endgame database contained many six piece endgames and five or fewer piece positions. Before the second match, the chess knowledge of the program was fine tuned by grandmaster Joel Benjamin. The opening library was provided by grandmasters Miguel Illescas, John Fedorowicz, and Nick de Firmian.[19] When Kasparov requested that he be allowed to study other games that Deep Blue had played so as to better understand his opponent, IBM refused. However, Kasparov did study many popular PC games to become familiar with computer game play in general.[citation needed]

Writer Nate Silver suggests that a bug in Deep Blue's software led to a seemingly random move (the 44th in the first game of the second match) which Kasparov misattributed to "superior intelligence".[20][21] Subsequently, Kasparov experienced a drop in performance due to anxiety in the following game.[21] Kasparov rejects this interpretation.[22]

Computer scientists believed that playing chess was a good measurement for the effectiveness of artificial intelligence, and by beating a world champion chess player, IBM showed that they had made significant progress.[23]

After the loss, Kasparov said that he sometimes saw deep intelligence and creativity in the machine's moves, suggesting that during the second game, human chess players had intervened on behalf of the machine, which would be a violation of the rules. IBM denied that it cheated, saying the only human intervention occurred between games. The rules provided for the developers to modify the program between games, an opportunity they said they used to shore up weaknesses in the computer's play that were revealed during the course of the match. Kasparov requested printouts of the machine's log files but IBM refused, although the company later published the logs on the Internet.[24] Kasparov demanded a rematch, but IBM refused and dismantled Deep Blue.[25] Owing to an insufficient sample of games between Deep Blue and officially rated chess players, a chess rating for Deep Blue was not established.[citation needed]

In 2003 a documentary film was made that explored these claims. Entitled Game Over: Kasparov and the Machine, the film interviewed some people who suggest that Deep Blue's victory was a ploy by IBM to boost its stock value.[25]

One of the cultural impacts of Deep Blue was the creation of a new game called Arimaa designed to be much more difficult for computers than chess.[26]

One of the two racks that made up Deep Blue is on display at the National Museum of American History in their exhibit about the Information Age;[citation needed] the other rack appears at the Computer History Museum in the "Artificial Intelligence and Robotics" gallery of the Revolution exhibit.[27] Reports that Deep Blue was sold to United Airlines appear to originate from confusion between Deep Blue itself and other RS6000/SP2 systems.[28]

\index{Stockfish}
Stockfish current best chess program. See Github
\href{https://github.com/official-stockfish/Stockfish}{Stockfish}.

\subsection{Logistello}
\index{Logistello}\index{Othello}
\cite{buro1997othello,buro1995logistello,buro2003evolution}
{\bf why? use of statistical pattern learning}

Computer Othello program Logistello defeated the world champion Takeshi Murakami with a score of 6–0.


Logistello is a computer program that plays the game Othello, also known as Reversi. Logistello was written by Michael Buro and is regarded as a strong player, having beaten the human world champion Takeshi Murakami six games to none in 1997 — the best Othello programs are now much stronger than any human player. Logistello's evaluation function is based on disc patterns and features over a million numerical parameters which were tuned using linear regression.
\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/othello}
\caption{Othello}\label{fig:othello}
\end{center}
\end{figure}

\subsection{General Game Playing}
GGP
\cite{pell1996strategic,genesereth2005general,thielscher2009answer,schiffel2007fluxplayer,thielscher2010general,thielscher2011general,schofield2012hyperplay,michulke2009neural,schofield2015lifting,finnsson2010learning,bjornsson2009cadiaplayer,sironi2016comparison,sironi2017line,wang2018search}
{\bf why? new claim for Drosophila (less visible, mainstream
  Drosophila is Go). Highly ambitious aim to develop technology toward AGI in gaming}


General game playing (GGP) is the design of artificial intelligence
programs to be able to play more than one game successfully.[1] For
many games like chess, computers are programmed to play these games
using a specially designed algorithm, which cannot be transferred to
another context. For example, a chess-playing computer program cannot
play checkers. A general game playing system, if well designed, would
be able to help in other areas, such as in providing intelligence for
search and rescue missions.

There are other general game playing systems, which use their own
languages for defining the game rules. In 1992, Barney Pell defined
the concept of Meta-Game Playing, and developed the "MetaGame"
system. This was the first program to automatically generate game
rules of chess-like games, and one of the earliest programs to use
automated game generation. Pell then developed the system
Metagamer.[8] This system was able to play a number of chess-like
games, given game rules definition in a special language called Game
Description Language, without any human interaction once the games
were generated.[9] 

\subsection{Poker}
{\bf why? world class imperfect information program. Mention both UofA
  Hyperborean, Polaris
and CMU Libratus}

Poker AI Libratus individually defeated each of its 4 human
opponents—among the best players in the world—at an exceptionally high
aggregated winrate, over a statistically significant sample.[58] In
contrast to Chess and Go, Poker is an imperfect information game.[59]

bowling

Poker is a game of imperfect information (because some cards in play are concealed) thus making it difficult for anyone (including a computer) to deduce the final outcome of the hand. Because of this lack of information, the computer's programmers have to implement systems based on the Bayes theorem, Nash equilibrium, Monte Carlo simulation or neural networks, all of which are imperfect techniques.

AIs like PokerSnowie and Claudico have been created by allowing the computer to determine the best possible strategy by letting it play itself an enormous number of times. This seems to be the current approach to poker AI, as opposed to attempting to make a computer that plays like a human. This results in odd bet sizing and a much different strategy than humans are used to seeing.

Methods are being developed to at least approximate perfect poker strategy from the game theory perspective in the heads-up (two player) game, and increasingly good systems are being created for the multi-player game. Perfect strategy has multiple meanings in this context. From a game-theoretic optimal point of view, a perfect strategy is one that cannot expect to lose to any other player's strategy; however, optimal strategy can vary in the presence of sub-optimal players who have weaknesses that can be exploited. In this case, a perfect strategy would be one that correctly or closely models those weaknesses and takes advantage of them to make a profit, such as those explained above.

Research groups[edit]
Computer Poker Research Group (University of Alberta, Canada)[edit]
A large amount of the research into computer poker players is being performed at the University of Alberta by the Computer Poker Research Group, led by Dr. Michael Bowling. The group developed the agents Poki, PsOpti, Hyperborean and Polaris. Poki has been licensed for the entertainment game STACKED featuring Canadian poker player Daniel Negreanu. PsOpti was available under the name "SparBot" in the poker training program "Poker Academy". The series of Hyperborean programs have competed in the Annual Computer Poker Competition, most recently taking three gold medals out of six events in the 2012 competition. The same line of research also produced Polaris, which played against human professionals in 2007 and 2008, and became the first computer poker program to win a meaningful poker competition.

In January 2015, an article in Science[1] by Michael Bowling, Neil Burch, Michael Johanson, and Oskari Tammelin claimed that their poker bot Cepheus had "essentially weakly solved" the game of heads-up limit Texas hold 'em.[2][3][4]

School of Computer Science from Carnegie Mellon University[edit]
T. Sandholm and A. Gilpin from Carnegie Mellon University have started poker AI research in 2004 beginning with unbeatable agent for 3-card game called Rhode-Island Hold 'em. Next step was GS1 which outperformed the best commercially available poker bots. Since 2006 poker agents from this group have participated in annual computer competitions. "At some point we will have a program better than the best human players" – claims Sandholm. His bot, Claudico, faced off against four human opponents in 2015. In 2017 the program's latest software, Libratus, faced off against four professional poker players. By the end of the experiment the four human players had lost a combined \$1.8 million.[5]



\subsection{DOTA2}
{\bf why? first multi player program}

An OpenAI-machined learned bot played at The International 2017 Dota 2 tournament in August 2017. It won during a 1v1 demonstration game against professional Dota 2 player Dendi.[61]

\subsection{Go}
\index{AlphaGo}
{\bf why? the Drosophila. The game of intelligence par
  excellence. Only mention program names. Chapter 10 will gie much
  more detail about technology and matches.}


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/go}
\caption{Go}\label{fig:go}
\end{center}
\end{figure}
1989 GNU go: minimax. The idea is based on the
article "Programming the Game of Go. Byte, Vol.6 No.4" by
J. K. Millen. Man Lung Li, et al., Houston
\cite{millen1981programming}\index{GNU Go}

1996 NeuroGo Enzenberger \index{NeuroGo}\cite{enzenberger1996integration}

1993 Brugmann Monte Carlo Go
\cite{brugmann1993monte,bouzy2004monte}\index{Monte Carlo Go}
1995 Buro Logistello \cite{buro1995statistical}\index{Logistello}
2006 MCTS Coulom\index{MCTS}
2006 UCT Kocsis Szepesvari \cite{kocsis2006bandit}\index{UCT}
2007 Silver \cite{gelly2007combining,silver2009reinforcement}
2013 DQN Atari
2016 AG Sedol \index{Lee Sedol}\index{Ke Jie}\index{AlphaGo}\cite{silver2016mastering}

\section{Summary}

%checkers, chess (turing, russians, deep blue-kasparov)

% 1950 Turing paper

% 1960 Samuel

% 1994 Checkers

% 1997 Kasparov

% 2016 Sedol



%\section{Theory}



%Philosophy of Intelligence; behavioral view of intelligence. very briefly. Further: see appendix

%turing 1950

%show the search-eval architecture

%\section{Practice} Example: a Tic Tac Toe program

%or: Hex. or 9x9 go.

%\section{Challenge} Understand that Lookahead is intelligence





==> chapters/old08dqn.tex <==
%% 5: dqn
%% section: generalizing states, net based, fucntion approximation, feature learning, representaion learning, deep learning
%% section: dqn: deep reinforcement learning
%% *section: Atari papers, Gym, optimal control dynamic systems
%% *section: rainbow enhancements to DQN
%% section: system 1 and system 2: this is system 1
%% section: go layers in keras
The theme of this book is to find best moves in large state spaces. The theme of this part of the book is to go beyond hand-crafted heuristics, how to learn good function approximation methods.  
The {\bf problem} of this chapter is to overcome delayed credit
assignment. In reinforcement learning the distance between rewards and
states is large, in contrast to
supervised learning, where for each state a direct label is
present. Deep reinforcement learning is unstable due to the credit
assignment distance, and correlation  between subsequent states and values.
The {\bf topic} in this chapter is to show how stable training has
been achieved in a deep Q-learning network (DQN) in end-to-end
training of classic Atari arcade videogames such as Space Invaders.

\section*{Learning Goals}
\begin{itemize}
%\item {\bf It is exciting to see supervised transfer to RL. Atari story is great. Now also explain the problems that were overcome. Emotion is that RL can also achieve the AI deep learning success}
\item learn end to end features for reinforcement learning, better than handcrafted
\item generalization performance. Benchmarks. result: Atari
\item stable search (deadly triad)
%\item Reinforcement Learning: delayed rewards, stability
%\item Mnih: DQN: policy gradient,  REINFORCE, replay buffer
%\item Benchmarks: Atari, ALE, Gym, Mujoco
\end{itemize}
%H8 thread: dqn make end to end features, generalize, stable. Dqn=replay buffer

The goal of function approximation is to find the determining features of a
high dimensional and state space that is so large
that not all states can be seen. In machine learning and game playing
this has originally been done with manually 
crafted heuristics (Chapter~\ref{chap:search}. Chapter~\ref{chap:mcts}
used averaged random playouts. Chapter~\ref{chap:super} showed that
neural nets can be good function approximators. See Table~\ref{tab:architecture8}
for the Search-Eval architecture.


\begin{table}[ht]
\begin{center}
\input searcheval
\caption{Search-Eval Architecture}\label{tab:architecture8}
  \end{center}
\end{table}



To quote Mnih et al.~\cite{mnih2013playing}:
``Recent breakthroughs in computer vision and speech recognition have
relied on efficiently training deep neural networks on very large
training sets. The most successful approaches are trained directly
from the raw inputs, using lightweight updates based on stochastic
gradient descent. By feeding sufficient data into deep neural
networks, it is often possible to learn better representations than
handcrafted features.''

Unfortunately,  training function approximators in reinforcement
learning can be unstable. Sutton and Barto~\cite{sutton2018introduction} mention the deadly triad of
function approximation, off-policy learning, and value
bootstrapping causing the instability. The goal of this chapter is to show through which
methods stable deep reinforcement learning can be achieved.


The previous chapter introduced us to function approximation with
neural networks. The chapter covered supervised learning, an important
learning method that assumes a database of labeled examples. The topic
of this chapter is  reinforcement learning, where agents learn
control actions through interaction with their 
environment. In reinforcement learning each sample of the environment
comes at the cost of an interaction. One of the 
defining features of reinforcement learning is delayed rewards
calculation. We will see the that  reinforcement learning in
deep networks can converge, with the DQN algorithm, short for deep Q-learning network.

{\bf now I have said it 3 times. need to consolidate texts}

\section{Delayed Rewards}\index{DQN}
We are concerned with the problem of intelligent decision making in
complex situations. The search-eval architecture separates this
problem in a search and an eval part. Please refer to Table~\ref{tab:architecture8}.

For search, we progressed from
smart enumeration of the states to adaptively selecting promising
states and speculatively exploring new states.

For eval, we progressed from manually coded domain specific
heuristics, to machine learned function approximators, provided enough
labeled examples were available, and enough compute power. In this
chapter we will see how learning a function approximator of the state value
is  possible in reinforcement learning. 

This chapter will not introduce new search methods, it will only be
concerned with state evaluation.

Function approximation of states is highly valuable for large state
spaces in
reinforcement learning, as was already mentioned in
Section~\ref{sec:approx}. It allows value functions and policy 
functions to be approximated, which can then be used in
planning algorithms such as MCTS.

Unfortunately, translating the successes of supervised learning to
reinforcement learning is not straightforward. In reinforcement learning there
is no label available 
for each training state. All we have is an environment with which we
can act to receive delayed reward feedback, to learn about the world. 
Furthermore, reinforcement learning is unstable or divergent with a
nonlinear function approximator. 

In this chapter we will discuss one example where a method was found
to approximate state functions in reinforcement learning successfully:
Atari.




%\section{RL: No Labels, only Action-Rewards}

\subsection{Discounted Future Reward}
An essential difference between supervised learning and reinforcement
learning is that in reinforcement learning credit assignment is
delayed. In supervised learning for each training example an immediate
output label is available, allowing an error function to be
calculated, and gradients to be adapted. In reinforcement learning
output signals are infrequent and/or delayed, and must be calculated depending on
previous states. Now the Bellman equation specifies how values
should propagate, however, when function values are only
approximations, and, worse, values between different states may be correlated,
then performing  Bellman updates may not converge to the correct reqrd
value. Indeed, it was shown that off policy algorithms such as Q-learning combined with non
linear function approximation and bootstrapping may cause the network to
diverge~\cite{tsitsiklis1997analysis,baird1995residual}. Furthermore, in many
reinforcement learning applications the delay between reward and state
is long, causing the effect of small amounts of noise to accumulate
quickly, and the network to diverge.

Interestingly, these findings contradict the success of TD-gammon~\cite{tesauro1995td}
that used an algorithm similar to Q-learning approximating the value
function with a simple neural network with one hidden layer, based on
heuristic features. Since attempts to replicate the approach in Chess, Checkers and Go did
not achieve success, it was believed for some time that Backgammon was a special
case.

However, more recently  there have been other reports of successful
applications of deep neural networks  in a reinforcement learning
setting~\cite{heess2012actor,sallans2004reinforcement}.



\subsection{Atari  2600  Games}


%\section{Search-Eval Architecture}




%\section{Evaluation by Generalization}
Learning actions
directly from high dimensional sensory inputs such as sound and vision
is one of the long standing challenges of AI and reinforcement
learning. In 2013, one year after the Krizhevsky
success in supervised learning~\cite{krizhevsky2012imagenet}, a paper
was published that took the reinforcement learning  works a step
further in this direction. Mnih et al.~\cite{mnih2013playing} 
published a ground breaking work on {\em end to end\/} reinforcement
learning in Atari games~\cite{bellemare2013arcade}. Their work is end
to end in the sense that they 
learn actions directly from the raw visual state, the raw pixels, without the
intermediate step of hand crafted heuristic features.

The Atari games
that they used are well known applications that are both challenging and appealing to
researchers and the general public alike.  Mnih et
al.~\cite{mnih2013playing} applied deep learning to play 1980s Arcade
Atari 2600 games, such as Space Invaders, Pong, and Breakout, directly
from the raw television screen pixels. Being able to close the loop
from For six games they were able to
achieve human level of play. In a follow up article in 2015~\cite{mnih2015human} 
they improved on their 2013 work and were able to achieve a level of play
equal to human play for 49 Atari games that were in the test
set.

It should be noted that there were a few Atari games that proved
difficult to achieve strong play at. Notably  games
that required more planning, such as Montezuma's Revenge, were a
problem. Delayed credit assignment over long periods is still hard.

Nevertheless, a single architecture was able to successfully learn
control policies for different games. Only minimal prior knowledge was
used, and the net only processed the pixels and the
game score. The same network architecture and training procedure was
used on each game. 


%\section{Deep Q Learning}.

\subsubsection{Arcade Learning Environment}\index{Atari}
The impressive results  by Mnih et al.\ stimulated much further work in the area of
deep reinforcement learning, or deep Q networks (DQN) as they are
often abbreviated. The combination of end to end learning with delayed
credit assignment caused much interest among other researchers. We
will therefore look into some depth into their methods and 
experiments.


The Arcade Learning Environment~\cite{bellemare2013arcade}  is a
testbed designed to provide challenging reinforcement learning
tasks. It consists of Atari 2600 games, a games console first marketed
in 1977 (see figure~\ref{fig:console}). It presents agents with a high dimensional visual input
($210\times 160$ RGB video at $60$Hz) of tasks that were designed to
be interesting and challenging for human players (see
Figure~\ref{fig:atarigames}). The game cartridge ROM typically holds
the game code (2-4kB), while the console RAM is small, just 128 bytes.
The actions can be input via a joystick, and a fire button (18 actions).


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/console}
\caption{Atari 2600 Console}\label{fig:console}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=10cm]{figures/atarigames}
\caption{Screenshots of 4 Atari Games (Breakout, Pong, Montezuma's Revenge, Private Eye)}\label{fig:atarigames}
\end{center}
\end{figure}


The experiments were performed with seven Atari games:
Beam Rider, Breakout, Enduro, Pong, Q*bert, Seaquest, and Space Invaders.


In their 2013 work~\cite{mnih2013playing} the net performed better than an expert human
player on Breakout, Enduro, and Pong. On Seaqest, Q*Bert, and Space
Invaders perfofrmance was far below that of a human. In these games a
strategy must be found that extends over longer time periods. In their
2015 work~\cite{mnih2015human} the net performed better than human level play in 29 of 49
Atari games. Again, games with longer credit delay are more
difficult. Training was performed on  50 million frames in total.





\subsubsection{Network Architecture}
The Atari task is a control task: the network learns a policy directly from
pixel frame input. 
The network used consists of three hidden layers, which is simpler
than used in most supervised learning.

The images are high dimensional data, working with the full resolution
of $210\times 160$ with 128 colors at 60 frames per second would be computationally
intensive. Therefore, first the images are preprocessed. The 
$210\times 160$ with $128$ color palette is reduced to gray scale and
$110\times 84$ pixels cropped to $84\times 84$. The first hidden layer convolves
16 $8\times 8$ filters with stride 4 and ReLU. The second hidden layer
convolves 32 $4\times 4$ filters with stride 2 and ReLU. The third
hidden layer is fully connected and consists of 256 ReLU neurons. The
output layer is also fully connected with one output per action (18
actions for the joystick). The outputs correspond to the  Q values of
the individual action. The network receives the change in game score
as a number from the emulator, reprocessed to $\{-1,0,+1\}$ to indicate
deterioration, no change, or improvement of the score.

Recall that convolutional nets are also known as ``shift-invariant,''
or feature recognizers,
and fully connected nets allow $n\times m$ mapping. The networks
structure allows mapping of any features (shapes) to any action.

To reduce
computational demands further frame skipping was used. Only one in
every 3-4 frames was used, depending on the game.

As history, the net takes as input the last four resulting frames,
allowing movement to be seen by the net.
As optimizer RMSprop was used.

A variant of $\epsilon$-greedy is used, that starts with an $\epsilon$
of 1 (exploring) going down to $0.1$ (90\% exploiting).

\section{Divergence}
The algorithm used is a form of Q-learning.
However, it  has been shown that off policy algorithms such as Q-learning combined with non 
linear function approximation may cause network training to
diverge~\cite{tsitsiklis1997analysis,baird1995residual}.

Deep learning algorithms for supervised learning typically assume that
examples are independent. In reinforcement learning, subsequent states
are typically correlated, and so are reward values, causing divergent
optimization. Furthermore,  
small updates to Q may significantly change the policy and therefore
change the data distribution (which was correlated)~\cite{mnih2015human}.

\subsection{Experience Replay}\index{experience replay}
The important contributions are a method to efficiently randomize
example states, and a method to break the correlations with target
values~\cite{mnih2015human}.


The first method is a replay buffer. This is a  biologically
inspired
mechanism~\cite{mcclelland1995there,o2010play,lin1993reinforcement}. It
 randomizes over the data removing
correlations in the sample sequence and smoothing over 
the data distribution.

Second,  Q values are only periodically adjusted towards target
values,  reducing correlations with target values.

\subsubsection{Replay Buffer}
Experience replay uses a replay buffer to randomize examples to be
learned from. It improves on 
Q-learning in 2 repects: (1) experience replay goes beyond learning
from consecutive samples. Randomizing the order in which samples
are learned breaks the correlations between consecutive samples, and
therefore reduces the variance of the 
updates. (2) experience replay prevents unwanted feedback
loops, which would arise when the game makes moves in a certain area
that it cannot escape from, getting stuck in a poor local
minimum, or even diverge
catastrophically~\cite{tsitsiklis1997analysis}. By averaging the
bahavior distribution over the
previous states experience replay smooths out learning and avoids oscillations or
divergence in the parameters.

Experience
replay is off policy because current
parameters are different from those used for the sample, hence
the choice for Q-learning~\cite{sutton2018introduction}.

Experience replay samples uniformly in the replay memory, but could be
enhanced by prioritized sampling methods such as prioritized sweeping~\cite{moore1993prioritized}.

\subsubsection{Infrequent Target Updates}
Infrequent updates of the target values reduces correlations and
possible divernce and oscillations caused by loops and local
optima. It works by using a
separate network for generating the targets of the update of the $Q$
value. Every $x$ updates the network $Q$ is cloned to
obtain a target network $\hat Q$, which is used for generating the
targets for the following $x$ updates to $Q$.

This second network improves stability of Q learning,
where normalle an update that increases $Q(s_t,a_t)$ often also
increases $Q(s_{t+1},a)$ for all $a$, and therby also increases the
target, quite possibly
leading to oscillations and divergence of the policy. Generating the
targets using an older set of parameters adds a delay between the time
an update to $Q$ is made and the time the update changes the targets,
breaking the feedback loop or at least making oscillations less likely.

Experience replay is an impoortant
technique for the success of deep reinforcement
learning~\cite{mnih2013playing}. Related ideas can be traced
to earlier works.

Gradient TD methods have been proven to converge
for evaluating a fixed policy with a non linear value
approximator~\cite{bhatnagar2009convergent}.  Relaxing the fixed
control policy the neural fitted Q learning algorithm (NFQ) has been
reported to work  for non linear control with
deep networks~\cite{riedmiller2005neural}. NFQ builds on~\cite{gordon1995stable,ernst2005tree} and
experience replay~\cite{lin1992self}, and more recently~\cite{lagoudakis2003least}.

There has been progress towards non linear control function approximation in
reinforcement learning.

These advances in reinforcement learning occurred in parallel to the
work in supervised learning, showcased by 
Krizhevsky et al.~\cite{krizhevsky2012imagenet}.




\subsubsection{In context}
The  breakthroughs in computer
vision~\cite{krizhevsky2012imagenet} rely on  training
on large labeled training sets. The Krizhevsky et al. and later works
are trained directly from the raw inputs, using quick updates by stochastic
gradient descent. The representations that are learned in this way are
odten better representations than handcrafted or heuristic features.

End to end reinforcement learning of behavior policy from raw visual
input, without any heuristics, is an impressive feat. Some critique
notes that the Atari 2600 games are games of skill. The games are
difficult for humans, because they require dexterity and quick hand
eye coordination. Playing the games builds reflexes. The games are not
so much designed as games of strategy (such as Chess, Checkers, Go,
Backgammon, Othello, or even Tic Tac Toe).
Atari 2600 games are not games of the reasoning kind of intelligence,
they are reflex games (thinking fast, not  thinking slow).

Despite this obervation, the algorithmic feat of breaking through the
divergence and oscillation of reinforcement learning with long delays
in credit assignment is impressive, and the Atari results are highly
imaginative, and have stimulated large amounts of subsequent research.

\subsection{Atari Breakout Code}
The Atari papers come with code. For reference, the original DQN code
from~\cite{mnih2015human} is  at 
\href{https://github.com/kuz/DeepMind-Atari-Deep-Q-Learner}{Atari
  DQN}.\footnote{\url{https://github.com/kuz/DeepMind-Atari-Deep-Q-Learner}} This code is the original code, in LUA, without new
developments.
Note that DQN can be complicated to get working. There are many little
details to get right. In addition, the
experiments often have to run for a long time which means that
debugging and improving is slow if you have just one GPU. 

A better start is the Tensorflow implementation in Python of DQN for the Atari game
Breakout, at \href{https://github.com/floodsung/DQN-Atari-Tensorflow}{Atari
  Breakout Code}.\footnote{\url{https://github.com/floodsung/DQN-Atari-Tensorflow}} This may get you up to speed more quickly.  The code
is readable, and follows the concepts discussed in this
chapter. However, the
code is too large to cover in detail here.

To get really started with deep reinforcement learning, DQN and many
of the other algorithms, are available at the OpenAI  Keras RL library at
\href{https://github.com/keras-rl/keras-rl}{Keras RL}\footnote{\url{https://github.com/keras-rl/keras-rl}}
\cite{plappert2016kerasrl}. 

\section{Practice}
\subsection{Benchmark Suites}
It should also be noted that progress in methods was greatly
facilitated by the existence of suitable benchmark suites and
competitions~\cite{bellemare2013arcade}. Just as the game of Chess
stimulated large progress in heuristic search, by offering clear
rules, motivating competitions, and a challgenging problem, and MNIST
and ImageNet for supervised learning, so does
the Arcade Learning Environment for reinforcement learning for agents
playing video games.

Other well known benchmark suites are the OpenAI
Gym~\cite{brockman2016openai} for video games, and
Mujoco~\cite{todorov2012mujoco} for simulated robot tasks.



The benchmarks can be found here:\index{Arcade Learning
  Environment}\index{Atari 2600}\index{benchmarks}\index{Gym}\index{MuJoCo}
\begin{itemize}
  \item
    \href{https://github.com/mgbellemare/Arcade-Learning-Environment}{Arcade
      Learning Environment}\footnote{\url{https://github.com/mgbellemare/Arcade-Learning-Environment}} \cite{bellemare2013arcade}
  \item \href{https://gym.openai.com/}{OpenAI Gym}\footnote{\url{https://gym.openai.com/}} \cite{brockman2016openai}
  \item \href{http://www.mujoco.org/}{MuJoCo}\footnote{\url{http://www.mujoco.org/}} \cite{todorov2012mujoco}
\end{itemize}

Furthmore, the use of benchmarks is of great importance for
reproducible reinforcement learning
experiments~\cite{henderson2017deep}.

\subsection{Cartpole}
OpenAI provides baseline implementations of important reinforcement
learning algorithms~\cite{baselines}. A good implementation of DQN for the Atari
Learning Environment and for Gym is available, and for other
algorithms. Installation instructions for Ubuntu and MacOS are provided. 


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/Cart-pendulum}
\caption{Cartpole Experiment}\label{fig:cartpole}
\end{center}
\end{figure}


Cartpole is a basic experiment in which an agent must learn to balance
a stick on a cartpole by reinforcement learning. A nice video of a
real life cartpole experiment is at
\href{https://www.youtube.com/watch?v=5Q14EjnOJZc}{Cartpole
  Video}\footnote{\url{https://www.youtube.com/watch?v=5Q14EjnOJZc}}
(as opposed to the simulated cartpole that is most often used in
reinforcement learning experiments, see Figure~\ref{fig:cartpole}).
At \href{https://github.com/openai/baselines/tree/master/baselines/deepq}{OpenAI
  Cartpole
  baseline}\footnote{\url{https://github.com/openai/baselines/tree/master/baselines/deepq}}
  working example code for the Cartpole experiment 
is available.


The high level code is simple, as listing~\ref{lst:cartpole} shows. To really
understand what is going on you have to look into the implementations of
\verb|deepq.learn| which has implements DQN in few hundred lines of code.


\lstset{label={lst:cartpole}}
\lstset{caption={Cartpole code~\cite{baselines}}}
\lstinputlisting[language=Python,float]{python/cartpole.py}




%Atari paper,
ALE

Gym
\subsubsection{Exercises}
\begin{itemize}
\item ALE/Gym
  \item Mountain Car
  \item Balancing Pole
    \item 9x9 Go??? in Gym!!!
  \end{itemize}

%\section{Challenge}
approximating function, state-action/array/mapping/function

generalizing states


\section{Summary}
H8 thread: dqn make end to end features, generalize, stable. Dqn=replay buffer

\begin{itemize}
\item Reinforcement Lernign: delayed rewards, perforamnce geenralization, stability
  \item Atari work Mnih. end to end
\item DQN, policy gradient,  REINFORCE, replay buffer
  \item Benchamrsk: ALE, Gym, Mujoco
\end{itemize}
Deep supervised learning generalizes features from large databases. Using large
databases it is often possible to learn features that are better than
handcrafted heuristic features. The examples
in these databases are independent, and training converges towards an
optimum. With correlated states, reinforcement learning training
processes diverge. Using a replay buffer Mnih et al. were able to
decouple the states enough to cause convergence to good control
networks.

In their paper they state the following:
``a single architecture can successfully learn control policies in a
range of different environments with only very minimal prior
knowledge, receiving only the pixels and the game score as inputs, and
using the same algorithm, network architecture and hyperparameters on
each game, privy only to the inputs a human player would have.''

This architecture, 
DQN, was demonstrated on Atari games. This has the benefit that the
success was shown on a wide
variety of games that are challenging for humans. The disadvantage may
be that the games were more aimed at skill than at intelligence. The
games were challenging for humans because of difficult hand eye
coordination, and not so much because of difficult reasoning
processes.
This will be part of Chapter~\ref{chap:plan}.

\subsubsection{Fast and Slow}
Fast and slow: this is fast (learned features to
recognize). generalization. Just like in Chapter~\ref{chap:super}.
Again, in this chapter the kind of intelligence is that of Thinking
Fast, in humans. System 1 thinking, reflex-thinking.


\section*{Historical and Bibliographical Notes}
NeuroGo~\cite{enzenberger1996integration} and NeuroGammon~\cite{tesauro1990neurogammon} used small nets to learn the coefficients of
heuristics evaluation functions of the state. They were written in a time when no such compute
power was avaliable, nor had the necessary advances in deep learning
training algorithms occurred, to learn features directly from the state.



Silver et al.~\cite{silver2012temporal} discuss the use of temporal
difference search in Go, comparing MCTS with TD reinforcement learning.

Lai~\cite{lai2015giraffe} experiments with DQN in Chess.



==> chapters/old10a0g.tex <==

%% 6: plan
%% section: search-eval integration: generating examples by planning to learn, and using learned eval to search
%% section: convergence/divergence: tunnelvision through self learning. off policy/on policy
%% section: system 1 and system 2: this is combination: 1+2=3
%% *section: implement 15 puzzle, diplomacy, SAT, GTOC, chess, checkers
%% *section: run on Cloud
%% *section: check transfer learning, hyper parameter optimization
%% *section: do more advanced net structures, do net structure optimization
%% *section: do build up small nets and then expand to larger nets
%% section: implement 9x9 go learner in a0g

% {\bf a pity that AlphaGo is so much technical text.
% many open questions: why resnets?
% why no more exact method/approximation hybrids?
% move 1+2=3 text to section on fast and slow?
% move early games text to historical notes? It is a bit of a dry
% summary without much insight or intuition.
% }

In this chapter planning and training come together. The most advanced exact
algorithm of the search-eval architecture (MCTS) and the most advanced approximation
algorithm (DQN) join forces. Together they form a Go player  that is
strong enough to beat the strongest humans (AlphaGo).

The problem that we encounter is again to achieve (1) stable and (2) high performance
generalization in a large and high dimensional state space. First we will see how with meticulous care correlations
between states are avoided in database learning in AlphaGo. Second, and more
importantly, we will see how, when learning from databases runs out of
steam, self-play is used to learn higher and higher levels of play, in
AlphaGo Zero. A third  system, AlphaZero, not only learns very well,
but is also quite general, learning to play from scratch in Chess and
Shogi, even beating the best conventional players.

Two things stand
out. It is quite
remarkable that these new algorithms beat the conventional players,
built on years of conventional game playing research.
%(MCTS+DQN+self-play versus
%alpha-beta+heuristics+manual tuning)
 It is even more remarkable
that  the new players learn to play at world champion level in a
matter of days, where humans need years.

These results have had a large impact on AI research,  and many new  
startups in reinforcement learning and AI have appeared.

In addition to planning and training coming together, the search-eval architecture will be 
getting a new paradigm: an extra learning loop is added around the
search-eval functions, creating the self-learning, recursive  self-play
architecture that is able to do tabula rasa learning (see
Table~\ref{tab:paradigms10}, Table~\ref{tab:arch10}, and Figure~\ref{fig:selfplay}).



%% \section*{Learning Goals}
%% \begin{itemize}
%% %\item {\bf it is exciting: this whole alphago chapter is one big exciting chapter}
%% \item self-play: planning and learning loop. AlphaGo
%% \item self-play: tabula rasa. AlphaGo Zero
%% \item self-play: general. Alpha Zero. GGP
%% \item AlphaGo matches, Ke Jie, Lee Sedol, effect on Go, impact on AI
%% \end{itemize}


\begin{table}
\begin{center}
\input diag/paradigm
\caption{Four Reinforcement Learning Paradigms}\label{tab:paradigms10}
  \end{center}
\end{table}

\begin{table}
\begin{center}
\input diag/searcheval
\caption{Search-Eval Architecture}\label{tab:arch10}
  \end{center}
\end{table}

\begin{figure}[t]
    \centering{\input diag/selfplay3
     \caption{Conceptual Self-Play Loop}\label{fig:selfplay}}
\end{figure}

\subsubsection{The Challenge of Self-Play}
Self-play is exciting. It is the holy grail of AI:
intelligence emerging out of basic interactions between
agents~\cite{leibo2019autocurricula}. 
It has intrigued researchers since the start of
game playing research. Interestingly, the basic minimax algorithm works like
self-play:  find your own best move by playing yourself as your
opponent.
%Self-Play:  a program teaching itself how to perform
%intelligent actions surely is the pinnacle of AI.

Many researchers have tried  self-play for their
games, and there have been some good results. Table~\ref{tab:programs} on page~\pageref{tab:programs}
lists some of the better known programs (look for {\em self-play\/} in the
Data column).

Self-play combines exact planning with approximate learning. The main challenges of approximate methods in reinforcement learning are the ones
we have seen in the previous chapters:
\begin{enumerate}
\item {\em Strong generalization\/} achieving learning in the face of long distance
  credit assignment needs strong examples to learn from---no
  underfitting, no overfitting. 
\item {\em Diversiit, stability\/} achieving stable training when there are
correlations between subsequent states and target values. Correlations
between consecutive states can lead to cylces and local
optima. We need diverse examples.
\end{enumerate}

% {\bf heeft dit allemaal zin? wat wil ik eigenlijk zeggen? dat self
% play beter kan worden dan een database? that mcts generates the
% training examples? All this will come later. it is voorbarig het nu al
% te doen. Maar, verderop moeten ze wel besproken worden: transcend db
% play, and mcts de training examples genereert. }

These are challenges facing all game playing programs. 
Achieving strong and stable generalization is hard in self-play. There
are fewer controls to influence the learning process than in heuristic
planning and deep learning, since the learning process is left to its
own devices: the examples to train from are now generated as part of the
learning process. In Go and Backgammon self-play was able to  achieve generality and stability in an elegant
and simple way. AlphaGo is a complex program that builds on supervised
and reinforcement learning. AlphaGo Zero, using self-play, achieves even higher performance,
in a way that is more elegant and simpler.

%% Supervised learning of board patterns has a long history in game
%% playing. In Othello, Go, and Checkers successful improvements of
%% playing strength have been documented (see
%% Table~\ref{tab:programs}). Databases allow learning of randomized,
%% uncorrelated, positions, with immediate labeks, without the need for
%% stable propagation of credit assignment over a long sequence of
%% states.

%% However, the level of play of database learning is limited by the
%% quality of play by the grandmasters whose games were recorded. Also,
%% database learning is copying of examples. Straightforward remembering
%% can hardly be called creative learning. To
%% transcend the level of play of databases, and to achieve true
%% learning, a reinforcement setting is better suited.
%% When we can overcome the problem of long range credit assignment and
%% achieve stable trainning, the potential benefits of self-play are
%% larger.

%% The previous chapters have covered many techniques to achieve a stable
%% and general learning process. The Atari papers introduced experience
%% replay and separate taget networks, and the rainbow paper discussed
%% actor critic and many other enhancements.

%% Planning algorithms are good at overcoming the
%% distance between states and rewards, they look ahead, at the cost of
%% computation to search though exponentially many possibilities.

%% Function approximation algorithms are good at generalization. Deep
%% hierarchies of layers can learn to distinguish features in states.

%% Let us see how 
%% self-play integrates eval and search.

%% \subsubsection{Integrating Evaluation and Search}
%% To be able to learn you need to be able to compare your current play
%% with a source of
%% better quality play.
%% This can be a database with best moves, a simulator (as with Atari) or
%% other programs (as has been done in~\cite{schraudolph1994temporal}) or self-play.

%% In self-play the evaluation function is a function approximator.
%% The search function, the planner, is used to generate high quality
%% targets for the function approximator to train on.
%% Thus, self-play adds an extra loop to the training procedure. In
%% supervised learning training consists of going through the database of
%% examples until the approximator is sufficiently trained.
%% In self-play, the planner generates a set of training examples that
%% the approximator is trained on. Then the extra loop comes in, since
%% that new approximator is then used by the planner to generate a new
%% set of examples, which is used for training an even better (hopefully)
%% approximator. And so on.

%% Altough both Atari and AlphaGo both are examples of reinforcement
%% learning, there is an important difference.
%% Atari's DQN is a ``flat'' training process against  the environment,
%% the Gym simulator. The environment is static, non learning.
%% On the other hand, in AlphaGo's recursive self-play, the training
%% examples are generated from its net, improved by lookahead search
%% by MCTS using an old version of the nets. The environment is moving,
%% it is learning.

%% Planning works hand in hand with learning.

\section*{Core Concepts}
\begin{itemize}
\item AlphaGo: Database of Positions, supervised+reinforcement
\item AlphaGo Zero: Self-Play, a form of reinforcement learning. MCTS, ResNets, Tabula Rasa
\item AlphaZero: Generalize to Go, Chess, Shogi
\end{itemize}


\section{Search-Eval Architecture}
Let us see how self-play fits in the search-eval
architecture. Self-play programs such as TD-Gammon and AlphaGo have a
search function and 
an evaluation function. In most modern programs the search function is
MCTS, and the evaluation function is a deep network (or more than one).
A self-play program also has an extra element, the self learning loop
(see Figure~\ref{fig:selfplay}).

\subsection{Evaluation}
Eval is a function approximator that
consists of a deep neural net. The function approximator is trained,
and is then queried during play. 
\begin{enumerate}
\item eval is the {\em learning element\/} of the self-play scheme, that is
trained in the training phase of self-play
\item eval is a {\em value function\/} to be queried for the value of
  the state during play.
  
\end{enumerate}
As we shall see shortly, in AlphaGo  function approximators are used in three
places, (1) as
policy function, (2) in the playout part, and (3) in the move
selection part of MCTS,  inside the MCTS 
tree. See Figure~\ref{fig:mcts10} for the four operations of MCTS.


\begin{figure}[t]
    \centering{\includegraphics[width=14cm]{figures/mctsalgo}
     \caption{Monte Carlo Tree Search~\cite{chaslot2006monte}}\label{fig:mcts10}}
\end{figure}


\subsection{Search}
In self-play search also has two roles: to  look ahead to generate examples
and to look ahead during actual play. For both roles the look ahead
algorithm  does exactly the same thing. It is only that its
role in the self-play scheme is different during training and use.
\begin{enumerate}
\item search  generates the examples for the training phase. By looking ahead, it
generates better quality examples as target for the
training. 
\item next, when the self-play training has finished, and the program is
used for a normal game, search
performs lookahead using the net to find the best action in actual
play.
\end{enumerate}
The roles are somewhat like the training and test phases in supervised
learning.
% setting, the first item would be the
% training data set, and the second item the test data set, to see if
% the training has created a good player.
% (see Section~\ref{sec:trainset}). 

\subsection{Self-Play Loop}\index{self-play}
Conceptually self-play is simple: it is a training loop around a
standard 
search-eval player. See Listing~\ref{lst:selfplay} and 
Figure~\ref{fig:selfplay} for code and a conceptual picture. 
In the
first line of the code there is
an outer loop that determines for 
how many iterations we want to perform the self-play learning. This
single line of code (line 1) is the self-play loop.

Although conceptually  and code-wise simple, there are subtle
interactions occurring during self-play that have an effect on
generalization and stability. Researchers have worked
to understand this for their games. We will explain them in this chapter. 

Figure~\ref{fig:selfplay} illustrates the concept of self-play: a
searcher that does look ahead and calls a value network as evaluator,
generating examples that are  input for the subsequent training phase
to improve the same kind of value net for the next iteration. $s$ is the state, $\pi$ the policy, $\theta$
are the network parameters (the weights) and $z$
the reward for the state $s$. Listing~\ref{lst:selfplay} provides the
pseudo-code. 

These game
outcomes are collected in the examples buffer (when the buffer is
full, the oldest entries are deleted, see  the second line).

Then, in the third line, an inner loop performs a few episodes  of
self-play games with the current net as eval (a mini tournament,
fourth line). The games of this tournament are (state, action) 
pairs, together with the game outcome $z$ (win, loss, or draw).

On the last
line this buffer
is then used to 
train the network (using a replay buffer with randomized sampling to break
correlations). The newly trained network is then used in the next self
play iteration as the evalution function by the searcher. Then another
tournament is played, using the searcher's lookahead to generate high
quality examples.

\lstset{label={lst:selfplay},numbers=left}
\lstset{caption={Self-Play Loop}}
\lstinputlisting[language=Python,float]{python/selfplay.py}

The principle of self-play is simple. Getting the details to work to
yield a very high level of play required
many years of research.

Among the challenges  is creating good quality training targets
of sufficient generality (diversity) so that quality of play kept improving,
without hitting a plateau, or degenerating into a limited kind of
play. The task of MCTS lookahead is to generate good quality training samples.
Another challenge is convergent training, for which the randomized
replay
buffer is used to break correlations between consecutive
states. 


\section{AlphaGo}
AlphaGo made AI history by defeating the best human Go
players. Interestingly, the
DeepMind team did not stop after that. After they won with AlphaGo, they
continued to improve their work. So far, no less than three major
results have been published in science's most prestigious journals, all  named after Alpha:
AlphaGo~\cite{silver2016mastering}, AlphaGo
Zero~\cite{silver2017mastering}, and
AlphaZero~\cite{silver2018general}.\footnote{Work on a fourth program,
  AlphaStar, for StarCraft, is also under
  way~\cite{alphastar2018}. Also, a related approach, called AlphaFold, is successful in
  protein folding~\cite{nussinov2019computational}.} We will discuss them in sequence.

\begin{table}[t]
  \begin{center}
    \begin{tabular}{c|c|c|c|c|c}
      {\bf program} & {\bf method} & {\bf positions} & {\bf networks}
      & {\bf search} & {\bf input/output} \\ \hline
      AlphaGo & superv. \& reinf. & grandm. \& gener.
                                                     & 3: policy,
                                                       playout, value
      &  MCTS & Go\\ \hline
      AlphaGo Zero & self-play & generated & 1: policy and value
                                             head & MCTS & Go \\ \hline
      AlphaZero & self-play & generated & 1: policy and value
                                             head & MCTS &Go, Chess,
                                                           Shogi \\
      \hline
    \end{tabular}
    \caption{AlphaGo, AlphaGo Zero, AlphaZero}\label{tab:alphago}
    \end{center}
    \end{table}
      

The first porogram, AlphaGo, is the most complicated. See Table~\ref{tab:alphago}. It uses
supervised learning, reinforcement learning, and three neural
networks. For the reinforcement learning part a highly tuned database of self-play
positions is used.  The second program, AlphaGo Zero, has a simpler
architecture, it does not use databases of positions, all training is
based on positions generated by self-play only. The third program,
AlphaZero, uses the same architecture, and plays Go, Shogi and
Chess. Its main purpose is to showcase the generality of the Zero architecture.

When we compare these three programs, an interesting phenomenon can be
noted. The later works are more simple and elegant than the earlier
works. Especially the early work, on AlphaGo, is  quite a complicated
system, with multiple networks and training types. Conceptually, the
easiest sections to understand are the two later sections, on AlphaGo Zero
and AlphaZero. Despite this, in this book we present the works in chronological
order, as they were published in 2016, 2017, and 2018. This order of presentation shows the
progression towards increasing conceptual elegance. Therefore a warning is appropriate: if you get confused, it  
might actually help to first read how Alpha(Go) Zero works in
Section~\ref{sec:alphagozero} and \ref{sec:alphazero}, and then 
return to AlphaGo in Section~\ref{sec:alphago}. So, you may want to
skip ahead to  page~\pageref{sec:alphagozero}.



\section{Games Played}
We will now briefly look at some of the games played by AlphaGo. 
Appendix~\ref{chap:matches} contains all games played in the Fan Hui
tournament, the Lee Sedol tournament, and the Ke Jie tournament.


{\em Fan Hui}
The games against Fan Hui were  games played in October 2015
as part of the development effort of AlphaGo. Fan Hui was the 2013, 2014, and
2015 European Go Champion rated at 2p dan. He described the program as very
strong and stable. ``It seems like a wall. I know AlphaGo is a
computer, but if no one told me, maybe I would think the player was a
little strange, but a very strong player, a real person.''



{\em Lee Sedol}
In international Go, although there is no official world wide  ranking,  Lee Sedol
was at the time considered one of the four best players in the world.

The games against Lee Sedol were part of a very high profile, much
publicized man-machine tournament. A one and a half hour \href{https://www.youtube.com/watch?v=9gzMQOa5MD4}{movie} was
made of the event.\footnote{\url{https://www.youtube.com/watch?v=9gzMQOa5MD4}}  The match
took place in March 2016. Lee Sedol is a 9p dan professional Go player, with 18
international titles when he played AlphaGo. He has been 9p since 2003. The match ended in a 1-4
win for AlphaGo.


\begin{figure}[ht]
    \centering{\includegraphics[width=7cm]{figures/leesedolmove37}
     \caption{``Speechless'' Move 37 by AlphaGo  in Game 2}\label{fig:leesedolmove37}}
\end{figure}


In Game 2 Alphago played a shocking move on the right-hand side
of the board, see Figure~\ref{fig:leesedolmove37}. Commentators said
that it was a very strange move, or thought that it was a mistake. Lee
Sedol took nearly fifteen minutes to
formulate a response. Fan Hui, who has experience playing AlphaGo, at
first also could not believe his eyes. But then he saw the beauty in
this rather unusual move.
Indeed, the move changed the course of the game and  AlphaGo went on
to win.
At the post-game press conference Lee Sedol was in
shock. He said: ``Yesterday, I was surprised,'' referring to his loss
in Game One.\label{sec:beauty}
``But today I am speechless. If you
look at the way the game was played, I admit, it was a very clear loss
on my part. From the very beginning of the game, there was not a
moment in time when I felt that I was leading.'' 

Fan Hui gives more commentary, which shows why this move seems so profound
from a human perspective.
He writes: ``Black 37 is one of the two moves from this match sure to
go down in Go history. This move proved so stunning that, when it
appeared on the screen, many players thought the stone had been put
down in the wrong place.  

% ``Because my main duty was to count the score at the end of the game,
% I had nothing in particular to do in the meantime. However, for such a
% historic event, it would be a terrible shame if there were no one to
% record the scene in the playing room, so I took this role upon
% myself. Though I had no prior experience, my aim was simple: to
% capture the atmosphere, the players' expressions, even their gestures,
% and in this way to communicate the experience of the match. 

``On seeing Black 37, I wrote down the following: "Here?! This goes
beyond my understanding. Globally, there's nothing wrong with it, it's
going in the right direction [$\dots$] and AlphaGo always pays special
attention to coordinating the stones. It seems anything is possible in
Go! Everyone will be talking about this move! A human would never dare
play it, it's too difficult to estimate. But AlphaGo can. Perhaps this
move is a sign of its confidence." 

``This move made a deep impression on me during the game. I
experienced first confusion, then shock, and finally delight. It
reminded me of an old Chinese saying: "A beginner plays the corners,
an average player the sides; but a master controls the center." These
days, due to the convergence of strengths and the pressure of
competition, something close to the opposite is true, with most
players focusing on the corners and sides. In contrast, AlphaGo's
talent for central control is second to none. Perhaps, through
AlphaGo, we too can become the "masters" of which the proverb speaks. 

``Returning to the game, we may say that Black 37 casts an invisible
net across the board. Together with the lower side, Black's shoulder
hit creates potential all across the center. Although it helps White
make territory on the right, the presence of White A means that a
Black invasion there would not have been valuable anyway. Of course,
Black should be reluctant to give away fourth-line territory too
easily, but one must give to get. 

``After the match, when I examined the data back at DeepMind, I saw
that AlphaGo had not even been thinking about 37 only a few moves
before. It had been expecting a different move, and its data indicated that a
human player would hardly consider the shoulder hit a possibility. It
was only when White played 36 that AlphaGo discovered 37, and boldly
decided that this move would work even better. 

``The pace of the game was much slower than the previous day, so Lee had
already gone out to smoke before 37. The minute he caught sight of
AlphaGo's reply, he stared blankly at the board. Then he smiled, sat
down, and started thinking. The longer he thought, the more serious
his expression became, while the clock ran down little by
little''~\cite{fanhui2016deepmind}. And indeed, this game was won by AlphaGo.



%% ``On March 9, Lee played black and lost the first game by
%% resignation.[15] On March 10, he played white and lost the second game
%% by resignation.[16] On March 12, he played black and lost the third
%% game as well.[17] On March 13, he played white and won the fourth
%% game, following an unexpected move at White 78 described as "a
%% brilliant tesuji", and by Gu Li 9 dan as a "divine move" and
%% completely unforeseen by him. (See Figure~\ref{fig:game4sedol}.) GoGameGuru commented that this game was
%% "a masterpiece for Lee Sedol and will almost certainly become a famous
%% game in the history of Go".[18] Lee commented after the victory that
%% he considered AlphaGo was strongest when playing white (second). For
%% this reason, and because he thought winning a second time with black
%% would be more valuable than winning with white, he requested that he
%% play black in the final fifth game, which is considered more risky
%% when following Chinese go rules.[19] On March 15, he played black and
%% lost the fifth game, to lose the Go series 1-4.[20]''



%% \begin{figure}[h]
%%     \centering{\includegraphics[width=7cm]{figures/game4sedol}
%%      \caption{``Divine'' Move 78 by Lee Sedol in Game 4}\label{fig:game4sedol}}
%% \end{figure}




{\em Ke Jie}
Ke Jie was ranked  number one in
the Korean, Japanese, and Chinese ranking systems at the time of the match.  He was also first among all human
players worldwide  under Remi Coulom's ranking system
~\cite{goratings}.

On 23--27 May 2017 a three game match was played in Wuzhen, China. The
match was won
3-0 by AlphaGo.
AlphaGo was subsequently awarded a professional 9-dan title by the
Chinese Weiqi Association. 

Before the match, DeepMind had organized a 60 game online tournament against
top pros from 29 December 2016 to 4 January 2017. This version of AlphaGo used 4
TPUs in a single machine. It achieved  an Elo rating of
4858~\cite{silver2017mastering}, or 3 stone stronger than the version
that defeated Lee Sedol.\index{TPU} DeepMind named this match version {\em
AlphaGo Master}. Its architecture is the same as AlphaGo, with a
combination of  supervised and reinforcement learning (even though DeepMind
was, at the time, already working on AlphaGo Zero).



\subsection{*AlphaGo}\index{AlphaGo}\label{sec:alphago}
The first publication describes the details of
AlphaGo~\cite{silver2016mastering}. AlphaGo is the program that beat
Fan Hui in London in 2015 in a training match, Lee Sedol in Seoul
in March 2016, and Ke Jie in Wuzhen in May 2017. Three
prominent members of the AlphGo team are Demis Hassabis, David Silver,
and Aja Huang. Their pictures are shown in Figure~\ref{fig:fanhui}. 
\index{David Silver}\index{Aja Huang}\index{Demis Hassabis}
\index{Fan Hui}\index{Lee Sedol}\index{Ke Jie}


\begin{table}[t]
\begin{center}
\input figures/fanhui
\caption{Fan Hui, Lee Sedol, Ke Jie; Demis Hassabis, David Silver, Aja
Huang (Left-to-right, top-to-bottom)}\label{fig:fanhui}
\end{center}
\end{table}

\subsubsection{Training}
AlphaGo uses a mix of supervised learning (grandmaster games) and
reinforcement learning (a database of positions from self-play) all
coordinated by an MCTS 
searcher. Supervised learning on grandmaster games was used to
achieve a certain level of play, and then positions from self-play
were used to improve further.
In AlphaGo, the reinforcement learning  agent is thus an MCTS/neural net program
that trains against through interaction with an environment that consists of a
database with games against a
copy of itself (hence the name self-play for this part of the
training). Note that quite some preparation is used to tune and
de-correlate the training positions.
%% In this case the agent is a function
%% approximator, a neural net, that is trained against examples from an
%% environment/simulator. The examples  are  generated by MCTS during
%% self-play in which older version of that net was used.

AlphaGo is a complicated program.  It uses supervised and
reinforcement learning, and two
separate policy networks and a value network. First, a game database
is used to train 
two policy networks by supervised learning. A fast roll out policy
network is created for MCTS simulations based on $3\times 3$
patterns.\footnote{Recall the four MCTS  
operations: select, expand, roll out and backup.} Second, another
database of 160,000 grandmaster games  is used to train a slower selection
policy network by supervised learning (28 million positions).  This
policy network is used in the MCTS selection operation. The supervised network is 
further trained by reinforcement learning. Next a value network is
trained based on a database of 30 million self play positions.

For the MCTS leaf values a mix is
used of the value network and the outcome of  MCTS roll outs using
the fast roll out policy network. Note that in AlphaGo the random play
outs of MCTS are replaced by play outs using the fast policy net.

To summarize, AlphaGo uses three networks:\index{AlphaGo networks}
\begin{enumerate}
\item a ``fast'' roll out policy net trained by supervised learning from human games,
  used for MCTS roll out
  \item a ``slow'' selection policy net, first trained by supervised learning from
  grandmaster games, then further refined through self-play positions
\item  a value net for position evaluation value, trained by self-play
  learning from separate  games to prevent overfitting due to
  correlation between subsequent game states
\end{enumerate}



\subsubsection{Performance of the Three Networks}
We will now discuss these  networks in more detail.

{\em Fast Roll Out Policy Network}\index{AlphaGo!fast roll out policy network} The 
fast roll out policy network is based on $3\times 3$ patterns. Its
function is to replace (or enhance) the random roll outs of MCTS. It achieves 24\%
accuracy on a test set, but it replies with an answer in $2\mu s$,
which is 1500 times faster than the slow policy network, on the
hardware used by the AlphaGo team.

{\em Selection Policy Network}\index{AlphaGo!slow selection policy network}
The network trained by supervised learning is trained on 29 million
positions for classification of expert moves on a data set of internet
games (split into a test set of one million positons, and a training
set of 28 million positions). This policy network achieves 57\%
accuracy of  correct actions
after training. Its time to compute  an answer is 3 ms.
It is trained by asynchronous stochastic gradient descent.
The supervised training took three weeks; 340 million training steps
were performed.


The policy network is further refined by
reinforcement learning with self-play positions. It was trained for one full day of
self-play of 10,000 mini-batches of 128
games, carefully managed to prevent correlations using positions from
a pool of opponents. 
The training algorithm is policy gradient descent, with the REINFORCE\index{REINFORCE}
algorithm~\cite{sutton2018introduction}. 
This network performs quite well, without any search at all, it won 85\% of
games against Pachi, 
a strong open source MCTS program. The reinforcement learning is
important, since a no-search network based on
supervised learning won only 11\% against Pachi.\index{Pachi}
Interestingly, it is the weaker supervised net that was used in MCTS
selection in AlphaGo.  The paper speculates that this is because
of greater variation in the supervised network it chooses from a wider
repertoire of ``best'' moves, whereas, the reinforcement
network chooses always the single best move. Whatever the reason, it
is surprising that a weaker network is used in favor of a stronger
network and more work is needed to fully understand the reasons.


{\em Value Network}\index{AlphaGo!value network}
The value network is trained as a  regression  of the policy
network. The value represents the probability of winning for the
states. For this, 30 million training positions were used from self
play games. To avoid overfitting the training positions were created
so as not to be correlated, using a small self-play search based on the
positions that were used for the supervised selection policy
network.
The training algorithm is stochastic gradient descent as in the
supervised training phase, based on the mean squared error between the
predicted values and the observed rewards.
This training phase took 50 GPUs one week.

AlphaGo is a complicated program. The preceding overview gives some
of the relevant details. Many more  details of the various training
methods can be 
found in the original publication~\cite{silver2016mastering}. 

\subsubsection{Search Algorithm}
The search algorithm of AlphaGo is MCTS (see also
Section~\ref{sec:mcts} and~\cite{browne2012survey}). The four MCTS
operations are implemented as follows. 

{\em Selection}
For selection, a variant of P-UCT~\cite{rosin2011multi,matsuzaki2018empirical}\index{P-UCT} is used, which
allows integration of prior information into the UCT selection
formula. This is especially important for new, unexplored children, to
be able to use the 
information of the policy net. With the policy net, AlphaGo does not employ the all-moves-as-first or
rapid action value estimation heuristics used in most other programs,
since the policy net provides  priors of better quality. In addition AlphaGo does not use progressive
widening~\cite{chaslot2008progressive}, dynamic komi~\cite{baudivs2011balancing} or an opening book, which most other Go
programs do.

The constant  $C_p$ determines the exploration/exploitation trade-off.\index{$C_p$}
 A high value means more exploration. AlphaGo uses 
$C_p=5$. This  is high compared to most Go programs, where values of $C_p<0.75$ or even
$C_p\approx 0$ were
used~\cite{gelly2006modification,chaslot2010monte}. AlphaGo  favors a
considerable amount of exploration compared to earlier Go
programs.\index{$C_p$} Section~\ref{sec:explexpl} discusses the performance
sensitivity of $C_p$. 


{\em Expansion} Children of leaves of the MCTS tree are expanded  when
the visit count exceeds a threshold.  New children get prior
probabilities from the policy network, and  are put in the
queue for evaluation by the GPU with both the policy and the value
network. The threshold is determined by 
the length of the work queue for the GPU.

{\em Roll out}
Leaves in AlphaGo are evaluated both by the value network (GPU queue)
and  roll outs with the fast roll out network. Results are
combined with a parameter $\lambda=0.5$ (half roll out, half value
network).\index{$\lambda$, AlphaGo mixing parameter}

{\em Backup}\index{virtual loss}\index{lock free}
The roll out statistics are updated as usual in MCTS (visit count and
win count). AlphaGo is a tree parallel program~\cite{chaslot2008parallel}, which
means that multiple processes can update the MCTS tree
concurrently. AlphaGo uses standard techniques for ensuring efficient
parallel selection (virtual loss~\cite{segal2010scalability,mirsoleimani2017analysis}) and
correctness of the tree (lock free
updates~\cite{enzenberger2009lock,mirsoleimani2018lock}).


\subsubsection{Network Architecture}
For the fast roll out policy network, the function approximator is actually based on a hash
table. The fast roll out policy is based on small ($3\times 3$) patterns that
are also found in other Go
programs~\cite{gelly2006modification,gelly2007combining}. It is based
on a  hash table of the {\em last good reply\/}
heuristic~\cite{baier2010power}.

The function approximator for the selection policy is based on a 13 layer
convolutional neural network. It has 12 convolutional hidden layers (plus one input
layer and one fully connected output layer). The first convolutional
layers uses a kernel size of $5\times 5$, the other hidden layers use
$3\times 3$. A ReLU unit is applied at each layer.

The network for the value network has one convolutional layer more
than the policy network, for a total of 14 layers.

\subsubsection{Input/Output Features}
The input layer is  $19\times 19\times 48$ with $48$ feature
planes. The inputs to the AlphaGo nets are more than just the stones
on the board. The features of each point include stone color, how many
times ago a turn 
was played, the number of liberties, how many opponent stones would be
captured, how many own stones would be captured, the number of
liberties after the move is played, ladder status, ladder escape, if a
point fills an own eye, and color to play. 

The output layer is a fully connected layer with a softmax function
for the policy network and a single $\tanh$ unit for the value network.

\subsubsection{Compute Hardware}
Training the networks occurs off line, before a match is played, and large
amounts of computation power and time are available. During a match
the time to compute is limited. Function approximation does not come cheap.  Position
evaluation requires evaluating multiple networks, which costs
orders of magnitude  more computation than traditional heuristic
programs. Combining MCTS
with deep neural networks has required quite some software engineering. 
AlphaGo uses an asynchronous multi-threaded search that executes
simulations on CPUs, 
and computes policy and value networks in parallel on GPUs. AlphaGo
used 40 search threads, 48 CPU cores, and 8 GPUs. A distributed
version was also developed, to make use of a cluster of machines. It
has been run on  1,202 CPUs and 176 GPUs.

In 2016 Google developed a special kind of GPU especially optimized
for tensor computations in 
TensorFlow, named {\em TPU},\index{TPU} for Tensor Processing Unit.
DeepMind started using TPUs for AlphaGo in 2016. TPUs are designed for
high througput low precision computations (as low as 8 bit precision)
whereas GPUs are typically optimized for 32 or 64 bit precision
operations, and memory throughput is often a bottleneck~\cite{jouppi2017datacenter}.

\subsubsection{Playing Strength}
Quite some development and
experimentation were needed for AlphaGo to reach the level of play that it did.

Figure~\ref{fig:agElo} shows the Elo rating of AlphaGo  compared
to other programs and Fan Hui. AlphaGo is clearly superior. The graph indicates a playing strength
of 5p dan. Since publication of the
article in 2016, the performance of Alphago has continued to improve, due to
further refinement. The version playing against Lee Sedol and  Ke Jie
was significantly stronger, at 9p dan.

AlphaGo has an elaborate architecture, with three
networks. Therefore, it is instructive to see how each network 
influences performance. Figure~\ref{fig:agNetworks} shows the impact
of turning some of the 
three networks off. We see that each network has a significant
contribution, and that the contribution of the networks is independent
in the sense that they 
improve each other. 

AlphaGo also uses a significant amount of compute
power. Therefore, it is interesting to see how more computers
influence playing strength. Figure~\ref{fig:agDistr} shows the impact
of the extra hardware for 
the distributed version of AlphGo. Clearly the use of more than one
GPU is advantageous, as is the use of multi-threading. The use of a
cluster of machines (dark blue, distributed) gives an increase in
performance of around 200 Elo points.



\begin{figure}[ht]
    \centering{\includegraphics[width=5cm]{figures/agElo}
     \caption{AlphaGo Elo Rating (pale red is 4 handicap stones) \cite{silver2016mastering}}\label{fig:agElo}}
\end{figure}


\begin{figure}[ht]
    \centering{\includegraphics[width=7cm]{figures/agNetworks}
     \caption{AlphaGo Networks \cite{silver2016mastering}}\label{fig:agNetworks}}
\end{figure}


\begin{figure}[ht]
    \centering{\includegraphics[width=5cm]{figures/agDistr}
     \caption{Elo Rating of AlphaGo Distributed Versions \cite{silver2016mastering}}\label{fig:agDistr}}
\end{figure}





\subsubsection{Open Questions}
The AlphaGo team made important scientific progress, they strongly pushed the
field of reinforcement learning forward, and the worldwide attention
generated by the 2016 and 2017 matches did much to strengthen the
worldwide interest in AI. The successes and the design of AlphaGo
attracted much attention by  AI researchers  and others.
However, AlphaGo is a complicated program, and a natural question is
if the approach could be simplified. Among the questions raised by the
AlphaGo success were the following:

\begin{itemize}\label{sec:open}
\item  DeepMind trained its networks for weeks. An important
question is how to increase training speed. This question was already addressed by Google, with the development of
TPUs. It was clear that AI and machine learning needed all the power
they could get, and TPUs provide more speed, specifically optimized for
neural network training. 
\item Looking more specifically at AlphaGo, a natural question to ask is:
``Why does the supervised learning policy network work better in
MCTS selection, whereas the reinforcement learning policy network has
higher accuracy?''
\item
Furthermore, at the leaf nodes of the MCTS tree both fast roll outs
are computed and a value function from the value network is used. The two are
mixed by the $\lambda$ parameter. Would a more elegant solution exist?
\item
The overall architecture is complicated, with four training methods
for three nets. Is a simpler architecture possible? 
Can self-play replace supervised learning entirely?
\item
The network architecture is elaborate with 13 or 14 layers. Its design
and tuning cost time and
effort. Can  this network architecture and the tuning of
hyperparameters be made simpler?
% \item
% Training takes multiple weeks, which is a long time, can
% it be shortened? Are there, in addition to TPUs, other ways to speed
% this up?
\item
Then, just as with Deep Blue/Kasparov,
the  natural question was raised: ``What next?''
With the
human Go champions defeated, what was to be the next Drosophila?
Was it to be learning from scratch, would it be taking on general
intelligence, or would there be  another
game?
\end{itemize}
As to the last question,  DeepMind did all three, as we shall see next.


\subsection{AlphaGo Zero}\index{AlphaGo Zero}\index{Tabula Rasa}\label{sec:alphagozero}
After defeating three of the top human Go masters ten years before
most AI experts were counting on this to happen, the team did not
rest. The DeepMind motto is ``solving intelligence'' and although this may
seem overly ambitious, they did continue with a hard problem, and they
succeeded.

The year after the AlphaGo publication, they again did what no one had done
before in AI, they learned to play the game of Go 
from scratch~\cite{silver2017mastering}.\footnote{The field
of General Game Playing\index{GGP} has 
this goal as well, and more: to learn how to play any game from
scratch. Although GGP methods may be more general, Go is a significantly
more complex game than typical GGP games are.} Only the rules
of the game were known, and the program learned to play beyond world
championship level all by itself. Tabula rasa, no heuristics at all.
Of course, the rules of the game had to be coded in some way, and the
input and output layer of 
the net were specifically designed for Go, and  quite some
refinement went into the network architecture and choice of hyperparameters for the self-play to work. All these are described meticulously
in their publication~\cite{silver2017mastering} and discussed in talks
at scientific conferences. 

\subsubsection{Less is More}
The great British computer scientist
Tony Hoare is credited with saying: ``Inside every large problem
there is a small problem struggling to get out.''
This certainly applies to AlphaGo. The original AlphaGo  is a
complicated program. The team redesigned the program from four
learning methods and three function approximators to one each: only
self-play, and one net (a two-headed net, a net with a policy head and a
value head). 

Furthermore, MCTS in AlphaGo Zero did no longer do any play outs at all. At 
leaves of the MCTS tree the value function provided by
the value head of the single network was used. No
more mixing parameter $\lambda$. In fact, since MCTS no longer does
random playouts, the MC in its name no longer applies. The algorithm
should really be called something else.

AlphaGo Zero no longer initialized its nets with grandmaster
games before it started the reinforcement learning bootstrapping  with
self-play states. It learned all knowledge from scratch. 
From a reinforcement learning point of view the fact that the entire
spectrum of play was learned, from absolute beginner to world class,
is an impressive achievement. Clearly, problems with generality of the knowledge
and the convergence of the training  were overcome in AlphaGo Zero.

Another change that was made was that the network switched from two
convolutional nets to a single residual net (resnets are discussed in 
Section~\ref{sec:resnet}).\index{ResNet} 

It may seem counterintuitive that a simpler architecture, with just a single two headed
evaluation network would work better for such a complex game, although Tony Hoare would disagree.
The simpler architectures are easier to understand and improve. Simplicity
may have helped the team to 
reach the impressive reinforcement learning results.

The main change in the training scheme is that MCTS is now inside a 
reinforcement training loop, where in the previous AlphaGo examples
were taken from a database of self-played positions. Each MCTS search
gets 1600 simulations, which is enough to get high quality
and de-correlated training examples, giving better generalization and
more stable search.

%{\bf curriculum learning! faster!}
To play stronger, AlphaGo Zero does {\em not\/} use the boost that
initialization with grandmaster games provides. In order to reach higher, the play
starts lower. This requires
a  more stable reinforcement training process. The slightest problems in overfitting
or correlation between states that throws off the training will show
up as low accuracy in  testing.

In fact, the result of the more accurate self-play is not only {\em better\/}
but also {\em faster\/} training, from weeks for AlphaGo to days for AlphaGo
Zero.\label{sec:days}
The reason is known as {\em curriculum learning\/}~\cite{bengio2009curriculum}: it
is quicker to learn a goal in many small steps from easy to hard, than
in one large step. In self-play, AlphaGo Zero's neural 
network always trained against an opponent of a comparable
level, or  slightly better. Learning to play against a slightly
better opponent costs less  computational effort than training against
grandmaster games, where the network has to learn to overcome a large
error  in one big step. In self-play, the net is always
training against an opponent of its own level, allowing a 
smoother  learning path, and, importantly, requiring less computational
effort~\cite{silver2017mastering}. 
It is easier to learn a big problem by learning it in many smaller
steps. This phenomenon was named curriculum learning by Bengio
et al.~\cite{bengio2009curriculum}. See also Section~\ref{sec:curr}. 

The AlphaGo Zero paper provides a comparison with the
old AlphaGo showing how in relatively little training time self-play
reinforcement learning is able to surpass supervised database
learning (see Figure~\ref{fig:slrl}). 


\begin{figure}[ht]
    \centering{\includegraphics[width=6cm]{figures/slrl}
     \caption{Comparison of Supervised Learning and Self-play
     Reinforcement Learning~\cite{silver2017mastering}}\label{fig:slrl}}
\end{figure}

Of course, it still is important to ensure diversity, since it is all
too easy for the self-play opponents to teach each other into a certain
obscure part of Go knowledge, without discovering the breadth of the game.

\subsubsection{Detailed Self-Play Training}
Let us look in more technical detail how self-play is implemented in
AlphaGo Zero~\cite{silver2017mastering}. The neural network is trained as follows. A self-play
reinforcement learning algorithm uses MCTS to play each move. First, the neural network
is initialized to random weights $\theta_0$. At each subsequent iteration $i$,
games of self-play, or episodes, are generated, consisting of a sequence of
moves. For each move of each episode  $t$, an MCTS
search $\pi_t$ is performed using the previous neural network
$\theta_{i-1}$ and a move is played sampled from $\pi_t$.
The game $t$ terminates when both players pass at step $T$ at which
point the game is scored $z=\{-1,+1\}$. The data are stored in a
state-policy-distribution-reward-triple $(s_t, \pi_t, z_t)$ as examples
in the example buffer for training the network parameters
$\theta_i$. The network $(p,v)=f_{\theta_i}(s)$ is trained by sampling uniformly over the
example triples of all time steps (episodes) of the last iterations of
self-play. A loss function is chosen to minimize the error between
predicted value $v$ and self-play outcome $z$, and to maximize the
similarity of predicted move probabilities $p$ and search
probabilities $\pi$.
Policy and value were used as a combined loss function that sums over
the mean squared value error and cross entropy policy
losses:\index{loss function AlphaGo Zero}
$l=(z-v)^2-\pi^T\log p + c\|\theta\|^2 $
where $c$ is the controlling parameter for L2 weight regularization to
prevent overfitting~\cite{goodfellow2016deep,silver2017mastering}.


\subsubsection{Network Architecture}
The new function approximation architecture is  simpler than in AlphaGo. It
consists of one residual network (see 
Section~\ref{sec:resnet}) instead of a value net, a slow selection
policy net, and a 
fast roll out policy net. The resnet has one input and two outputs: a
policy head and a value head. The resnet is trained by self-play, the
databases of positions for supervised and reinforcement learning have
disappeared. MCTS no longer does roll-outs, so the fast
roll-out net has gone as well.

It is reported that combining policy and value  into a single network slightly
reduces move prediction accuracy, but also reduces the value error. It
improved playing performance in AlphaGo Zero by 600 Elo points, in
part because the dual objective regularizes the network better.


Figure~\ref{fig:convnetresnet} shows the difference in performance
between the combined dual policy/value network and the separate
networks, and the convolutional and residual networks~\cite{silver2017mastering}.


\begin{figure}[ht]
    \centering{\includegraphics[width=5cm]{figures/convnetresnet}
     \caption{Comparison of Dual and Separate, and of Convolutional
     and Residual Networks~\cite{silver2017mastering}}\label{fig:convnetresnet}}
\end{figure}

The resnets consist of blocks of convolutions~\cite{he2016deep} with batch
normalization~\cite{ioffe2017batch} and ReLU units. Interestingly,
after experimenting with 40 block 
ResNets against 20 block resnets, the team decided to use the 20 block
net in the tournament version of the player. The added complexity of 40 block nets did not increase
performance enough to outweigh computational cost. 

As before, neural network parameters are optimized by stochastic gradient descent
with momentum and learning rate annealing. 
In a comparison against AlphaGo the resnet was more accurate, achieved lower error and
improved performance in AlphaGo by over 600 Elo~\cite{silver2017mastering}.

The input to the neural network is a $19 \times 19 \times 17$ image
stack comprising 17 binary feature planes. The 17 feature planes
contain the current board and a history of the 8 previous moves, both
for black and for white, and the color to play. The input features 
are processed by a residual network tower. The tower consists of a single
convolutional block followed by either 19 or 39 residual blocks, one
of which is shown in Figure~\ref{fig:resnetblock}. The total network
depth, in the 20 or 40 block network, is thus 39 or 79 parameterized
layers, plus  2 layers for the policy head and 3 layers for the value
head, consisting of a  block ending in a fully connected layer. See
the paper for details~\cite{silver2017mastering}.


\begin{figure}[ht]
    \centering{\includegraphics[width=4cm]{figures/resnetblock.jpg}
     \caption{AlphaGo Zero Residual Block~\cite{silver2017mastering}}\label{fig:resnetblock}}
\end{figure}



\subsubsection{Compute Hardware}
Originally, each neural network was trained with TensorFlow, with 64 GPU workers
and 19 CPU parameter servers. Later, TPUs were used.
Figure~\ref{fig:power} shows the
difference in total dissipated power consumption between the different versions of
AlphaGo.

\begin{figure}[ht]
    \centering{\includegraphics[width=10cm]{figures/power}
     \caption{Comparison of Power Consumption for Training~\cite{googlecloud2018}}\label{fig:power}}
\end{figure}

\subsubsection{Search Algorithm}
The search algorithm of AlphaGo Zero is MCTS. For selection, the same
P-UCT~\cite{rosin2011multi} variant was used, that incorporates priors from the policy head,
and not RAVE. This MCTS did not use roll outs at the leaves of the
MCTS tree, but value head lookups. In the self-play, a total of 25,000
games  were played in each self-play iteration. MCTS performs 1600
simulations for each move. %  Since there are no roll outs in this version,
% there is no $\lambda$ parameter.
MCTS hyperparameters were selected by Gaussian process
optimization~\cite{shahriari2016taking}. 


\subsubsection{Input/Output Features}
The input planes of AlphaGo Zero are simpler than in AlphaGo. Only the
board information is used, no additional information such as ko, or
liberties, is used. Even the basic heuristic of not playing moves that
would fill the player’s own
eyes is excluded. AlphaGo Zero learns from scratch. No heuristic
information is given to the program. 

\subsubsection{Playing Strength}
Silver et al.~\cite{silver2017mastering} describe that learning
progressed smoothly throughout training, and did not suffer 
from the oscillations or catastrophic forgetting that have been
noted in previous
literature~\cite{foerster2017stabilising,heinrich2016deep}.

Training progressed quickly. AlphaGo Zero
outperformed the original AlphaGo after just 36 hours. The training time for the
version of  AlphaGo that played Lee Sedol was  several
months. Furthermore AlphaGo Zero used a single machine with 4 tensor
processing units, whereas AlphaGo Lee was distributed over many
machines and used 48 TPUs. Figure~\ref{fig:ag0perf} shows the
performance of AlphaGo Zero. Also shown is the performance of the raw
network, without MCTS search. The importance of MCTS is large, around
2000 Elo points.


\begin{figure}[ht]
    \centering{\includegraphics[width=13cm]{figures/ag0perf}
     \caption{Performance of AlphaGo Zero}\label{fig:ag0perf}}
\end{figure}


\subsubsection{Reinforcement Learning versus Self-play}
Taking a step back, it is instructive to compare the self-play of
AlphaGo Zero and the DQN of Atari to the reinforcement
learning frame of agent and environment (see Figure~\ref{fig:rl}).

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/agent.png}
\caption{Reinforcement Learning}\label{fig:rl}
\end{center}
\end{figure}

{\em Environment\/}
In Atari the OpenAI Gym simulator is the environment. For each DQN action
Gym provides a new state and reward. In AlphaGo Zero the AlphaGo MCTS player is the
simulator that provides the states and rewards. Samples from
different games are used in the value function to prevent 
correlations/overfitting. 

{\em Agent\/}
In Atari the DQN net is the agent. The agent is trained to have good
actions/values by playing against the environment, provided by Gym.
In AlphaGo too the MCTS/network player is the agent. The net is
trained against MCTS generated plays of earlier 
versions of itself (the MCTS environment). 

The principle of the self-play scheme is not new. Training by
self-play, by self-generated examples, is the same as TD-Gammon  did
in 1995, and has been tried in different ways by others. What is new
is the success of this particular implementation, with MCTS, deep
networks, and GPUs/TPUs, on the full game of Go, far surpassing human ability.



\subsubsection{Tabula Rasa}
AlphaGo Zero's reinforcement learning is truly learning from
scratch. The paper notes that
AlphaGo Zero discovered a remarkable level of Go knowledge during
its self-play training process. This included not only fundamental
elements of human Go knowledge, but also non standard strategies
beyond the scope of traditional Go knowledge.

Joseki are standard
openings that Go players learn. Joseki are corner plays. There are
beginner's and advanced joseki. Over the course of its learning,
AlphaGo Zero progressed through learning these
joseki. It is interesting to study how it did so, as it reveals the
progression of AlphaGo Zero's Go intelligence. Figure~\ref{fig:joseki}
shows how the program learned over the 
course of a few hours of self-play.




\begin{figure}[ht]
    \centering{\includegraphics[width=13cm]{figures/joseki}
     \caption{AlphaGo Zero is Learning Joseki~\cite{silver2017mastering}}\label{fig:joseki}}
\end{figure}

The top row shows five joseki that AlphaGo Zero discovered. The first
joseki is one of the standard beginner's openings out of Go theory. As
we move to the right, more difficult joseki are learned, with playing
stones in looser configurations.

The bottom row shows five joseki favored at different stages of the
self-play training. It starts with a preference for a weak corner
move. After 10 more hours of training, a better 3-3 corner sequence
is favored. More training reveals more, and better, variations.

For a Go player, it is remarkable to see the kind of progression in
computer play, reminding them of the time when they themselves
discovered these joseki. It is hard not to anthropomorphisize AlphaGo
Zero (think of the computer as a human being).


\subsubsection{Open Questions}
Most of AlphaGo's  open questions on page \pageref{sec:open} are addressed by AlphaGo
Zero. The new program has a simpler architecture, and it addressed a
major AI question: learning from scratch,  with surprising success.

The architecture of the program has changed fundamentally: from a
combination of supervised and reinforcement
learning based on databases of positions, to a self-play loop in which
the searcher was incorporated in the training loop (Figure~\ref{fig:selfplay}/Listing~\ref{lst:selfplay}). Surely earlier
works on self-play were an inspiration for AlphaGo Zero (see
Section~\ref{sec:early}). In any 
event, an important open question was answered. 

%% Chapter~\ref{chap:conv} showed us that a major concern in
%% reinforcement learning is overfitting due to 
%% correlated training data. The work on AlphaGo Zero answers this issue
%% elegantly. The stability of the training is greatly improved when
%% training targets are close to the current level of knowledge.
%% {\bf dit is toch helemaal niet waar?}


A remaining question was one of the Drosophila questions. Can we
construct a player that plays different games, the GGP
question~\cite{pell1996strategic,genesereth2005general}?



\subsection{AlphaZero}\index{AlphaZero}\label{sec:alphazero}
After defeating the best human Go players, and after having created
the first Tabula Rasa self learning Go computer, the team went on to tackle
this other long standing challenge in AI: constructing a general game
player. If AlphaGo 
Zero's architecture was able to learn Go from scratch, then perhaps it
would  be able to learn {\em any\/} game? A year after the AlphaGo Zero
publication they published
a positive result, showing how AlphaGo Zero's design could also play
Chess and Shogi.

At the end of 2017 a preprint~\cite{silver2017shogi} reported that
the AlphaGo Zero approach also worked on Chess and 
Shogi (a kind of Japanese Chess). A year later the formal publication
followed~\cite{silver2018general}. The team had been able to teach the
same network architecture (20
resnet blocks) to learn Go, Chess and Shogi, thus achieving a limited
form of {\em general\/}
tabula rasa learning. The program, named AlphaZero, beat the strongest
players in Go, Chess and Shogi (respectively AlphaGo Zero, the program
Stockfish,
and the program Elmo).

Note that the hand-crafted input and output layers of the networks are different
for each game. Furthermore, the weights in the trained networks are
also different. Strict transfer learning was not achieved: a trained Shogi net
is not able to play Go.

AlphaGo Zero's achievement is remarkable for more than one reason.
First, it is remarkable that self-play is so powerful that it can learn
from scratch {\em and\/} become so strong that it beats the current
world champions.
Second, it is remarkable that different games can be learned by the same
network architecture.
Apparently, some kind of element of general learning must have been
learned and hidden in the resnets of AlphaZero.
Third, it is amazing that for Chess and Shogi,  all strong programs
were based on the heuristic planning approach of alpha-beta with domain
specific heuristics~\cite{ramanujan2010adversarial}; and are now they
are beaten by a general approach using self-play function approximation.

\subsubsection{Go, Chess and Shogi}\index{Shogi}\index{Elmo}\index{Stockfish}
That AlphaZero can play three different games with one architecture is surprising.
The three games, though all board games, are quite different. Go is a
static game of strategy. Stones, once placed, do not move, and are
rarely captured. Each stone played is therefore of strategic
importance. In Chess the pieces move, it is a  dynamic game
where tactics are important, and sudden death is an important element
of play. In Chess it is
possible to win in the middle of the game by capturing the king. No such
concept exists in Go. Indeed, one element of human Chess play is to
move the king to a safe position to reduce the level of stress in the game. Shogi,
sometimes called Japanese Chess, is
even more dynamic. Pieces, once captured, can be returned in the
game, changing loyalty, creating even more complex game dynamics.\footnote{Pieces
are of the same color, but are wedge-shaped, and change orientation
when switching sides.}

It appears that since the kinds of move patterns, the tactics, and the
strategies to be learned are very different, that it  requires
a different kind of program. Indeed, this is the conventional 
approach: a  developer crafts a program specifically for a
certain game, incorporating all kinds of game specific knowledge and
heuristics into the code.  For Go, the game is so subtle
and difficult that no 
scientist was able to elicitate successful heuristics, and knowledge
had to be learned by machine learning from carefully crafted game databases (initially, in
AlphaGo) or through self-play 
(eventually, in AlphaGo Zero).

The conventional game-specific
approach has worked well for Chess, Shogi and  other games so
far. The general programs created by GGP generally trade-off
generality for playing strength. AlphaZero is the first to show that it is
possible to be general {\em and\/} strong.



As all top Chess programs,  Stockfish follows the classic search-eval
design of alpha-beta  and a heuristic
evaluation function, that we have seen in
Sunfish (see Section~\ref{sec:sunfish}) and Deep Blue (see
Section~\ref{sec:deepblue}). Among the enhancements of Stockfish are
forward pruning,
iterative deepening, transposition tables, quiescence, piece-square
tables, null window, null move, history heuristics, 
search extensions, search reductions, static exchange evaluation, an
opening book and
an end game database. Chapter~\ref{chap:idtt} provides background
explanations on
most of these enhancements. In Stockfish, all these enhancements have been carefully
tested and tuned, for many years~\cite{stockfish}.

The state space complexity of Shogi is  substantially larger than
Chess: $O(10^{71})$ versus
$O(10^{47})$~\cite{allis1994searching,iida2002computer}. The strongest
Shogi programs have recently started defeating human
champions~\cite{shogi}. Elmo, one of these programs, is
designed like Chess programs, around alpha-beta search and a heuristic
evaluation function, with many carefully tuned and tested game
dependent enhancements.

\subsubsection{One General Architecture}
Although it would seem that the different kinds of games
require a different program design, AlphaZero's results have proven this
conventional wisdom wrong, at least for the three board games. All that needed to be changed were the
input and output layers of the function approximator. The self-play training
algorithms, network architecture, search algorithm, training
parameters and compute hardware
are all the same. The self-play
program was then able to learn to play the game beyond world class
level. Either the game dynamics of Go, Chess and Shogi are less
different than they seemed, or the resnet is learning some knowledge of
quite general applicability (or, more likely, a bit of both).

\subsubsection{Input/Output Features}
The input and output
layers are different for each game.
For Go, the same $19\times
19\times 17$ planes as in AlphaGo Zero were used in AlphaZero, where 8
moves of history is encoded in addition to the stones on the
board. Move encoding in Go is simply a coordinate of a stone.

For Chess, a similar encoding scheme is used, although more elaborate
using many more planes. The scheme encodes all possible moves from
a position in different binary planes. In Chess there is a greater
variety of possible moves, and the encoding scheme therefore uses more planes
than in Go, $8\times 8\times 73$.\footnote{Silver et al.~\cite{silver2018general} contains the
details of their elaborate encoding. The encoding scheme is quite complex, although it is noted that simpler
encoding schemes also work.}

Shogi has an even greater variety of
moves, leading to a stack of $9\times 9\times 139$ planes as
input. The paper mentions that experiments with different coding
schemes worked as well, altough training efficiency was affected somewhat.

\subsubsection{Playing Strength}
The Elo rating of AlphaZero in Chess, Shogi and Go is shown in
Figure~\ref{fig:azelo}. Also shown is the Elo rating of the programs
Stockfish, Elmo,  AlphaGo Zero~\cite{silver2017mastering} and
AlphaGo Lee~\cite{silver2016mastering}.

We can see how AlphaZero is
stronger than the other programs, all through learning by self-play. In Chess, a field that has benefited from work
by a large community of researchers for as long as computers existed,
the difference is the smallest. For Shogi the difference in playing
strength is larger.

Interestingly, AlphaZero slightly outperforms AlphaGo Zero. There are sall
differences between AlphaZero and AlphaGo Zero. AlphaZero updates the
neural network continually whereas in AlphaGo Zero the new net is only
accepted if it wins 55\% of the times against the old
network. AlphaZero does not exploit Go symmetries. 


\begin{figure}[ht]
    \centering{\includegraphics[width=13cm]{figures/azelo}
     \caption{Elo Rating of AlphaZero in Chess, Shogi, and Go~\cite{silver2018general}}\label{fig:azelo}}
\end{figure}

\subsubsection{Compute Hardware}
Both Stockfish and Elmo ran with 44 threads on 44 cores (2 Intel Xeon
Broadwell CPUs with 22 cores) with 32 GB transposition tables and 3 hour
per match time controls with 15 seconds per move extra. AlphaZero ran
on a single machine with 44 CPU cores, and 4 first-generation TPUs.



%\subsection{Reimplementations of AlphaZero}
\subsection{Open Reimplementations of Alpha Zero}\label{sec:reimp}
When the AlphaGo papers were published, this caused great
interest in the research community. The DeepMind team has not yet published
their code, but the
publications~\cite{silver2016mastering,silver2017shogi}
(and especially~\cite{silver2017mastering}) provide enough detail for 
researchers to create their own versions, some of which are open
sourced on Github.

\subsubsection{A0G: AlphaZero General}
Thakoor et al.~\cite{nair2017learning} created\index{A0G}\index{AlphaZero General}
a self-play system as part of a course project.  The system is called AlphaZero
General (A0G), and is
on \href{https://github.com/suragnair/alpha-zero-general}{Github}.\footnote{\url{https://github.com/suragnair/alpha-zero-general}} It
is implemented in Python and Tensorflow, Keras and PyTorch, and
suitably scaled down for smaller computational resources. It has
implementations for $6\times 6$ Othello, Tic Tac Toe, Gobang, and
Connect4, all small games of significantly less complexity than
Go. Its main network architecture is a four layer CNN followed by 
two fully connected layers. The code is  easy to understand
in an afternoon of study, and is well suited for educational purposes.
The course project write-up provides some \href{https://github.com/suragnair/alpha-zero-general/raw/master/pretrained\_models/writeup.pdf}{documentation} for A0G~\cite{nair2017learning}.


\subsubsection{Facebook ELF}
ELF stands for Extensible Lightweight Framework. It is a framework for game
research  in C++ and Python~\cite{tian2017elf}. Originally developed
for real time strategy games by Facebook, it includes the Arcade Learning Environment and
the \href{https://github.com/facebookresearch/darkforestGo}{Darkforest}\footnote{\url{https://github.com/facebookresearch/darkforestGo}}
Go program~\cite{tian2015better}. ELF can be found
at \href{https://github.com/pytorch/ELF}{Github ELF}.\footnote{\url{https://github.com/pytorch/ELF}}
ELF  also contains the program OpenGo~\cite{ELFOpenGo2018}, a reimplementation of  
AlphaGo Zero (in C++).\index{ELF}\index{OpenGo}

\subsubsection{Leela}
Another reimplementation of AlphaZero is
 Leela. Both a Chess and a Go version of Leela
 exist. The \href{https://github.com/LeelaChessZero/lczero}{Chess}\footnote{\url{https://github.com/LeelaChessZero/lczero}}
 version is based on Chess engine
 Sjeng. The \href{https://github.com/gcp/leela-zero}{Go}\footnote{\url{https://github.com/gcp/leela-zero}}
 version is based on Go engine Leela.  Leela does not come with
 trained weights of the network. Part of Leela  is a community effort
 to compute these weights.\index{Leela}  


\subsubsection{PhoenixGo}\index{PhoenixGo}
PhoenixGo is a strong Go program by Tencent~\cite{PhoenixGo2018}. It
is based on the AlphaGo Zero architecture. It can be
found at \href{https://github.com/Tencent/PhoenixGo}{Github
PhoenixGo}.\footnote{\url{https://github.com/Tencent/PhoenixGo}} A
trained network is available as well. 

\subsubsection{Deep Reinforcement Learning}
Finally, a Python implementation of self-play
is
\href{https://github.com/AppliedDataSciencePartners/DeepReinforcementLearning}{DeepRL}.\footnote{\url{https://github.com/AppliedDataSciencePartners/DeepReinforcementLearning}}
DeepRL provides  code for a nice on line tutorial on AlphaZero-based self
play. It implements the game Connect4.


\subsection{1+2=3}\label{sec:123}
The link between planning, training, self-play on the one hand and
thinking fast and slow on the other has been noted
in~\cite{anthony2017thinking}. When we look at the search-eval
architecture (Figure~\ref{fig:arch10} we see three elements: the
search procedure, the evaluations procedure, and the self-play
loop.  Evaluation, system 1, is thinking fast, a reflex-like
network. Planning, system 2, is
thinking slow, a reasoning-like rational brain.  Self-play takes evaluation (system 1) and planning
(system 2) and adds a third system, a training loop, to create a self
learning system. The third system, the self-training
loop, allows the reasoning system to feed training examples to the
network to improve the reflexes.  Note that
Kahneman~\cite{kahneman2011thinking} does not identify a third system.

Already in 1959 Samuel~\cite{samuel1959some} introduced the idea of
learning by self-play in his  Checkers program. In his program,
the coefficients of the heuristic function were updated towards the value of the search after black and
white had each played one move. 

Concurrently to the work by the DeepMind
team, Anthony et al.~\cite{anthony2017thinking}\index{ExIt} worked on a similar
idea for tabula rasa learning 
based on self-play, combining MCTS and DQN. The name of their work is
ExIt, for Expert Iteration. They did not use Go, but
Hex, a simpler game, to show their methods. They do make the link with
Kahneman's work explicit in the title of their paper.


Supervised learning, as in Neurogammon, uses a database to learn by
example from good moves.
Self-play is different. In minimax and MCTS, the look ahead
searcher is alternately playing  the role of the player and of its
opponent, to determine the best move. In self-play, the look ahead
searcher generates more 
difficult training examples, on which the evaluation network is
trained. The improved searcher is then used to generate more difficult
training examples, on which the evaluation network is trained again,
etc.\footnote{
Note that the self-play searcher internally also uses MCTS to
alternately play the role of player and opponent.}

By this recursive mechanism the system grows in strength, assuming
there are no pitfalls along the way. Among the pitfalls to take care of
are a convergent training process, and an all encompassing, diverse, training
process. A
Chess player who is an expert in pawn play but does not know how to
use the knight well is not an all-round player. The Chess player may
play well against a similarly myopic player trained in the same
specialization, but will fail against a fresh
test opponent trained in other areas. The AlphaGo Zero publication
provides few hints on how to achieve this.

\subsection{Earlier Works}\label{sec:early}
The success of AlphaZero builds on other research in
self-play. Self-play and self-learning have fascinated many AI
researchers, and a large literature of 
self-play systems exists. In self-play the first two parts of this
book come together: planning and training. The search-eval
architecture gets an extra loop (see
Figure~\ref{fig:selfplay}).
To understand the current
methods of AlphaZero, where they came from, and what solutions we can
expect for current challenges, we will now take some time to look
deeper into  previous work on self-play.


AlphaGo was not created in a vacuum. There is a large body of research
of which we will now discuss some of the more notable successes.

Turing's original article on a paper chess program introduced the basic
search-eval architecture, with the basics of minimax state space
search, and feature-based
eval. % Putting an extra reinforcement learning loop around
% it,  allows a virtuous circle of learning from self-play: a planner
% that generates examples to train the value function approximator,
% which is then used in the next iteration as an improved evaluation
% function by the planner to generate even better examples, etc.

As many developments in science, the AlphaGo success builds on a large
body of previous work. Table~\ref{tab:programs} lists some  of the
notable works on games, with an emphasis on the training part. The
first column contains the name of the program, if given in the
paper. The second column lists which game(s) the program plays. The third column is
the planning algorithm, if applicable. The fourth column is the
learning algorithm, if applicable. CNN stands for convolutional neural
net, FCN for fully connected net. The fifth column contains the data
with which the learning took place. For supervised learning this is
typically a database of grandmaster games, and for reinforcement
learning self-play, or databases with self-played games, are often used. The sixth column is the network
architecture. Only the hidden layers are noted. For the older papers
this is often a small number of hidden layers (and neurons). After the
advent of GPUs in 2012 larger nets became feasible. The seventh column
lists the evaluation method. This can be a linear combination of
heuristic features, a system where the network learns the coefficients
of heuristic features, or a full end-to-end learning system from  raw board
input. Last is a reference to a major work describing the approach of
the program. Only the name of the first author is noted. Some programs
were developed over many years by different authors.   


\begin{table}
\begin{center}
\input diag/programs
\caption{Evolution of Planning, Learning and Self-play in Game
Playing}\label{tab:programs} 
  \end{center}
\end{table}

We will now discuss how the methods of the programs developed. These
methods are mostly aimed at position evaluation, although some are also
used for (selective) search.

\subsubsection{Shapes and Patterns}
Shapes and patterns are of great importance in many games. For this
reason, many early works focused on learning shapes and patterns.
In the Checkers program Chinook much of its strength came from its
endgame database. The endgame database contained all board positions
with 8 or fewer pieces. As soon as the database was reached by the
search, perfect knowledge was reached. The end game database greatly
contributed to the strength of
Chinook~\index{Chinook}\cite{schaeffer1996chinook}. In Chess, Deep
Blue had a database that was accessed as soon as 5 or fewer pieces
were on the board~\cite{campbell2002deep}.

In Go, the emphasis is on small local patterns. Stoutamire used hashed sets of patterns  to
find good and bad shapes~\cite{stoutamire1991machine}. Van
der Werf used neural networks and automatic feature extraction to
predict good local moves from game
records~\cite{van2002local,van2004ai}. 

In the contexts of MCTS, many researchers were working on combining MCTS with
learned patterns, especially to improve the random roll outs of MCTS. Supervised learning on grandmaster games
was used to improve playouts and also to improve UCT selection. Gelly \& Silver  et 
al.\ published notable works in this area~\cite{gelly2006modification,silver2007reinforcement,gelly2008achieving}. The
program MoGo\index{MoGo} achieved good results around 2006-2009.

\subsubsection{Regression}
Patterns are also important in Othello. Around 1995 very good results were achieved by
Logistello~\cite{buro1995logistello}\index{Othello}\index{Logistello}. Logistello
used logistic regression on patterns. The author also successfully
introduced probabilistic depth reduction methods~\cite{buro1997experiments}.

\subsubsection{Game Databases}\index{supervised learning}
Many researchers have tried supervised learning on  databases of
grandmaster games.

Tesauro's 1989 Neurogammon\index{NeuroGammon} achieved good results in
Backgammon with supervised learning of the coefficients of an evaluation
function with handcrafted features. It used a single hidden
layer~\cite{tesauro1990neurogammon}. 
In Go,  Enderton used
neural networks in the search, for move ordering and forward pruning of
selective search in his Golem Go program~\cite{enderton1991golem}. Enzenberger's Neurogo\index{NeuroGo} used a neural network for
position evaluation~\cite{enzenberger1996integration}.

Much later, Maddison et al.\ published work on a 12-layer convolutional
neural net for move predicition in Go~\cite{maddison2014move}, laying
a foundation for the supervised learning of AlphaGo.
Facebook's AI Research lab created
Darkforest\index{darkforest} for end-to-end deep learning of Go
positions and MCTS~\cite{tian2015better}. Graf et al.~\cite{graf2015adaptive} describe experiments with adaptive
playouts in MCTS with deep learning.
Convolutional neural nets were also used in Go by Clark and
Storkey~\cite{clark2014teaching,clark2015training} who had used a CNN for supervised learning
from a database of human professional games, showing that it
outperformed GNU Go and scored wins against Fuego.

In Chess, the program Deepchess\index{DeepChess} by
David et al.~\cite{david2016deepchess} performed end-to-end deep
learning in Chess, achieving results on par with Falcon and Crafty,
two  alpha-beta based programs.

In Checkers,
Blondie24~\cite{chellapilla1999evolving,fogel2001blondie24} used a
network to evolve board features, also achieving good results. 


\subsubsection{Temporal Difference  Learning}\index{temporal difference}
After the success with supervised learning in Neurogammon, Tesauro
tried temporal difference learning from the raw board in a small neural network in 1992. This
was further augmented with expert designed features, resulting in
play at  world class level. TD-Gammon's success was the first widely
published  success of
self-play~\cite{tesauro1995temporal,tesauro2002programming}.\index{TD-Gammon} 
Tesauro's success inspired many others to try temporal difference learning.

Wiering et al. and Van der
Ree~\cite{wiering2010self,van2013reinforcement} report on self-play
and TD learning in Othello and Backgammon.


In Go Schraudolph et al.~\cite{schraudolph1994temporal} used temporal difference to
learn position evaluation from board networks. They note that to be
successful, networks should reflect spatial organization of input signals.
Huang et al.~\cite{huang2003learning} used self-play of 16 different players to learn
opening strategies in Go.

Silver, in his PhD thesis~\cite{silver2009reinforcement}, applied reinforcement
learning to search in Go, and Silver et
al.~\cite{silver2007reinforcement} and
Gelly \& Silver~\cite{gelly2008achieving,gelly2007combining,gelly2012grand}
studied reinforcement learning of local shape patterns.
Silver et al.~\cite{silver2012temporal} further combined temporal difference learning
in MCTS.

In Chess,
Thrun's Neurochess\index{NeuroChess}~\cite{thrun1995learning} tried
temporal difference feature learning.
The program Knightcap~\cite{baxter1999knightcap,baxter2000learning}\index{Knightcap} and
Beal et al.~\cite{beal2000temporal} also use temporal difference learning on evaluation
function features. Veness et al.\cite{veness2009bootstrapping} use
self-play to learn evaluation function weights. They name their
approach {\em search bootstrapping\/} and, referencing Samuel's Checkers program, describe it as follows: ``The idea of search
bootstrapping is to adjust the parameters of a heuristic evaluation
function towards the value of a deep search.'' This sentence captures
the idea of self-play, as used in AlphaZero, quite well.
Arenz~\cite{arenz2012monte} applied MCTS to Chess.

Inspired by the progress in deep learning, in
2015 Matthew Lai tried end-to-end learning in Chess: he went beyond
evaluation function weight 
tuning with Giraffe~\cite{lai2015giraffe},\index{Giraffe} using DQN, 
and self-play, including feature extraction and pattern recognition
for end-to-end reinforcement learning. Giraffe reached master level
play.
Heinz also reported on self-play experiments in
Chess~\cite{heinz2000new}. He later joined the AlphaZero team.

In other games, Guo et al.~\cite{guo2014deep} report on the use of MCTS to play Atari
games, their combination of MCTS and DQN outperforms DQN on Atari.

In Poker,\index{Poker} an imperfect information game, impressive results have been
published~\cite{bowling2015heads,moravvcik2017deepstack} with
combinations of planning and learning algorithms, most notably
counterfactual regret minimization and self-play.


In some of the early works the small size of the networks limited
success. In others the temporal difference  learning or self-play is based on handcrafted or
heuristic features of the state space, possibly introducing  bias
or errors. End-to-end 
learning, from the raw board or pixels requries more computational
power. When first done successfully end-to-end
(AlexNet~\cite{krizhevsky2012imagenet},
Atari~\cite{mnih2013playing,mnih2015human}) the papers generated much
research interest. 







\subsection{Impact}


\subsubsection{Popular Media}
The Lee Sedol match of AlphaGo has  had a large impact in
the popular media. The vision of computers being smarter than highly
intelligent human champions continues to attract attention, as much as
it did in the days of Deep Blue--Kasparov. AI shot to
prominence and many AI researchers were interviewed on questions
ranging from when we would see self driving cars,
to the future of the human race.

Many newspaper articles appeared, a quite entertaining movie\footnote{\url{https://www.youtube.com/watch?v=9gzMQOa5MD4}} was
made, and many blogs were written for enthusiasts on how to build your
own AlphaGo/AlphaZero. This, by the way, turns out to be quite doable on the
algorithmic side (see Section~\ref{sec:reimp}) but  acquiring the computational power to
train the function approximators is a challenge.

\subsubsection{Impact on Go}
It is interesting to see how human Go players respond to the matches,
and to see how the style of human play changes. Despite some sadness,
mostly reactions were positive, Go 
players were enthusiastic about the innovations and new style of play
that AlphaGo exhibited. Players were eager to learn more about their
game. Books have been written about the new go theory that was
created (for example, Zhou~\cite{zhou2018}). The publicity around the
matches created much new interest in the game. 

\subsubsection{Impact on Science}\label{sec:science}
The AlphaGo matches have also had quite an impact on science. The interest
from society in AI has increased significantly, with companies and
governments investing in AI research labs. Also within
science there has been much interest in multidisciplinary
collaborations, to see how machine learning can transfer to fields
ranging from astronomy, physics, pharmacology, chemistry, medicine,
biology, psychology, sociology, economics, archeology, linguistics,
literature, history, policy science, law, philosophy, to the arts.

\subsubsection{Impact on AI}
On AI the AlphaGo matches and the self-play results of Alpha(Go) Zero
have had a large impact as well. Machine learning has attracted many
new talents, and especially reinforcement learning has
ballooned. Work on benchmarking and reproducibility~\cite{henderson2017deep,khetarpal2018re,islam2017reproducibility}\index{reproducibility} in reinforcement
learning has increased. Popular suites are ALE~\cite{bellemare2013arcade},\index{ALE}\index{Gym}
Gym~\cite{brockman2016openai}, ELF~\cite{ELFOpenGo2018},\index{ELF}
Starcraft~\cite{uriarte2015benchmark,koeman2018starcraft,vinyals2017starcraft},
and Mario~\cite{karakovskiy2012mario}.\index{StarCraft}\index{Mario}
There is also much interest in 
solving further challenges of self-play (see the open questions in
Section~\ref{sec:questions} on page~\pageref{sec:questions}). 

\subsubsection{Future of Self-Play}
Self-play has been an active area of research for many years. The
AlphaZero results have shown the power of the paradigm, and the
successes have created much research interest into fundamental
questions and applications of self-play. 


%\subsubsection{Open Questions}
\label{sec:questions}
Many questions remain. Among them are:
\begin{itemize}
\item
Why is performance of self-play levelling off? Is the network
saturating? How can learning be
improved further? Can learning be sped up, can learning efficiency be improved?
\item
For which other domains can self-play work? Does self-play only work
for board
games, or also for other Markov problems, or for non-Markovian problems?
\item
Did self-play kill the deadly triangle? Is training stability no
longer a problem? Is overfitting solved?

\item
Why do resnets perform so well in self-play? Are there other
architectures that work better? Can the network architecture be
optimized automatically? 
\item
So far, general methods have been enhanced with domain dependent
methods (Chapters~\ref{chap:idtt} and \ref{chap:conv}). Which
enhancements work well in self-play?
\item
How general are the concepts learned by self-play? How can learned
concepts be transferred to other games? (Note that in AlphaZero each
game needed to start training from scratch.)
\item
Hierarchical reinforcement learning studies how multiple layers of
abstraction can order state spaces, and solve more complicated
problems. Will it work for self-play?
\item
Does self-play work well in imperfect information games such as
Bridge, Poker, and Starcraft? 
\item
There is much  research in flat DQN (training without planning). Self-play appears to crucially depend on
planning to generate high quality examples. Will exact methods  make a come
back or will DQN find ways to train for the long credit assignment
distances that planning is so good at?
\item
Evolutionary Strategies have been successful in some studies. Will they
play a role of importance in (general) self-play?
\end{itemize}

\section{Practice}
The AlphaZero General (A0G) code base is well suited for experimentation with
self-play. A0G can be found 
at \href{https://github.com/suragnair/alpha-zero-general}{A0G}.\footnote{\url{https://github.com/suragnair/alpha-zero-general}} Note
that you also have to install TensorFlow and Keras. They are
at \href{https://www.tensorflow.org}{tensorflow.org}.


\subsubsection{Exercises}
\begin{enumerate}
\item Install and run A0G Othello 6x6. Play against the computer. 
\item Observe the learnign processes of the different games Tic Tac
  Toe, Connect4, Gobang. See how self learning progresses 
\item Vary learning rate, vary MCTS Nsims, vary iterations. How is
  performance impacted? How is learning time impacted?
\item Try different net architectures. How is performance impacted?

\item Take a traditional alpha-beta Othello program, for
example \href{http://dhconnelly.com/paip-python/docs/paip/othello.html}{Othello}.\footnote{\url{http://dhconnelly.com/paip-python/docs/paip/othello.html}} See
if A0G can learn a strong enough player to beat it.
\item Choose a simple game, and implement it in A0G. Does it learn quickly?
\item *Implement Chess input and output layers in A0G, learn it tabula rasa, and play
  against Sunfish. You may want to have a look at LeelaZero Chess or ELF OpenGo for inspiration.
\end{enumerate}

\section{Summary}
%{\bf central concept: self-play works well through curriculum
%learning}
In this chapter we analyzed in-depth the performance of AlphaGo,
AlphaGo Zero, and AlphaZero. Three of the strongest human Go players
were resoundingly defeated by the AI, causing great interest in AI by
science and society.

Issues of generalization, overfitting and training stability (the deadly triad)
were overcome by the AlphaGo team in an impressive show of science and
engineering prowess, for which they received many accolades.

The main conceptual innovation of this
chapter is the impressive performance of self-play, as a combination
of a planning and training loop,  as a combination of MCTS and
DQN. Self-play, Figure~\ref{fig:selfplay}, takes Evaluation (System 1) and Planning
(System 2) and adds a third item, a learning loop, creating a
self-learning system. 

The self-play loop uses MCTS to generate high-quality examples,
which are used to train the neural net, which is then used in a
further self-play iteration to refine the network further (and again,
and again, and again).
Alpha(Go) Zero thus learns from zero knowledge, tabula rasa. And, just
as impressively, the same self-play architecture can learn tabula rasa
Chess and Shogi as well, defeating decades of heuristic refinement.

MCTS is changed significantly in the self-play setting. Gone are the
random play-outs that gave MCTS the name Monte Carlo, and much of the
performance is through a high-quality policy and value approximation
residual network. The name DQN-TS for DQN Tree Search would be more appropriate.

Self-play creates a natural form of curriculum learning. We will
look deeper into curriculum learning in the next chapter.


Reproducibility in science is of great importance to
progress~\cite{henderson2017deep}. The impact of benchmarks and open
source algorithms in this respect is important. The reimplementations
of the self-play results in A0G, ELF OpenGo, PhoenixGo and Leela will stimulate
experimentation and are
of  importance to progress towards general learning systems.





\section*{Historical and Bibliographical Notes}
The work on AlphaGo is a landmark achievement in AI. Every AI
researcher is encouraged to study it well.
The primary source of information for AlphaGo are the three AlphaGo
papers by Silver et
al.~\cite{silver2016mastering,silver2017mastering,silver2018general}. The
papers contain a wealth of information, and are well written, although
can be a bit overwhelming at times. Many blogs and popular press
articles have been written about AlphaGo, and also many Youtube videos
exist explaining things in a way that might be  more
accessible.

Do not forget to watch the AlphaGo movie. Although it does not go too
deep into the details, it is a fascinating account of the match, and
its significance in AI. It is
at \href{https://www.youtube.com/watch?v=9gzMQOa5MD4}{AlphaGo Movie}.\footnote{\url{https://www.youtube.com/watch?v=9gzMQOa5MD4}}

As happened after Deep Blue-Kasparov, there has been a fan out of
AlphaGo like technology to other fields, where similar decision making
questions are present.
Other applications: retrosynthesis of molecules in
chemistry~\cite{segler2018planning}.

Self-play works: Samuel, Tesauro, 


==> chapters/old11transfer.tex <==

%% The problems of this chapter are performance and applicability: we
%% wish to increase the 
%% quality of self-play, and we wish to enlarge the range of applications
%% that it can be applied to. We will 

Self-play has been used in AI since the early days, yet there are
still many opportunities for enhancing performance. 
In this chapter we will discuss ways to deepen our understanding of self-play, to
enhance performance, and to increase the number and kinds of problems that
self-play can be applied to.

We start with the open questions from the previous chapter, that were
mostly concerned with learning efficiency. Since
the advances in self-play are still young, many of the enhancements
discussed in 
this  chapter are suggestions for future studies in the relevant
application domains.

\begin{itemize}
\item (understanding) why does self play work? [curriculum
  learning/convergence: example buffer]
\item (improvement) how can it be further improved? [better understanding/visualize net]
\end{itemize}


%% \section*{Learning Goals}
%% \begin{itemize}
%% \item stability: learning process improvements. deadly triad?
%% \item generalization to other problems. arch, hier rl, other self play work
%% %% \item
%% %% For which other domains can self play work? Does self play only work
%% %% games, or also for other Markov problems, or for non-Markovian problems?
%% %% \item
%% %% Why is performance of self play levelling off? How can learning be
%% %% improved further? 
%% %% \item
%% %% Did self play kill the deadly triangle? Is learning stability no
%% %% longer a problem? Is overfitting solved?
%% %% \item
%% %% Can learning be sped up, can learning efficiency be improved?
%% %% \item
%% %% Can the network architecture be learned automatically?
%% %% \item
%% %% Why do resnets perform so well in self play? Are there other
%% %% architectures that work better?
%% %% \item
%% %% How general are the concepts learned by self play? How can learned
%% %% concepts be transferred to other games? (Note that in AlphaZero each
%% %% game needed to start training from scratch.)
%% %% \item
%% %% Does self play work well in imperfect information games such as
%% %% Bridge, Poker, and Starcraft? 
%% \end{itemize}

%% These questions can be grouped into two categories: questions about
%% the training process, and questions about generalization towards more
%% applications.

This chapter will deal with curriculum learning and transfer learning.

We saw that curriculum learning was mentiojned as explanation for the
faster learning of AlphaZero.

\section{curriculum learning}
summarize bengio, weinshal, silver.

bengio 2009

deep training is hard

Elman 1993: curriculum: start small increase difficulty, also: small capacity
learn possible unlearnable
multi-stage curriculum strategies improved generalization and faster convergence

Bengio writes: deep architecture training. Some have good solutions in local minima that are almost impossible to find by random initialization. (Erhan 2009)
Deep learning attempts to learn feature hierarchies. Features at
higher levels are formed by composition of lower level
features. Automatically learning multiple levels of abstraction,
creating a complex function mapping from input to output, without
depending on human crafted features.

Training deep architectures involves a potentially intractable
optimiztation problem. Before Hinton 2006 there were no good
algorothms for training fully-connected deep architectures, when they
introduced greedily training one layer at a time. It exploits
an unsupervised generative learning algorithm for each layer: a
restricted Boltzmann Machine.  Now, it is conceivable that by training
each layer one after the other, we first learn the cimpler concepts,
represented in the first layer, then silightly more abstract concepts
in the second layer, etc. Further works introduced other algorithms
for training deep architectures, all showing advantage of deep
architectures over shallow ones, and using unsupervised pre-training. 

Out of the study for better deep learning algorithms, and the success
of unsupervised pre-training, curriculum
learning arose. Unsupervised pre-training starts the supervised
poptimzation in a region of parameter space that were not much better
in terms of final trainign error, but substantially better in terms
of test error (they generalized better). This suggests a dual effect
of unsupervised pre-training. It helps opitmization by starting in
better basins of attraction of the descent procedure in parameter
space, and as a kind of regularizer.

A curriculum can be seen as a sequence of training criteria. Each
training criterion in the sequence is associated with a different set
of weights on the training examples. Initially, the weights favir
easier examples, or examples illustrating the simplest concepts, that
can be learned most easily. The next training criterion involves a
slight change in the weightingof examples that increases the
probability of sampling more difficult examples. At the end of the
sequence, the reweighting of the examples is uniform and we train on
the target training set of the target training distribution.

Advantage of a curriculum strategy is: faster training in the online
setting because the learner wastes less time with the noisy or harder
to predict examples (when it is not ready to incorporate them).

And guiding training towards better regions in parameter space, into
basins of attraction (local minima) of the descent procedure
associated with better generalization: a curriculum can be seen as a
particular continuation method. (...)

Curriculum strategies are also connected to transfer (or mukti-task)
learning
Curriculum strategies are also connected to transfer (or multi-task)
learning and lifelong learning (Thrun, 1996). Curriculum learn- ing
strategies can be seen as a special form of trans- fer learning where
the initial tasks are used to guide the learner so that it will
perform better on the final task. Whereas the traditional motivation
for multi- task learning is to improve generalization by sharing
across tasks, curriculum learning adds the notion of guiding the
optimization process, either to converge faster, or more importantly,
to guide the learner to- wards better local minima.


Weinshall:
in human learning supervision is often accompanied by a
curriculum. Thus the order of presented examples is rarely random when
a human teacher teaches another human. Like- wise, the task may be
divided by the teacher into smaller sub-tasks, a process sometimes
called shaping (Krueger \& Dayan, 2009) and typically studied in the
context of reinforcement learning (e.g. Graves et al., 2017). Although
it remained for the most part in the fringes of machine learning
research, curriculum learning has been identified as a key challenge
for machine learning throughout (e.g., Mitchell, 1980; 2006; Wang \&
Cottrell, 2015). 

We focus here on curriculum learning based on ranking (or weighting as
in (Bengio et al., 2009)) of the training exam- ples, which is used to
guide the order of presentation of examples to the learner. Risking
over simplification, the idea is to first present the learner
primarily with examples of higher weight or rank, later to be followed
by examples with lower weight or rank. Ranking may be based on the
dif- ficulty of each training example as evaluated by the teacher,
from easiest to the most difficult. 

curriculum learning, when given the ranking of training points by
their difficulty thus defined, is expected (probabilistically) to
significantly speed up learn- ing especially at the beginning of
training. This theoretical result is supported by empirical evidence
obtained in the deep learning scenario of curriculum learning
described in Section 3, where similar behavior is observed. We also
show that when the difficulty of the sampled training points is fixed,
convergence is faster when sampling points that incur higher loss with
respect to the current hypothesis as suggested in (Shrivastava et al.,
2016). This result is not al- ways true when the difficulty of the
sampled training points is not fixed.
But such ideal ranking is rarely available. In fact, the need for such
supervision has rendered curriculum learning less useful in machine
learning, since ranking by difficulty is hard to obtain.

However, self play

Learning rate is always faster with curriculum learning, especially at
the beginning of training. (ii) Final generalization is sometimes
improved with curriculum learn- ing, especially when the conditions
for learning are hard: the task is difficult, the network is small, or
when strong regularization is enforced. These results are consistent
with priorart(see e.g. Bengioetal.,2009). 

\section{pre-training as transfer learning for curriculum learning}
Join both.

Pre-training with a curriculum strategy might act similarly to
unsupervised pre-training, acting to find better local minima and as a
regularizer, and help to reach faster convergence to a minimum of the
error function.

Curriculum is like transfer from stage to stage.
Pre training.

notion of transfer discussed in (Bengio et al., 2009) in the context
of multi-task and life- long learning (Thrun \& Pratt, 2012), where
knowledge is transferred from earlier tasks (e.g. the discrimination
of easy examples) to later tasks (e.g. the discrimination of difficult
examples).


Continuation methods (smoothing)?

\section{transfer learning}
Summarize transfer learning.
normal training adjust net for each new example.
for an example the net is not blank, but initialized by the previous
training examples.
pre-training is that another batch of examples are used as
initializer, possibly per layer.

transfer learning is that another batch of examples is use for entire
net as inistializer

curriculum learning, is that examples are increasingly difficult

curriculum learning takes other examples (input to training)
transfer learning takes other weights (result of training)

while doing curriculum leanring, the intermediate results are used as
in transfer learning. It learns from different examples.
doing transfer learning thus needs different examples as input


pre-training.




\section{self play as curriculum learning}
Self play is curriculum. Self play is pre training. Self
play is transfer.

\section{transfer learning as general game playing}
But also: alphazero 3 games is transfer. And: it is
not. No transfer of learnd weights. Need more research there.  Net viz
to learn knowledge.




 



\section{Curriculum Learning}
\subsection{curriculum learning is...}
speed of curriculum learnign, speed of convergence, weinshall
theorectical result
CONVERGENCE RATE DECREASES WITH DIFFICULTY

empirical study

\subsection{beyond trial and error}
shaping is able to learn things that are beyond trial and error
(Krueger and Dayan)
 
\subsection{curriculum leanring  in supervised learning}

behgio: faster AND find better local minima


A theoretical motivation for deep architectures comes from complexity theory: some functions can be represented compactly with an ar- chitecture of depth k, but require an exponential size architecture when the depth is restricted to be less than k (Hastad \& Goldmann, 1991; Bengio, 2007). How- ever, training deep architectures involves a potentially intractable non-convex op- timization problem (Bengio, 2007), which complicates their analysis. There were no good algorithms for training fully-connected deep architectures before 2006, when Hinton et al. (2006) introduced a learning algorithm that greedily trains one layer at a time. 

\subsection{curriculum learning in slf play}
\subsection{curriculum learning as generalizaiton}
\subsection{curriculum learning as transfer leartinng}
bengio
staged learning

weinshall says curriculum learning is difficult to do in the real
world, since there is infrequently a teacher that ranks the examples
from easy to hard. until self-play.
amd because what a human finds hard, a machine learnign may not find
hard. Self-play, obvisoulys, does not have that probelem, and
automatically generates the right level of hardness for the learners.

never ending learning

\section{Transfer Learning}
relation of curriculum learning with transfer learning: transfer from
easy to har dacoorus in curriculum learning often. Curriculum learning
as generealized/iterated transfer learnign.
\subsection{all training is generalization}
transfer from one example to othe rexample

\subsection{transfer learning as different examples learning}
all learning is transfer learning, generealization to different
examples

\subsection{transfer learning as pre training}

\subsection{pretraining as curriciulum learning as transfer learning}  

curriculum lkearnig transfers knwoledg efrom teacher to student.




\section{Training}\label{sec:curr}\index{curriculum
learning}\index{transfer learning} 
The open questions of the previous chapter are concerned with the  efficiency of the
training process, and with generalization of training results
(transfer learning). We will first discuss the efficiency of the
training process.

%% \subsection{Learning Stability}
%% Issue: Stability: correlations
%% solution: replay buffers
%% self-play: with replay buffers seems solved
%% saturation does not seem to be caused by stability issues.

%% Previously, training reinforcement learning function approximators
%% required careful attention to stability, due to correlations between
%% subsequent states and target values. Replay buffers were introduced,
%% and actor critic networks, to achieve sufficiently stable
%% training. Training sets were large, to provide sufficient variation in
%% training examples, causing training times to be large.

%% Self play combines planning and learning. Examples are generated by a
%% planner (such as MCTS). This lookahead creates examples of higher quality and
%% greater independence, creating a more  diverse  and stable training
%% process.

%% The ``deadly triad'' of function approximation, bootstrapping and  off policy
%% learning did not occur in AlphaZero, or, if it did, it did not
%% preclude reaching a high level of play.

%% {\bf
%%   Did others encounter this in self play? other studies into learning stability of self play?}

%% well, bengio curriculum learning, epstein perfect teacher, tesauro add heuristics


%% It should be noted that no in depth study 
%% Stable learning? more efficient self play due to suitable opponent?
%%  Did self play kill the deadly triangle? Is learning stability no
%%  longer a problem? Is overfitting solved?

%% Is curriculum learning, learning by small steps, applicable to more
%% problems?

%% This remains very much an open question
 
\subsection{Training Efficiency}
\subsubsection{Curriculum Learning}
In the previous chapter we  saw  that supervised and
reinforcement learning can be slow when there is a large gap between
training targets and  the initial state of the approximator, as was
the case with AlphaGo. When errors are
large, convergence is slow.

Tabula rasa self-play creates a different convergence process. It has
the advantage that the  network outputs are not too far from the  
training examples. The errors on the output layer tend to be
small. The training targets are 
generated in lock step with the trainee, both trainer and trainee grow
in playing quality together. 

Thus each AlphaZero self-play training iteration converges  quicker then when large
steps must be taken as with AlphaGo data base learning. Indeed, this has been
observed in other works as 
well. It has been called curriculum
learning by Bengio et al.~\cite{bengio2009curriculum,matiisen2017teacher}, or
pre-training~\cite{erhan2010does}. Specifically, the pre-training has
been reported to guide the learning towards basins of attraction of
minima that support better generalization from the training data
set~\cite{erhan2010does,bengio2012practical}. Recently, Weinshall et
al.\ studied curriculum
learning in relation to transfer
learning~\cite{weinshall2018curriculum}. Curriculum learning is 
also important for life long learning, or never ending
learning~\cite{mitchell2018never}, and has been reported to be
necessary for other domains as well~\cite{zaremba2014learning,graves2017automated}.

Curriculum learning has not yet been studied extensively in the
context of self-play. There is room for future work on this topic.


\begin{figure}[ht]
    \centering{\includegraphics[width=6cm]{figures/slrl}
     \caption{Comparison of Supervised Learning and Self-play
     Reinforcement Learning}\label{fig:slrl11}}
\end{figure}

\subsubsection{Why is learning Levelling Off?}
Another important question  is why performance of self-play is levelling
off (see, for example, Figure~\ref{fig:slrl11}). A better understanding
of this question may yield ways to push this point  further off, just
like a better understanding of learning principles such as curriculum
learning allowed AlphaGo Zero to achieve  a higher level of play than
AlphaGo, as Figure~\ref{fig:slrl11} shows.

Perhaps the curve is levelling off because there is nothing left to
learn in $19\times 19$ Go? If this were true, then AlphaZero would
have found the global optimum, the ultimate Go wisdom. Although this
could conceivably be true, given the
complexity of the domain, it is more likely that the training has
gotten stuck in a local optimum. We can try to get out of the local
optimum by changing training parameters, by restarts, or
normalization.

%% If it is truly 
%% suspected that $19\times 19$ Go has been learnt to perfection, then
%% a different board size can be tried. On a larger board the level off
%% should not occur within a reasonable training time, and on a smaller
%% board it should happen sooner. 
%% unlikely, this question can be tested, for example by running the
%% program on different sized. If the program has learned all
%% there is to learn about $19\times 19$ Go, then on the larger boards it
%% should continue to learn as training time increases, and at the
%% smaller board it should start levelling off sooner, as th.

Perhaps the capacity of the network is too  small, and it is
underfitting? This can be tested by  increasing the
network size. The AlphaGo Zero paper describes a comparison
between 20 block and 40 block residual nets, finding the improvement
of the larger network to be
small~\cite{silver2017mastering}. If the smaller network had been
underfitting, then the larger network
would have performed significantly better.
Another solution is to change the network architecture in a more
fundamental way, by adding or removing layers of different types. 

Perhaps there is a more fundamental limit to what self play can teach
a neural net? This situation is described by Tesauro in his TD-gammon
papers. His single layer network did not learn more complicated
patterns, and he added a small amount of planning (a two level search) and
certain hand crafted heuristic knowledge, improving performance of the
program significantly~\cite{tesauro2002programming}.


Perhaps the self play training scheme should be improved. Already
Epstein~\cite{epstein1994toward,epstein1993toward} noted the importance of a good
trainer in self play, and has suggestions on how to avoid self play training
pathologies. Or perhaps the planner needs to improve as the level of
play increases, for example by increasing the number of MCTS
simulations, or changing the amount of explorarion that MCTS does.

Perhaps the local minima in the state space have become too hard to find? 
The question how to improve learning  further may well be the most
important question to ask in machine learning. There are still many
parameters and elements of the program left to explore and understand.
This remains very much an open question that will be actively
researched in the field.



\subsection{Learning Architecture}
\subsubsection{Hyperparameter Optimization}

Deep learning and self play systems have many hyper
parameters. AlphaGo Zero lists many (see
Table~\ref{tab:hyp}~\cite{silver2017mastering}).

\begin{table}[ht]
\begin{center}
\begin{tabular}{c|c}\hline\hline
{\bf hyper parameter} & {\bf value}\\ \hline\hline
self play games per iteration & 25000\\ \hline
MCTS simulations & 1600\\ \hline
exploration temperature & 1 for first 30 moves, 0
afterwards \\ \hline
Dirichlet noise & $\eta=0.03, \epsilon=0.25$ \\ \hline
resignation threshold & 5\%\\ \hline
regularization parameter & $c=10^{0.4}$\\ \hline
mini batch size & 2048, 32 per worker \\ \hline
self play positions & 500,000 \\ \hline
learning rate&annealed with momentum par 0.9\\ \hline
CE loss/MSE  weighting&  equal in the loss
function\\ \hline
optimization checkpoint & 1000\\ \hline
self play evaluator &  400\\ \hline
win margin for acceptance & 55\% \\ \hline
network architecture & 19 residual blocks\\ \hline \hline
\end{tabular}
\caption{AlphaGo Hyper Parameters~\cite{silver2017mastering}}\label{tab:hyp}
\end{center}
\end{table}

The effects of some of these hyperparameters interfere. A basic
premise of AI is
that some decision making tasks are best left to computers. This holds
also true
for hyper parameters. Finding the
optimal setting for all parameters is a daunting task, best left to
machine optimization.\footnote{just as finding the best coefficients for an
evaluation funciton of hand crafted heuristics is best left to machine
learning, and, for that matter, crafting the evaluation features
themselves  is also best left to machine learning, and crafting a database of
training positions is best left to self play. Some would even say that
crafting machine learning algorithms is best left to machine learning,
but that is a topic for another book.} Many optimization algorithms
have a large set of hyper parameters, and hyper parameter optimization
is an active field of research. Well known methods are exhaustive
search~\cite{hoos2004stochastic}, random search~\cite{bergstra2012random,wang2016bayesian},
Bayesian optimization~\cite{bergstra2011algorithms,hutter2011sequential,thornton2013auto,snoek2012practical}, gradient based methods (including neural
networks and SVM)~\cite{bergstra2011algorithms,chapelle2002choosing},
and evolutionary
optimization~\cite{back1993overview,burke2013hyper,pappa2014contrasting,van2015optimally}.
Some
software packages for hyperparameter optimization are
\href{https://github.com/automl/SMAC3}{SMAC}\footnote{\url{https://github.com/automl/SMAC3}}~\cite{hutter2011sequential},
\href{https://automl.github.io/auto-sklearn/stable/}{auto-sklearn}\footnote{\url{https://automl.github.io/auto-sklearn/stable/}}~\cite{feurer2015efficient},
\href{http://www.cs.ubc.ca/labs/beta/Projects/autoweka/}{Auto-WEKA}\footnote{\url{http://www.cs.ubc.ca/labs/beta/Projects/autoweka/}}~\cite{kotthoff2017auto},
\href{https://scikit-learn.org/stable/}{scikit-learn}\footnote{\url{https://scikit-learn.org/stable/}}~\cite{pedregosa2011scikit},
  \href{http://iridia.ulb.ac.be/irace/}{irace}\footnote{\url{http://iridia.ulb.ac.be/irace/}}~\cite{lopez2016irace}
  and
  \href{https://code.fb.com/ai-research/nevergrad/}{nevergrad}\footnote{\url{https://code.fb.com/ai-research/nevergrad/}}~\cite{nevergrad}.\index{nevergrad}\index{irace}\index{scikit-learn}\index{AutoML}\index{AutoWeka}\index{auto-sklearn}\index{SMAC}

AlphaGo Zero optimized its hyper parameters with Bayesian optimization,
AlphaZero used the same set of hyper parameters. 


\subsubsection{Network Architecture}
The  architecture of the network is
also a  hyper parameter to optimize. Among the decisions to make are
how many layers, of what type, and how many
neurons, also of what type, whether to have cells, and how they are
connected. Getting the architecture 
right for your problem can be a timeconsuming problem, perhaps also
best left to machine learning.

Network architecture optimization is an active field of research, and
can be based the same methods as for 
hyper parameter optimization. Random search, Bayesian
optimization~\cite{yoshinari2018probabilistic}, 
evolutionary
algorithms~\cite{kitano1990designing,van2018automatic,jaderberg2017population,miikkulainen2019evolving},
are popular methods, although reinforcement learning has also been
used~\cite{zoph2016neural,baker2016designing}. Two surveys
  are~\cite{yao1999evolving} and \cite{elsken2018neural}. A standard
  work on evolutionary strategies is B\"ack~\cite{back1996evolutionary}.

\subsubsection{Network Type}
In Chapter~\ref{chap:super} we saw an evolution of different network
types for image recognition, and in Chapter~\ref{chap:dqn} the same
occurred in  reinforcement learning. For AlphaGo Zero
Figure~\ref{fig:slrl} compared convolutional and residual nets. So
far, there is little other work reported that compares different
network types. A
complicating factor is that running self-play experiments is
computationally expensive. Running experiments to find out what type
of network and which
hyper parameters work best for a problem is currently  computationally
infeasible for large problems. 

\subsubsection{Network Optimization}
An important element of all neural network function approximators is
the optimization algorithm. Stochastic gradient descent has been the
optimization algorithm of
choice, although alternatives exist. Recently works
report on evolution
strategies~\cite{chrabaszcz2018back,salimans2017evolution,wierstra2008natural}. An
advantage of evolution strategies is that they are well suited for
parallelization, providing possible speedups for the training phases
of self-play.

%\subsubsection{Generalization in Reinforcement Learning}
%To improve performance several ideas to further develop reinforcement
%learning are being pursued.

%\subsubsection{hierarchical RL}
%\cite{barto2003recent}
%\cite{bakker2004hierarchical}
%\subsubsection{Meta learning}




\section{Transfer Learning: Generalization to other Problems}\index{transfer learning}
Self-play has shown promise by achieving  good training performance,
and by generalizing to other games. We will now turn to the
generalization question.

There are two kinds of generalization that we are interested in:
system generalization and transfer learning. In system
generalization the question is to build a system that can learn to
solve multiple problems. This is the kind of generalization that GGP
seeks to achieve. AlphaZero succeeded in this aspect for three
board games. Algorithms, network architecture and hyperparameters generalized to three
games, although it needed hand crafted input and output
layers, and, significantly, the network had to be retrained from
scratch for each game. The trained nets do not generalize accross
games.
% Extending system generalization tries to extend this to more
% and different kinds of problems.

The goal of transfer learning is to learn knowledge in one domain and
apply it in a different domain, including the trained net. Transfer
learning  tries to
transfer knowledge that is learned in one domain to solve problems in
another domain, without
retraining~\cite{pratt1993discriminability,thrun2012learning}. Surveys
on transfer learning are~\cite{taylor2009transfer,pan2010survey}.

Before we look at how to apply self-play in different domains, we
will now look briefly into how we can learn which knowledge has been
learned by the net.

\subsection{Visualizing Neural Net Weights}\label{sec:zflayers}
Deep networks can be used for feature learning, or
representation learning. The layers learn concepts of increasing
generality~\cite{bengio2013representation,lecun2015deep}, creating a
hierarchy of concepts. How general are the concepts learned by self-play?
What do they ``look'' like, can they be represented as a two
dimensional picture for us to interpret?

Montavon et al.~\cite{montavon2018methods} provides an tutorial of
methods for interpreting deep nets.
Zeiler and Fergus ZF paper~\cite{zeiler2014visualizing} gives
insightful pictures of the different layers (one of which is
reproduced in Figure~\ref{fig:zfnetlayers11}). They developed a
visualization technique to interpret the layers of a CNN.
Noh et al.~\cite{noh2015learning} use deconvolution for semantic segmentation.


\begin{figure}[t]
    \centering{\includegraphics[width=10cm]{figures/zfnetlayers}
     \caption{ZFnet layers\cite{zeiler2014visualizing}}\label{fig:zfnetlayers11}}
\end{figure}

During supervised learning the accumulating knowledge is refined with
each training epoch and is generalized in the deep layer. In
self-play, there is an extra dimension, in addition to epoch and
layer. In 
each self-play iteration the level of difficulty of the concepts learned
increases. AlphaGo Zero's joseki picture illustrates well
how over time the self players learned each other more advanced concepts  (see Figure~\ref{fig:joseki11}).
Table~\ref{tab:concepts11} summarizes the three kinds of self play learning.
  
\begin{figure}[ht]
    \centering{\includegraphics[width=13cm]{figures/joseki}
     \caption{AlphaGo Zero is Learning Joseki~\cite{silver2017mastering}}\label{fig:joseki11}}
\end{figure}

\begin{table}
  \centering{
    \begin{tabular}{c|c|c}
      {\bf supervised} & {\bf self-play} & {\bf learn}\\ \hline
      epoch & epoch & optimize  error\\ \hline
      layer & layer & generalize concept \\ \hline
      -     & iteration & playing strength
    \end{tabular}
    \caption{Three Kinds of Learning in Supervised and Self
      Play}\label{tab:concepts11}
  }
\end{table}

Self-play has a long history in research, starting with Samuel's
Checkers player. The recent breakthrough by
AlphaGo Zero, and the subsequent reimplentations (A0G, Elf OpenGo,
PhoenixGo and Leela) will stimulate research in this area.
Future work should find other insightful ways to visualize knowledge accumulation.



\subsubsection{Recent Self-Play Work}
Much work in reinforcement learning is on ``flat'' DQN, on learning
without planning. Not all reinforcement
learning can be folded into a deep function approximator. For
self-play a planning component is 
convenient to generate the training targets. The use of exact methods
will also depend on the dimensionality of the problem. For 
high dimensional problems approximation is a necessity, but for low
dimensional problems exact methods will yield better answers. 


There are, however, recent works on self-play that explore the idea
further. Sodhani and Pahuja~\cite{sodhani2018memory} augment self-play
with memory resulting in faster exploration of the environment.
Charlesworth~\cite{charlesworth2018application} applies self-play in a
multi-player game of imperfect information.
Sukhbaatar et al.~\cite{sukhbaatar2018learning} experimemt with
self-play in hierarchical reinforcement learning to automatically
learn sub-goals. Previously, they studied intrinsic
motivation and curriculm learning through
self-play~\cite{sukhbaatar2017intrinsic}.
Zhao et al.~\cite{zhaotraining} study self-play in modern games.

\section{Practice}
\subsubsection{Exercises}
A0G:
\begin{enumerate}
\item Play with tensorboard to look inside the brain/training process and understand training process
\item Do of hyper parameter tuning of A0G
\item Play with different net architectures
\item Can single agent optimization problems benefit from self-play?
Implement the 15 Puzzle in A0G. And travelling salesperson.
\item See if transfer learning of 4x4 Othello, to 6x6 to 8x8 works, and
works faster. Are we seeing  curriciulum learning?
\end{enumerate}

\section{Summary}
{\bf central concept: learning generalization: hyper par optim,
network arch; transfer/generalization to other problems: hier rl, imperfect info}
\begin{itemize}
\item learning process improvements. deadly triad?
\item generalization to other problems
\end{itemize}
This is still an active field of research. Improving performance of
the learning process through automation with optimization
methods. Visualizing knowledge, generalizing it to other domains. 

\section*{Historical and Bibliographical Notes}
Hyperparameter
optimization~\cite{bergstra2011algorithms,hutter2011sequential}.

Evolutionary Strategies the reference is~\cite{back1993overview}.

Curriculum learning~\cite{bengio2009curriculum,matiisen2017teacher}.

For GGP go to~\cite{genesereth2005general}.

Readable and insightful introduction into the field of Abstraction in
deep representation learning are~\cite{bengio2013representation,lecun2015deep}.

For Network visualization start with the ZFnet paper
insight~\cite{zeiler2014visualizing}.

Poker~\cite{bowling2015heads}
\cite{moravvcik2017deepstack}
\cite{brown2018superhuman}




==> chapters/old2-02games.tex <==
%% 2: games
%% section: behaviorist view of intelligence: memory, reasoning, and learning. turing test
%% section: games in ai: drosophila: simpler reality, strict rules
%% section: history checkers, chess (turing, russians, deep blue-kasparav)
%% section: lookahead: search-eval architecture
%% section: example: 9x9 go in python, or hex or ttt

%FIRST WRITE TOP DOWN STRUCTURE

%add words to the sections $\rightarrow$ make subsections

%Landmarks

%Methods

The topic of this chapter is to introduce the behavioristic approach to
intelligence, and further narrow the scope of the study of artificial
intelligence to games: domains  with clear and well defined rules, yet
providing exciting challenges to human intelligence, to be precise, board games such
as Chess, Checkers, and Go. We will provide a short historic overview
of early work in these fields.

We will learn about the age old dream
of mechanical intelligence, and the first attempts by the pioneers of
computer science to make intelligent apparatuses. And, surprisingly,
the earliest approaches of Shannon and Turing can still be traced in
the architecture of today's AlphaGos.
\section*{Learning Goals}
\begin{itemize}
  \item intelligent behavior and games
  \item history of games
\end{itemize}


\section{AI and Strategic Reasoning}
What is intelligence? Intelligence implies reasoning, memory, learning,
problem solving skills, emotion, adaptivity, and creativity. But,
human intelligence is also embodied, humans are conscious,
self-aware.  The former is about {\em
acting\/} intelligent. The latter list is about {\em being\/}
intelligent.

We will now discuss these aspects in more depth.

\subsection{Cognition}
Cognitive aspects of intelligence include logical reasoning, planning,
problem solving, learning, creativity, understanding, self-awareness, and
emotional knowledge~\cite{kahneman2011thinking}

Intelligence gives us the cognitive abilities to learn, form
concepts, and reason. These abilities allow us to recognize patterns, comprehend
ideas, plan, solve problems, and use language to
communicate. They enables humans to experience and think.

These last two elements bring us closer to the point that human
intelligence is embodied intelligence.

\subsection{Embodied vs. Computational, Connectionist vs. Symbolic}
Embodied intelligence stresses our ability to {\em perceive\/} information,
to use it as knowledge in adaptive behaviors within an environment, in
an embodied sense~\cite{francisco1991embodied}.


The embodied mind thesis challenges other theories, such as
computationalism, which states that
thoughts are a form of computation of a set of laws for the relations
among representations.

This discussion in psychology has also occurred in AI. Symbolic AI
stressed the importance of logic reasoning, and assumes that
knowledge is grounded in symbols. On the other side,
connectionism and robotics are biologically inspired and regard
intelligence as emerging bottom up from interaction of artifacts with an
environment~\cite{nilsson2009quest,stone2016artificial}.

Interestingly, the work in this book draws on both streams of
thought. Reinforcement learning draws on the idea of learning through interaction with
the environment, and neural nets are inspired by
connectionism. Planning, and heuristic search, on the other hand, are
from the logic reasoning side of AI. In self play, symbolic and
connectionist, reasoning and reinforcement, come together.


\subsection{History of AI}
It appears the concept of artificial intelligence is as old as human
thought. The first recorded dreams of intelligent machines  go back to Indian
philosophies 1500 BC~\cite{mccorduck2009machines}. 

By attempting to describe human thought as the mechanical manipulation
of symbols classical philosophers were th first to described= ideas of
{\em modern\/} AI. This work on mathematicsal reasoning culminated in
the invention of the 
 digital computer in the 1940s. The advent of the first computers  and the ideas
behind it prompted  scientists to start serious
discussions on the possibility of creating an electronic brain. 

The field of AI research was subsequently founded in the summer of 1956 at a
workshop at Dartmouth College. Among those present were John McCarthy, Marvin
Minsky, Nathaniel Rochester, Claude Shannon, Allen Newell, Herbert
Simon, Arthur Samuel, John Nash, Warren McCulloch, who would all
become  leaders of AI research for decades. There
was  much optimism then,  and many predicted that human level  machine
intelligence would exist within 20
years~\cite{moor2006dartmouth,mccorduck2009machines}.  
Eventually it became clear that they had  underestimated the
difficulty of this project, although many unexpected  results did
happen, such as search engines, social networks, and recommender
systems.

Interest in AI has been high  again after 2000, because of
machine learning successes in vision, speech, robotics and other applications in
academia and industry.

\subsection{Turing Test and General Intelligence}
Most AI researchers are interested in  intelligent behavior,  machines that
           exhibit  reasoning, knowledge, planning, learning,
           communication, perception, and the ability to interact with
           the physical environment. By which methods the machines
           exhibit this behavior is irrelevant. Consciousness and self-awareness
           are not on the agenda, and simulating the brain is not necessary.

\subsubsection{Behavior: Turing Test}
In 1950 Alan Turing proposed a test on how to determine if a machine
exhibits  intelligence. The machine passes the test when its behavior
is indistinguishable from that of a human. In the Turing test a human
evaluator judges a natural language conversation between a human
and a machine. The evaluator
is aware that one of the two participants  is a
machine, and both participants are separated from one another by a
screen.
Participants are restricted to a text-only,  such as through
keyboard and screen. (Natural language technology is deemed too hard.)
If the evaluator cannot  tell which conversation is from the machine,
the machine is considered to have passed the test. Note that the test
results do not always have to be correct, only how closely the answers
resemble those a human would give counts. It might even be the case
that making deliberate mistakes is a good idea, for example, when the
domain would be a game of Chess, then a Chess machine could be
identified by being much stronger than a human would be.

The paper introducing the Turing test was titled: ``Computing
Machinery and Intelligence.''  It opens with the words: ``I
propose to consider the question, 'Can machines
think?`''~\cite{turing1950computing}.   


           
\subsubsection{Special and General Intelligence}
Machines that are intelligent in a single domain, such as Chess, are
said to have specific or {\em special\/} intellligence. Artificial
{\em general\/} intelligence (AGI) woudl be the intelligence of a machine
that can  perform any intellectual task that a human can. AGI is the
holy grail of  AI research, and favorite  topic in science fiction and future
studies. AGI is sometimes called {\em strong AI\/} although that term
is used by some researchers to mean machines that experience
consciousness~\cite{searle2008mind}.  

As of 2017, over forty organizations worldwide are doing active
research on AGI~\cite{baum2017survey}.


\subsubsection{Limited Scope}
General intelligence is clearly a challenging goal. Although ultimately intelligent behavior has to be measured in real world
settings, the real world, however, is complex, and quite
a challenge to master. It is better to start with a model that
captures an essential and interesting aspect of reality, but is otherwise
simpler. For this reason, ever since the start of AI, games have played an important
role. The rules of the game limit its scope, making it much more
suited as a first object of study than the full complexity of reality.

\subsubsection{Drosophila Melanogaster}
 In 1965, the Soviet mathematician Aleksandr Kronrod called chess the
Drosophila Melanogaster of Artificial Intelligence~\cite{landis2001aleksandr},
see Fig.~\ref{fig:drosophila}. Drosophila Melanogaster, a type of
fruit fly, has been used by developmental biologists in genetics
experiments, because of it fast procreation cycle. Researchers could see quickly results of their
experiments.
\index{Drosophila Melanogaster}

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/drosophila.jpg}
\caption{Drosophila Melanogaster (fruit fly)}\label{fig:drosophila}
\end{center}
\end{figure}

Such an experimenter's favorite experimental tool with quick
turnaround times is  useful in AI research. Chess, the game
of intelligence par excellence, was a convenient domain
that was well suited for such experimentation. It is clearly a game of
intelligence, requiring many years of  dedication and study to achieve
proficiency.




\subsubsection{Clear Rules}
In addition to a limited scope, a second advantage of games is the
clarity of the rules. Games have a clear goal, and the possible
actions are well defined by the rules. In this, games differ from the
real world, where goals and rules are often implicit and vague. Thus, games are
easier to solve than many real world tasks, a clear advantage for
researchers.

\subsubsection{Clear Performance}
Games also allow for a clear and undisputed way to measure
progress. Game rules
define win and loss, and the intelligence of programs can be measured by
letting them play against eachother or against humans. Many types of games have
rating systems, such as in tennis, where the best of the world are
ranked based on how many wins have been scored against other
players. An often used measure is the  Elo-rating,
a system devised by the Hungarian-American physicist  Arpad Elo. The
basis of the Elo rating is pairwise comparison \cite{elo1978rating}.

\subsubsection{Special Intelligence}
In  the original Turing test {\em any\/} question
can be asked of the machine. It is a  test for General
Intelligence, the same kind of intelligence that humans have. Limiting
the scope of our domain to a single game clearly cannot be used to
achieve to pass the general Turing test, all we can hope is to achieve special
intelligence, the kind of intelligence needed to win a certain
game. Still, achievements in special intelligence, such as by Deep
Blue, Watson and AlphaGo, attract large publicity. This may be in part
because the human mind generalizes easily, and
anthropomorphizes\footnote{I.e., treat as if human.}
easily. When we see a device do something in a particular domain for
which a human must be incredibly smart, we automatically assume that the device
must {\em be\/} smart, and will do  as well in another domain {\em
because that is what a human would do}. It is easy to let us forget that a machine is
not a human, something that writers of science fiction books and Hollywood movies eagerly exploit. Machine intelligence is highly specialized, and this is
quite unhuman-like. 

Indeed, one of the great challenges of AI is to create a machine that
has general  intelligence, or at least in AIs that are
intelligent in more than one domain.
The field of transfer learning studies how knowledge that is learned
in one domain can be transfered to another
domain. Chapter~\ref{chap:transfer} discusses transfer learning.


Games are a suitable testbed for AI
experimentation~\cite{mandziuk2007computational}. The first 
game to be heavily studied was Chess,  the game of
intelligence par excellence. For this reason Kronrod named Chess the
Drosophila Melanogaster, or experimental testbed of choice, of AI. And
indeed, for many decades many researchers used it to their advantage,
developing many ingenious computational methods to
achieve a level of play, ultimately beating the strongest human minds
in the world.

Indeed, dedicated research groups  all over the world worked in Chess,
creating quick
progress. In just three decades the dream of beating the human world
champion was realized. On May 11, 1997 Garry Kasparov, then the highest
rated human chess player ever, was defeated by the computer
program \textsc{Deep Blue}, in a highly publicized six game match in
New York~\cite{hsu2004behind,schaeffer1997kasparov}.  


\section{A Short History of Computer Games}
Then, a new Drosophila had to be found, which would become Go.

But we are getting ahead of ourselves. In order to get a good
understanding of the field, let us start with a short overview of some
of the better known games in the history of AI. We will start with two
paper designs, and then continue with the first real game playing programs.


\subsection{Claude Shannon}
Claude Elwood Shannon (1916–2001) was an American mathematician,
electrical engineer, and cryptographer. Shannon is primarily known as
``the father of information theory.''  

In 1949 Shannon presented a paper titled ``Programming a Computer for
playing Chess.'' The paper describes a design for how to program a
computer to play chess based 
on position evaluation and move selection. The paper describes  strategies
for restricting the number of possibilities to be
considered. Shannon's paper is  one of the first articles
published on the topic of 
programming a computer to play chess~\cite{shannon1988programming}. 



\subsection{Alan Turing}
In 1948 Alan Turing (1912-1954) worked with David Champernowne on writing a chess
program for a computer that did not yet exist. They named their
program Turbochamp. In 1950, the program was finished. In 1952, Turing
tried to implement it on a Ferranti Mark 1, but the computer was
unable to execute the program. Turing wanted to play a game, so he
executed the program by hand, flipping through the pages of the
algorithm and carrying out its instructions on a 
chessboard. This took about half an hour per move.
The program is the first full Chess program, even though it was
executed on paper~\cite{turing1953digital}. Turbochamp had an
evaluation function and a search function, a design that is still used
by today's programs.


\begin{figure}[t]
\begin{center}
\includegraphics[width=3cm]{figures/turing}
\caption{Alan Turing}\label{fig:turing}
\end{center}
\end{figure}
\index{Alan Turing}

\subsection{Christopher Strachey}
Christopher Strachey (1916-1975) was a preeminent computer scientist
at Oxford, well known
for his work on denotational semantics and programming language
design. In 1951, Christopher Strachey wrote a Checkers program for the
Ferranti Mark 1 computer of the University of 
Manchester. It could play a complete game of Draughts (Checkers) at
reasonable speed~\cite{strachey1952logical}.

\subsection{Arthur Samuel}
Arthur Samuel (1901-1990) startd in 1949 to write a Checkers program
for the IBM 701 computer. It was among the world's first successful
self-learning programs, adapting weights in the evaluation function
based on the outcome of the search~\cite{samuel1959some}. 

The main driver of the program was a
search tree of the board positions reachable from the current
state. To reduce memory consumption Samuel implemented a version of what is now called alpha-beta pruning.
He used a heuristic evaluation function based on the position of the
board to prevent having to search to the end of the game. He also used
a method to memorize search results, and later versions used
supervised learning from professional games and from self play. Around
the 1970s the program had progressed to amateur level~\cite{schaeffer2008one}.




\subsection{TD-Gammon}
{\bf why? first world class level games program. self play
  reinforcement learning eval. neural net, mostly eval. Inspiration
  for the moderns: Atari and AlphaGo}
  
1992 TD Gammon \cite{tesauro2002programming} Tesauro. A
reimplementation in Tensorflow is at
\href{https://github.com/fomorians/td-gammon}{TD-gammon}.

TD-Gammon, a backgammon program written by Gerry Tesauro, demonstrates
that reinforcement (learning) is powerful enough to create a
championship-level game-playing program by competing favorably with
world-class players.

During play, TD-Gammon examines on each turn all possible legal moves
and all their possible responses (two-ply look-ahead), feeds each
resulting board position into its evaluation function, and chooses the
move that leads to the board position that got the highest score. In
this respect, TD-Gammon is no different than almost any other computer
board-game program. TD-Gammon's innovation was in how it learned its
evaluation function. 

TD-Gammon's learning algorithm consists of updating the weights in its
neural net after each turn to reduce the difference between its
evaluation of previous turns' board positions and its evaluation of
the present turn's board position—hence "temporal-difference
learning". The score of any board position is a set of four numbers
reflecting the program's estimate of the likelihood of each possible
game result: White wins normally, Black wins normally, White wins a
gammon, Black wins a gammon. For the final board position of the game,
the algorithm compares with the actual result of the game rather than
its own evaluation of the board position.[1] 

Unlike previous neural-net backgammon programs such as Neurogammon
(also written by Tesauro), where an expert trained the program by
supplying the "correct" evaluation of each position, TD-Gammon was at
first programmed "knowledge-free".[1] In early experimentation, using
only a raw board encoding with no human-designed features, TD-Gammon
reached a level of play comparable to Neurogammon: that of an
intermediate-level human backgammon player. 

Even though TD-Gammon discovered insightful features on its own,
Tesauro wondered if its play could be improved by using hand-designed
features like Neurogammon's. Indeed, the self-training TD-Gammon with
expert-designed features soon surpassed all previous computer
backgammon programs. It stopped improving after about 1,500,000 games
(self-play) using 80 hidden units.[2]

Backgammon expert Kit Woolsey found that TD-Gammon's positional
judgement, especially its weighing of risk against safety, was
superior to his own or any human's.[1] 

TD-Gammon's excellent positional play was undercut by occasional poor
endgame play. The endgame requires a more analytical approach,
sometimes with extensive lookahead. TD-Gammon's limitation to two-ply
lookahead put a ceiling on what it could achieve in this part of the
game. TD-Gammon's strengths and weaknesses were the opposite of
symbolic artificial intelligence programs and most computer software
in general: it was good at matters that require an intuitive "feel"
but bad at systematic analysis.


\subsection{Schaeffer Checkers 1994}
{\bf why? first world champion program. Also: first solved game (after
TTT (picture), nine Men's Morris (picture), Connect4 (picture), etc)}
           
\cite{schaeffer1992world,schaeffer1996chinook}
\index{Chinook}
\index{Checkers}
\index{Tinsley}
English draughts (checkers) world champion Tinsley resigned a match
against computer program Chinook. Chinook defeated 2nd highest rated
player, Lafferty. Chinook won the USA National Tournament by the
widest margin ever. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/checkers}
\caption{Checkers}\label{fig:checkers}
\end{center}
\end{figure}
\cite{schaeffer2008one}
Chinook is the first computer program to win the world champion title
in a competition against humans. In 1990 it won the right to play in
the human World Championship by being second to Marion Tinsley in the
US Nationals. At first the American Checkers Federation and English
Draughts Association were against the participation of a computer in a
human championship. When Tinsley resigned his title in protest, the
ACF and EDA created the new title Man vs. Machine World Championship,
and competition proceeded. Tinsley won with four wins to Chinook's
two, with 33 draws. 

In a rematch, Chinook was declared the Man-Machine World Champion in
checkers in 1994 in a match against Marion Tinsley after six drawn
games, and Tinsley's withdrawal due to pancreatic cancer. While
Chinook became the world champion, it never defeated the best checkers
player of all time, Tinsley, who was significantly superior to even
his closest peer.[1] 

In 1995, Chinook defended its man-machine title against Don Lafferty
in a 32-game match. The final score was 1–0 with 31 draws for Chinook
over Lafferty.[2] After the match, Jonathan Schaeffer decided not to
let Chinook compete any more, but instead try to solve checkers. At
the time it was rated at 2814 Elo. The solution was achieved, and the
result published in 2007.[3]

Chinook's program algorithm includes an opening book, a library of
opening moves from games played by grandmasters; a deep search
algorithm; a good move evaluation function; and an end-game database
for all positions with eight pieces or fewer. The linear handcrafted
evaluation function considers several features of the game board,
including piece count, kings count, trapped kings, turn, runaway
checkers (unimpeded path to be kinged) and other minor factors. All of
Chinook's knowledge was programmed by its creators, rather than
learned with artificial intelligence. 

\subsection{Deep Blue Kasparov 1996/1997}\label{sec:deepblue}
{\bf why? first world champion chess program, the Drosophila. classic search
  eval, purely heuristic. excellent example of the field ``heuristic
  search''. Very high profile, impact in public perception of humans
  as the sole proprietors of intelligence on the planet. Now
  superseded by open source program Stockfish.}

\index{Deep Blue}
\index{Kasparov}
\index{Chess}
In 1996 IBM Sponsored the first match between the human world Chess
champion Garry Kasparov and IBM's Chess supercomputer Deep
Blue at the ACM Compuing Conference in Philidelphia. Kasparov won the match ...
A year later, in May 1997, the rematch was played in New
York. Kasparov was defeated in a highly publicized match. Several
accounts of the match, its historical significance, and the technology
have been
written~\cite{schaeffer1997kasparov,campbell2002deep,hsu1990grandmaster,hsu2004behind,levy1991computers}. 

Reference on how computers play chess is \cite{levy1991computers}.

The Deep Blue chess machine (IBM) defeats the (then) world chess
champion, Garry Kasparov.

Deep Blue was a chess-playing computer developed by IBM. It is known
for being the first computer chess-playing system to win both a chess
game and a chess match against a reigning world champion under regular
time controls. 

Deep Blue won its first game against a world champion on 10 February
1996, when it defeated Garry Kasparov in game one of a six-game
match. However, Kasparov won three and drew two of the following five
games, defeating Deep Blue by a score of 4–2. Deep Blue was then
heavily upgraded, and played Kasparov again in May 1997.[1] Deep Blue
won game six, therefore winning the six-game rematch 3½–2½ and
becoming the first computer system to defeat a reigning world champion
in a match under standard chess tournament time controls.[2] Kasparov
accused IBM of cheating[3] and demanded a rematch. IBM refused and
retired Deep Blue. 

Development for Deep Blue began in 1985 with the ChipTest project at
Carnegie Mellon University. This project eventually evolved into Deep
Thought, at which point the development team was hired by IBM.[4] The
project evolved once more with the new name Deep Blue in
1989. Grandmaster Joel Benjamin was also part of the development team.

The project was started as ChipTest at Carnegie Mellon University by
Feng-hsiung Hsu, followed by its successor, Deep Thought. After their
graduation from Carnegie Mellon, Hsu, Thomas Anantharaman, and Murray
Campbell from the Deep Thought team were hired by IBM Research to
continue their quest to build a chess machine that could defeat the
world champion.[5] Hsu and Campbell joined IBM in autumn 1989, with
Anantharaman following later.[6] Anantharaman subsequently left IBM
for Wall Street and Arthur Joseph Hoane joined the team to perform
programming tasks.[7] Jerry Brody, a long-time employee of IBM
Research, was recruited for the team in 1990.[8] The team was managed
first by Randy Moulic, followed by Chung-Jen (C J) Tan.[9] 

After Deep Thought's 1989 match against Kasparov, IBM held a contest
to rename the chess machine and it became "Deep Blue", a play on IBM's
nickname, "Big Blue".[10] After a scaled-down version of Deep Blue,
Deep Blue Jr., played Grandmaster Joel Benjamin, Hsu and Campbell
decided that Benjamin was the expert they were looking for to develop
Deep Blue's opening book, and Benjamin was signed by IBM Research to
assist with the preparations for Deep Blue's matches against Garry
Kasparov.[11] 

In 1995 "Deep Blue prototype" (actually Deep Thought II, renamed for
PR reasons) played in the 8th World Computer Chess Championship. Deep
Blue prototype played the computer program Wchess to a draw while
Wchess was running on a personal computer. In round 5 Deep Blue
prototype had the white pieces and lost to the computer program Fritz
3 in 39 moves while Fritz was running on an Intel Pentium 90 MHz
personal computer. In the end of the championship Deep Blue prototype
was tied for second place with the computer program Junior while
Junior was running on a personal computer.[12] 

Design[edit]
Deep Blue employed custom VLSI chips to execute the alpha-beta search
algorithm in parallel,[13] an example of GOFAI (Good Old-Fashioned
Artificial Intelligence) rather than of deep learning which would come
a decade later. It was a brute force approach, and one of its
developers even disclaimed that it was artificial intelligence at
all.[14]

Deep Blue, with its capability of evaluating 200 million positions per
second, was the fastest computer to face a world chess
champion. Today, in computer chess research and matches of world class
players against computers, the focus of play has often shifted to
software chess programs, rather than using dedicated chess
hardware. Modern chess programs like Houdini, Rybka, Deep Fritz or
Deep Junior are more efficient than the programs during Deep Blue's
era. In a November 2006 match between Deep Fritz and world chess
champion Vladimir Kramnik, the program ran on a computer system
containing a dual-core Intel Xeon 5160 CPU, capable of evaluating only
8 million positions per second, but searching to an average depth of
17 to 18 plies in the middlegame thanks to heuristics; it won
4–2.[30][31] 

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/chess}
\caption{Chess}\label{fig:chess}
\end{center}
\end{figure}
\cite{campbell2002deep,hsu2004behind}

\subsubsection{Impact of Deep Blue Win}
how chess is now learned
Watson, medical diagnoses.

Deep Blue and Kasparov played each other on two occasions. The first
match began on 10 February 1996, in which Deep Blue became the first
machine to win a chess game against a reigning world champion (Garry
Kasparov) under regular time controls. However, Kasparov won three and
drew two of the following five games, beating Deep Blue by a score of
4–2 (wins count 1 point, draws count ½ point). The match concluded on
17 February 1996. 

Deep Blue was then heavily upgraded (unofficially nicknamed "Deeper
Blue")[15] and played Kasparov again in May 1997, winning the six-game
rematch 3½–2½, ending on 11 May. Deep Blue won the deciding game six
after Kasparov made a mistake in the opening, becoming the first
computer system to defeat a reigning world champion in a match under
standard chess tournament time controls. 

The system derived its playing strength mainly from brute force
computing power. It was a massively parallel, RS/6000 SP Thin
P2SC-based system with 30 nodes, with each node containing a 120 MHz
P2SC microprocessor, enhanced with 480 special purpose VLSI chess
chips. Its chess playing program was written in C and ran under the
AIX operating system. It was capable of evaluating 200 million
positions per second, twice as fast as the 1996 version. In June 1997,
Deep Blue was the 259th most powerful supercomputer according to the
TOP500 list, achieving 11.38 GFLOPS on the High-Performance LINPACK
benchmark.[16] 

The Deep Blue chess computer that defeated Kasparov in 1997 would
typically search to a depth of between six and eight moves to a
maximum of twenty or even more moves in some situations.[17] David
Levy and Monty Newborn estimate that one additional ply (half-move)
increases the playing strength 50 to 70 Elo points.[18] 


Kasparov in 1985
Deep Blue's evaluation function was initially written in a generalized
form, with many to-be-determined parameters (e.g. how important is a
safe king position compared to a space advantage in the center,
etc.). The optimal values for these parameters were then determined by
the system itself, by analyzing thousands of master games. The
evaluation function had been split into 8,000 parts, many of them
designed for special positions. In the opening book there were over
4,000 positions and 700,000 grandmaster games. The endgame database
contained many six piece endgames and five or fewer piece
positions. Before the second match, the chess knowledge of the program
was fine tuned by grandmaster Joel Benjamin. The opening library was
provided by grandmasters Miguel Illescas, John Fedorowicz, and Nick de
Firmian.[19] When Kasparov requested that he be allowed to study other
games that Deep Blue had played so as to better understand his
opponent, IBM refused. However, Kasparov did study many popular PC
games to become familiar with computer game play in general.[citation
  needed] 

Writer Nate Silver suggests that a bug in Deep Blue's software led to
a seemingly random move (the 44th in the first game of the second
match) which Kasparov misattributed to "superior
intelligence".[20][21] Subsequently, Kasparov experienced a drop in
performance due to anxiety in the following game.[21] Kasparov rejects
this interpretation.[22] 

Computer scientists believed that playing chess was a good measurement
for the effectiveness of artificial intelligence, and by beating a
world champion chess player, IBM showed that they had made significant
progress.[23] 

After the loss, Kasparov said that he sometimes saw deep intelligence
and creativity in the machine's moves, suggesting that during the
second game, human chess players had intervened on behalf of the
machine, which would be a violation of the rules. IBM denied that it
cheated, saying the only human intervention occurred between
games. The rules provided for the developers to modify the program
between games, an opportunity they said they used to shore up
weaknesses in the computer's play that were revealed during the course
of the match. Kasparov requested printouts of the machine's log files
but IBM refused, although the company later published the logs on the
Internet.[24] Kasparov demanded a rematch, but IBM refused and
dismantled Deep Blue.[25] Owing to an insufficient sample of games
between Deep Blue and officially rated chess players, a chess rating
for Deep Blue was not established.[citation needed] 

In 2003 a documentary film was made that explored these
claims. Entitled Game Over: Kasparov and the Machine, the film
interviewed some people who suggest that Deep Blue's victory was a
ploy by IBM to boost its stock value.[25] 

One of the cultural impacts of Deep Blue was the creation of a new
game called Arimaa designed to be much more difficult for computers
than chess.[26] 

One of the two racks that made up Deep Blue is on display at the
National Museum of American History in their exhibit about the
Information Age;[citation needed] the other rack appears at the
Computer History Museum in the "Artificial Intelligence and Robotics"
gallery of the Revolution exhibit.[27] Reports that Deep Blue was sold
to United Airlines appear to originate from confusion between Deep
Blue itself and other RS6000/SP2 systems.[28] 

\index{Stockfish}
Stockfish current best chess program. See Github
\href{https://github.com/official-stockfish/Stockfish}{Stockfish}.

\subsection{Logistello}
\index{Logistello}\index{Othello}
\cite{buro1997othello,buro1995logistello,buro2003evolution}
{\bf why? use of statistical pattern learning}

Computer Othello program Logistello defeated the world champion
Takeshi Murakami with a score of 6–0. 


Logistello is a computer program that plays the game Othello, also
known as Reversi. Logistello was written by Michael Buro and is
regarded as a strong player, having beaten the human world champion
Takeshi Murakami six games to none in 1997 — the best Othello programs
are now much stronger than any human player. Logistello's evaluation
function is based on disc patterns and features over a million
numerical parameters which were tuned using linear regression. 
\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/othello}
\caption{Othello}\label{fig:othello}
\end{center}
\end{figure}

\subsection{General Game Playing}
GGP
\cite{pell1996strategic,genesereth2005general,thielscher2009answer,schiffel2007fluxplayer,thielscher2010general,thielscher2011general,schofield2012hyperplay,michulke2009neural,schofield2015lifting,finnsson2010learning,bjornsson2009cadiaplayer,sironi2016comparison,sironi2017line,wang2018search}
{\bf why? new claim for Drosophila (less visible, mainstream
  Drosophila is Go). Highly ambitious aim to develop technology toward AGI in gaming}


General game playing (GGP) is the design of artificial intelligence
programs to be able to play more than one game successfully.[1] For
many games like chess, computers are programmed to play these games
using a specially designed algorithm, which cannot be transferred to
another context. For example, a chess-playing computer program cannot
play checkers. A general game playing system, if well designed, would
be able to help in other areas, such as in providing intelligence for
search and rescue missions.

There are other general game playing systems, which use their own
languages for defining the game rules. In 1992, Barney Pell defined
the concept of Meta-Game Playing, and developed the "MetaGame"
system. This was the first program to automatically generate game
rules of chess-like games, and one of the earliest programs to use
automated game generation. Pell then developed the system
Metagamer.[8] This system was able to play a number of chess-like
games, given game rules definition in a special language called Game
Description Language, without any human interaction once the games
were generated.[9] 

\subsection{Poker}
{\bf why? world class imperfect information program. Mention both UofA
  Hyperborean, Polaris
and CMU Libratus}

Poker AI Libratus individually defeated each of its 4 human
opponents—among the best players in the world—at an exceptionally high
aggregated winrate, over a statistically significant sample.[58] In
contrast to Chess and Go, Poker is an imperfect information game.[59]

bowling

Poker is a game of imperfect information (because some cards in play
are concealed) thus making it difficult for anyone (including a
computer) to deduce the final outcome of the hand. Because of this
lack of information, the computer's programmers have to implement
systems based on the Bayes theorem, Nash equilibrium, Monte Carlo
simulation or neural networks, all of which are imperfect techniques. 

AIs like PokerSnowie and Claudico have been created by allowing the
computer to determine the best possible strategy by letting it play
itself an enormous number of times. This seems to be the current
approach to poker AI, as opposed to attempting to make a computer that
plays like a human. This results in odd bet sizing and a much
different strategy than humans are used to seeing. 

Methods are being developed to at least approximate perfect poker
strategy from the game theory perspective in the heads-up (two player)
game, and increasingly good systems are being created for the
multi-player game. Perfect strategy has multiple meanings in this
context. From a game-theoretic optimal point of view, a perfect
strategy is one that cannot expect to lose to any other player's
strategy; however, optimal strategy can vary in the presence of
sub-optimal players who have weaknesses that can be exploited. In this
case, a perfect strategy would be one that correctly or closely models
those weaknesses and takes advantage of them to make a profit, such as
those explained above. 

Research groups[edit]
Computer Poker Research Group (University of Alberta, Canada)[edit]
A large amount of the research into computer poker players is being
performed at the University of Alberta by the Computer Poker Research
Group, led by Dr. Michael Bowling. The group developed the agents
Poki, PsOpti, Hyperborean and Polaris. Poki has been licensed for the
entertainment game STACKED featuring Canadian poker player Daniel
Negreanu. PsOpti was available under the name "SparBot" in the poker
training program "Poker Academy". The series of Hyperborean programs
have competed in the Annual Computer Poker Competition, most recently
taking three gold medals out of six events in the 2012
competition. The same line of research also produced Polaris, which
played against human professionals in 2007 and 2008, and became the
first computer poker program to win a meaningful poker competition. 

In January 2015, an article in Science[1] by Michael Bowling, Neil
Burch, Michael Johanson, and Oskari Tammelin claimed that their poker
bot Cepheus had "essentially weakly solved" the game of heads-up limit
Texas hold 'em.[2][3][4] 

School of Computer Science from Carnegie Mellon University[edit]
T. Sandholm and A. Gilpin from Carnegie Mellon University have started
poker AI research in 2004 beginning with unbeatable agent for 3-card
game called Rhode-Island Hold 'em. Next step was GS1 which
outperformed the best commercially available poker bots. Since 2006
poker agents from this group have participated in annual computer
competitions. "At some point we will have a program better than the
best human players" – claims Sandholm. His bot, Claudico, faced off
against four human opponents in 2015. In 2017 the program's latest
software, Libratus, faced off against four professional poker
players. By the end of the experiment the four human players had lost
a combined \$1.8 million.[5] 



\subsection{DOTA2}
{\bf why? first multi player program}

An OpenAI-machined learned bot played at The International 2017 Dota 2
tournament in August 2017. It won during a 1v1 demonstration game
against professional Dota 2 player Dendi.[61] 

\subsection{Go}
\index{AlphaGo}
{\bf why? the Drosophila. The game of intelligence par
  excellence. Only mention program names. Chapter 10 will gie much
  more detail about technology and matches.}


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/go}
\caption{Go}\label{fig:go}
\end{center}
\end{figure}
1989 GNU go: minimax. The idea is based on the
article "Programming the Game of Go. Byte, Vol.6 No.4" by
J. K. Millen. Man Lung Li, et al., Houston
\cite{millen1981programming}\index{GNU Go}

1996 NeuroGo Enzenberger \index{NeuroGo}\cite{enzenberger1996integration}

1993 Brugmann Monte Carlo Go
\cite{brugmann1993monte,bouzy2004monte}\index{Monte Carlo Go}
1995 Buro Logistello \cite{buro1995statistical}\index{Logistello}
2006 MCTS Coulom\index{MCTS}
2006 UCT Kocsis Szepesvari \cite{kocsis2006bandit}\index{UCT}
2007 Silver \cite{gelly2007combining,silver2009reinforcement}
2013 DQN Atari
2016 AG Sedol \index{Lee Sedol}\index{Ke Jie}\index{AlphaGo}\cite{silver2016mastering}

\section{Summary}

%checkers, chess (turing, russians, deep blue-kasparov)

% 1950 Turing paper

% 1960 Samuel

% 1994 Checkers

% 1997 Kasparov

% 2016 Sedol



%\section{Theory}



%Philosophy of Intelligence; behavioral view of intelligence. very briefly. Further: see appendix

%turing 1950

%show the search-eval architecture

%\section{Practice} Example: a Tic Tac Toe program

%or: Hex. or 9x9 go.

%\section{Challenge} Understand that Lookahead is intelligence





==> chapters/old201intro.tex <==
\section{Tuesday March 15, 2016}
Tuesday  March 15, 2016 is an important day in the history of intelligence. That
day was the final day of a five game match in which a computer
challenged one of the strongest Go players known to
humanity. Go is an ancient game of strategy, played by millions around
the world, originating in South-east Asia. Playing the game well
requires  years of training and a considerable amount of intelligence. Dedicated
Go-schools exist in China, Korea, and Japan, and professional Go
players achieve star-status in their countries and can live well from
their prize money.



\begin{figure}[t]
\begin{center}
\includegraphics[width=12cm]{figures/fourseasons}
\caption{AlphaGo versus Lee Sedol}\label{fig:fourseasons}
\end{center}
\end{figure}


On March 15, at the luxurious Four Seasons hotel in Seoul, the computer program
AlphaGo beat top Go-professional Lee Sedol (see
Figure~\ref{fig:fourseasons}). The prize money, 1 million dollars, was donated by DeepMind
to charities. Lee Sedol received 170,000 dollars for his
efforts.  The match consisted  of 5 games, the human
champion was beaten 4-1. A subsequent match in 2017 against
champion Ke Jie was
also won by the computer. Commentators described AlphaGo's level of
play as very strong, and the style of play as refreshing, with a few highly
surprising moves. AlphaGo was awarded a 9 dan professional rank, the
highest rank possible, by the Chinese Weiqi association, and the journal
Science chose the event as one of the {\em breakthrough of the year\/} runners
up. Today, human Go players are taking inspiration from the games
played by AlphaGo, trying to learn from its deep insights and unusual moves~\cite{zhou2018}.

To add insult to injury, in 2017 the
DeepMind team went  further. They created a version of AlphaGo,
AlphaGo Zero, that learned
to play the game from scratch, with zero human knowledge added, no
grandmaster games studied, and no Go knowledge
preprogrammed
\cite{silver2016mastering,silver2017mastering,silver2017shogi,silver2018general}. The
AlphaGo Zero work is  considered to be even more impressive than the
AlphaGo-wins,  since its learning   closely
resembles learning processes in human children (this will be discussed
further in Chapter~\ref{chap:fast}).

The breakthrough performance of AlphaGo came as a surprise. The level
of play of computer Go programs had been languishing around the strong
amateur level for years. Experts in computer games had expected grand
master level play to be at least ten years away, let alone beating the
world's strongest players.


The DeepMind AlphaGo Zero work is truly senstional. Beating
    the human Go champions has shaken the world of AI, indeed it has
    shaken the world. The goal of this book is to teach you how they
    did it by allowing you to gradually
    replicate the cornerstones of their work.

    In the first Part, we will cover the basics of games and
    reinforcement learning. Then, in the second
    Part (``Plan''), to 
    appreciate where we are coming from, you will experiment with an
    old school heuristic Chess 
    program. You can also
    build an MCTS program, and understand how it works, and see
    how very different it is from the heuristic approach.

    In the
    third Part (``Train''), we will
    discuss the essential elements of   deep learning, and you will understand another 
    important field, deep {\em reinforcement\/} learning, and
    replicate the Atari experiments that set off the reinforcement
    learning interest.

    Finally, in the fourth Part (``Plan + Train''), you can put it all together and
    build a version of a game playing program that achieves  one of the
    major feats of recent AI: self learning. The program learns to play games from
    scratch (tabula rasa).

\subsubsection{Excitement}
This book is built on excitement---excitement because the advances in
game playing are so large that they appear to be
approaching true intelligence; excitement because  the
intelligent architectures seem to work in more than one domain, giving a glimpse
of that holy grail of AI, {\em general\/} intelligence. On a more
technical note there is excitement among AI researchers
because in modern self-play two old 
schools in AI, symbolic and connectionst, have joined forces. From the
perspective of methodology there is also reason for excitement. A large part of the
progress in games research is caused by the free and open availability
of test data sets and algorithms, allowing easy replication and
improvement of results.

Open science works, and allows you, the
reader, to benefit. After learning the concepts and algorithms of
reinforcement learning in games, you should be ready to help create
the future.
%% excitement because likewise planning and learning are working
%% together; excitement because we are leaving behind the world of
%% heuristic (special) knowledge, to enter the world of general methods;
%% excitement because, simply, it is exciting to understand what is
%% inside a Chess machine and to know what makes a Go machine tick;
%% excitement because the path of discovery  reads like
%% a detective story with many unexpected turns of events; and finally
%% excitement because this knowledge might enable {\em you\/} to take us further
%% on the road to machine intelligence $\ldots$  
    

    % This book is built on two
    % pillars of excitement: the excitement of knowing you are learning one of the
    % most significant AI developments of the decade, and the excitement of
    % thinking of what this might hold for the future. After
    % reading this book, you should be ready  to help create that future.



% The rest  of this chapter will give an overview of the contents of
% this book.

\section{Four Stories}
The story of reinforcement learning in games is a story of magnificent
scientific achievements. That 
is the {\em first}, and obvious, story: an account of how
intelligence can be programmed, and an outlook into our future. This
level of the book is built on excitement, as we just mentioned.

This
book also contains a {\em second\/} story, an ordinary computer
science story, with
algorithms, code, and explanations, all about the techniques of reinforcement learning in
games.  We will discuss the algorithms to build intelligent game playing programs. Section~\ref{sec:planlearn} expands on this algorithmic level.

This book contains a {\em third\/} story, the story of unfolding
discoveries from specific heuristics to general learning methods,
discoveries that shaped the science of artificial intelligence
itself. Section~\ref{sec:heurlearn} expands on generalization in
artificial intelligence.

Finally, this book contains a {\em fourth\/} story, the story of
scientific discovery itself. This final story illustrates how the experimental
approach to scientific discovery has used games as an experimenter's
tool to find intelligence. The front cover picture of two Drosophilas
illustrates this fourth  story.

This fourth story contains the most important lesson that you
might take away from 
  this book: how to use the experimental approach to creating
  intelligent problem 
  solvers of amazingly good performance. Try, understand, generalize/automate, try
  again. At  first sight this may seem to be a book that teaches
  methods and algorithms of the quest towards artificial general intelligence in games. Although we cover some pretty
  powerful methods in 
  this book,  I hope that what you will take away from this
  book is an approach to research itself, an experimenter's mentality, that allows you to
  keep inventing better methods yourself, to work towards Artificial
  General Intelligence: {\em Try,
  Fail.  Try again, Fail better.} 


% The story in this book is  a history. It is a history of a specific kind of AI, the history of
% computer playing intelligent board games. That history shows how
% technology evolved, form the specific to the general---from
% exploitative enumerative search and domain specific heuristics, to
% exploration, generalization and domain specific features that are
% learned by general methods.

% At a deeper level, this is the story of
% AI---from specific to general.  It is the story of a how a young field
% with limited computional power tried to model a game of intelligence
% through manual heuristics,
% and through roadblocks and setbacks develops more general methods that
% are applicable to other domains, that can learn and generalize. It is the story of how two areas of AI
% that were quite distinct---symbolic AI and connectionist AI---came
% together to create a success. It is the story of planning and learning. It is
% also the story of one constant: 
% the search-eval architecture.

% These are the first baby steps on the road to
% Artificial General Intelligence---a history worth to be documented and
% learned from. Hold on tight, for the story of 70 years of artificial intelligence.




% \begin{itemize}
%   \item architecture: search-eval/exact-approx/slow-fast/plan-learn
% \item two trends: performance and generalization. 
%   First start with problem description, do a shortcut towards high
%   performance, exploiting heuristic specifics, then understand what is
%   going on, and generalize the specific features through
%   learning.
%   \item 
%   \item Try harder, and always in the direction of more automation/learning/generalization
%   \item (4) minimax+heuristic, (5) ab, id/tt, search extensions, quiescence, coeff
%     learning, (6) avg backup, monte carlo eval, exploration selection,
%     (7) function approx, (8) stable learning, (9) performance
%     learning, (10) self tuning through self play, (11) hyper par
%     optim
%     \item from rigid to flexible to learned flexibility (which is even
%       more flexible than hard coded ``flexibility'')
%     \item 
% \end{itemize}


% \section*{Learning Goals}
% \begin{itemize}
% \item {\bf It  is exciting to learns about the quest for machine intelligence, and the 4 paradigms. Bring the emotion in understanding our own thinking}
%   \item 
%   \item Thinking=Fast+Slow
%   \item AI=Plan+Learn
%   \item Learning=Generalized planning examples (Fast is internalized Slow)
% \end{itemize}



%% section: topic (background) legitimization (why this book): to explain the tech behind the big breakthrough
%% section: problem statement
%% section: methods: theory and running practic eexample
%% section: outline

% \section{Homo Ludens}
% This is a book about intelligence and a book about games. In 1938 the great
% Dutch historian and cultural theorist Johan Huizinga published Homo
% Ludens. In this book he discussed the importance of the element of play in
% human culture~\cite{huizinga1938homo}. In education and psychology the
% concept of learning through play is well known. This book is not about human
% culture or human learning, but about  artificial
% intelligence. This book is about the
% importance of the element of self play for learning, and
% intelligence. AI is about creating mechanical devices that exhibit
% intelligent behavior.  AI is a study of how
% intelligence can be realized outside the human body. This book is
% about how, through self play, computers can learn to play games of
% intelligence (Go, Chess, and Shogi). The links of self play, and
% reinforcement learning, between learning in AI and learning in
% children is inescapable. To provide a glimpse of this link we will
% highlight parallels between chapters of this book and the book
% ``Thinking, Fast and Slow,'' a book by psychologist and behavioral
% economist Daniel Kahneman~\cite{kahneman2011thinking}.



\subsubsection{Problem Statement}
The main question that we are concerned with in this book is
the following:
\begin{quotation}
  
{\em   What machine learning methods are
used in  Chess and Go that achieve such a high level of play?}

\end{quotation}
Among the technologies used are heuristic search methods, neural nets, and
compute power in the form of GPUs and cloud-computing. This book
provides an in depth introduction to them all, how they work, with example
code, and with many references to the literature for more details. 

The core of this book is about the  search-eval
architecture. This architecture allows advanced planning and learning
methods to work synergistically together. We describe the
architecture and the technologies
that have been so successful, from heuristic search,
to deep Q-learning. 

% Planning (more
% specifically Bandits and MCTS) and
% Learning (more specifically DQN) are separate and active fields of study in their own
% right. When they came together, in Turing's classic search-eval
% architecture, they
% caused a quantum leap, in Go. Getting techniques from two fields
% to work together requires large efforts to understand (1) two fields and
% (2) how they can work together. It is our hope that the explanations in
% this book stimulate more efforts of scientists like
% the DeepMind team to
% cross boundaries and join efforts in both fields, allowing AI to solve
% harder and harder problems.

% An alternative problem statement, and a driving question, is: {\em Or
%   more precise:  for Chess and Go, games for which humans 
% require intelligence, what  mechanical methods work? And what kind of
% problems can these methods solve, and how can these methods be
% extended?}

Although the methods for Chess and Go are quite
different,
%there is a  commonality in both approaches, which is called the
%search-eval architecture in this book.
this architecture, devised by
Turing around the time of the Second World War, is still at the center of many
intelligent machines. 




% \section{Symbolic and Connectionist}
% Throughout the history of AI there have been two dominant schools of
% thought: symbolic AI and connectionist AI. The school of symbolic AI
% is rooted in logic and reasoning, and gave rise to expert systems. The
% idea is that many aspects of intelligence can be studied
% thorugh the manipulation of symbols. Symbolic AI is sometimes seen as
% top down, theory driven. Dichotomies are always oversimplifications,
% but if forced, planning and search would be symbolic AI.

% Connectionist AI is bottom up, it believes that intelligence emerges
% out of interactions of complex networks with their environment. Neural
% networks and deep learning are prime examples of connectionist
% AI. Learning would be connectionist.

% As noted, forcing the real world into dichotomies does not always do
% justice to the complexity of the real world. Learning may be
% connectionist, but if an important part of the success of deep
% learning is due to efficient backpropagation optimizers. And
% optimizers are search algorithms, or symbolic AI.

% It will be clear by now that this book is about the success of both: planning and
% learning, symbolic and connectionist AI. 



\subsubsection{Intended Audience}
%The following chapters will describe the methods. We will
We take a
hands on approach to artifical intelligence. After each new method is
described, we will show you how the concepts can be implemented in 
 examples, exercises and small  programs. Games-AI is an open field. Researchers have released
their  algorithms and codes allowing replication of results. This is a  sharing-oriented research
 field. We point you to code bases at Github throughout the book. Although you
probably do not have access to Google-scale compute power, at the end of
this book, you will be able to create a fully functional self-learning
program, and you can comfortably enter the active community
of reinforcement learning researchers.

\subsubsection{Graduate Course}
This book can be used for a 
graduate course in Reinforcement Learning in Games. The material
is organized in chapters that should roughly correspond to the lectures of a
single semester 
course. The availability of source code should provide for practical
assignments where you can get your hands dirty and immerse
yourself in this fascinating topic. Pieces of working 
code   can be extended to your liking for further study and research.
%The book
%will be used for such a Master-level course at Leiden University.

\subsubsection{Prerequisite Knowledge}
Since there are few other comprehensive books in this fast moving field,
this book is designed to be self-contained. Necessary pieces of
information from other fields have been included:
basic introductions into
Markov Decision Processes, reinforcement learning and deep learning are
provided. To 
do the exercises in this book,  undergraduate level proficiency in Python is
necessary. An undergraduate level understanding of artificial intelligence
and neural networks is also presumed.


\section{Artificial Intelligence:  Mathematics +
  Biology}\label{sec:schools}\index{symbolic AI}\index{connectionist AI}
Artificial intelligence is the 
study of machines that exhibit behavior for which humans need 
intelligence.  Main topics in the study of AI are cognitive functions
such as learning and problem 
solving~\cite{russell2016artificial}.

Artificial intelligence research is based on two fields of science,
mathematical logic and biology~\cite{nilsson2009quest}. One of the early ways of modeling thought
processes is the top down deductive approach that has come to be known
as symbiolic AI. In symbolic AI logic reasoning is used to draw
inferences and conclusions from underlying facts and assumptions about
the world. Intelligence is considered to be equivalent to a top down reasoning
process. This school has yielded progress in expert systems, 
reasoning systems, and theorem proving systems. Well known examples
are the  STRIPS planner~\cite{fikes1971strips}, the Mathematica and
Mathlab computer algebra systems~\cite{buchberger1982computer}, 
the programming language PROLOG~\cite{clocksin2012programming}, and
also semantic (web)
reasoning~\cite{berners2001semantic,antoniou2004semantic}. Part II of
this book, on heuristic planning, has grown out of the  symbolic approach. Symbolic AI
is inspired by mathematical logic.

A second school of thought is the connectionist approach to AI.
It purports that intelligence
emerges out of interaction processes between many small
elements. Embodied intelligence
(robotics)~\cite{brooks1991intelligence}, nature inspired algorithms
such as Ant Colony Optimization~\cite{dorigo1997ant}, swarm
intelligence~\cite{kennedy2006swarm,bonabeau1999swarm}, genetic
algorithms and  evolutionary
strategies~\cite{fogel1994introduction,holland1992genetic,back1993overview}, and, last but not least, neural
networks~\cite{haykin1994neural,lecun2015deep} are examples of the
successes of this approach. Part III of this book, on training, has
grown out of the connectionist approach. Connectionism is inspired by
biology.


Machine learning is the field of research that studies algorithms
that learn relations between variables  that were not explicitly
pre-programmed. It encompasses both symbolic and connectionist
methods. Machine learning algorithms find patterns, categorize
data, or  make decisions.  Machine Learning consists of three groups
of methods: 
supervised learning, reinforcement learning and unsupervised
learning~\cite{bishop2006pattern}.

In supervised learning a (typically large) database of labeled
examples exists, from which the type of relation between variables is
inferred. The labels have to be provided beforehand, by humans, or by 
other means.

In reinforcement learning there is no database of labeled examples,
interaction is the key. In reinforcement learning an agent can
interact with its environment, which returns a new state and a reward
after each action. By probing the environment, the
reinforcement learning agent can learn relationships that hold in the
environment. Reinforcement learning problems are often modeled as
Markov Decision Processes~\cite{sutton2018introduction}. Most games can be modeled as reinforcement
learning problems.

Unsupervised learning algorithms find patterns in data without the
need for human labeling. Typical unsupervised algortithms cluster data
based on inherent properties such as distance between variables.

In this book we study reinforcement learning algorithms in
games. Reinforcement learning is interesting in that it lives on the
middle ground between the two approaches, drawing inspirations from
symbolic AI (exact planning, mathematics, Markov Decision Processes) and
connectionist AI (approximate training, cognition,
interaction). Especially in Part IV, Plan + Train, we see how the two
schools of thought in AI join to achieve great success.


\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/arch.jpg}
\caption{Search--Eval Architecture}\label{fig:arch}
\end{center}
\end{figure}

\section{Architecture: Search + Eval}
Since the earliest days of game playing research, the search-eval
architecture has been the cornerstone of game playing programs. The
architrecture is simple,  see
Figure~\ref{fig:arch}. It consists of two functions, a search
function and an evaluation function. The search function traverses
possible game positions, and the evaluation function scores the
position with a value function. Search-eval programs solve a specific
class of
reinforcement learning problems, i.e., games, and work especially
well in two-player zero-sum perfect-information games. (The Figure
also introduces the words {\em plan\/} and {\em trained\/}. These
terms are of great importance, as we will see in the next section.) 

Although
the insides of the search-eval architecture have changed immensely
over the decades, this organization in two functions has remained.
Many new  mechanisms have been 
invented since the days of Turing: Monte Carlo evaluation,
Deep Q-networks, self-guided search, generalization, and
self-play. Where in the Chess  domain specific knowledge had to be encoded 
in the program, now
programs learn to play better than  the
strongest human, without being told  more than the rules of the
game. In Chapter~\ref{chap:search} the search-eval architecture will
be explained in detail.

\subsubsection{History}
The search-eval architecture is old, yet has been at the basis of
progress in reinforcement learning in games since the beginnging in
the 1950s. Its central role in the development of artificial
intelligence in games allows us  to show the history of these
developments.  Chapter~\ref{chap:games} contains a brief overview of
major achievements.



\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=5cm]{figures/dragon.jpg} &
\includegraphics[width=5cm]{figures/DrawingHands.jpg}
\end{tabular}
\caption{A Dragon biting in its own Tail and Escher's Self-drawing Hands}\label{fig:dragon}
\end{center}
\end{figure}

\section{Methods: Plan + Train}\label{sec:planlearn}

Please refer to Figure~\ref{fig:arch} again. The essence of the search-eval architecture is an intricate interplay
between two reinforcement learning methods: planning and
training. First, in the planning phase an exact lookahead algorithm generates
possible future states of the game. Second, these future states are then
scored by an approximating value 
function. This value function can  use domain specific 
knowledge %% (such as: more pieces is better than fewer pieces)
or it can use a
neural network, or any other approximating function. Often, the
approximating value function uses some kind of training to improve its
approximations.

In self-play, the outcome of  tournaments is
used as input for the value function to train from,
which is then used as input for more tournaments and more training, etc.   This kind of behavior, of feeding off itself, is called recursion, see Figure~\ref{fig:dragon}.
In Chapter~\ref{chap:selfplay} we will describe self-play in
detail.

\subsubsection{Model-based and Model-free}\index{model-based}\index{model-free}
An often-used distinction in reinforcement learning
  is between 
model-based and model-free methods.
Planning is a model-based method: it can be used when a model of the
environment is available, such as the rules of the game, or a
simulator. Training works in model-free situations, when such a model
does not exist, and the goal is to create such a model. Together,
planning and training are the two building blocks of this book.

\subsubsection{Planning, Training, and Learning}
In the field of artificial intelligence, the word {\em learning\/} is used frequently to indicate many
different kinds of action retention, from simple remembering to complex adaptive methods. This is
fine, of course, and we will use the regular terminology of machine
learning, supervised learning, and reinforcement learning.  In this book
we will try, when possible, to be a bit more precise. We will use the term {\em planning\/}
for reinforcement learning methods that traverse large state
spaces to find good values. We will use the term {\em training\/} for reinforcement learning methods
that train neural network function approximators. We will use the term
{\em learning\/} for reinforcement learning methods that use a combination of
planning and training to learn to play a game. 

%% The search-eval architecture makes such a virtuous circle of
%% planning and training possible, where planner and trainer help each
%% other to improve their outcomes, 
%% learning  an ever improving quality of play (well, in theory, at least).
%% See Fig..
% 
% The goal of this book is to familiarize the reader with this
% architecture, and to discuss in depth the techniques that constitute
% machine intelligence, so that the reader is well equipped to take the
% next steps and perhaps help bring the field forward.



\subsection{Specific + General}\label{sec:heurlearn}
The methods in this book go from specific to general, from model-based
to model-free to integrated. The early chapters describe
methods that need domain specific heuristics, and we 
end with methods that are able to generalize features in many
domains. Together the chapters tell a story  how AI progressed from
Artificial Specific (or Narrow)
Intelligence to Artificial General Intelligence.



%% %\section{Learning to Learn}
%% % This book also documents the progression  towards self learning systems.
%% This has been a long road, that started with trying to
%% mimic human knowledge by coding heuristic rules,\index{heuristics}
%% approximations of what were thought to be relevant domain specific
%% knowledge. Quickly, a planner (or searcher) was put on top, to resolve
%% tactical and strategic issues. Then, adaptive search was used, and
%% later on generalization. As the success of general learning systems
%% increased, the role of heuristics steadily diminished. Two parallel
%% developments enabled the success of learning systems:  the availability of large training databases
%% with labeled examples, and the availability of large amounts of
%% compute power, especially in the form of GPUs.\index{GPU}

This book covers the technologies behind the major AI breakthroughs in
games. Computer Chess, Atari, and Go required
surprisingly diverse techniques, from specific heuristic planning to 
deep learning self-play.
%% :
%% \begin{itemize}
%% \item Heuristic Planning includes heuristic evaluation functions and
%%   alpha-beta search, and many important enhancements such as iterative
%%   deepening and transposition tables, all necessary ingredients for
%%   world championship level Chess
%% \item Monte Carlo Tree Search is an adaptive search algorithm at the basis of the
%%   breakthrough in Go. The theories that explain how and why MCTS works
%%   are  reinforcement learning and bandit theory\index{bandit theory}
%% \item Deep learning and deep reinforcement learning 
%%   caused a sensation by playing Atari Arcade games end-to-end:
%%   directly from
%%   the raw pixels of the screen all the way to the joystick actions
%% \item Self-play, the technology behing AlphaZero, which enables  learning
%%    to world championship level  in
%%   Go, from first principles, without   any heuristic input
%% \item Current research topics in reinforcement learning are discussed:
%%   imperfect information, transfer 
%%   learning, curriculum learning, and hierachical reinforcement
%%   learning. We also discuss how these techniques may develop and
%%   influence the   future of AI and the quest to that elusive goal, artificial general
%%   intelligence 
%% \end{itemize}
Figure~\ref{fig:layersch}) gives an overview of the topics of this book. The early chapters describe methods that work for
specific games, heuristic search. The next chapters describe increasingly general methods that adapt themselves to different domains. In the end, self-play methods are described, that even teach themselves which examples to learn from. 

This book is  the story of AI researchers that were learning how to
make algorithms that can learn to learn.

% \section{Plan to Learn}
% Table~\ref{tab:concepts} connects the main concepts covered in this
% book from AI
% and Psychology (or better, Kahneman). Note that Kahneman does not
% feature reinforcement learning prominently, and does not label
% explicitly the activity of using rational planning to generate
% examples to train the patterns from. Since this training is quite
% important in our architecture, we took the liberty of adding as 
% a system 3, a system in which rational reasoning creates examples from 
% which fast reflexes are trained.

% Table~\ref{tab:paradigms} translates the main concepts to paradigms
% for planing and learning on which the game players are based.

% Table~\ref{tab:techniques} relates these paradigms  the techniques that
% are used in the players.


% Table~\ref{tab:architecture} concerns the search-eval and provides
% details of the different algorithms that are used in the search, eval,
% and two other important elements of the game players.




% \begin{table}[ht]
% \begin{center}
%   \begin{tabular}{c|c}
%     \hline\hline
%      {\bf AI} &  {\bf  Kahneman}\\ \hline
%     Feature Recognition  & System 1, Thinking Fast
%     \\ \hline
%     Planning, Reasoning & System 2, Thinking Slow \\ \hline
%     Reinforcement Learning & {\em System 3, Training Very Slowly?}\\ \hline\hline
%   \end{tabular}
%   \caption{Concepts in Artificial Intelligence and Psychology}\label{tab:concepts}
%   \end{center}
% \end{table}

% \begin{table}[ht]
% \begin{center}
% \input paradigm
% \caption{Four Reinforcement Learning Paradigms}\label{tab:paradigms}
%   \end{center}
% \end{table}

% \begin{table}[ht]
% \begin{center}
% \input technique
% \caption{Techniques}\label{tab:techniques}
%   \end{center}
% \end{table}

% \begin{table}[ht]
% \begin{center}
% \input searcheval
% \caption{Search-Eval Architecture}\label{tab:architecture}
%   \end{center}
% \end{table}

\section{Thinking: Fast + Slow}
The philosophical implications of the AlphaGo achievement are
large. Of course, some humans knew that we are not the only intelligent race on
the planet (ask any dog, monkey or dolphin trainer). Yet,  the realization
that we are now able to create a machine that can  learn to play such a
tremendously challenging and rich game of strategy, beating the
smartest professionals, who have devoted their lives to learn the
intricacies of the game, is baffling. Indeed, for many researchers the
goal of artificial intelligence research is to understand
intelligence, and here, we  have made a
tremendous 
step. It now certainly is the case, 
at least for the narrow domain of  complicated board games,
that we have succeeded in replicating parts of learning and reasoning
processes  at human level. 

Daniel Kahneman is a psychologist and winner of the Nobel prize in
Economics. His works have helped  found the field of behavioral
economics. In his works, such as on prospect theory, he  combines
psychology and economics. 
He has written a highly accessible book, which has been
on best seller lists since it was published in 2011. It is called  
{\em Thinking Fast and Slow}~\cite{kahneman2011thinking}. In this book he presents the topics of his
most famous papers. Central in Kahneman's book is System 1 
thinking, or fast, approximate, intuitive human thinking, and System 2
thinking, or exact, slow,
reasoned, human thinking. These two concepts fit well with our AI methods
at the basis of the search-eval architecture.

Therefore we will highlight links between the  methods described
here and the 
concepts in Kahneman's book. While this book focuses on technical AI
methods, the philosophical
implications of   progress in artificial intelligence are  important. We 
refer to the work of Kahneman for some  of these
implications.
%
%% If
%% you think of this book as the companion of Kahneman's book for
%% mechanical thinking,
%% then that is somewhat appropriate, although current AI technology is
%% just starting to be intelligent in a very limited way. But the model
%% of thinking fast and slow is present in this book. We call it planning and
%% training. 
%
Kahneman's book describes fast and slow thinking in human
intelligence. This book does the same for artificial intelligence.
(see Chapter~\ref{chap:fast}).

\begin{figure}[t]
\begin{center}
\input diag/layerchapters
\caption{Stack of Chapters, with increasingly advanced Mappings from
Problems to Methods (from bottom to top)}\label{fig:layersch}
  \end{center}
\end{figure}



\subsubsection{State Spaces}
A major element in reinforcement learning in games is to model
decision problems as state spaces of all possible game positions. For most
interesting problems these
state spaces are very large, and much of AI is concerned with  
efficiently finding solutions in these very large state spaces. In the following chapters, we will describe in depth the 
methods that do so.

\section{Outline}
The  purpose of this book is to show which methods  
game playing programs use to
exhibit intelligent behavior in two person games. The material in this book is
organized in a logical order (see 
Figure~\ref{fig:layersch}). The chapters are a sequence of
increasingly advanced mappings between problems and solution
methods.

\subsubsection{*Starred Chapters and Sections}
The chapters are organized in parts, from planning to training to self
play, with chapters on the main techniques. Three chapters contain 
advanced material. Depending on your interests, or the aim of the
course, some material can be
skipped. Figure~\ref{fig:overview} shows 
the structure of the chapters. The further to the right, the more
technical the chapters are.


Chapters and sections whose name starts
with a *star are  advanced material, which is essential for high
performing implementations, but may be skipped when in a hurry, without missing the main thread.

\subsubsection{The Parts}
{\em Part I\/} We start, 
in Chapter~\ref{chap:games},
with the question why, in artificial intelligence, the study of games
plays such an important role. We provide a historic overview of
notable achievements in the history of game playing programs. Next,
in Chapter~\ref{chap:rl}, we review reinforcement learning as a
common language for the study of game playing programs.

{\em Part II\/} Then, in
Chapter~\ref{chap:search} we  introduce the first methods: minimax
and heuristics, methods that map quite directly to the state spaces of Chess and
Checkers. The next chapter describes enhancements to transcend this
direct (and somewhat rigid) mapping, to achieve higher
performance. Chapter~\ref{chap:trial} then introduces a planning
method that is inherently adaptive, which was necessary 
for  the next domain, Go.

{\em Part III\/} We continue our path to more general methods that adapt themselves to their domain
in the next Chapters,~\ref{chap:super}-\ref{chap:conv}, with
training of function approximators using
databases of examples. These training methods work for image
recognition and for playing Atari arcade
games.

{\em Part IV\/} Chapter~\ref{chap:plan} goes a step further and introduces  
self-play. In self-play two versions of the program play tournaments
against each other. Self-play is a method that adaptively generates high quality examples with
which to train the function approximator. As we will see, this works
amazingly well in Go, and generalizes to other 
games. Chess and Go are two-player perfect information games. The next chapters then look
at future  developments for intelligent methods for even more complicated
games (multi-player, imperfect information) that contain more elements
of real world decision making.
% The chapters describe methods of increasing generality and build upon each other.



\begin{figure}
\begin{center}
\input diag/overview
\caption{Overview of the Chapters of this Book. Roman: General
  Content {\bf Bold: Technical Content} {\em Italics: Advanced Content}}\label{fig:overview}
  \end{center}
\end{figure}



\subsubsection{The Chapters}
Let us now discuss the chapters in more detail.
We will
start in Chapter~\ref{chap:games} with early thoughts on intelligence
and intelligent
machines. We then provide a brief historic overview of some of the
important game 
playing programs, starting with the early designs of Claude Shannon,
Christopher Strachey and Alan Turing.
%The techniques are rooted in different paradigms
%(see Table~\ref{tab:paradigms}.)

Next, in chapter~\ref{chap:rl}, we introduce reinforcement
learning. The concepts and formalizations of reinforcement learning
are at the basis of the historic advances in artificial intelligence
that we have recently witnessed. Concepts such as  policy and
Q-learning are discussed in this chapter.


In chapter~\ref{chap:search}, we 
introduce heuristic planning. Heuristic planning in games
uses domain specific knowledge to reduce the size of the state space, and then
uses minimax planning to traverse that reduced state space.
In this chapter we discuss the  principles of the search methods
that are at the basis of  AI breakthroughs in
Checkers and Chess. 

The planning methods of heuristic planning are simple and rigid, and it turns out that many
enhancements are needed to achieve good performance in real game
playing programs. The
following chapter, Chapter~\ref{chap:idtt}, introduces
enhancements that  overcome some of the rigidity of the minimax
approach. In this chapter variable-depth and variable-width
enhancements are introduced.

In the next chapter, Chapter~\ref{chap:trial}, we delve deeper into  the
principles of learning by trial and error. Major topics in this
chapter are the 
exploration/exploitaiton trade-off and the concept of evaluation by
random play-out, leading to the Monte Carlo Tree Search algorithm
(MCTS). The algorithm in this 
chapter is variable-depth and variable-width by design, and great performance improvements, especially in $9\times 9$ Go,
are achieved with MCTS. The chapter also discusses enhancements of MCTS.

Then, we switch from planning to training. We focus on the evaluation
function, and try to generalize features from the states. We start in
Chapter~\ref{chap:super} with a short review of deep learning
methods for supervised learning. Among other things, convolutional
networks are discussed, and the problem of overfitting. In 2012 deep learning methods caused a
breakthrough in image recognition performance. Much of the
current interest in artificial intelligence is caused by this
breakthrough for which Bengio, Hinton and LeCun received the 2018
Turing award, also known as the Nobel prize of computer science.  

Chapter~\ref{chap:dqn} looks at how these methods can be used in a
reinforcement learning setting:
generalization of features in deep neural networks for learning by
trial and error, or Deep Q Networks,
DQN. Q-learning with function approximation and bootstrapping is in principle unstable,
and  a few important enhancements had to be developed to achieve stable
training. With these enhancements, we find that  DQN can be an effective way to improve
on heuristic evaluation functions. 

In the next chapter, Chapter~\ref{chap:conv}, we look deeper into
enhancements to achieve stable training in supervised and
reinforcement learning. %% Specifically,
%% we cover impediments, such as overfitting and myopia,  deep
%% reinforcement learning.


Chapter~\ref{chap:plan} combines planning and training %% or MCTS and
%% DQN, the two major building 
%% blocks of AlphaGo. Here we  see how planning and learning can be combined
to create self-learning systems. The
kind of learning of these systems resembles human learning. Finally,
we conclude in Chapter~\ref{chap:conclusions} by reflecting on the
artificial intelligence progress, and  in chapter~\ref{chap:fast} on the relations to natural
intelligence. We discuss possible future resesarch directions.\\

After this overview, let us begin our journey.


%% \begin{table}\label{tab:arch}
%%   \begin{center}
%%     \begin{small}
%% \input tab-arch
%%   \caption{Search-Eval Architecture in different chapters}
%%   \end{small}
%%   \end{center}
%% \end{table}

% \section{From Special to General}

% \section{Stories}
% There are many stories in this book, and they are all related. 
% See Figure~\ref{fig:stories}.

% \begin{figure}
% \begin{center}
% \input stories2
% \caption{Overview of the Story Lines in this Book}\label{fig:stories}
%   \end{center}
% \end{figure}

% \begin{itemize}
% \item In Eval, From Heuristics to Learning is Special to General is
%   Weak to Powerful
% \item In Search (planning), From alpha-beta to MCTS is Rigid to Adaptive
  
%   \item From Plan to Learn to Self Play is Plan+Learn
    
% \item From Slow to Fast to ??? (become a pro in $x$ in 10,000 hour of training?)
%   \item From Symbolic to Connectionist is indeed from Heuristics to
%     Learning
%     \item Heuristics is not search, Learning is not eval

%   \item A constant is the search-eval architecture---in all programs
%     there is a search component interacting with an eval component
%     (except Atari)
%   \item The coming of age of Self Play---Learning to Play

% \end{itemize}
% And: note that computers are now learning faster than humans. AlphaZero
% learns to play Go in a few days, where humans take years to master the
% game.

% If you forgive the blatant anthropomorphization, not only are computers better
% at playing Chess and Go, they are now also better at {\em learning\/} to
% play Chess and Go, and what is more, they teach themselves.

% \section{Outlook}
% \begin{itemize}
% \item Self play works
% \item  Computers can now learn faster than humans and they teach themselves.
%   \item Future research will yield many new developments in self learning:
%   \begin{itemize}
%   \item in applications, such as medicine, and new uses of intelligent
%     decision making
%     \item in fundamental learning. Through self play, learning will
%       be  more powerful
%   \end{itemize}
% \item The reason is that self play generates an efficient curriculum
%   learning method for self learning
 
% % \item Message: Self Play is Plan + Learn. We need Plan. Machine
% % learning needs reasoning 
% \end{itemize}
% Students studying AI should learn about this, hence this book.

%% \section{Old Stuff}
%% % This stuff is more like a preface
%% \section{why this book}
%% To explain what makes alphago tick, this book explains the recent leaps in reinforcement learning.

%% The AlphaGo Nature papers explained. The AlphaGo technology is truly
%% breathtaking. As any good science, the technology has been published
%% in scientific papers. The Nature publications of 2015, 2016, and 2017
%% by the DeepMind team are the prime source of information
%% \cite{mnih2015human,silver2016mastering,silver2017mastering}. They are
%% well written, explaining all details. However, the articles are full
%% with details, and expect much background knowledge. Even for insiders
%% it is a daunting task to understand all details. The purpose of this
%% book is to collect all necessary information and to explain it in a
%% comprehensive way to make it easier to understand. For AI researchers,
%% and for those aspiring to become one. 

%% \section{intended audience}
%% Researchers and Graduate Students interested in planning and learning,
%% the technology behind AlphaGo. I have tried to make the text self
%% contained, and as accessible as possible to a wider audience, since
%% the field of computer games has traditionally thrived by the attention
%% and contributions of scientists and non-scientists alike. 

%% This book is the reult of three lectures on the technology behind the
%% successes of modern reinforcement learning. The first was an early
%% lecture in October 2016 for the KNAW, for a general audience, given
%% together with my colleagues Max Welling and Tom Heskes. The second was
%% a guest lecture in the Master course Reinforcement Learning at Leiden
%% University. The lecture was crammed with details, I talked as fast as
%% I could, and there was not nearly enough time to explain many of the
%% deep concepts in full. Thus, the idea for a longer treatment was
%% born. The third lecture was for an audience of physicists, at
%% Innsbruck University. In all lectures, the audience wanted to know all
%% details to understand, essentially, how AlphaGo thinks. In all three
%% lectures there was barely enough time to scratch the surface. This
%% book is my way of making amends to these three audiences.  

%% \section{what we will discuss}
%% planning and learning

%% \section{contributions}
%% The search-eval architecture has been with us since the start of AI,
%% it was the basis of the first chess program design. Now, with AlphaGo,
%% a new incarnation has shown the great power of this classic
%% architecture. The architecure may be old, but the technology inside is
%% brand new. This book explains both the architecture and the
%% technology inside needed to make a truly self-learning computer
%% program for one of the hardest games known to mankind.
%% The question is, where can it lead us further, what kind of
%% problems can be solved next?

%% \begin{itemize}
%% \item First coherent treatment of planning and learning, the two
%%   technology working in synergy in AlphaGo (see nature paper)
%% \item document important new incarnation of search-eval architecture
%%   as it allowed step towards general artifical intelligence  (see
%%   nature paper)
%% \item comprehensive overview of all necessary technology, from
%%   minimax, hash tables, to nets and DQN 
%% \item the book has two main threads: A practical one, in each chapter
%%   you will build elements of a working Hex program (or 9x9 go?); A
%%   philosophical one, in each chapter the learned mechaisms are
%%   compared with what we know of human thought, thinking fast and
%%   slow. 
  
%% \end{itemize}  


==> chapters/old202games.tex <==
%% 2: games
%% section: behaviorist view of intelligence: memory, reasoning, and learning. turing test
%% section: games in ai: drosophila: simpler reality, strict rules
%% section: history checkers, chess (turing, russians, deep blue-kasparav)
%% section: lookahead: search-eval architecture
%% section: example: 9x9 go in python, or hex or ttt

%FIRST WRITE TOP DOWN STRUCTURE

%add words to the sections $\rightarrow$ make subsections

%Landmarks

%Methods

This chapter introduces the field of study of this book: artificial
intelligence and games. As we will see, artificial intelligence takes
a behavioristic approach to intelligence. We will also look at
computer programs for playing games.
We will see that board games
have a long history  in AI. They are a
testbed of choice for studying new methods for artificial
intelligence.
% For games, we limit
% ourselves to games that cha e topic of this chapter is to introduce the behavioristic approach to
% intelligence, and further narrow the scope of the study of artificial
% intelligence to games.
% : domains  with clear and well defined rules, yet
% providing exciting challenges to human intelligence, to be precise, board games such
% as Chess, Checkers, and Go.
% We will provide a short historic overview
% of important early work in this field.

The dream of creating artificial intelligence is  old, perhaps as
old as humankind. It was this dream that spurred the creation of
computing machinery. One of the first things the pioneers of
computer science did was to make  machines  that reason.
% And, surprisingly,
% we will see later on that the basic architecture of  Shannon's and
% Turing's design can still be traced in 
% the architecture of today's programs in Go, Poker, and StarCraft.

The learning goals of this chapter are: (1) we wish to
understand why games play such an important role in artificial
intelligence, and (2) we provide an overview of landmark game playing
programs in the history of AI in games of intelligence.
% wish to understand the challenges that AI
% developers face when building game playing programs.

% \section*{Learning Goals}
% \begin{itemize}
%   \item intelligent behavior and games
%   \item history of games
% \end{itemize}

\section*{Core Concepts}
\begin{itemize}
\item Games as Drosophila of AI
\item Early work: Shannon, Turing,  Samuel
\item Successful programs: TD-Gammon, Chinook, Deep Blue, AlphaGo
%\item General Game Playing
\end{itemize}

\section{Intelligence}
What is intelligence? Intelligence  includes recognition,
reasoning,  memory,  learning, 
problem  solving, adapting to your environment, and creativity. In
addition, human 
intelligence is embodied, human beings have emotion,  are
self-aware, and  have a will. Most artificial intelligence research is
focused on the former list.  Essential elements studied in AI are recognition,
reasoning, memory and learning~\cite{russell2016artificial}.
%, of intelligent behavior, of {\em 
%acting\/} intelligent.
Intelligent decision making is at the core of
AI research. Artificial intelligence research mostly studies
intelligent behavior (as opposed to {\em being\/} intelligent). 

We will now discuss these concepts in more depth.

\subsection{Cognition}
% Cognitive aspects of intelligence include logical reasoning, planning,
% problem solving, learning, creativity, understanding, self-awareness, and
% emotional knowledge~\cite{kahneman2011thinking}.
%
Psychology teaches us  that intelligence includes  cognitive
abilities, the abilities to learn, form
concepts, and reason. These abilities allow us to recognize patterns, comprehend
ideas,  allow us to plan, solve problems, and use language to
communicate. Cognitive abilities enable intelligent
behavior. These abilities also enable us to experience and think.

Experience and conscious thought are elements of 
%These last two elements bring us closer to the point that human
%intelligence is
embodied intelligence.
%\subsection{Embodied vs. Computational, Connectionist vs. Symbolic}
The theory of embodied intelligence stresses our ability to {\em
  perceive\/} information, 
to use it as knowledge in adaptive behaviors within an environment, in
an embodied sense~\cite{francisco1991embodied}.

A rival theory is the theory of 
computationalism. Computationalism states that
thoughts are a form of computation of a set of laws for the relations
among representations. Computationalism regards the brain as  a big
computer~\cite{mccorduck2009machines}. The field of reinforcement
learning has elements of both schools. Reinforcement learning is about
adaptive learning in response to stimuli from an
environment. Reinforcement learning is a field in psychology and in
artificial intelligence. Chapter~\ref{chap:rl} provides a formal introduction.

In AI a similar  discussion between  two schools of
thought  has taken place, as we have seen in
Section~\ref{sec:schools}. In AI, the concept of {\em symbolic\/} AI  
stresses the importance of logic reasoning, and assumes that
knowledge is grounded in the reasoning with and manipulation of symbols. Symbolic AI is inspired by
mathematical logic. On the other hand,
{\em connectionist\/} AI  regards
intelligence as emerging bottom up from interaction of artifacts with an
environment~\cite{nilsson2009quest,stone2016artificial}. Connectionism
is inspired by biology, specifically by the neurons and synapses that make up our
brain.

Surprisingly, the work in this book draws on both schools of
thought. Reinforcement learning looks at learning that occurs through
interaction with 
the environment, and neural nets are inspired by
biology. On the other hand, planning, and heuristic search, are 
from the logic reasoning side of AI.
%In self-play, the two schools of symbolic and
%connectionist  come together, achieving breakthrough success.
% 
The breakthroughs of Chess are mostly due to symbolic
AI. Breakthroughs in Atari are due to connectionism. Breakthroughs in
AlphaGo (and other self-play programs) 
in part~\ref{part:selfplay} rely on both schools of thought,
and their success is a success of an integrated approach to AI,
expressed in a reinforcement learning framework. For other combined
approaches, see~\cite{valiant2008knowledge,garcez2015neural}.


\section{Artificial Intelligence}
Artificial intelligence is old. There are indications that the first
ideas on mechanical thought are
as old as human 
thought. The first recorded dreams of intelligent machines  go back to Indian
philosophies 1500 BC~\cite{mccorduck2009machines,wujastyk2003roots}. In Greek the word
automaton means {\em acting on one's own will}. In Greek mythology,
Homer's Iliad describes automatons,  self-operating machines, that
open doors automatically. There are many more examples of automata in
Greek mythology,
such as an artificial person of bronze, or watchdogs of gold and
silver. In Chinese text mechanical engineers, or artificers, are
described, as well as artificial wooden flying birds~\cite{needham1965science,koetsier2001prehistory}.

By attempting to describe human thought as the mechanical manipulation
of symbols, classical philosophers were the first to describe ideas of
modern AI. This work on mathematical reasoning culminated in
the invention of the  digital computer in the 1940s. The advent of the
first computers  and the ideas 
behind it prompted  scientists to start serious
discussions on the possibility of creating an electronic brain. 


\begin{figure}[t]
\begin{center}
\includegraphics[width=12cm]{figures/dartmouth2}
\caption{Dartmouth AI Workshop 1956}\label{fig:dartmouth}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
\includegraphics[width=12cm]{figures/winter}
\caption{AI Winters~\cite{lim2018}}\label{fig:winter}
\end{center}
\end{figure}


The modern field of AI research was subsequently founded in the summer of 1956 at a
workshop at Dartmouth College, NH (see Figure~\ref{fig:dartmouth}). Among those present were John McCarthy, Marvin
Minsky, Nathaniel Rochester, Claude Shannon, Allen Newell, Herbert
Simon, Arthur Samuel, John Nash, and Warren McCulloch. These would all
become  leaders of AI research in the following decades. There
was  much optimism then,  and many predicted that human level  machine
intelligence would exist within 20
years (this was in 1956)~\cite{moor2006dartmouth,mccorduck2009machines}.  
Eventually, however, it became clear that they had  underestimated the
difficulty of this project. An AI winter followed in which funding for
AI research all but dried up (see
Figure~\ref{fig:winter}~\cite{lim2018}). The figure shows that despite
the funding drought, progress was made, and another period of inflated
expectations followed, followed by another winter. Achievements in the
1990s heralded the current AI summer that we are still enjoying. After 2000 interest in AI has been high
again, because of 
machine learning successes in search, vision, speech, robotics and
other applications in academia and industry. In fact, many other
inventions that were 
not expected did happen, such as search engines (what is the market
capitalization of Google and Baidu?), social networks (what is the
market capitalization of Facebook and Tencent?), recommender
systems (what is the market capitalization of Amazon, Alibaba and Netflix?) and
multi-touchscreen communicators (what is the market capitalization of
Apple, Samsung, and Huawei?).



\begin{figure}[t]
\begin{center}
\includegraphics[width=10cm]{figures/bhl3}
\caption{Geoffrey Hinton,  Yann LeCun and Yoshua Bengio}\label{fig:bhl}
\end{center}
\end{figure}

In 2018 the highest recognition in computer science, the Turing award,
was awarded to three key researchers in deep learning: Bengio, Hinton
and LeCun (Figure~\ref{fig:bhl}).\index{Yoshua Bengio}\index{Yann LeCun}\index{Geoffrey Hinton}


\subsection{Turing Test and General Intelligence}
Most AI researchers are interested in  intelligent behavior,  machines that
exhibit  reasoning, knowledge, planning, learning,
communication, perception, and the ability to interact with
the physical environment.  The focus is on behavior; by which methods the machines
exhibit this behavior is less relevant. Consciousness and self-awareness
are not (yet) on the mainstream agenda, and simulating the human brain is not part of
AI research.

In contrast to some parts of psychology, AI is less interested
in defining the essence of 
intelligence (``being intelligent'') as it is in intelligent behavior, with a strong focus on
creating intelligent systems. The AI approach is a pragmatic approach.

Note that the strict separation between behavior and being is
becoming somewhat less strict. The focus on behavior of AI fits
  the  school of symbolic AI especially well, where intelligence is based on
  human logic, and not on human hardware. The other school,
  connectionism, is emphatically inspired by biology and 
  neurology, i.e., a simulation of human hardware.


\begin{figure}[t]
\begin{center}
\includegraphics[width=10cm]{figures/turingtest}
\caption{Turing Test}\label{fig:turingtest}
\end{center}
\end{figure}


\subsubsection{Behavior: Turing Test}\index{Turing test}
In 1950 Alan Turing proposed a test on how to determine if a machine
exhibits  intelligence. The machine passes the test when its behavior
is indistinguishable from that of a human. In the Turing test a human
evaluator engages in a natural language conversation with a human
and with a machine (Figure~\ref{fig:turingtest}). The evaluator
is aware that one of the two participants  is a
machine, and both participants are separated from one another by a
screen.
Participants are restricted to text-only,  such as through
keyboard and screen (speech technology is deemed too hard).
If the evaluator cannot  tell which conversation is from the machine,
the machine is considered to have passed the test. Note that the
machine may make mistakes as long as they are mistakes that humans
would also make. The Turing test is an imitation game. It might even
be the case 
that making deliberate mistakes is a good idea, for example, when the
domain would be a game of Chess, then a Chess machine could be
identified by being much stronger than a human would be.

The paper that introduced the Turing test was titled: ``Computing
Machinery and Intelligence''~\cite{turing1950computing}.  It opens
with the words: ``I 
propose to consider the question, 'Can machines
think? `'' and is a classic in AI.   


           
\subsubsection{Specialized and General Intelligence}
Machines that are intelligent in a single domain, such as in Chess, are
said to have narrow or  special intelligence. Artificial
{\em general\/} intelligence (AGI) would be the intelligence of a machine
that can  perform any intellectual task that a human can. AGI is the
holy grail of  AI research, and a favorite  topic in science fiction and future
studies. AGI is sometimes called {\em strong AI\/} although that term
is used by some other researchers to mean machines that experience
consciousness~\cite{searle2008mind}.  

As of 2017, one study found that over forty organizations worldwide are doing active
research on AGI~\cite{baum2017survey}.

Most game playing programs still achieve high performance by focussing on
a single domain. This situation is slowly changing. In
Chapters~\ref{chap:plan} and \ref{chap:fast} we will see General Game Playing (GGP) and
AlphaZero attempt to achieve high performance (``true
intelligence'') in multiple domains: general intelligence.


\subsubsection{Limited Scope}
General intelligence is clearly a challenging goal. Although
ultimately intelligent behavior has to be measured in a real world
setting, the real world is complex, and might be too 
much of a challenge to master. Researchers typically choose to start with a model that
captures an essential and interesting aspect of reality, but is otherwise
simpler. For this reason, ever since the start of AI, games have played an important
role. The rules of the game limit its scope, making it  better
suited as a first object of study than the full complexity of reality.

\subsubsection{Drosophila Melanogaster}
In 1965, the Soviet mathematician Aleksandr Kronrod called Chess the
Drosophila Melanogaster of artificial intelligence~\cite{landis2001aleksandr}. Drosophila Melanogaster,
see Figure~\ref{fig:drosophila}, is a type of
fruit fly that is used by developmental biologists in genetics
experiments, because of its fast reproduction cycle. The fast
reproduction allowed quick experiments.
\index{Drosophila Melanogaster}

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/drosophila.jpg}
\caption{Drosophila Melanogaster (fruit fly)}\label{fig:drosophila}
\end{center}
\end{figure}

Such an experimenter's  tool with quick
turnaround times is  useful in AI research. Chess was a convenient domain
that was well suited for such experimentation. It is clearly a game
for which humans need 
intelligence, requiring many years of  dedication and study to achieve
proficiency.




%\subsubsection{Clear Rules}
In addition to having a limited scope, a second advantage of games is the
clarity of the rules.  Possible
actions are well defined by the rules and the end of a game is also
well-defined. In this, games differ from the 
real world, where goals and rules are often implicit and vague. Thus, games are
easier to solve than  real world tasks, a clear advantage for
researchers who want quick success.


\begin{figure}[t]
\begin{center}
\includegraphics[width=4cm]{figures/elo2}
\caption{Arpad Elo}\label{fig:elo}
\end{center}
\end{figure}


\subsubsection{Clear Performance}\label{sec:elo}
Games also allow for a clear and undisputed way to measure
progress. Game rules
define win and loss, and the intelligence of programs can be measured by
letting them play against each other or against humans. Many  games have
rating systems, such as in tennis, where the best of the world are
ranked based on how many wins have been scored against other
players. An often used measure is the  Elo-rating,
a system devised by the Hungarian-American physicist  Arpad Elo (see Figure~\ref{fig:elo}). The
basis of the Elo rating is pairwise
comparison~\cite{elo1978rating}.\index{Arpad Elo}\index{Elo} 

\subsubsection{Specific Intelligence}
In  the original Turing test {\em any\/} question
can be asked of the machine. It is a  test for General
Intelligence, the  kind of intelligence that humans have. Limiting
the scope of our domain to a single game clearly cannot be used for
the general Turing test, all we can hope for is to achieve special 
intelligence, the kind of intelligence needed to win a certain
game. Still, achievements in specific intelligence, such as by Deep
Blue, Watson and AlphaGo, attract large publicity. This may be in part
because the human mind generalizes easily, and
anthropomorphizes\footnote{I.e., treat as if human.}
easily. When we see a device do something in a particular domain for
which a human must be incredibly smart, we automatically assume that the device
must {\em be\/} smart, and will do  as well in another domain {\em
because that is what a human would do}. It is easy for  us to forget that the machine is
not a human, something that writers of science fiction books and
Hollywood movies eagerly exploit. Current machine intelligence is almost
always highly specialized, which is quite unhuman-like. 

% Indeed, one of the great challenges of AI is to create a machine that
% has general  intelligence, or at least has intelligence in more than one domain.
% The field of transfer learning studies how knowledge that is learned
% in one domain can be transfered to another
% domain. Chapter~\ref{chap:transfer} discusses transfer learning.
In
Chapter~\ref{chap:fast} the issues of artificial and human
intelligence will be revisited, including the topics of learning, and
specialized and general intelligence.  By then, we will have acquired a
deep understanding of how to create artificial intelligence in games.


%% Games are a suitable testbed for AI
%% experimentation~\cite{mandziuk2007computational}. The first 
%% game to be heavily studied was Chess,  the game of
%% intelligence par excellence. For this reason Kronrod named Chess the
%% Drosophila Melanogaster, or experimental testbed of choice, of AI. And
%% indeed, for many decades many researchers used it to their advantage,
%% developing many ingenious computational methods to
%% achieve a level of play, ultimately beating the strongest human minds
%% in the world.

%% Indeed, dedicated research groups  all over the world worked in Chess,
%% creating quick
%% progress. In just three decades the dream of beating the human world
%% champion was realized. On May 11, 1997 Garry Kasparov, then the highest
%% rated human chess player ever, was defeated by the computer
%% program \textsc{Deep Blue}, in a highly publicized six game match in
%% New York~\cite{hsu2004behind,schaeffer1997kasparov}.  


\section{Game Playing Programs}
% Then, a new Drosophila had to be found, which would become Go.
%
% But we are getting ahead of ourselves.
In order to get a good
understanding of the field, let us start with a short overview of some
of the better known game players in the history of AI. First we discuss two
hypothetical game players described only in scientific papers, and
then continue with the first real game playing programs. 


\begin{figure}[ht]
\begin{center}
\includegraphics[width=7cm]{figures/shannon}
\caption{Claude Shannon}\label{fig:shannon}
\end{center}
\end{figure}
\index{Claude Shannon}

\subsection{Claude Shannon 1949}
Claude Elwood Shannon (1916–2001, see Figure~\ref{fig:shannon}) was an
American mathematician, 
electrical engineer, and cryptographer. Shannon is primarily known as
the father of information theory (but he also knew how to juggle).  

In 1949 Shannon presented a paper titled ``Programming a Computer for
playing Chess.'' The paper describes a design of how to program a
computer to play chess based 
on position evaluation and move selection. The paper describes  strategies
for restricting the number of possibilities to be
considered. Shannon's paper is  one of the first articles
published on the topic of 
programming a computer to play chess~\cite{shannon1988programming}. 



\begin{figure}[ht]
\begin{center}
\includegraphics[width=11cm]{figures/ferranti}
\caption{Ferranti Mark 1}\label{fig:ferranti}
\end{center}
\end{figure}
\index{Ferranti Mark 1}

\begin{figure}[ht]
\begin{center}
\includegraphics[width=4cm]{figures/turing}
\caption{Alan Turing}\label{fig:turing}
\end{center}
\end{figure}
\index{Alan Turing}


\subsection{Alan Turing 1950}
In 1948 Alan Turing (1912-1954, see Figure~\ref{fig:turing}) worked with David Champernowne on  a chess
program for a computer that did not yet exist. They named their
program Turbochamp. In 1950, the program was finished. In 1952, Turing
tried to implement it on a Ferranti Mark 1, see Figure~\ref{fig:ferranti}, but the computer was
unable to execute the program, so he
executed the program by hand, flipping through the pages of the
algorithm and carrying out its instructions on a 
chessboard. Reportedly, this took about half an hour per move.
The program is the first to have played a full Chess game, even though it was
executed on paper and by hand~\cite{turing1953digital}. Turbochamp had an
evaluation function and a search function, a design that is still used
in today's programs.


\begin{figure}[ht]
\begin{center}
\includegraphics[width=4cm]{figures/strachey}
\caption{Christopher Strachey}\label{fig:strachey}
\end{center}
\end{figure}
\index{Christopher Strachey}


\subsection{Christopher Strachey 1951}
Christopher Strachey (1916-1975, see Figure~\ref{fig:strachey}) was a preeminent computer scientist
at Oxford, well known
for his work on denotational semantics and programming language
design. In 1951, Christopher Strachey wrote a Checkers program for the
Ferranti Mark 1 computer of the University of 
Manchester. It could play a complete game of Draughts (Checkers) at
reasonable speed~\cite{strachey1952logical}.

\begin{figure}[ht]
\begin{center}
\includegraphics[width=8cm]{figures/samuel}
\caption{Arthur Samuel}\label{fig:samuel}
\end{center}
\end{figure}
\index{Arthur Samuel}

\subsection{Arthur Samuel 1959}
Arthur Samuel (1901-1990, see Figure~\ref{fig:samuel}) started in 1949 to write a Checkers
 program
for the IBM 701 computer. It was among the world's first successful
self-learning programs, adapting coefficients in the evaluation function
based on the outcome of the search~\cite{samuel1959some}. 

The main driver of the program was a
search tree of the board positions reachable from the current
state. To reduce memory consumption Samuel implemented a version of what is now called alpha-beta pruning.
He used a heuristic evaluation function based on the position of the
board to prevent having to search to the end of the game. He also used
a method to memorize search results, and later versions used
supervised learning from professional games and from self play. Around
the 1970s the program had progressed to amateur level~\cite{schaeffer2008one}.





\begin{figure}[ht]
\begin{center}
\includegraphics[width=6cm]{figures/gtesauro_ai_350_2}
\caption{Gerald Tesauro}\label{fig:tesauro}
\end{center}
\end{figure}
\index{Gerald Tesauro}

\begin{figure}[t]
\begin{center}
\includegraphics[width=5cm]{figures/Backgammon}
\caption{Backgammon}\label{fig:bg}
\end{center}
\end{figure}

\section{Modern Game Playing Programs}
Playing strength of game playing programs has since increased
steadily. Computer hardware has become more powerful, and better
algorithms have been found. Most of these algorithms are described in
this book.

After the pioneers we will now skip a few years. We will pick up after 1990, where some
programs started  playing at world champion level. We  will
discuss these world champion programs now.

\subsection{TD-Gammon 1992}\index{TD-Gammon}
At the end of the 1980s Gerald Tesauro (see Figure~\ref{fig:tesauro}) worked on Backgammon
programs. Figure~\ref{fig:bg} shows a Backgammon board.


His programs were based on neural networks that learned good patterns of
play. His first program, Neurogammon, was trained using supervised
learning. It achieved an intermediate level of
play~\cite{tesauro1989neurogammon}. His second program,
TD-Gammon, was based on temporal difference learning and self-play, a form of
reinforcement learning (see Chapters~\ref{chap:rl} and \ref{chap:dqn}). Combined with hand
crafted heuristics, in 1992 it played at world-class human championship
level, becoming the first computer program to do so in a game of
skill~\cite{tesauro2002programming}. 

TD-Gammon updates  its
neural net after each move, reducing the difference between the
evaluation of previous and current positions. It uses a well-known method from
reinforcement learning called {\em temporal-difference
learning}, hence the name of the program. % The score of a position is a set of four estimates  of the
% likelihood that White wins normally, Black wins normally, White wins a
% gammon, or Black wins a gammon. For the final board position
% the algorithm compares to the actual result of the game.


In Tesauro's previous program  Neurogammon an expert trained the program by
supplying the "correct" evaluation of each position. In contrast,
TD-Gammon initially learned knowledge-free, or {\em tabula rasa}.
Tesauro describes TD-Gammon's self-play as follows: ``The move that is selected is  the move with maximum expected
outcome for the side making the move. In other words, the neural
network is learning from the results of playing against itself. This
self-play training paradigm is used even at the start of learning,
when the network's weights are random, and hence its initial strategy
is a random strategy.''~\cite{tesauro1995temporal}

The self-play version used
only a raw board encoding,  without any hand-crafted heuristic
features. It reached a level of play comparable to Neurogammon: that of an
intermediate-level human Backgammon player. By adding a simple
heuristic search it reached world-class level.

TD-Gammon's
success  inspired many other researchers to try 
neural networks and self-play approaches, culminating in recent high
profile results in  Atari~\cite{mnih2013playing} and
AlphaGo~\cite{silver2016mastering,silver2017mastering}  
(see Chapters~\ref{chap:dqn} and \ref{chap:plan}). 

Interestingly, a modern
reimplementation of TD-Gammon in TensorFlow is available on Github
\href{https://github.com/fomorians/td-gammon}{TD-Gammon}.\footnote{\url{https://github.com/fomorians/td-gammon}}

\begin{figure}[t]
\begin{center}
\includegraphics[width=7cm]{figures/schaeffer}
\caption{Jonathan Schaeffer}\label{fig:schaeffer}
\end{center}
\end{figure}
\index{Jonathan Schaeffer}

\begin{figure}[t]
\begin{center}
\includegraphics[width=4cm]{figures/tinsley}
\caption{Marion Tinsley}\label{fig:tinsley}
\end{center}
\end{figure}
\index{Marion Tinsley}


\subsection{Chinook 1994}
The Checkers program Chinook is the first computer program to win the
world champion title 
in a competition against humans. It was developed by Canadian Jonathan
Schaeffer, see Figure~\ref{fig:schaeffer}.
Based on his experience as a Chess player and programmer
 Schaeffer decided to write a Checkers program, 
believing that the technology existed to achieve world
championship level. 


Chinook's architecture follows the standard search-eval approach, based
on alpha-beta search and a hand-crafted heuristic evaluation function, both with
many enhancements (see Chapter~\ref{chap:idtt})~\cite{schaeffer1992world,schaeffer1996chinook}. Apart from meticulous
testing and tuning, Chinook derived much of its strength from its 
endgame database that contained perfect knowledge for any board
position with fewer than 8 pieces.\footnote{This endgame database
  technology allowed Schaeffer 
and his team to go on to solve the game and create a proof that Checkers, with perfect play, is a draw~\cite{schaeffer2007checkers}. 
\index{Chinook}
\index{Checkers}
}

Schaeffer started development in 1989. At first progress came
swift. In 1990 Chinook won the right to play in the 
human World Championship by being second to Marion Tinsley in the US
Nationals (see Figure~\ref{fig:tinsley}). Tinsley had reigned supreme for such a long time in
Checkers, that he enjoyed having a strong opponent again. % However, then controversy started, and the American
% Checkers Federation and English 
% Draughts Association ruled against the participation of a computer in a
% human championship. Tinsley, for his part, disagreed, and amazingly
% resigned his title in protest, since he wanted to play the computer so 
% much~\cite{schaeffer2008one}. The ACF and EDA then created the new
% title Man vs.\ Machine World Champion, 
% and the competition could proceed after all. Tinsley won with four wins to Chinook's
% two, with 33 draws. 


In  1994 Chinook was declared
the Man-Machine World Champion. In 1995, Chinook defended its
Man-Machine title against Don Lafferty 
in a 32-game match. The final score was 1–0 with 31 draws for Chinook
over Lafferty. At
the time it was rated at 2814 Elo. After the match, Chinook retired from competitive
playing. Later, Schaeffer and his team used Chinook to solve Checkers,
proving  in 2007 that with perfect play by both sides, Checkers is a
draw)~\cite{schaeffer2007checkers}.  


Chinook's win is made all the more impressive because of the
opponent: Dr. Marion Tinsley. Tinsley,
a professor of mathematics, played Checkers at a level that was
unheard of. He was
world champion from 1955–1958 and 1975–1991 and never lost a world
championship match, and lost only seven games  in his 45-year career,
two of which to  
Chinook~\cite{schaeffer2008one}. He withdrew from
championship play during the years 1958–1975, relinquishing the title
during that time. It was said that Tinsley was to Checkers what
Leonardo da Vinci was to science, what Michelangelo was to art and
what Beethoven was to music~\cite{madrigalcheckers}. Schaeffer
recalls  one particular event. In one game from
their match in 1990, Chinook, playing with white pieces, made a
mistake on the tenth move. Tinsley instantly remarked, ``You're going to regret
that.'' And, yes, after they played on, Chinook resigned after move
36, fully 26 moves later, when it saw its loss.  Schaeffer looked back into the database and
discovered that Tinsley picked the only strategy that could have
defeated Chinook from that point and Tinsley was able to see his win
64 moves into the future~\cite{schaeffer2008one}.

% In
% 1994 Chinook was declared the Man-Machine World Champion, a first in
% the history of AI.

\begin{figure}[ht]
\begin{center}
\includegraphics[width=5cm]{figures/hsu}
\caption{Feng-hsiung Hsu}\label{fig:hsu}
\end{center}
\end{figure}
\index{Feng-hsiung Hsu}

\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/garrykasparov}
\caption{Garry Kasparov}\label{fig:garrykasparov}
\end{center}
\end{figure}


\begin{figure}[ht]
\begin{center}
\includegraphics[width=8cm]{figures/DeepBlue_Team}
\caption{1996 Deep Blue Team: Chung-Jen Tan, Murray Campbell, Joe Hoane, Feng-hsiung Hsu, and Jerry Brody}\label{fig:team}
\end{center}
\end{figure}


\begin{figure}[ht]
\begin{center}
\includegraphics[width=11cm]{figures/kasparov}
\caption{Excitement in 1997. Game 6, Caro Kahn. Kasparov resigned
  after 19 moves}\label{fig:kasparov}
\end{center}
\end{figure}



\subsection{Deep Blue 1997}\label{sec:deepblue}\index{Deep Blue}
If the Checkers events caused excitement, then Chess did doubly so. In 1985
Feng-hsiung Hsu (see Figure~\ref{fig:hsu}), a PhD student at Carnegie
Mellon University, started work on a Chess program that, after much
development, showed enough promise for IBM to become involved.
After
quite some more years of development, performance had improved enough
for IBM to sponsor a match against the human world Chess 
champion Garry Kasparov (Figure~\ref{fig:garrykasparov}). The match
took place at the ACM Computer Science Conference in
Philidelphia. Figure~\ref{fig:team} shows a team photo from those days. On
February 10, 1996, Deep
Blue won its first game against human champion Kasparov, making Chess
history. However, Kasparov went on to win three games and draw two,
winning the six-game match by 4-2.


A year later, in May 1997, the rematch was played in New
York at the 35th floor of the Equitable Center (see
Figure~\ref{fig:kasparov}).\index{Garry Kasparov} An upgraded version of 
Deep Blue played Kasparov again, this time capable of evaluating 200
million positions per second, 
twice as fast as the 1996 version. Kasparov was defeated $3\frac{1}{2}-2\frac{1}{2}$
in a highly publicized match. Deep Blue became the first computer system to
defeat a reigning world champion 
in a match under standard Chess tournament time controls. Several 
accounts of the match, its historical significance, and the technology
behind it, have been
written~\cite{schaeffer1997kasparov,campbell2002deep,hsu1990grandmaster,hsu2004behind,levy1991computers,newborn2013deep}. 

Deep Blue started out as a hardware design project, when Feng-hsiung
Hsu wanted to see if he could create a
special purpose VLSI Chess move generator chip. This project evolved into a
full-fledged Chess program, which was named Deep Thought, after the 
fictional computer in Douglas Adam's {\em The Hitchhiker's Guide to the
Galaxy}, who computed the answer to Life, the Universe, and
Everything.\footnote{which, as you may know, is
42.}  After their 
graduation from Carnegie Mellon, Hsu, Thomas Anantharaman, and Murray
Campbell were hired by IBM Research to
continue their quest to build a Chess machine that could defeat the
world champion. IBM named the machine
Deep Blue.  Anantharaman subsequently left IBM
and Joe Hoane and Jerry Brody joined the team in 1990. %  The team was managed
% first by Randy Moulic, followed by Chung-Jen Tan.
Figure~\ref{fig:team} shows the Deep Blue team.  %After a
%scaled-down version of Deep Blue, 
%Deep Blue Jr., played
Grandmaster Joel Benjamin was signed up by IBM Research to
assist with the preparations for Deep Blue's matches against Garry
Kasparov.\index{Deep Blue}\index{Garry Kasparov}\index{Chess}\index{ChipTest}




The design of Deep Blue followed the standard search-eval architecture, with quite a
number of special enhancements. To start with, the evaluation function used 480
specially developed hardware chips, allowing it to evaluate 200 million
positions per second in parallel. The search algorithm was also heavily
parallelized, running on a 30 node IBM RS/6000 system.
Deep Blue  would
typically search to a depth of 6-8 moves and to a
maximum of more than 20 moves in some situations.
The opening library was provided by grandmasters Miguel Illescas, John
Fedorowicz, and Nick de Firmian. It had an endgame database of
positions with 5-6 pieces.

Deep Blue's evaluation chips were highly customizable, containing
8000 individual parts, and a database of master games was used to tune their
weights.  
The success of Deep Blue was rightfully billed as the success of
brute force, due to the impressive number of 200 million evaluations
per second. However, the fact that the evaluation weights were
initially tuned by supervised learning, and not by hand, would equally
allow a claim to a victory  due to machine learning (although it did
not use neural nets nor did {\em Deep\/} Blue use {\em deep\/}
learning).
% One of its  
% developers even disclaimed that it was artificial intelligence at
% all.   When a technology becomes sufficiently well understood, it ceases
% to be AI.



Before the matches, Kasparov could not practice against Deep
Blue to familiarize himself with the play style of the
computer. However, Kasparov did study many popular PC  
games to become familiar with computer game play in general.

Kasparov was quite upset during the match.
After the loss in game 2, he said that he sometimes saw ``deep intelligence
and creativity'' in the machine's moves, implying  that during the
second game, humans had intervened on behalf of the
machine. IBM denied, saying the only human intervention occurred {\em between\/}
games, but not {\em during\/} games. The rules allowed the developers
to fix errors between rounds, 
an opportunity they  used, and which may have caused apparent
differences in play 
style between games. % Kasparov requested printouts of the machine's log files,
% which were subsequently published on the
% Internet. In 2003 a documentary film was made that explored these
% claims. Entitled Game Over: Kasparov and the Machine, the film
% interviewed some people who suggest that Deep Blue's victory was a
% ploy by IBM to boost its stock value.


In its time, Deep Blue, with its capability of evaluating 200 million positions per
second, was the fastest computer to face a world chess
champion. Since then, the focus has shifted to
software, rather than using dedicated chess
hardware. Chess algorithms have progressed, and modern chess programs
such as Stockfish, Houdini, or Deep Fritz are more efficient than the
programs of Deep Blue's 
era. Today less hardware is needed to achieve the same performance. In a
November 2006 match between Deep Fritz and world chess 
Champion Vladimir Kramnik, the program ran on a computer system
containing one dual-core Intel Xeon 5160 CPU, capable of evaluating only
8 million positions per second, but searching to an average depth of
17 to 18 plies in the middlegame, thanks to fast heuristics and search
extensions (see Chapter~\ref{chap:idtt}).\index{Stockfish}
Stockfish is currently one of the strongest Chess programs. It is open
source, available on Github 
\href{https://github.com/official-stockfish/Stockfish}{here}.\footnote{\url{https://github.com/official-stockfish/Stockfish}} 

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/othello}
\caption{Othello}\label{fig:othello}
\end{center}
\end{figure}
\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/mburo}
\caption{Michael Buro}\label{fig:buro}
\end{center}
\end{figure}\index{Michael Buro}

\subsection{Logistello 1997}
\index{Logistello}\index{Othello}
Logistello is a computer program that plays the game of Othello, also
known as Reversi. Logistello was written by Michael Buro  (see
Figure~\ref{fig:buro}) and is
  a very strong player, having beaten the human world champion
Takeshi Murakami with a score of 6-0 in 1997. The best Othello programs
are now much stronger than any human player.

Logistello's evaluation
function is based on disc patterns and has over a million
numerical parameters which were tuned using  advanced logistic linear regression~\cite{buro1997othello,buro1995logistello,buro2003evolution}. 



\begin{figure}[ht]
\begin{center}
\includegraphics[width=4cm]{figures/david}
\caption{David Silver}\label{fig:silver}
\end{center}
\end{figure}
\index{David Silver}


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/go}
\caption{Go Board}\label{fig:go}
\end{center}
\end{figure}

\subsection{AlphaGo 2016}\index{AlphaGo}\index{Go}

After the 1997 Chess match Go (Figure~\ref{fig:go}) became the next  Drosophila of AI, the benchmark
game, and research interest intensified.

Traditionally, computer Go programs followed the conventional Chess
setup of alpha-beta search with an influence-based heuristic evaluation
function. The GNU Go program is a good example of this
approach~\cite{millen1981programming}\index{GNU Go}. The Chess
approach, however, did not work for Go. The level of play
was stuck at mid-amateur level for quite some time.

However, the game
of Go worked very well as Drosophila. 
Many researchers have produced  interesting findings. New
algorithms have been developed, such as Monte Carlo tree search, % there
% is much interest in the theory of
% multi-armed bandits,
progress has been made
in supervised learning and reinforcement learning, and neural networks
are actively used.  In 2015-2017 the DeepMind AlphaGo team, headed by
David Silver (see Figure~\ref{fig:silver}) played three matches
beating all human champions that it played. %  Finally, computer self play has
% been shown to be able to learn the game of Go from scratch in a period
% of days, something that takes humans years of hard study. On the
%  domain of Go, computers have now out-learned humans.
 Books are
being written analyzing the theoretical innovations that AlphaGo has
unlocked for human Go masters.


We will cover all these developments in quite some depth in this
book. Chapter~\ref{chap:trial} covers the search algorithm, Chapters~\ref{chap:super} and
\ref{chap:dqn} cover machine learning, and
Chapter~\ref{chap:plan} goes in depth into self play.

Appendix~\ref{chap:go} contains a brief tutorial on the rules of Go.

\subsection{Poker 2018}\index{Poker}
In contrast to board games such as Chess, Checkers, and Go, Poker is a
card game. Since some of the cards are hidden from the player, it is
a game of imperfect information. Because of this,  computing 
the possible moves is much more difficult. This has held back the
development of strong Poker programs for some time.

\begin{figure}[t]
\begin{center}
\includegraphics[width=6cm]{figures/bowling}
\caption{Michael Bowling}\label{fig:bowling}
\end{center}
\end{figure}\index{Michael Bowling}

\begin{figure}[t]
\begin{center}
\includegraphics[width=35mm]{figures/sandholm}
\caption{Tuomas Sandholm}\label{fig:sandholm}
\end{center}
\end{figure}\index{Tuomas Sandholm}

Recently, however, impressive progress has been made by groups from
Alberta headed by
Bowling~\cite{bowling2015heads,bowling2009demonstration,moravvcik2017deepstack}
(Figure~\ref{fig:bowling}) and CMU headed by
Sandholm~\cite{sandholm2010state,brown2018superhuman}
(Figure~\ref{fig:sandholm}) in heads-up (2 person)
variants of Poker. Programs DeepStack and Libratus have defeated some
of the strongest human Poker players in one-on-one
play~\cite{brown2018depth}.\index{DeepStack}\index{Libratus} Tuomas
Sandholm is the 2003 recipient of the IJCAI Computers and Thought award.

% At the basis of the Poker players is a method called counterfactual
% regret minimization (CFR)~\cite{zinkevich2008regret}\index{CFR} that determines the best possible strategy by letting it play
% itself recursively (somewhat like the MCTS algorithm in perfect
% information games).


Research in computer Poker is an active field, with versions of
research programs  being licensed for commercial entertainment
purposes. Section~\ref{sec:poker} provides more information on the
Poker methods.


\begin{figure}[t]
\begin{center}
\includegraphics[width=10cm]{figures/starcraft}
\caption{StarCraft}\label{fig:starcraft}
\end{center}
\end{figure}\index{StarCraft}



\subsection{StarCraft 2018}\index{StarCraft}\index{AlphaStar}
StarCraft is a popular real time strategy video game.  It combines imperfect
information with multi-player aspects,  long term strategy and
tactics. The imperfect information aspect is that the game map is only
partially visible, and the actions of the other players are not all
known. Armies have to be build up (strategy) and battles have to be
played (tactics).

StarCraft combines imperfect information, multi-player, strategy and
tactics. It combines more aspects of real life in a single
game than games such as Chess or Poker. StarCraft is  a popular game, with
strong human 
champions. For these reasons researchers have become interested in
using the game as a testbed for AI. Since 2010 academic competitions
have been organized, that stimulated much research~\cite{togelius2010multiobjective,ontanon2013survey}.  In 2017, DeepMind
and Blizzard together have created an easy to use Python interface to
the game~\cite{vinyals2017starcraft}.

In 2018 DeepMind's player AlphaStar played two-person test matches
against some of the world's strongest players, which it
won~\cite{alphastar2018}. StarCraft is becoming an active field of
research, and more research on StarCraft can be expected.

Section~\ref{sec:starcraft} provides more information on StarCraft
methods.

\section{Summary}
In this chapter we started by discussing key aspects of AI:
recognition, reasoning, memory and learning. AI takes a behavioral
approach to intelligence, which is operationalized with the Turing
Test, introduced by Alan Turing in 1950. We then proceeded with a
brief history of AI, starting with the 1956
Dartmouth College workshop. A list of ambitious goals for AI were
formulated, which turned out to be overly ambitious, causing an AI
winter. However, after research picked up by the turn of the
millennium, a number of  AI 
technologies (such as search, social networks, deep learning, and recommender
systems) had deeply affected society. 


Games have been a favorite test-bed for AI research. Games such as
Chess and Go have been called the Drosophila of AI, after
the fruit fly from genetics research. 
An important difference between human intelligence and artificial 
 intelligence is that human intelligence is general, and
artificial intelligence is special. Human intelligence can solve many
problems, an AI program can solve only one, such as playing good
chess. Research is under way into artificial general intelligence. 

The chapter provided a short overview of important designs and
programs. We listed the early designs by Shannon, Strachey, Turing, and Samuel. The
programs featured were TD-Gammon (Backgammon), Chinook (Checkers),
Deep Blue (Chess),  Logistello (Othello), AlphaGo (Go), Libratus and
DeepStack (Poker) and AlphaStar (StarCraft). 

Games are a favorite experimenter's tool for AI.
Many breakthroughs in intelligence and learning have taken place in a
variety of games, each with their own characteristic.

The early designs established some of the basic algorithms and
approaches, such as the search-eval architecture, minimax, alpha-beta,
heuristics, and learning. Computers were not yet powerful enough to
reach strong levels of play. The later programs all did, using highly
enhanced versions of the original blueprints, as well as new
techniques, such as deep learning.

In the following chapters we will look in detail which techniques are
used to achieve the breakthrough performance reported so widely in the media and
the research articles. 




\section*{Historical and Bibliographical Notes}
We conclude each chapter with a brief summary of entry points to the
scientific literature. The works mentioned here may be more accessible
than some of the more technical papers, in which you can find all
details. 

In this chapter we now list  three such works. An excellent popular and
all-encompassing standard text book of AI is Russel and
Norvig~\cite{russell2016artificial}. If you have taken an undergraduate
course in AI, chances are that you already own a copy.

A highly
accessible popular psychology book is Thinking Fast and Slow by
Kahneman~\cite{kahneman2011thinking}. Kahneman is one of the founders of
the field of behavioral economics, and his approach to intelligence
fits well with the search-eval architecture that is prevalent in
artificial intelligence in games.

Game playing programs solve reinforcement learning problems. 
A standard work for reinforcement learning is Sutton and
Barto~\cite{sutton2018introduction}. The recent  second
edition is even more comprehensive than the first edition. Sutton and
Barto divide reinforcement learning into exact tabular methods and approximate
methods. This distinction maps nicely to Kahneman's categories of
thinking Slow and thinking Fast, and Shannon and Turing's search-eval
architecture.

Insightful and entertaining accounts have been written about the human
and scientific side of writing world champion level game playing
programs. Schaeffer's account, now in its second edition, of how he
and his team created Chinook, is especially memorable, not just
because of his side of the story, but also because of the picture that
it paints of Marion Tinsley, the amazing Checkers
champion~\cite{schaeffer2008one}. 

Much has been written about the Chess match between Deep Blue and Garry
Kasparov. Feng-hsiung Hsu's account gives the story behind their ``quest
to build the mother of all Chess machines.'' It is an awe-inspiring
story of this moment in the history of Chess-playing intelligence
versus computer programming intelligence~\cite{hsu2004behind}.

A good reference on how computers play Chess is
\cite{levy1991computers}, and Chapters~\ref{chap:search} and
\ref{chap:idtt} cover much of the techniques that are used in Chess programs.






==> chapters/org08dqn.tex <==

% %% 5: dqn
% %% section: generalizing states, net based, fucntion approximation, feature learning, representaion learning, deep learning
% %% section: dqn: deep reinforcement learning
% %% *section: Atari papers, Gym, optimal control dynamic systems
% %% *section: rainbow enhancements to DQN
% %% section: system 1 and system 2: this is system 1
% %% section: go layers in keras


% The topic of this chapter is deep reinforcement learning. As in
% supervised learning, great advances have been made in recent years,
% stimulating AI research immensely.

% The structured  state space, and the relation with long range
% credit assignment, are  major challenges, especially since we work
% with approximation due to the size of the state space.  In this
% chapter we show how stable policy learning can be achieved. %  despite
% % long range credit assignment, despite correlated states, and despite
% % the large size of the state space.

% Supervised learning infers a classification function from a database of
% example-label pairs. Reinforcement learning infers a policy or value
% function from state-action or state-value
% pairs. It has no database of
% examples, but is provided with an environment. Reinforcement learning
% is learning by interaction with its environment. 

% In  supervised learning states and rewards are present in pairs, in reinforcement learning  the distance between rewards and
% states is large. There are no labeled images, only rewards that may
% have to be propagated over many states before they reach the goal state. Due to
% this long distance deep approximate reinforcement learning can be unstable.
% Achieving a stable policy training process is a non-trivial
% problem.

% In this chapter we will see compelling examples of how  stable training has
% been achieved in a deep Q-learning network (DQN). This was achieved on
%  end-to-end
% policy training  of classic Atari arcade games, such as Space Invaders.

% %\section*{Learning Goals}
% The learning goals of this chapter are to understand stable training
% of  end-to-end reinforcement learning. How  can it learn concepts that 
% are better than hand-crafted features, overcoming a ``deadly triad'' of
%  off-policy learning, bootstrapping, and function approximation? 
% End-to-end training is training from pixels to joystick action,
% without any intermediate handcrafted features to ``help'' the training.


% \begin{table}[ht]
% \begin{center}
% \input diag/searcheval
% \caption{Search-Eval Architecture}\label{tab:architecture8}
%   \end{center}
% \end{table}





% Unfortunately,  training function approximators in reinforcement
% learning can be unstable. % Sutton and Barto~\cite{sutton2018introduction} mention the ``deadly triad'' of
% % function approximation, off-policy learning, and value
% % bootstrapping as a cause of the instability.
% The goal of this chapter is to show through which
% methods stable deep reinforcement learning has been
% achieved.%\index{deadly triad}

% % This chapter will not introduce new search methods, it will only be
% % concerned with state evaluation.

% %% The previous chapter introduced us to function approximation with
% %% neural networks. The chapter covered supervised learning, an important
% %% learning method that assumes a database of labeled examples. The topic
% %% of this chapter is  reinforcement learning, where agents learn
% %% control actions through interaction with their 
% %% environment. In reinforcement learning each sample of the environment
% %% comes at the cost of an interaction. One of the 
% %% defining features of reinforcement learning is delayed rewards
% %% calculation. We will see the that  reinforcement learning in
% %% deep networks can converge, with the DQN algorithm, short for deep Q-learning network.

% %% {\bf now I have said it 3 times. need to consolidate texts}

% To orient ourselves, how DQN fits in the big picture, the search-eval architecture is shown again in Table~\ref{tab:architecture8}.
% The goal of function approximation in most reinforcement learning
% problems is to find a value function or a
% policy function that
% maximizes reward. (In most supervised learning problems the goal is to
% minimize categorization error.) Deep learning will do this through
% the formation of  features of 
% high dimensional states in a state space  that is so large
% that not all states will be seen for training. In Chapter~\ref{chap:search} 
% this was done with hand-crafted heuristics. Chapter~\ref{chap:trial}
% used averaged random samples, and Chapter~\ref{chap:super} 
% employed generalizing neural nets.

% \section*{Core Problems}
% \begin{itemize}
% \item Size of state space for end-to-end learning
% \item Unstable learning
% \end{itemize}

% \section*{Core Concepts}
% \begin{itemize} 
% \item End-to-end Policy Learning, Deep Q-learning Network (DQN)
% \item Stable long range credit assignment,  Deadly Triad, Replay Buffer.  
% \end{itemize}

% Let us now look at deep Q-networks, or DQN.


\section{Deep Reinforcement Learning}\index{DQN}
\label{sec:dqn}
Deep reinforcement learning is one of the success stories of
artificial intelligence. Before it became a success, there were quite
some obstacles that had to be overcome. In this section we will
discuss these problems and the methods that have been found to address
them.




story:
hand crafted features does not work
end-to-end requires scale up
scale up requires approximation
approximation cause unstable search due to deadly triad: correlations
between states, and approximation causing loops
solved in part by replay buffer to break correlations
and infrequent weight updates
and many more (rainbow)


There are two important differences between supervised learning and
reinforcement learning: (1) the way that information is presented 
(database or  interaction) and (2) whether the
information is present for all or for some states.

First, supervised learning can infer a  function for a database of 
example-label pairs, when the ground truth is given. Reinforcement learning infers a function for state-action 
pairs. It has no fixed database of
examples with ground truth labels. Positive or negative rewards are only
provided after interaction with an environment. The set of examples is
not fixed, and may change from learning process to learning process. 

The second difference is that in supervised learning ground truths are
present for all 
example-label pairs. The state space is fixed  and dense, and stable learning
methods have been devised. In reinforcement
learning problems the state space is often sparse,  the outcome of an action may only be known after many
further steps, and the rewards are
only available for some of the state-action pairs. For other
state-action pairs the rewards may
have to be propagated over a long distance of intermediate states
before the reward of a state-action pair is known. This gives rise to
the credit assignment 
problem, and, as we shall see in the next section, some
forms of reinforcement learning may be unstable. For deep
reinforcement learning, achieving a stable  training process is
a non-trivial 
problem.

Also note that the functions to be learned are different. In
supervised learning  a classification function is typically learned. In
reinforcement learning the function is a policy or a value function.

Achieving stable deep learning has long been a challenge, yet, as we
will see in this chapter, in recent years  compelling examples of how  stable training has
been achieved in a deep Q-learning network (DQN), with
policy training  of classic Atari arcade games, such as Space Invaders.

%% We are concerned with the problem of intelligent decision making in
%% complex situations. The search-eval architecture separates this
%% problem in a search and an eval part. Please refer to Table~\ref{tab:architecture8}.

%% For search, we progressed from
%% smart enumeration of the states to adaptively selecting promising
%% states and speculatively exploring new states.

%% For eval, we progressed from manually coded domain specific
%% heuristics, to machine learned function approximators, provided enough
%% labeled examples were available, and enough compute power. In this
%% chapter we will see how learning a function approximator of the state value
%% is  possible in reinforcement learning. 


%% Function approximation of states is highly valuable for large state
%% spaces in
%% reinforcement learning, as was already mentioned in
%% Section~\ref{sec:approx}. It allows value functions and policy 
%% functions to be approximated, which can then be used in
%% planning algorithms such as MCTS.

%% Unfortunately, translating the successes of supervised learning to
%% reinforcement learning is not straightforward. In reinforcement learning there
%% is no label available 
%% for each training state. All we have is an environment with which we
%% can act to receive delayed reward feedback, to learn about the world. 
%% Furthermore, reinforcement learning is unstable or divergent with a
%% nonlinear function approximator. 

%% In this chapter we will discuss one example where a method was found
%% to approximate state functions in reinforcement learning successfully:
%% Atari.




%\section{RL: No Labels, only Action-Rewards}

\subsubsection{Delayed Credit Assignment in Deep Reinforcement Learning}
An essential difference between supervised learning and reinforcement
learning is that  credit assignment is
delayed. In supervised learning for each training example an immediate
output label is available, allowing an error function to be
calculated, and weights to be adapted. In reinforcement learning 
output signals from the environment are infrequent or delayed, may be
``polluted'' by old values, and are calculated using values from
other states that may be approximated. When the path between state and
reward 
is long,  the effect of small amounts of noise in the propagated rewards accumulates
quickly, unstable learning may follow,  and the network may learn no
useful information. 
The Bellman equation specifies how values
should propagate. However, when function values are 
approximations, % and, worse, when values between different states are
                % correlated, 
then   Bellman updates may not converge to the correct 
value.  Indeed, as we shall further discuss in
Section~\ref{sec:stable}, it was shown that the combination of off-policy
learning, non-linear function approximation and bootstrapping may
cause the learning process to
diverge~\cite{tsitsiklis1997analysis,baird1995residual}. Since in reinforcement learning training examples are generated
in interaction with the environment, divergent training processess
have consequences for the set of training examples. In unstable
reinforcement learning the training set is not fixed, but of
undetermined size, and changing. The size of the
training set may be infinite or vary in size, as the training process
itself influences which examples are generated. 

\subsubsection{TD-Gammon and Stable Training}\index{TD-Gammon}
Interestingly,  the success of TD-Gammon~\cite{tesauro1995td}
suggested that there must be ways around instability. 
TD-Gammon's training did converge.\footnote{Note, however,
that TD-Gammon used shallow learning.} It used a temporal difference
algorithm similar to Q-learning, approximating the value 
function with a shallow neural network with one hidden layer, based on
heuristic features. Of course, TD-Gammon's success
prompted attempts with TD-learning in Checkers~\cite{chellapilla1999evolving}, and Go~\cite{sutskever2008mimicking,clark2014teaching}. The
success could not be replicated in these games, and it was believed
for some time that Backgammon was a special
case well-suited for reinforcement learning and
self-play~\cite{pollack1997did,schraudolph1994temporal}.  One
suggestion was that perhaps the randomness of the dice 
rolls helped exploration 
and smoothing of the value function of the state space.


However,   there have also been a few reports of early successful
applications of deep neural networks  in a reinforcement learning
setting~\cite{heess2012actor,sallans2004reinforcement}. Of course, the 
results in Atari (2013) and Go (2016) have now provided clear evidence that stable
and general reinforcement learning is possible. (See also the
historical and bibliographical notes of this chapter.)

Let us now look in more detail into the Atari 2600 experiments.

\subsection{Atari  2600  Games}


%\section{Search-Eval Architecture}



\begin{figure}[t]
\begin{center}
\includegraphics[width=4cm]{figures/mnih}
\caption{Volodymyr Mnih}\label{fig:mnih}
\end{center}
\end{figure}


%\section{Evaluation by Generalization}
Learning actions
directly from high dimensional sensory inputs such as sound and vision
is one of the long standing challenges of AI. In 2013, one year after the AlexNet
success in supervised learning, a paper
was published that took the reinforcement learning  works a major step
further. Mnih et al.~\cite{mnih2013playing} 
published a ground breaking work on {\em end-to-end\/} reinforcement
policy learning in Atari games. Their work is end-to-end in the sense that they 
learn joystick actions directly from the  visual state, the raw pixels, without the
intermediate step of hand crafted heuristic features, as has been done
before. The network was named DQN, for Deep-Q-network. Figure~\ref{fig:mnih} shows a picture of Volodymyr Mnih.


\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{figures/console}
\caption{Atari 2600 Console}\label{fig:console}
\end{center}
\end{figure}



Mnih et al.\ applied deep learning to play 1980s Arcade
Atari 2600 games, such as Space Invaders, Pong, and Breakout, directly
from the raw television screen pixels. Figure~\ref{fig:console} shows
a picture of the Atari 2600 console, and the joystick. % The Atari games are  both
% challenging for  
% researchers and well known to the general public.

Being able to close the loop
from from pixels to best play is a major achievement. For six games
Mnih et al.\ were able to
achieve human level of play in their original 2013 workshop paper. In a follow up article in 2015 
they improved on their  work and were able to achieve a level of play
equal to humans for 49 of the games that were in the test
set~\cite{mnih2015human,bellemare2013arcade}.

It should be noted that there are a few Atari games that proved
difficult to achieve strong play at. Notably  games
that required more long range planning, such as Montezuma's Revenge, were a
problem. Delayed credit assignment over long periods is still
hard.\index{Montezuma's Revenge}\label{sec:montezuma}

Nevertheless, a single architecture was able to successfully learn
control policies for many different games. Minimal prior knowledge was
used, and the neural network only processed the pixels and the
game score. The same network architecture and training procedure was
used on each game. 


%\section{Deep Q Learning}.

\subsubsection{Arcade Learning Environment}\index{Atari}\index{ALE}
The impressive results  by Mnih et al.\ stimulated much further work in the area of
deep reinforcement learning. Successful end-to-end reinforcement
learning created much interest among  researchers, and many related
algorithms were developed. We
will  look into some depth into their methods and 
experiments.

The games that were used for DQN are from a standard benchmark, the
Arcade Learning Environment (ALE)~\cite{bellemare2013arcade}. ALE  is a 
testbed designed to provide challenging reinforcement learning
tasks. Among other things it contains an emulator of the Atari 2600
console, a gaming console first marketed 
in 1977 (see Figure~\ref{fig:console}). ALE presents agents with a high
dimensional\footnote{That is, high dimensional for machine
  learning. $210\times 160$ pixels is not exactly High Definition
  video quality.} visual input
($210\times 160$ RGB video at $60$Hz) of tasks that were designed to
be interesting and challenging for human players (see
Figure~\ref{fig:atarigames}). The game cartridge ROM typically holds
the game code (2-4 kB), while the console RAM is small, just 128
bytes. This is not a typo, really only 128 {\em bytes}.
The actions can be input via a joystick, and a fire button (18 actions).


\begin{figure}[t]
\begin{center}
\includegraphics[width=10cm]{figures/atarigames}
\caption[Atari Games]{Screenshots of 4 Atari Games (Breakout, Pong, Montezuma's Revenge, Private Eye)}\label{fig:atarigames}
\end{center}
\end{figure}


The original experiments were performed with seven Atari games. Training was performed on  50 million frames in total.


In their 2013 work~\cite{mnih2013playing} the neural network performed better than an expert human
player on Breakout, Enduro, and Pong. On Seaqest, Q*Bert, and Space
Invaders performance was far below that of a human. In these games a
strategy must be found that extends over longer time periods. In their
2015 work~\cite{mnih2015human} the net performed better than human level play in 29 of 49
Atari games. Again, games with longer credit delay were more
difficult. 



Let us look in more detail at the network architecture of the 2013
 experiments.

\subsection{Network Architecture}
The Atari task is a control task: the network trains a behavior policy directly from
pixel frame input. The task of processing raw frames involves a high
computational load. Therefore, the 2013 training architecture contains a
number of reduction steps. 
The network that is used consists of three hidden layers, which is simpler
than what is used in most supervised learning tasks.

The images are high dimensional data. Since working with the full resolution
of $210\times 160$ with 128 colors at 60 frames per second would be
 computationally too
intensive,  the images are preprocessed. The 
$210\times 160$ with $128$ color palette is reduced to gray scale and
$110\times 84$ pixels cropped to $84\times 84$. The first hidden layer convolves
16 $8\times 8$ filters with stride 4 and ReLU. The second hidden layer
convolves 32 $4\times 4$ filters with stride 2 and ReLU. The third
hidden layer is fully connected and consists of 256 ReLU neurons. The
output layer is also fully connected with one output per action (18
actions for the joystick). The outputs correspond to the  Q-values of
the individual action. The network receives the change in game score
as a number from the emulator, derivate updates are reprocessed to $\{-1,0,+1\}$ to indicate
decrease, no change, or improvement of the score (Huber loss~\cite{openaibaseline2017}).


To reduce
computational demands further frame skipping was used. Only one in
every 3-4 frames was used, depending on the game.
For history, the net takes as input the last four resulting frames,
allowing movement to be seen by the net.
As optimizer RMSprop was used.
A variant of $\epsilon$-greedy is used, that starts with an $\epsilon$
of 1 (exploring) going down to $0.1$ (90\% exploiting).

The network architecture consists of convolutional layers and a fully
connected layer. Convolutional nets are  shift-invariant feature recognizers.
Fully connected nets allow $n\times m$ mapping. The feature
recognizers together with the $n\times m$ mapping allow mapping of
any feature (shape) to any action. 



\section{Stable Training}\label{sec:stable}
% An early success of reinforcement learning is TD-Gammon, Tesauro's
% backgammon playing program that played at world champion
% level~\cite{tesauro1995td}. TD-Gammon learnt to play  backgammon by
% reinforcement learning and self-play. It did so using a simple neural network
% with one hidden layer.
Deep Q-learning is a search process where the training examples to be
used are influenced by the search itself, introducing the possibility
of unstable or self-reenforcing learning. Dealing with divergence and
instability of the search is of prime importance in DQN.

As noted before, attempts to follow up on TD-gammon's success with
neural nets and 
self-play in  Checkers and Go were not
successful at first.

Much research into stability of reinforcement learning has been
performeed. We will discuss the deadly triad, long range credit assignment,
correlation between states, and fluctuations in the data distribution.

\subsection{Deadly Triad}
Tsitsiklis and Van Roy~\cite{tsitsiklis1997analysis}
showed in 1997 that combining off-policy reinforcement 
learning with non-linear function
approximators (such as neural networks)  could cause
the training to diverge. Deep reinforcement learning combines
bootstrapping, function approximation, and often also off-policy learning. Sutton and Barto~\cite{sutton2018introduction} call the combination of
bootstrapping, function approximation and off-policy learning the
{\em deadly triad}, because these three together cause instability in the
training process. For some time, most further research  in reinforcement
learning focused on linear function approximators, which have 
better convergence guarantees. 



{\em Function approximation\/} may have inaccuracies in the
attribution of values to states. Whereas exact methods are designed to
recognize individual states, neural networks are
often designed to recognize individual features of states. These features may be
shared by different states, and values attributed to those features
are shared as well by states. In a reinforcement learning process
where new states are generated on the fly, this sharing of values among states may cause 
loops or 
other forms of instability. If the accuracy of the approximation of
the true function values is good enough, then states may be identified
well enough to prevent most loops or divergent training processes. 

{\em Bootstrapping\/} of values increases the efficiency of the training because
values do not have to be calculated from the start, but previously
calcuated values are reused. Bootstrapping is at the basis of the
recursive Bellman equation. However, errors or
biases in initial values may persist, and even spill to other states,
as values are propagated Bellman-style, and error values become
correlated between states. With function
approximation inaccuracies in values are alomst guaranteed. Bootstrapping can thus lead to unstable learning,
and training loops getting stuck in one area of the state space.

An example of training getting stuck in Chess can be the
following. Imagine a program 
that knows everything about center control but 
nothing about king safety, and therefore looses if it encounters a differently
trained agent that will outplay it in the king-safety domain. We can
try to counter this effect by preventing 
correlations between states in the training set in some way, as we
will see soon.

{\em Off-policy\/}  learning uses a  behavior policy that is different from
the target policy (see Section~\ref{sec:off-policy}). When the target
policy is improved, the off-policy 
values are not, and the algorithm does not converge by this
action. Off-policy learning converges generally less well than
on-policy learning, especially when combined with function
approximation~\cite{sutton2018introduction}. 


% 0. deadly triad, work by sutton \& tsitsiklis after TD (on-policy)
% (approximation mixes states causing loops and instability,
% bootstrapping uses old values to build 
% on: bias which may through approximation spill to other states as
% well, off-policy keeps old errors preveting convergence)


% - approximation
% what goes wrong?
% mixes the targets of different states
% what can we do about it?
% hope that states are similar enough that they deserve similar targets

% - bootstrapping
% what goes wrong?
% tunnelvision. you strap yourself in a certain direction, the initial
% values determine much of the rest of the expansion process
% what can we do about it?
% uncorrelate choice of successors, make sure entire state space is
% explored

% - off policy learning
% what goes wrong?
% follows behavior distribution that explores, that are not updated and
% thus not converge
% may stay in old and existing areas of state. convergence problems
% updates off the target policy
% what can we do about it?
% only update the target policy (on policy)

% Furthermore, it was shown that combining model-free reinforcement
% learning algorithms such as Q-learning with non-linear function
% approximators [25], or indeed with off-policy learning [1] could cause
% the Q-network to diverge. Subsequently, the majority of work in
% reinforcement learning focused on linear function approximators with
% better convergence guarantees [25] \cite{tsitsiklis1997analysis}

Especially when training takes place in an environment where the
distance of credit assignment is long, the consequences of the deadly
triad may preclude stable learning to occur. 

\subsection{Long Range Credit Assignment}
A defining feature of reinforcement learning is long range credit
assigment. Long range credit assignment presents
a great challenge for deep reinforcement learning, because of the
deadly triad. % In reinforcement learning credit assignment is
% a challenge. There can be a long delay between actions and resulting
% rewards.
The Bellman equation provides an update rule how to
propagate reward values through the state space. In the tabular case
these intermediate credit assignments will 
always arrive at the correct state, since all states are uniquely
stored in the table data structure.

When the state space is too large for tables, methods for 
function approximation are typically used. States can no longer be
addressed uniquely, but values are approximated through  features (be
they hand crafted or learned) as discovered by neural
networks. Value propagation  in combination with 
approximation makes credit assignment unreliable, since the
propagation path through the states may contain omissions, shortcuts
and loops.

\subsection{Correlated States}
In supervised learning data samples (states) are  independent and
assumed to be distributed uniformly over the state space. In the database of static images, there is no relation
between subsequent images, and examples are independently sampled. Each image is separate, in contrast to a
movie, where many intertemporal relations between frames are
present. In reinforcement learning a sequence of states is generated
by a simulator or game playing program. The states are often
correlated between states, differing only by one move or one stone. Such a correlated and myopic training set, covering only a
part of the state space, will not work well with standard supervised
learning training algorithms. The  correlated
states create the possibility of feedback loops, and the training
algorithm may well  get stuck in a part of the feature space.

In addition to encountering loops and local features learning  from correlated consecutive
samples is inefficient and has a high variance. Little new information is contained in two
states that are almost the same. The low learning efficiency translates
into a smaller effective data set,  much training is done, yet little
is learned.
% high variance, since the effective information content is low, and
% basic statistics teaches us that (when all other things are equal) a small data set has a higher
% variance than a large data set.
Randomizing the samples breaks these
correlations and therefore reduces the probability to get stuck. 


The deadly triad would suggest to use on-policy instead of off-policy
learning, to improve 
the training convergence. However, when learning on-policy the current
network determines the next data sample to be trained on. Mnih et
al.~\cite{mnih2013playing} give an example of how on-policy learning
might also lead
to training divergence. Assume that  
the maximizing action is to move left. With on-policy learning the
training samples will be dominated by samples from the left-hand side;
if, for some reason, the maximizing action then switches to the right,
then the training distribution will 
also switch. In this way unwanted feedback loops may arise
and the network will get stuck in self reinforcing features, or
diverge~\cite{tsitsiklis1997analysis}. 

\subsection{Fluctuating Data Distribution}
In supervised learning the training examples are all in a static
database,  the distribution of the training data does not change
during training. In reinforcement
learning the data distribution changes as the algorithm learns new
behaviors. This  has two consequences, one desired, one undesired. In
the short term, learning new behaviors may casue myopia or getting
stuck in the state space by feeding on its own behavior as described in
on-policy learning. This short term training behavior can be smoothed
with a replay buffer by providing data from a larger landscape.

In the longer term, learning new behaviors may
actually be desirable. Forgetting bad behaviors can also be a way to
escape ineffective parts of the state space. Thus, the replay buffer
should not be too large. In Chapter~\ref{chap:plan} we will
learn more about this  in the context of self-play.

% ,
% causing instability in the learning. The fluctuating data distribution
% brings the  need to be able to {\em forget\/} in order to prevent
% continued  bootstrapping on an old basis.

We will see in the next section that the replay buffer smooths the
fluctuating data distribution.




% =================================================
% replay buffer is off-policy

% correlated data and non-stationary distributions

% The reasons for instability
% - approximation
% - bootstrapping
% - off policy learning
% together may lead to instability

% - target correlations
% - state/position distribution non-stationarity

% - long range credit assignment

% pictures

% - target correlations what goes wrong? what can we do about it?
% - state/position correlations what goes wrong? what can we do about it?

% - long range credit assignment what goes wrong? what can we do about it?
% w


% In contrast to TD-Gammon and similar online approaches, we utilize a technique known as expe- rience replay [13] where we store the agent’s experiences at each time-step, et = (st, at, rt, st+1) in a data-set D = e1 , ..., eN , pooled over many episodes into a replay memory. During the inner loop of the algorithm, we apply Q-learning updates, or minibatch updates, to samples of experience, e ∼ D, drawn at random from the pool of stored samples. After performing experience replay, the agent selects and executes an action according to an ε-greedy policy. Since using histories of arbitrary length as inputs to a neural network can be difficult, our Q-function instead works on fixed length representation of histories produced by a function φ. The full algorithm, which we call deep Q-learning, is presented in Algorithm 1.


\subsection{Divergence}
% In the work on DQN 
%   The training algorithm used is a form of Q-learning, which, when
% %However, it  has been shown that off policy algorithms such as
% %Q-learning
% combined with non 
% linear function approximation can cause network training
% divergence~\cite{tsitsiklis1997analysis,baird1995residual}.

% Deep learning algorithms for supervised learning typically assume that
% examples are independent. In reinforcement learning, and in games, subsequent states
% are typically correlated, and so are reward values, causing divergent
% optimization. Furthermore,  
% small updates to Q may significantly change the policy and therefore
% change the data distribution~\cite{mnih2015human}.

%\subsubsection{Experience Replay}\index{experience replay}
The DQN algorithm has methods to overcome  divergent training. It breaks the
correlations with two mechanisms. 
The important contributions  of Mnih et al.\ are a method to efficiently randomize
example states~\cite{mnih2013playing}, and, in 2015, a method to break the correlations with target
values~\cite{mnih2015human}.


The first method is a replay buffer. This is a  biologically
inspired
mechanism~\cite{mcclelland1995there,o2010play,lin1993reinforcement}.
It consists of a buffer of many previous states out of which it
randomly selects training examples. In doing so it randomizes over the
data removing some correlations in the sample sequence and smoothing over 
the data distribution.

Second,  Q-values are only infrequently adjusted towards target
values,  reducing correlations with target values.
We will now discuss these two methods.

\subsubsection{Replay Buffer}
Experience replay uses a replay buffer to randomize the training
examples. It improves on standard 
Q-learning in two respects: (1) randomizing the order in which samples
are used breaks the correlations between consecutive samples, and
therefore reduces the variance of the 
updates (high variance leads to ineffective training). (2) Experience
replay prevents unwanted feedback 
loops, which would arise when the game makes moves in a certain area
that it cannot escape from, getting stuck in local areas of the state space, or even diverge
catastrophically~\cite{tsitsiklis1997analysis}. By averaging the
behavior distribution over the
previous states, experience replay smooths out training and avoids
oscillations or divergence in the parameters.


% First, each step of experience is potentially used in many weight
% updates, which allows for greater data efficiency.

% Furthermore, the replay buffer randomly samples previous
% transitions, and thereby smooths the training distribution over many
% past behaviors 

% By using experience replay the behavior
% distribution is averaged over many of its previous states, smoothing
% out learning and avoiding oscillations or divergence in the
% parameters.
Training by experience replay is a form of  off-policy
learning, since the  current parameters are 
different from those used to generate the sample.

In practice, experience replay stores the last $N$ examples in
the replay memory, and samples uniformly  when
performing updates. A form of importance sampling might differentiate
important transitions.


%% Experience
%% replay is off policy because current
%% parameters are different from those used for the sample, hence
%% the choice for Q-learning~\cite{sutton2018introduction}.

%% A possible improvement of experiece replay i
%% Experience replay samples uniformly in the replay memory, but could be
%% enhanced by prioritized sampling methods such as prioritized sweeping~\cite{moore1993prioritized}.

\subsubsection{Infrequent Weight Updates}
The second improvement in DQN is infrequent weight updates.
Infrequent updates of the target weight values reduce correlations and
possible divergence and oscillations caused by loops and self
reinforcing features. It works by using a
separate network for generating the targets of the update of the $Q$
value. Every $x$ updates the network $Q$ is cloned to
obtain a target network $\hat Q$, which is used for generating the
targets for the following $x$ updates to $Q$.

This second network improves stability of Q learning,
where normally an update that increases $Q(s_t,a_t)$ often also
increases $Q(s_{t+1},a)$ for all $a$. This also increases the
target, quite possibly
leading to oscillations and divergence of the policy. Generating the
targets using an older set of parameters adds a delay between the time
an update to $Q$ is made and the time the update changes the targets,
breaking the feedback loop or at least making oscillations less likely.

%% There has been progress towards non linear control function approximation in
%% reinforcement learning.

%% These advances in reinforcement learning occurred in parallel to the
%% work in supervised learning, showcased by 
%% Krizhevsky et al.~\cite{krizhevsky2012imagenet}.


To conclude this chapter, now that we have discussed methods on how to achieve stable end-to-end
deep reinforcement learning, let use compare how this is achieved with
supervised learning.

\subsection{End-to-End Training}
Both the works on Atari and ImageNet succeed in end-to-end training. It
is interesting to compare end-to-end training in supervised and in
reinforcement learning. The  breakthroughs in computer
vision with AlexNet~\cite{krizhevsky2012imagenet},
and other ILSVRC-works, rely on  training
on large labeled training sets. In these and later research, networks
are trained directly from the raw inputs, using  updates by stochastic
gradient descent. The layered representations that are learned in this way are
often better representations than hand-crafted or heuristic features.

Mnih et al.\ achieved an end-to-end  behavior policy from raw visual
input, without any heuristics or intermediate features. The Atari 2600 games are games of skill. The games are
difficult for humans, because they require dexterity and quick
hand-eye coordination. Playing the games builds reflexes. The games
are not 
so much designed as games of strategy (such as Chess, Checkers, Go,
Backgammon, Othello, or even Tic Tac Toe), where planning algorithms shine.
The Atari 2600 games are are reflex games (thinking fast, not
 slow), that could be learned with a surprisingly simple neural
 network. In this sense, the problem of playing Atari well is not
 unlike an image database categorization problem: both problems are to
 find the right answer (out of a small set) that matches an input
 consisting of a set of pixels. Apparently, mapping pixels to
 categories is not that different from mapping pixels to joystick
 actions, and the long credit assignment problem has been
 overcome. This is a surprising result, to see such a deep connection
 between supervised and reinforcement learning. 

Despite this obervation, the algorithmic feat of breaking through the
divergence and oscillation of reinforcement learning with long delays
in credit assignment is impressive, and the Atari results are highly
imaginative, and have stimulated much subsequent research. Many blogs
have been written on replicating the result, which is not a trivial
task~\cite{openaibaseline2017}. 

Let us now look deeper in more advanced methods for generalization and
stable learning.


==> chapters/part1.tex <==
\part{Setting the Scene}
In this part we introduce the context of artificial intelligence and
game playing. We discuss why games play such a central role in
artificial intelligence. To give an idea of the progress that has been
made in artificial intelligence game playing, some 
milestone programs are discussed. Next, reinforcement learning is
introduced, a popular general framework well suited to formalize
important notions in game playing. It
forms the formal basis for the rest of the book.


==> chapters/part2.tex <==
\part{Planning}\label{part:plan}
In this part we introduce heuristic planning methods. We will start with
heuristic search algorithms with minimax as the basic paradigm. Minimax
is a simple paradigm: a fixed depth, fixed width algorithm, just a few
lines of code. Minimax algorithms, and all  algorithms derived from it, are
exact dynamic programming methods. 

We will also introduce the  search-eval architecture, an architecture
that consists of a search procedure and an eval procedure. For
minimax, typically a heuristic eval is used. Many enhancements have
been developed to 
achieve good performance with heuristic planning algorithms,  within the minimax paradigm.
Heuristics are approximation methods, they can generalize states,
allowing the size of very large state spaces to be reduced, so that
minimax, an exact method, can do its work.

Some of the games for which heuristic search works well have been
discussed in Chapter~\ref{chap:games}: Chess, Checkers, and
Othello. For these games many enhancements have been developed, to
achieve better performance. 

%A main thread in this part is how to achieve higher performance, by
%searching the state space in a more efficient way, first with
%heuristics, and then generalizing these
%approaches.
Chapter~\ref{chap:idtt} is devoted to heuristic
enhancements of search and eval functions. 

Chapter~\ref{chap:trial}  closes this part with  Monte Carlo Tree
Search (MCTS) an
algorithm that is based on 
a backup rule that is quite different from rigid minimax. Where in minimax efficient adaptive
and selective behavior had to be introduced via enhancements, in MCTS
adaptive and selective search are at  the core of the
algorithm. MCTS caused a breakthrough in performance in Go. MCTS is
also used successfully in other domains, and is one of the core elements of the
self-play methods of Chapter~\ref{chap:plan}. 
%Search, divide and conquer, table based


==> chapters/part3.tex <==
\part{Learning}\label{part:train}
%Generalization
In the part on Planning we discussed exact methods to perform
lookahead in  the state space. Exact methods are great since they provide exact values to
the value function, but  they may take
excessively long to compute when the state space is large. We 
also saw our first approximation methods, in the form of hand-crafted heuristic
evaluation functions, or averaged random playouts, as a way to shrink
the part of the state space 
that has to be traversed. However, in some cases the heuristic or random value
functions are not good enough. 

In the Planning part, most of our attention was on search, and the
evaluation function consisted of hand-crafted features, or randomization. In this part we shift our focus from the search part to the eval part.
We discuss machine learning  methods that go beyond hand-crafted heuristic or
randomized methods. These methods are called function approximation
methods. They  can automatically discover features from a (large) set of
training examples. The methods discover the essential features in a
training set. If trained well, these features should generalize to
similar sets of examples that were not seen during training. The
training reduces a large state space to essential features, allowing
the features to be used for 
classification and function approximation.  Deep
neural networks are frequently used for feature discovery.

For exact planning methods there is one relevant time where
computation takes place: the
(on line) time it takes to find the answer. For approximation methods,
both the time to train the approximator (off line) and the time to use
the approximator (on line) for the value lookup  are relevant. Training
occurs off line, and takes usually much longer than value lookup. In a
games tournament the on-line time to make a move is measured in minutes, the
off line time to train a network is sometimes measured in weeks.

The  approximate methods  train value
functions that can provide fast answers, and can often give a  good approximation of
that value of a state. (The training time of the aproximators may be
long, though.)

We will discuss two important training methods,  supervised learning (Chapter~\ref{chap:super})
and reinforcement learning (Chapter~\ref{chap:dqn}) and their
enhancements (Chapter~\ref{chap:conv}).


==> chapters/part4.tex <==
\part{Planning + Learning}\label{part:selfplay}
In this final part planning and traininglearning, exact and approximate, work
together. Self-play has a long history in game playing. Self-play is 
a recursive method, it feeds off itself, just as minimax planning. In minimax we determine our
best move by calculating our opponent's best reply, which
is based on our best reply, etc. In self-play we use a search-eval
player to train our own
evaluation function, by playing a small tournament against ourselves,
using the game record as training input, yielding an improved
evaluation function and playing for improved gain. Then we continue
our path of self improvement 
by doing another iteration of self-play, with the improved value
function.  The planning that is performed by the search function
ensures that the game record will be 
of a higher quality than the previous level of play on which the
current evaluation function is trained, so that the network is always trained
against higher quality examples. We will see that self-play is related
to curriculum learning, an efficient way of training neural nets. 

Self-play is at the basis of the successes of AlphaGo and
AlphaZero, and, some 25 years earlier, TD-Gammon.

% In this part the exact and approximate methods come together in an
% elegant self-play scheme: the exact methods are used
% to improve the approximate methods in a learning loop.



==> chapters/part5.tex <==
\part{Conclusion}


==> chapters/plan.tex <==

%% 6: plan
%% section: search-eval integration: generating examples by planning to learn, and using learned eval to search
%% section: convergence/divergence: tunnelvision through self learning. off policy/on policy
%% section: system 1 and system 2: this is combination: 1+2=3
%% *section: implement 15 puzzle, diplomacy, SAT, GTOC, chess, checkers
%% *section: run on Cloud
%% *section: check transfer learning, hyper parameter optimization
%% *section: do more advanced net structures, do net structure optimization
%% *section: do build up small nets and then expand to larger nets
%% section: implement 9x9 go learner in a0g


\section{Integrating Evaluation and Search}

A0G

search-eval interaction: plan to generate examples for DQN to learn
\section{Search-Eval Architecture}
Evaluation on trained features, mcts search, and self learning loop
\subsection{Evaluation by Generalization}
\subsection{Search: MCTS/UCT}
\subsection{Self learnig RL loop}


\section{Self learning: 1+2=3}

\section{*convergence, divergence, overfitting}
\subsection{Replay Buffer etc}

off policy, on policy

\section{*Future Ideas}
\subsection{15 Puzzle, SAT}

\subsection{Checkers, Chess}

\subsection{Cloud}

\subsection{Transfer Learning, Hyper Parameter Optimization}

\subsection{Net Structure}

\subsection{Evolve Net}



\section{Fast and Slow}
Fast and slow: this is fast and slow (planning+learning). really it is also learning of the third kind: using planning to generate examples from whcih to learn


%\section{Plan/Learn}
%search: UCT, eval: generalize
%\section{Theory}




\section{Practice: A0G 9x9 Go}
A0G examples

full a0g and keras 9x9 go





==> chapters/todo.tex <==
\begin{itemize}
%\item write all summaries (ch12,13)
%\item ch5 extra text on piece square tables etc
%\item ch6 add text picture mcts tree, picture Cp vs N
%\item ch7 extra text, explain how hard deep learning is, failed
%  attempts. voeg toe 3 subsections: on generalization (needs CNN,
%  explain CNN with pictures, explain diff with FCN), on vanishing
%  gradients (explain ReLU, 
%  picture ReLU, explain diff with sigmoid), on overfitting (explain
%  dropouts, with picture)
% \item ch8 extra text explain difficulty of correlated states,
%   difficulty of long range credit assignments (pictures of
%   correlation, of long range credit assignment)
% \item ch9 extra text time series, LSTM,
%\item ch11 extra text hierarchical reinforcement learning
%\item ch12 order is illogical, rearange, methods, levels, ggp, aiai,
%  agi, futu% re. methods should be a list, or incorporated in chapters. 
% \item ch13 rambling. tighten up. sys123, behavioral intell (again???
%   in ch 2???), agi (again??? in ch12), fast   learning, future.
%   too many items that have been
%   addressed elsewhe
%  re. need to say things only in 1 place
% \item Ch 1, ch 12, ch 13 contain various pieces of deep insight. These
%  should really be inserted into the main text, to make that better.
\item improve exercises; improve chapter bibliographical sections
  % \item rewrite intro. too much
\item read whole book. repetitions, clarity, main thread
% \item main theme: Search-Eval. Optimize=find
%   best. Search=Optimize. Heur=/=Optimize. Learn=Optimize. Search-eval
%   is two kinds of optimizations. It is all optimization, just with
%   different data structures. It is about what to optimize. The
%   details matter, all these papers are doing is setting up the right
%   kind of setting creating a new kind of optimization. Intelligence
%   is finding the right combination of settings/datastructures for
%   optimization. In this book, in this field of research,
%   Intelligence is Learning to Play, and Learning to Play is Learning
%   What to Optimize.
% \item What is the topic of this book? The topic of this book is the reinforcement learning methods for intelligent
%   behavior in games.
  % Explaining How does Self-Play work? Expose about the field of
  % computer games/reinforcement learning in games with highlights:
  % heuristic planning, learning function approximation, coming together in
  % self-play, with main threads shared architecture (search-eval) and shared
  % algorithm (optimization). This book is a 5-tuple: (heur plan,
  % learning func approx, self-play, search-eval, optim) providing an
  % overview of the field reinforcement learning in games, showing you
  % about creating intelligent behavior, preparing you for further
  % thesis research. The problem is that there are 5 things in the
  % 5-tuple, not one.  If it would be one, then it would be search-eval,
  % or the task of finding what to optim.

%\item
%   I will show you how to create Intelligent behavior in games using
%   multiple levels of recursively structured optimization. I will also
%   hint at future possibilities, extensions of these technologies,
%   towards general intelligence.  

% Essentie van het boek:
% H2: why\&background/past/related work. Setting the scene
% H3: the language\&definitions. Korter!!! Geen backprop en zo. Maak 3 korter. Puur de essentie. 
% H4: straightforward mapping of technology on problem, with apparent knowledge
% H6: one level further: adapting the mapping
% H7: more difficult: learning the mapping from examples
% H10: learning the examples for learning the mapping
% H12: even more difficult problems.
% picture (tikz) of the problems/chapters building on top of each other

% Veranderingen na Heel boek lezen:
% H1 ander outline essentie verhaal vertellen. Intelligent behavior from
% Recursively structured optimization. Van straightforward naar more
% difficult problem/method mapping. Learning= plan+ train

% H2 ggp er uit

% H3 alleen essentie. Korter

\item perform and execute code in practice and exercise sections
%\item replication. some things (such as deadly triad) are explained
%  many times. Go over book and write down all location where concepts
%  are discussed, and make sure it is only once. Kind of index, with at
%  most one entry per key-term
\item Language is sometimes dry. Note that this can be written more
  exciting.
% \item rewrite 12.1: a theory/framework on layers of recursive
%   optimization. The new search-eval. Rewrite Chapter 12 completely.
% \item check 11.2.1 GGP text for consistency
%  H10 haal teveel alphago detail er uit, naar appendix
% \item read whole book again
\item  Mike Preuss,  Thomas Moerland, Joost Broekens, Alfons Laarman,
  Thomas B\"ack, Michael Emmerich,  Felienne Hermans, 
  Vedran Dunjko, Jan van Rijn, Frank Takes, Walter Kosters, Jonathan Vis,
\item[Plan] Mark Winands, Matthijs Spaan, Tristan Cazenave,
  Bruno Bouzy, Aja Huang,  Simon Lucas, Remi Coulom, Sylvain
  Gelly, Olivier Teytaud,
\item[Train]  Herke van Hoof, Pascal Mettes, Marco Wiering, Thomas
  Moerland, Frans Oliehoek, Michael Lew, Wojtek Kowalczyk,
 \item David Silver,  Thore Graepel, Ilya 
    Sutskever, Pieter Abbeel, Volodymir Mnih, Sergey Levine, John
    Schulman, Emma Brunskill, Marc Lanctot
% \item add to Ch11 that the main problem of self-play is computational
%   cost. We must find a way to do it cheaper. More engineering, faster
%   training, faster play, smaller MCTS, parallel tournaments? Add to ch
%   10 the problem.
\item add an MCTS example (but how? how many passes to do?) Add
  supervised network example? 

\item publisher
\item check references \& clean up all arXiv
\item figures, copyrights
\end{itemize}


==> diag/actor-critic.tex <==
% Definition of circles
\def\firstcircle{(0,0) circle (1.5cm)}
\def\secondcircle{(0:2cm) circle (1.5cm)}

\colorlet{circle edge}{black!50}
\colorlet{circle area}{black!20}

\tikzset{filled/.style={fill=circle area, draw=circle edge, thick},
    outline/.style={draw=circle edge, thick}}

\setlength{\parskip}{5mm}
% Set A and B
\begin{tikzpicture}
    \begin{scope}
        \clip \firstcircle;
        \fill[filled] \secondcircle;
    \end{scope}
    \draw[outline] \firstcircle node [label=above:{Value
      function\ \ \ \ \ \ \ \ \ \ \  },label=below:{Value-based\ \ \ \  \ \ \ }] {};
    \draw[outline] \secondcircle node
    [label=above:{Policy},label=below:{\ \ \ \ \  \ \ \ Policy-based}] {};
%    \node[anchor=south] at (current bounding box.north) {$A \cap B$};
\end{tikzpicture}

==> diag/heursampgen.tex <==
\begin{tabular}{l|c|c|c|c}\hline\hline
     & {\bf Ch~\ref{chap:search}} & {\bf Ch~\ref{chap:trial}} & {\bf
                                                                  Ch~\ref{chap:dqn}}
  & {\bf Ch~\ref{chap:plan}} \\ \hline
{\bf name} & alpha-beta & MCTS & DQN & Self-Play\\ \hline\hline
{\bf select} & left-to-right& expl/expl           & -     & expl/expl\\ \hline
{\bf backup} & minimax    & average         & -     & average\\ \hline
{\bf eval}   & heuristic  & sample          & generalize   & generalize\\ \hline\hline  
\end{tabular}


==> diag/ontology.tex <==
\begin{tabular}{l|c|c}
               & special &  general\\ \hline \hline
  search=plan  & AB      &  MCTS   \\ \hline
  eval,learn   & heur    &  net \\ \hline \hline


==> diag/paradigm.tex <==
\begin{tabular}{l|c|c|c|c}\hline\hline
     & {\bf Ch~\ref{chap:search}} & {\bf Ch~\ref{chap:trial}} & {\bf Ch~\ref{chap:dqn}} & {\bf Ch~\ref{chap:plan}} \\ \hline\hline
{\bf paradigm} & {\bf plan} & {\bf plan} & {\bf train} & {\bf plan+train} \\ \hline
{\bf Kahneman} & slow       & slow            & fast  & slow+fast \\ \hline
{\bf technique}& enumerate  & adaptive        & generalize & self-play\\ \hline
{\bf program}  & Deep Blue  & MoGo, Zen       & Atari & Alpha(Go) Zero \\ \hline
\hline
\end{tabular}


==> diag/paradigm2.tex <==
  \begin{tabular}{l|c|c|c|c}
    \hline\hline &
      {\bf Ch~\ref{chap:search}} & {\bf Ch~\ref{chap:trial}} & {\bf
      Ch~\ref{chap:dqn}} & {\bf Ch~\ref{chap:plan}}
      \\ \hline
      paradigm & {\bf plan} & {\bf plan} & {\bf train} & {\bf plan+train}
      \\ \hline
      field & mathematics & statistics & func approx&
      self learning
      \\ \hline
      algorithm & AlphaBeta & MCTS & DQN & MCTS+DQN
      \\ \hline
     {\bf search} & smart enumeration & exploi/explor  & sample  & RL/MCTS
    \\ \hline
     {\bf evaluation} & man heuristic & rand playouts & gen features & gen features 
    \\ \hline
      backup & minimax & average & back prop & average/back prop 
    \\ \hline
    program & Deep Blue & MoGo, Zen & Atari & Alpha(Go) Zero
    \\ \hline
    Kahneman & slow & slow & fast & slow+fast
    \\ \hline\hline
  \end{tabular}


==> diag/searcheval.tex <==
\begin{tabular}{l|c|c|c|c}\hline\hline
     & {\bf Ch~\ref{chap:search}} & {\bf Ch~\ref{chap:trial}} & {\bf Ch~\ref{chap:dqn}} & {\bf Ch~\ref{chap:plan}} \\ \hline\hline
{\bf search} & alpha-beta& MCTS           & -     & MCTS\\ \hline
{\bf select} & left-to-right& UCT           & -     & P-UCT/policy net\\ \hline
{\bf backup} & minimax    & average         & -     & average\\ \hline
{\bf eval}   & heuristic  & roll-out          & DQN   & value net\\
  \hline
{\bf self-play}   & -  & -          & -   & self-play\\ \hline\hline  
\end{tabular}


==> diag/tab-arch.tex <==
  \begin{tabular}{c|c|c|c|c|c|c}
    \hline\hline
    {\bf Kahneman} &  {\bf AI} & {\bf Arch} & {\bf
      Ch~\ref{chap:search}} & {\bf Ch~\ref{chap:trial}} & {\bf
      Ch~\ref{chap:dqn}} & {\bf Ch~\ref{chap:plan}}
        \\ \hline
    Fast & Recog & Eval & Heuristic & Rnd Playouts
    & Deep Q Net & Deep Q Net
    \\ \hline
    Slow & Plan & Search & smart enumeration & expl/expl  & expl/expl
    & expl/expl 
    \\ \hline
    3 & Learn & Selfplay & $-$ & $-$ & Superv. \&
    RL & RL Self Play
    \\ \hline
    Program &  &  & Deep Blue & MoGo &
    AlphaGo & Alpha(Go) Zero \\ \hline\hline
  \end{tabular}


==> diag/technique.tex <==
\begin{tabular}{l|c|c|c|c}\hline\hline
     & {\bf Ch~\ref{chap:search}} & {\bf Ch~\ref{chap:trial}} & {\bf Ch~\ref{chap:dqn}} & {\bf Ch~\ref{chap:plan}} \\ \hline\hline
{\bf recognize}& heuristic& random playouts & generalize  & generalize\\ \hline
{\bf plan}   & enumerate  & expl/expl       & -           & expl/expl\\ \hline
{\bf learn}  & -          & -               & features    & best player\\ \hline
\hline
\end{tabular}


==> python/sunfish/sunfish.6 <==
.TH SUNFISH 6 "11 Feb 2014"
.SH NAME
Sunfish - A 111 line Chess Engine in Python
.SH SYNOPSIS
sunfish
.SH DESCRIPTION
Sunfish is a simple, but strong chess engine, written in Python, mostly for teaching purposes. Without tables and its simple interface, it takes up just 111 lines of code!

The great clarity of the Sunfish code provides a great platform for experimenting, be it with evaluation functions, chess heuristics or search. Fork it today and see what you can do! 
.SH GAMEPLAY
Sunfish presents chess board as a simple grid

  r n b q k b n r 
  p p p p p p p p 
  . . . . . . . . 
  . . . . . . . . 
  . . . . . . . . 
  . . . . . . . . 
  P P P P P P P P 
  R N B Q K B N R 

 Your move:

You make your move by typing source and destination coordinates.
Coordinates are represented by letters A through H on X-axis and numbers 1
through 8 on Y-axis, where bottom-left corner represents coordinate A1

 8  r n b q k b n r 
 7  p p p p p p p p 
 6  . . . . . . . . 
 5  . . . . . . . . 
 4  . . . . . . . . 
 3  . . . . . . . . 
 2  P P P P P P P P 
 1  R N B Q K B N R 

    A B C D E F G H

Player always begins. Player controls capital letters on the bottom.

To move Pawn on E2 to E4, player would type e2e4 on the "Your move:" prompt and
press return key.

.SH FEATURES
.IP \[bu]
Build around the simple, but deadly efficient MTD-bi search algorithm.
.IP \[bu]
Filled with classic as well as modern 'chess engine tricks' for simpler and faster code.
.IP \[bu]
Easily adaptive evaluation function through Piece Square Tables.
.IP \[bu]
Uses standard Python collections and data structures for clarity and efficiency.
.SH LIMITATIONS
Sunfish supports castling, en passant, and promotion. It doesn't however do minor promotion or draws of any kind. All input must be done in simple 'two coordinate' notation, as shown in the screenshot.

On the technical side there are a lot of features that could be interesting to add to Sunfish. For performance, the most important might be a piecelist to save the enumeration of all board squares at every move generation. Other performance optimizations include a reduced use of hashtables and a mutable board representation. Perhaps based on bitboards.

The evaluation in Sunfish is not very sophisticated. E.g. we don't distinguish between midgame and endgame. The search is limited in that no quince search is performed and so we can have horizon effects. Null move pruning is not done, and it is debatable wether it would be safe given our choice of MTD search. Finally Sunfish might benefit from a more advanced move ordering, including such things as killer move and SEE.
.SH COPYRIGHT
Copyright (C) 2014 Thomas Ahle

This program is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 3 of the License, or
(at your option) any later version.

This program is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with this program.  If not, see <http://www.gnu.org/licenses/>.
.SH AUTHOR
Thomas Ahle

